SoK: Certified Robustness for Deep Neural Networks

Great advances in deep neural networks (DNNs) have led to state-of-the-art performance on a wide range of tasks. However, recent studies have shown that DNNs are vulnerable to adversarial attacks, which have brought great concerns when deploying these models to safety-critical applications such as autonomous driving. Different defense approaches have been proposed against adversarial attacks, including: a) empirical defenses, which can usually be adaptively attacked again without providing robustness certification; and b) certifiably robust approaches, which consist of robustness verification providing the lower bound of robust accuracy against any attacks under certain conditions and corresponding robust training approaches. In this paper, we systematize certifiably robust approaches and related practical and theoretical implications and findings. We also provide the first comprehensive benchmark on existing robustness verification and training approaches on different datasets. In particular, we 1) provide a taxonomy for the robustness verification and training approaches, as well as summarize the methodologies for representative algorithms, 2) reveal the characteristics, strengths, limitations, and fundamental connections among these approaches, 3) discuss current research progresses, theoretical barriers, main challenges, and future directions for certifiably robust approaches for DNNs, and 4) provide an open-sourced unified platform to evaluate 20+ representative certifiably robust approaches.

==> contents/main_old.tex <==


\section{Introduction}

    \label{sec:intro}

    Machine learning techniques, especially deep neural networks~(DNNs), have been widely adopted in various applications, such as image classification~\cite{krizhevsky2009learning,he2016deep,szegedy2016rethinking}, natural language processing~\cite{vaswani2017attention,devlin2018bert,brown2020language}, and robotics~\cite{silver2017mastering,silver2018general}.
    However, despite their wide applications, recent studies~\cite{szegedy2013intriguing,goodfellow2014explaining} have shown that DNNs are  vulnerable to the carefully crafted adversarial attacks such as \textit{adversarial examples} ---  inputs with adversarial perturbation added that could mislead DNNs to make arbitrarily incorrect predictions~\cite{athalye2018obfuscated,brendel2017decision}.
    The existence of adversarial attacks leads to great safety concerns for DNN based applications, especially in the safety-critical scenarios such as autonomous driving.
    
    Different types of adversarial attacks have been proposed so far ~\cite{athalye2018obfuscated,brendel2017decision,goodfellow2014explaining,carlini2017towards,xiao2018generating,houdini2017cisse,madry2017towards}.
    To defend against these attacks, there are several work proposed to improve the robustness of  neural networks ~\cite{papernot2016distillation,samangouei2018defensegan,madry2017towards,buckman2018thermometer,guo2018countering}.
    However, many of such defenses  can be adaptively attacked again by sophisticated attackers~\cite{athalye2018obfuscated,tramer2020adaptive}.
    The everlasting competition between attackers and defenders motivates studies on the certifiably robust approaches for DNNs, which include both robustness verification and robust training approaches~(e.g. \cite{cohen2019certified,katz2017reluplex,singh2019beyond,singh2018robustness,wang2018efficient,wong2018provable,yang2020randomized}).
    The robustness verification approaches aim to provide the theoretically certified lower bound of robustness under certain perturbation properties, 
    such as the magnitude of perturbations.
    The corresponding robust training approaches aim to train neural networks in order to improve such lower bound of robustness.

    In this paper, we focus on recent research in certified robustness for DNNs, including both verification and robust training approaches.
    We provide the \textit{first} systematic taxonomy for the certifiably robust approaches, enabling researchers to further inspect each approach in details and understand their
    fundamental
    connections.
    In particular, we discuss both the \textit{deterministic verification} and emerging \textit{probabilistic verification} approaches for neural networks, along with the corresponding robust training approaches.
    
    We develop an open-sourced unified platform for the representative verification and training approaches.
    % \footnote{The platform is open-sourced at \textit{\url{https://github.com/AI-secure/VeriGauge}}.}
    Empirically, we benchmark over $20$ verification and robust training approaches for comparison.
    % \footnote{In addition, we maintain the leaderboard of state-of-the-art certified robustness at \textit{\url{https://github.com/AI-secure/Provable-Training-and-Verification-Approaches-Towards-Robust-Neural-Networks}}.}
    As far as we know, it is the \emph{first} large-scale benchmark on the certified robustness for 
    neural networks.
    Based on the taxonomy, analysis, and benchmark of existing approaches, we further provide discussion and analysis on current research progresses, theoretical barriers~(including a proposed one), and several promising future directions in certified robustness.
    % We also present additional theoretical analysis and improvements for existing robustness verification approaches based on exploiting the structure of SDP(semi-definite programming)-based verification problem.
    % We also present a theoretical barrier of randomized smoothing-based robustness verfication, and a novel acceleration strategy for SDP~(semi-definite programming)-based verification.
 

    Our main contributions are summarized as follows:
    % \begin{itemize}
    %     \item We provide the \textit{first} taxonomy of certified robustness approaches for neural networks, including both robustness verification and corresponding robust training approaches.
    %     \item We conduct comprehensive theoretical analysis and extensive empirical comparisons for different state-of-the-art approaches on robustness verification and training.
    %     \item 
    %     We theoretically show a barrier of current probabilistic robustness verification, and discuss possible future directions of certified robustness.
    %     % , and propose a novel acceleration strategy for SDP-based verification exploiting the tri-diagonal matrix structure of formulated SDP problem, which enables the SDP-based verification for larger DNNs. 
        
    %     \item We provide an open-sourced unified evaluation platform for over $20$ verification and training approaches, which we believe will facilitate the development and evaluation of research on certified robustness for~DNNs.\footnote{The extensive comparison of existing approaches and additional results are available at \texttt{\url{https://sokcertifiedrobustness.github.io}}.}
    % %   \bo{code link, blog} 
    % \end{itemize}


    \begin{itemize}
        \item  We provide the \textit{first} taxonomy of certifiably robust approaches for neural networks, including both robustness verification and corresponding robust training approaches.
        
        \item We conduct comprehensive theoretical analysis and extensive empirical comparisons for different state-of-the-art approaches on robustness verification and training.
        \footnote{The extensive comparison of existing approaches and additional results are available at \textit{\url{https://sokcertifiedrobustness.github.io}}~(link anonymized).}
        
        \item We discuss and analyze current research progresses, theoretical barriers~(including a new theoretic result), and challenges of current certifiably robust approaches. We further provide several potential future directions of certified robustness.
        
        \item We provide an open-sourced unified evaluation platform for over $20$ verification and training approaches, which we believe will facilitate the development and evaluation of research on certified robustness for~DNNs.
    \end{itemize}




\section{Notations and Preliminaries}
% \bo{1. notations of learning xxxx, 2. threat model: attack based on different norms, attack methods (fgsm, cw xxxx)-- certified is independent with the attack method -- claim the advantages, 3. chanlenges -- e.g. minmax hard to solve for nonconvex, ibp-- bound loss}
    
    In this section, we will introduce the basic notations and important preliminary concepts.
    
    \subsection{Notations}
        \label{sec:sec_notations}
        
        We denote $[n]$ as set $\{1,\,2,\,\dots,\,n\}$.
        % Throughout the text, we use $\epsilon$ or $r$ to represent the real-valued robust radius under consideration.
        To express the region of adversarial perturbation,
        when measured by $\cL_p$ norm, we use $B_{p,\epsilon}(x_0)$ to denote the corresponding ball centered at $x_0$ with $\epsilon$ radius, i.e., $B_{p,\epsilon}(x_0) := \{x: \|x - x_0\|_p \le \epsilon\}$.
        For matrix $\bM$, the $\bM^+ := \max\{\bM,\,\bzero\}$ is the elementwise positively filtered matrix, and the $\bM^- := \min\{\bM,\,\bzero\}$ is corresponding negatively filtered matrix.
        % The $\cN(\mu,\,\sigma^2)$ denotes normal distribution with mean $\mu$ and variance $\sigma^2$.
        % and $\cN(\mu,\bsigma)$ to represent the multivariate normal distribution with mean $\mu$~(vector) and co-variance matrix $\bsigma$.
        The function $\Phi(\cdot)$ is the cumulative density function~(CDF) of standard normal distribution $\cN(0,\,1)$.
        
        % The mathematical notations used are listed in \Cref{tab:notation}.
        % \begin{table}[!t]
        %     \centering
        %     \caption{Definition of mathematical notations.}
        %     \resizebox{0.48\textwidth}{!}{
        %     \begin{tabular}{c|l}
        %         \toprule
        %         Notation & Meaning \\
        %         \hline\hline
        %         $[n]$ & $\{1,\,2,\,\dots,\,n\}$  \\
        %         $x$ & Scalar or vector \\
        %         $\bM$ & Matrix \\
        %         $\epsilon$ or $r$ & The robustness radius under consideration \\
        %         $\|\cdot\|_p$ & Vector $\cL_p$ norm \\
        %         $\cL_p$ & The $\cL_p$ norm \\
        %         $B_{p,\epsilon}(x_0)$ & The $\cL_p$ ball with $\epsilon$ radius: $\{x:\, \|x - x_0\|_p \le \epsilon\}$ \\
        %         $\bM^+$ & $\bM^+ := \max\{ \bM ,\,\bzero \}$ elementwise \\
        %         $\bM^-$ & $\bM^- := \min\{ \bM ,\,\bzero \}$ elementwise \\
        %         $\cN(\mu,\,\sigma^2)$ & Single variable normal distribution with mean $\mu$ and variance $\sigma$ \\
        %         $\cN(\mu,\,\bsigma)$ & Multivariate normal distribution with mean $\mu$ and co-variance matrix $\bsigma$ \\
        %         $\Phi(\cdot)$ & CDF of standard normal distribution $\cN(0,\,1)$ \\
        %         \bottomrule
        %     \end{tabular}
        %     }
        %     \label{tab:notation}
        %     \vspace{-1em}
        % \end{table}
        We mainly focus on existing works on the classification task with neural networks. Specifically, a large portion of existing approaches mainly consider feed-forward ReLU networks (see \Cref{def:feed-forward-nn}).
        % \begin{definition}[Neural Networks for Classification]
            A \emph{neural network model} $f_\theta$ is modeled as a function: $\cX \mapsto \bbR^C$, where
            the input data $x \sim \cD$ is in a bounded $n$-dimensional subspace $\cX \subseteq [0,\,1]^n$, and the model provides confidence scores for all $C$ classes.
            $F_\theta(x) := \argmax_{i \in [C]} f_\theta(x)_i$ is the predicted class of model $f_\theta$ given input $x$.
            $\theta$ is the set of trainable parameters for $f$.
            For brevity, we will omit $\theta$ when there is no ambiguity.
            % \label{def:nn-for-classification}
        % \end{definition}
        % \bo{small English illustration}
        % 
        % We model the input domain as a bounded subspace, which is true for common applications.
        % For example, the pixel color of images is in $[0,\,255]$ and is usually normalized to range $[0,\,1]$.
        % The output of neural network $f$ is the confidence score for each class, and the model predicts the class with highest confidence score.
        Note that common neural networks may add a softmax layer on top of $f$ to normalize these confidence scores.
        Since it does not change the predicted class, we mainly focus on either $f(x)$~(refer to as \emph{logits layer} in the literature) or the final predicted label $F(x)$.
        % \linyi{Rewritten.}
        
        % More specifically, we call $f$ the \emph{logits layer} of the neural network.
        % After logits layer, neural networks often add a softmax layer to normalize these confidence scores which yields $\tilde{f}$.
        % The softmax layer is defined as such:
        % \begin{equation}
        %     \tilde{f}(x)_i = \dfrac{\exp\left(f(x)_i\right)}{\sum_{j=1}^C \exp\left(f(x)_i\right)}.
        %     \label{eq:softmax}
        % \end{equation}
        % Note that softmax layer does not change the relative size among classes, and thus does not change the predicted labels.
        % Therefore, we mainly care about the logits layer $f$, or the final prediction $F$.
        
        %A large portion of existing approaches mainly consider %feed-forward ReLU networks.
        \begin{definition}[Feed-Forward ReLU Networks]
            An $l$-layer feed-forward ReLU network $f_\theta$ is defined as such:
            \begin{equation}
                \small
                \left\{
                \begin{aligned}
                    & z_1 := x, \\
                    & \hz_{i+1} := \bW_i z_i + b_i, \quad & \text{for $i = 1,\,2,\,\dots,l-1$} \\ 
                    & z_{i} := \relu(\hz_{i}), \quad & \text{for $i = 2,\,\dots,l$} \\
                    & f_\theta(x) := \hz_l,
                \end{aligned}
                \right.
            \end{equation}
            where 
            % $z_1 := x$ and $f_\theta(x) := \hz_l$.
            % The ReLU function is 
            $\relu(z,\,0) = \max\{z, 0\}$.
            % 
            Each $z_i$ and $\hz_i$ is a vector in $\bbR^{n_i}$.
            In particular, $n_1 = n$ and $n_l = C$.
            The trainable parameters $\theta := \{ \bW_i, b_i:\, i \in [l-1] \}$.
            \label{def:feed-forward-nn}
        \end{definition}
        %Note that convolutional layers are affine transformations and can be expressed by $\hz_{i+1} := \bW_iz_i + b_i$ in \Cref{def:feed-forward-nn}.
        
    \subsection{Threat Model}
    
        In this paper, we focus on \textit{white-box evasion} attacks, which indicates the strongest adversary who has full knowledge about the target model including its parameters and architecture. The attacker could craft an imperceptible perturbation to the original input, generating a new sample known as \emph{adversarial example}~\cite{szegedy2013intriguing}, which fools the model to make wrong predictions.
        %The imperceptible perturbation is commonly characterized by $\cL_p$ norm.
        % , while other metrics will also discussed be discussed in this review.
        Specifically, we mainly consider \emph{$(\cL_p,\,\epsilon)$-adversary}~(\Cref{def:lp-adversary}), though 
        other types of attacks will also be discussed briefly.
        \begin{definition}[$(\cL_p,\,\epsilon)$-Adversary]
            For given $(x_0, y_0)$, where $x_0\in \cX$ is the input and $y_0 \in [C]$ is the true label, 
            the \emph{$(\cL_p,\,\epsilon)$-adversary} will generate a perturbed input $x \in B_{p,\epsilon}(x_0)$, such that $F_\theta (x) \neq y_0$.
            % any input $x \in B_{p,\epsilon}(x_0)$ where $B_{p,\epsilon}(x_0)$ is a ball centered at $x_0$ with radius $\epsilon$ under $\cL_p$ norm.
            % The goal of the adversary is to induce the model to make wrong prediction.
            (When the radius $\epsilon$ is not of interest, we will use \emph{$\cL_p$ adversary}).
            \label{def:lp-adversary}
        \end{definition}
        % \begin{remark*}
        %The goal of the adversary is to craft a perturbed input which is close to the original input, but misleads the model to make wrong prediction.
        The above definition conforms to \emph{untargeted attack}.
        We remark that \emph{targeted attack} which mislead the adversarial input to a predefined label $y_t$ can be defined similarly.
        % $B_{p,\epsilon}(x_0)$ is a ball centered at $x_0$ with radius $\epsilon$ under $\cL_p$ norm.
        % \linyi{Delete a redundant definition.}
        % The illustration of $\cL_p$ bounded ball for different $p$'s in 2-dimensional case is shown in \Cref{fig:different-norms}.
        %When $p \in \bbN_+ \cup \{\infty\}$, we adopt classical $\cL_p$ norm definition.
        %When $p=0$, we deem $\|x\|_0$ as the number of non-zero entries in $x$.
        In general, different literature also refers to an $(\cL_p,\,\epsilon)$-adversary as an $\cL_p$-bounded attack~(bounded by $\epsilon$).
        % \end{remark*}
        
        % \begin{figure}
        %     \centering
        %     \includegraphics[width=0.35\textwidth]{figures/different-norms.pdf}
        %     \caption{The $\cL_p$-bounded ball in 2-dimension space. From left to right are $p=1$, $p=2$, and $p=\infty$ ball centered at $x_0$ with radius $r$ respectively.}
        %     \label{fig:different-norms}
        % \end{figure}
        
        % Specifically, we care about the \emph{strongest $(\cL_p,\,\epsilon)$-adversary}.
        % \begin{definition}[Strongest $(\cL_p,\,\epsilon)$-Adversary]
        %     An $(\cL_p,\,\epsilon)$-adversary $\cA$ is called the strongest $(\cL_p,\,\epsilon)$-adversary \emph{if and only if}
        %     when model $f$ has adversarial examples given input $x_0$ whose true label is $y_0 \in [C]$, i.e., $\exists x \in B_{p,\epsilon}(x_0)$ s.t. $F(x) \neq y_0$, the adversary $\cA$ can \emph{always} find an adversarial example.
        %     \label{def:strongest-lp-adversary}
        % \end{definition}
        % \bo{define only one attack}
    
    \subsection{Robustness Verification and Training Approaches}
        \label{sec:definition-robust-verification-provable-defense}
        
        \para{Robustness verification.}
        \emph{Robustness verification} certifies the lower bound of model's performance against \emph{any} adversary under certain conditions 
        % (in this paper, we focus on $(\cL_p,\,\epsilon)$-adversary).
        , e.g., $\cL_\infty$-bounded attack.
        So far, there are two major branches of robustness verification approaches: \emph{deterministic verification} and \emph{probabilistic verification}.
        When the given input is non-robust against the attack, deterministic verification approaches are guaranteed to identify this non-robustness while the probabilistic verification approaches only succeed with certain probability (e.g. $99.9\%$) where the randomness is independent of input. Specifically, if the verification approach claims $x$ is non-robust if and only if it is indeed non-robust we call it \emph{complete verification}; otherwise \emph{incomplete verification}. See \Cref{def:verification-approach} for formal definition. 
        Moreover, the robustness verification can be modeled as an optimization problem~(\Cref{prob:verification-optimization-problem}).
        \begin{definition}[Robustness Verification]
            An algorithm $\cA$ is called a \emph{robustness verification} approach, if for any $(x_0, y_0)$, as long as there exists $x \in B_{p,\epsilon}(x_0)$ with $F_\theta(x) \neq y_0$~(adversarial example), $\cA(f_\theta,\,x_0,\,y_0,\,\epsilon) = \mathrm{false}$~(\emph{deterministic verification}) or $\Pr[\cA(f_\theta,\,x_0,\,y_0,\,\epsilon) = \mathrm{false}] \ge 1 - \alpha$~(\emph{probabilistic verification}), where $\alpha$ is a pre-defined small threshold.
            
            By definition, a robustness verification approach $\cA$ provides a sufficient condition for model robustness. If $\cA$ also provides a necessary condition for model robustness, $\cA$ is said to be \emph{complete}, otherwise \emph{incomplete}.
            
            %A \emph{robustness verification} approach $\cA$ is called a \emph{complete verification} approach if for $(x_0,y_0)$ such that any $x \in B_{p,\epsilon}(x_0)$ satisfies $F_\theta(x) = y_0$~(robust input), $\cA(f_\theta,\,x_0,\,y_0,\,\epsilon) = \mathrm{true}$.
            %In contrast, a \emph{robustness verification} approach $\cA$ is called an \emph{incomplete verification} approach if for some $(x_0,y_0)$ such that any $x \in B_{p,\epsilon}(x_0)$ satisfies $F_\theta(x) = y_0$~(robust input), $\cA(f_\theta,\,x_0,\,y_0,\,\epsilon) = \mathrm{false}$.
            \label{def:verification-approach}
            \label{def:complete-verification-approach}
        \end{definition}
        
        %\begin{remark*}
            %Robustness verification approach provides a sufficient condition for model robustness;
            %and complete robustness verification approach provides a sufficient and necessary condition.
            %Comparing to the adversaries, verification approaches can certify that the model is robust, i.e., no adversarial examples, while adversaries can show that there is adversarial example.
        %\end{remark*}
        
        % \linyi{Modified.}
        % , which is formalized in problem \ref{prob:verification-optimization-problem}.
        
        %We can also view robustness verification from optimization.
        \begin{problem}[Robustness Verification as Optimization]
            \label{prob:verification-optimization-problem}
            Given a neural network $f_\theta: \cX \mapsto \bbR^C$, input instance $x_0 \in \cX$, ground-truth label $y_0 \in [C]$, target label $y_t \in [C]$ and the radius $\epsilon > 0$, we define the following optimization problem:
            \begin{equation}
                \label{eq:verification-optimization-problem}
                    \cM(y_0,y_t) = \minimize_{x}\, f_\theta(x)_{y_0} - f_\theta(x)_{y_t}
                    \, 
                    \text{ s.t. }
                    \, 
                    x \in B_{p,\epsilon}(x_0).
            \end{equation}
            One can certify that $f_\theta$ is robust at $x_0$ within radius $\epsilon$ w.r.t. $\cL_p$ norm, as long as $\cM(y_0,y_t)\ge 0, \forall y_t\in[C]$.
        \end{problem}
        
        %\begin{remark*}
        %Given the solver for \Cref{prob:verification-optimization-problem}, we can enumerate all $C - 1$ different $y$'s and compute
        %\begin{equation}
        %    \label{eq:verification-optimization-problem-alternative}
        %    OPT := \min_{y \in [C]: y \neq y_0} \, f_\theta(x)_{y_0} - f_\theta(x)_{y}.
        %\end{equation}
        %$OPT > 0$ iff the model is robust~(at $(x_0,\,y_0)$ w.r.t $\cL_p$ norm with radius $\epsilon$), and $OPT \le 0$ iff the model is non-robust.
        %\end{remark*}
       Based on the optimization perspective in \Cref{prob:verification-optimization-problem}, if $\cM$ is exactly solved, the corresponding verification approaches would be complete. However, although complete verification is attractive, the optimization problem $\cM$ is shown to be \NP-Complete~\cite{katz2017reluplex}, and it is even intractable to approximate with constant approximation ratio~\cite{weng2018towards}. This intrinsic barrier impedes complete verification approaches from scaling up to common neural network size. To overcome this \emph{scalability challenge}, the incomplete verification approaches aim to solve the relaxed problem, i.e., by computing the lower bound of $\cM$ which is more tractable.  However, the relaxations in existing approaches are typically too loose, which induces another problem identified as the \emph{tightness challenge}. As a result, the tradeoff between scalability and tightness constitute the major obstacles for robustness verification.
       
        
        
        
        %Among deterministic verification approaches, those solving the exact value of the problem are complete verification approaches, which are usually based on branch-and-bound strategy or existing MILP solvers and cannot scale to large neural networks;
        %those computing the lower bound of the problem are incomplete verification approaches, which are usually based on linear relaxations and their bounds may be loose.
        %The probabilistic verification approaches are typically based on randomized smoothing.
        %Within our knowledge, all existing probabilistic verification approaches are incomplete.
        %They usually make the model predict the most frequent class when the input is sampled from a distribution centered at the original input.
        %So they are not directly related to this optimization problem.
        
        
        
        \para{Robust training.}
        We refer to a training approach as \emph{robust training} if the it either explicitly or implicitly enhances the robustness certification. Robust training is typically related to or derived from corresponding verification approaches. It usually improves the certified robustness by optimizing additional quantities such as regularization terms, certification bounds, or by adding uncertainty during training.
        % \linyi{What is add uncertainties to model layers?}
        Robust training ensures a non-trivial robustness certification, and it is a strong complement for robustness verification approaches.
        %We deem a training approach as a \emph{robust training} approach if the trained model has non-trivial certified robustness.
        %Note that we do not consider empirical defenses which train robust model against existing attacks but failed to be verified.
        %The robust training approaches are usually closely related to or derived from certain verification approaches.
        
        % \para{Robustness verification.}
        % The goal of the \emph{robustness verification} is to certify the lower bound of model accuracy against \emph{any} $(\cL_p,\,\epsilon)$-adversary.
        % % The algorithm reads the neural network model $f_\theta$, the original input $x_0\in\bbR^n$, the true label $y_0\in [C]$, and the required radius $\epsilon$.
        % % The norm type $p$ is also explicitly or implicitly specified.
        % % When the algorithm returns ``true'', the model $f_\theta$ is robust at point $(x_0,\,y_0)$ against the strongest $(\cL_p,\,\epsilon)$ Adversary.
        % Furthermore, we define \emph{complete verification} which returns ``true'' \emph{if and only if} the model $f_\theta$ is robust at point $(x_0,\,y_0)$ against any $(\cL_p,\,\epsilon)$ Adversary.
        % The \Cref{def:verification-approach} formulates them.
        % \bo{there are two point of views: deterministic and probabilistic. }
        % \begin{definition}[Deterministic Robustness Verification Approach]
        %     Whenever a \emph{deterministic robustness verification approach} $\cA(f_\theta,\,x_0,\,y_0,\,\epsilon)$ outputs true,
        %     there is no $x \in B_{p,\epsilon}(x_0)$ such that $F_\theta(x) \neq y_0$.
        %     % \emph{any} $(\cL_p,\,\epsilon)$ adversary cannot find $x \in B_{p,\epsilon}(x_0)$ such that $F_\theta(x) \neq y_0$.
        
        %     Furthermore, if $\cA(f_\theta,\,x_0,\,y_0,\,\epsilon)$ outputs false, there exists $x \in B_{p,\epsilon}(x_0)$ such that $F_\theta(x) \neq y_0$, then $\cA$ is a \emph{complete robustness verification approach}.
            
        %     If $\cA$ is a robustness verification approach but not complete, we call it \emph{incomplete robustness verification approach}, i.e., when $\cA(f_\theta,\,x_0,\,y_0,\,\epsilon)$ outputs false, there may exist $x \in B_{p,\epsilon}(x_0)$ such that $F_\theta(x) \neq y_0$.
        %     \label{def:verification-approach}
        %     \label{def:complete-verification-approach}
        % \end{definition}
        % \bo{A robustness verification algorithm xxx is defined as: whenever Axxx = \emph{true},  xxxxx}
        
        
        %     An algorithm $\cA_p(f_\theta,\,x_0,\,y_0,\,\epsilon)$ which reads neural network model $f_\theta$, input to the model $x_0\in\cX$, true class label $y_0 \in [C]$, and $\ell_p$ radius $\epsilon > 0$ is called a \emph{robustness verification approach} \emph{if and only if}
        %     the strongest $(\cL_p,\,\epsilon)$ adversary cannot find adversarial examples in model $f_\theta$ when original input is $x_0$ and true label is $y_0$ if $\cA$ return true.
        %     \label{def:verification-approach}
        % \end{definition}
        % \bo{need check}
        % An identical definition is:
        % \begin{equation}
        %     \resizebox{0.49\textwidth}{!}{
        %     $
        %     \begin{aligned}
        %         & \cA_p(f_\theta,\,x_0,\,y_0,\,\epsilon) \text{ is a robustness verification approach} \\
        %         \Longleftrightarrow 
        %         & \cA_p(f_\theta,\,x_0,\,y_0,\,\epsilon) = True \Longrightarrow \forall x \in B_{p,\epsilon}(x_0), F_\theta(x) = y_0.
        %     \end{aligned}
        %     $
        %     }
        %     \label{eq:eqdef-verification-approach}
        % \end{equation}
        % % that, for any $x' \in B_{p,\epsilon}(x)$, $F_\theta(x') = y$, if $\cA_p(f_\theta,\,x,\,y,\,\epsilon)$ returns true. 
        % \begin{definition}[Complete Robustness Verification Approach]
        %     A \emph{robustness verification approach} $\cA_p(f_\theta,\,x,\,y,\,\epsilon)$ is called \emph{complete robustness verification approach} \emph{if and only if}
        %     $\cA$ returns true~(resp. false) if the strongest $(\cL_p,\,\epsilon)$ adversary cannot~(resp. can) find adversarial examples in model $f_\theta$ when original input is $x_0$ and true label is $y_0$.
        %     \label{def:complete-verification-approach}
        % \end{definition}
        % An identical definition is:
        % \begin{equation}
        %     \begin{aligned}
        %         & \cA_p(f_\theta,\,x_0,\,y_0,\,\epsilon) \text{ is a robustness verification approach} \\
        %         & \Longleftrightarrow \\
        %         & \cA_p(f_\theta,\,x_0,\,y_0,\,\epsilon) = True \Longleftrightarrow \forall x \in B_{p,\epsilon}(x_0), F_\theta(x) = y_0.
        %     \end{aligned}
        %     \label{eq:eqdef-complete-verification-approach}
        % \end{equation}
        % %that, for any $x' \in B_{p,\epsilon}(x), F_\theta(x') = y$, \emph{if and only if} $\cA_p(f_\theta,\,x,\,y,\,\epsilon)$ returns true.
        
        % \bo{mention deterministicxxx, probabilistic is incomplete.... }
        
        % \begin{remark*}
        %     Robustness verification approach provides a sufficient condition for model robustness;
        %     and complete robustness verification approach provides a sufficient and necessary condition for model robustness.
        %     The robustness verification approaches are related with adversaries, but also different from them.
        %     Concretely, verification approaches can certify that the model is robust, i.e., no adversarial examples, while adversaries can show that there is adversarial example.
        %     % , i.e, the model is non-robust.
        % \end{remark*}
        
        % % If a verification approach is not complete, we call it \emph{incomplete robustness verification approach}.
        % The robustness verification approaches are related with adversaries, but also different from them.
        % Concretely, verification approaches can certify that the model is robust, i.e., no adversarial examples, while adversaries can show that there is adversarial example, i.e, the model is non-robust.
        % % However, verification approaches may fail to certify if the model is truly robust, and the adversaries may fail to find out adversarial example if the model is truly non-robust.
        % % When such failure is eliminated, we obtain the complete verification approach and the strongest adversary, and these two are essentially the same.
        % Their relation is depicted in \cref{fig:relation-verifier-attack}.
        % % The verification approaches are important since they can certify the robustness against any present and future adversaries.
        % \begin{figure}
        %     \centering
        %     \includegraphics[width=0.48\textwidth]{figures/fig-relation-verifier-attack.pdf}
        %     \caption{Relation between adversaries and robustness verification approaches.}
        %     \label{fig:relation-verifier-attack}
        % \end{figure}
        
        % There are also a growing number of probabilistic robustness verification approaches.
        % The \emph{probabilistic robustness verification approaches} are a family of randomized verification approaches.
        % For non-robust input, the probability of certifying it to be robust is non-zero, though usually be small.
        
        % % should be smaller than $1 - p$.
        % These verification approaches 
        % % , where the randomness comes from the private random seed.
        % We define $p$-confident probabilistic robustness verification approach in \Cref{def:probabilistic-verification-approach}.
        % Intuitively, for non-robust input, the probability of making wrong verification should be smaller than $1 - p$.
        % The confident level $p$ should be very high to validate such approaches.
        % For example, many of these approaches choose $p = 99.9\%$.
        % % Most probabilistic robustness verification approaches are derived from differential privacy and randomized smoothing
        
        % \begin{definition}[$\alpha$-Confident Robustness Verification Approach]
        %     A randomized algorithm $\cA^s(f_\theta,\,x_0,\,y_0,\,\epsilon)$ 
        %     % which reads neural network model $f_\theta$, input to the model $x_0\in\cX$, true class label $y_0 \in [C]$, and $\ell_p$ radius $\epsilon > 0$ 
        %     is called a \emph{$p$-confident robustness verification approach} 
        %     \emph{if} for any supported $f_\theta$, $x_0$, $y_0$, and $\epsilon$,
        %     $$
        %     \begin{aligned}
        %         & \exists x \in B_{p,\epsilon}(x_0), F(x_0) \neq y_0 \text{ (exists adversarial examples)} \\
        %         \Longrightarrow & \Pr_s[\cA^s(f_\theta,\,x_0,\,y_0,\,\epsilon) = \text{true}] \le 1 - \alpha, \\
        %     \end{aligned}
        %     $$
        %     where $s$ is the private random seed taken by $\cA$.
        %     \label{def:probabilistic-verification-approach}
        % \end{definition}
        
        % Many robustness verification approaches have limited range of supported neural networks.
        % For example, some support only feed-forward ReLU networks~(\Cref{def:feed-forward-nn}).%, though feedforward ReLU networks are widely used.
        
        % Based on different robustness verification approaches, there are corresponding training strategies to to optimize such objectives directly, and we will introduce them for both \emph{deterministic} and \emph{probabilistic} verification. 
        
        % \para{Optimization view of robustness verification.}
        % We can also view robustness verification from the optimization perspective.
        % \begin{problem}[Robustness Verification as Optimization Problem]
        %     Given trained neural network $f_\theta: \cX \mapsto \bbR^C$, the original input $x_0 \in \cX$, the true label $y_0 \in [C]$, the target label $y \in [C]$, and the radius $\epsilon > 0$, define the following optimization problem:
        %     \begin{equation}
        %         \begin{aligned}
        %             \minimize_{x}\quad & f_\theta(x)_{y_0} - f_\theta(x)_{y} \\
        %             \text{s.t.}\quad & x \in B_{p,\epsilon}(x_0).
        %         \end{aligned}
        %         \label{eq:verification-optimization-problem}
        %     \end{equation}
        %     % Let the $OPT$ be the optimal value of the optimization problem.
        %     \label{prob:verification-optimization-problem}
        % \end{problem}
        % \bo{use as problem no theorem}
        % \begin{remark*}
        %     Given the solver for \Cref{prob:verification-optimization-problem}, we can enumerate all $C - 1$ different $y$'s and compute
        %     \begin{equation}
        %         OPT := \min_{y \in [C]: y \neq y_0} \, f_\theta(x)_{y_0} - f_\theta(x)_{y}.
        %         % \tag{3b}
        %         \label{eq:verification-optimization-problem-alternative}
        %     \end{equation}
        %     $OPT > 0$ iff the model is robust~(at $(x_0,\,y_0)$ w.r.t $\cL_p$ norm with radius $\epsilon$), and $OPT \le 0$ iff the model is non-robust.
        %     Thus, a solver computing the \emph{lower bound} of the problem can be used for robustness verification;
        %     a solver computing the \emph{exact value} of \Cref{prob:verification-optimization-problem} can be used for complete robustness verification.
        %     % If a solver can compute the \emph{lower bound} of the problem, the algorithm can be used for robustness verification.
        %     % Furthermore, if a solver can \emph{exactly} solve the problem, the algorithm can be used for complete robustness verification.
        %     % Given the solver for \Cref{eq:verification-optimization-problem}, we can enumerate all $C - 1$ different $y$'s and compute the corresponding \Cref{eq:verification-optimization-problem} respectively, thus results in an algorithm solving
        %     % % Note that the objective function in \cref{eq:verification-optimization-problem} is equivalent to
        %     % \begin{equation}
        %     %     OPT := \min_{y \in [C]: y \neq y_0} \, f_\theta(x)_{y_0} - f_\theta(x)_{y}.
        %     %     % \tag{3b}
        %     %     \label{eq:verification-optimization-problem-alternative}
        %     % \end{equation}
        %     % % Thus, the algorithm can enumerate all $C - 1$ different $y'$s, solve the corresponding problems, and compute the minimum of them as $OPT$.
        %     % % 
        %     % The above theorem directly follows from the observation that $OPT > 0$ if and only if the model is robust at point $x_0$ with respect to $\ell_p$ norm with radius $\epsilon$.
        %     % The theorem implies that, robustness verification problem is equivalent to checking the emptiness of the space $B_{p,\epsilon}(x_0) \cap \{x:\, OPT(x) \le 0\}$.
        % \end{remark*}
        
        % \para{Certifiably robust defense.} 
        % Unlike heuristic defenses which target at defending existing adversaries, \emph{certifiably robust defenses}, or \emph{certifiable defenses} for short, chase for ``ultimate robustness'', i.e., no adversary can break.
        % We deem a training approach as a \emph{certifiably robust defense} if the trained model has non-trivial robustness against \emph{any} $(\cL_p,\,\epsilon)$-adversary with non-trivial radius $\epsilon$.
        % Though complete verification approach can verify the robustness, 
        % % as debriefed in \cref{sec:challenge-robust-verification}, 
        % it is usually computationally intractable.
        % Therefore, in practice we favor the defenses which yield non-trivial certifiable robustness even verified by incomplete verification approaches.
        
        % A powerful heuristic defense is adversarial training~\cite{madry2017towards}, which approximately solves min-max problem:
        % $$
        %     \min_\theta \max_{x \in B_{p,\epsilon}(x_0)} l(f_\theta(x),\,y_0),
        % $$
        % where $l$ is the regular loss function such as cross-entropy loss.
        % % measuring distance of model prediction $f_\theta(x)$ from the correct label $y_0$ such as cross-entropy loss.
        % The inner maximization is instrinsically hard to solve due to non-convexity, and is usually approximated by heuristic attacks such as PGD attack. 
        % The outer minimization optimizes model parameters. % using common optimizers.
        % % such as stochastic gradient descent or Adam optimizer~\cite{kingma2014adam}.
        % Many certifiably robust defenses use this framework, but substitute the inner maximization by the upper bound found by verification approaches.
        % % ~(as shown by \cref{thm:verification-optimization-problem}).
    
    
    
    %\subsection{Challenges of Robustness Verification}
    %    \label{sec:challenge-robust-verification}
    %    \para{Scalability Challenge.}
    %    A pessimistic result for robustness verification is that, the complete robustness verification is not only \NP-Complete~\cite{katz2017reluplex}, but also intractable even if we want to know only the robustness radius with constant approximation ratio~\cite{weng2018towards}.
    % ----------------------------------------------------
        % which is shown below as \cref{thm:hardness-1} and \cref{thm:hardness-2}.
        %
        % \begin{theorem}[\NP-Completeness, \citeauthor{katz2017reluplex}]
        %     The complete robustness verification $\cA$ which takes feed-forward ReLU network as the input is \NP-complete.
        %     \label{thm:hardness-1}
        % \end{theorem}
        % The theorem is proved by constructing a neural network which encodes arbitrary $3$-SAT formula so that complete robustness verification can be reduced to satisfiability check, thus the complete robustness verification problem is reduced to $3$-SAT satisfiability problem, which is a well-known \NP-complete problem.
        %
        % \begin{theorem}[Approximation Hardness, \citeauthor{weng2018towards}]
        %     A $k$-approximation to the complete robustness verification problem guarantees that if model $f$ is robust for any inputs in $B_p(x, r)$, then the algorithm $\cA_p(f_\theta,\,x_0,\,y_0,\,\epsilon)$ returns true for any $\epsilon \le r / k$.
        %
        %     Unless \P = \NP, there is no polynomial time algorithm that gives $(1 - o(1))\ln n$-approximation to the complete robustness verification problem for feed-forward ReLU networks.
        %     \label{thm:hardness-2}
        % \end{theorem}
        % The proof is also done by construction, which reduces the approximation to the complete robustness verification of classical Approximate $\mathsf{SET}\text{-}\mathsf{COVER}$ problem, which is known to be hard~\cite{raz1997sub,alon2006algorithmic,dinur2016mildly}.
        %
        % Viewing from optimization, the hardness falls in general $\NP$-hardness of solving non-convex optimization problems because of the non-convexity of neural networks.
        % Since neural networks are normally non-convex, the problem is generally hard to solve, 
        % To summarize, 
        %This intrinsic barrier impedes complete verification approaches from scaling up to common neural network size.
        % i.e., the \emph{scalability challenge}.
        
        %To qualify the scalability of verification approach, in later text we characterize the approach scalability by their supporting datasets.
        %Models for ACAS~\cite{katz2017reluplex} dataset typically have $< 300$ neurons.
        %Models for MNIST~\cite{lecun1998gradient} dataset typically have $1,000 - 10,000$ neurons.
        %Models for CIFAR-10~\cite{krizhevsky2009learning} dataset typically have $10,000 - 100,000$ neurons.
        %Models for ImageNet~\cite{russakovsky2015imagenet} dataset typically have $100,000$ - $1$ million neurons.
        %The scalability of approaches to be reviewed vary from ACAS to ImageNet.
        
        % \bo{deterministic, probabilistic xxxx}
        
        %\para{Tightness Challenge.}
        %One may turn to solving the relaxation of the verification problem, i.e., deriving the (incomplete) verification approach.
        %However, the relaxations in existing verification approaches are typically too loose.
        %The deterministic verification approaches usually fail to verify robustness even though the model is truly robust, unless the model is deliberately trained to be easily verified.
        %The probabilistic verification approaches usually fail to certify large radius $\epsilon$, especially against $\cL_\infty$ adversary.
        % A typical verification approach, interval bound propagation, propagates the intervals through the neural network layers.
        % However, direct interval bound propagation usually yields very loose bounds~\cite{gowal2019scalable}.
        % Besides this, many existing verification approaches are shown to be loose, i.e., usually fail to verify robustness even though the model is truly robust, unless the model is deliberately trained to be certifiably robust~\cite{xiao2018generating,wong2018provable}.
        %We call it \emph{tightness challenge}.
        
        %Both \emph{scalability} and \emph{tightness} are major challenges for robustness verification approaches.
        %And there exists a trade-off between them.
        % Moreover, for certifiably robust defenses, since they are usually based on bound found by verification approaches, they require even higher requirements to the verification approaches: nearly real-time computation speed, and the differentiability.
        % \bo{deterministic, probablistic xxx}

\section{Taxonomy of Robustness Verification and Robust Training Approaches}
    \label{sec:main-taxonomy}

    In this section, we will first provide a taxonomy of existing robustness verification and robust training approaches~(\Cref{fig:tree-categorization}), and then discuss several representative approaches and their connections in details.
    % \linyi{Change ``representative studides'' to ``representative approaches'' since here every object to discuss is a concrete approach.}
    % After that, we present some theoretical findings.
    % We close this section by a short discussion.

    % \bo{1. taxonomy based on optimization methods, + table 2. introduce the methods based on each category}
    
     \subsection{Taxonomy and Overview}
     
        % \begin{wrapfigure}{r}{0.48\textwidth}
        %     \centering
        %     \resizebox{!}{0.70\textheight}{\input{figures/approach-tree}}
        %     \caption{Classification of main $\cL_p$-based verification and certifiable robust defenses according to their main methods.
        %     The approaches are clustered hierarchically.
        %     Each leaf node represents a concrete approach.
        %     Among them, \colorbox{red!50}{red boxes} are pure verification approaches, \colorbox{red!20}{light red boxes} are pure defenses, and \colorbox{red!80}{dark red boxes} are those with both verification approaches and defenses.}
        %     \label{fig:tree-categorization}
        %     \vspace{-8mm}
        % \end{wrapfigure}
        \begin{figure*}
            % \hspace{-0.15\textwidth}
            \NoHyper
            \centering
            \resizebox{1.0\linewidth}{!}{\input{figures/approach-tree}}
            % \vspace{-1.5em}
            
            % \resizebox{!}{0.85\textheight}{\input{figures/approach-tree}}
            
            \caption{Taxonomy tree of representative robustness verification and training approaches against $\cL_p$ adversary.
            The approaches are clustered hierarchically based on their core methodology.
            The rounded boxes contain category names.
            The subsections where each category of the approaches is introduced in details are \textbf{bolded}.
            The leaf nodes contain references of corresponding approaches, where normal font denotes the {robustness verification approaches}, \textbf{bold} font denotes both robustness verification and training, and \textit{italic} font denotes robust training approaches.}
            \label{fig:tree-categorization}
            \vspace{-1.5em}
        \end{figure*}
     
        We present the taxonomy tree of major robustness verification and robust training approaches in \Cref{fig:tree-categorization}.
        % The main criteria is the core techniques of these approaches. 
        % \linyi{existing $\mapsto$ these.}
        Note that the robust training approaches are placed in the taxonomy tree alongside their closely-related verification approaches.
        In addition, we present an extended summary table of these approaches in \Cref{sec:adx-full-taxonomy-table}.
        
        In the following subsections, we will introduce the major verification and training approaches by category.
        \Cref{sec:complete-verification,sec:lp-relaxation-intro,sec:sdp-intro,sec:lipschitz-intro}
        introduce \textit{deterministic approaches}.
        Among them, \Cref{sec:complete-verification} introduces complete approaches, and \Cref{sec:lp-relaxation-intro,sec:sdp-intro,sec:lipschitz-intro} introduce incomplete approaches.
        The incomplete approaches can then be further divided into linear relaxations~(\Cref{sec:lp-relaxation-intro}), semi-definite programming~(SDP)~(\Cref{sec:sdp-intro}), and Lipschitz or curvature bound~(\Cref{sec:lipschitz-intro}).
        \Cref{sec:probabilistic-robustness-verification-root} will introduce the  \textit{probabilistic approaches}.
        We label the corresponding subsections for each category in the taxonomy tree~(\Cref{fig:tree-categorization}).
        
        To characterize the scalability of discussed verification approaches, we measure the scalability based on the largest model size for corresponding dataset.
        Models for ACAS~\cite{katz2017reluplex} dataset typically contain $<300$ neurons;
        MNIST~\cite{lecun1998gradient} --- $1,000 \sim 10,000$ neurons;
        CIFAR-10~\cite{krizhevsky2009learning} --- $10,000 \sim 100,000$ neurons;
        and ImageNet~\cite{russakovsky2015imagenet} --- $100,000 \sim 1$ million neurons.
        Thus, we can coarsely measure the scalability based on the supported datasets of the verification approaches.
        We observe that the scalability varies from ACAS to ImageNet.
        
        % % The defenses are usually based on verification approaches and specifically train models to be easier verified by the base verification approach, so we group them alongside the corresponding verification approaches.
        % The blue boxes are the category names, which usually indicate the main core methods.
        % The leaf nodes are concrete approaches, where normal red boxes stand for verification approaches, light red boxes stand for defenses, and dark red boxes stand for both verification approaches and defenses.
        
        % We also present an extended table of major verification and certifiably robust defenses against $\cL_p$ adversaries in \Cref{sec:adx-full-taxonomy-table}, which shows the supported $\cL_p$ norm, whether the verification is exact, whether the work contains certifiably robust defenses, and its scalability.
        % % The ``Main Techniques'' column summarizes the main techniques used in these works.
        % % The ``Verification'' column records whether the verification approach is complete, and the types of $\cL_p$ norms it supports.
        % % In ``Certifiably Robust Defenses'' column, the works which propose new certifiable robust defenses are labeled.
        % % Finally, we record the scalability of these approaches, which is measured by the largest dataset used in their conducted experiments.
        % % Normally, the larger the dataset is, the larger the neural network is, and the higher scalability it achieved.
        
        % At high level, these approaches can be divided into two large sectors: deterministic approaches and probabilistic approaches.
        % Among deterministic approaches, there are two main categories: complete verification, and incomplete verification~(relaxation-based verification approaches).
        % These incomplete verification approaches mainly use linear-based relaxation, semidefinite programming~(SDP) based relaxation, and local Lipschitz-based relaxation.
        % Another sector includes probabilistic approaches, which are incomplete and mostly based on randomized smoothing.
        % % In \cref{sec:probabilistic-robustness-verification-root} they are discussed in detail.
        % In following text, we discuss each major approach.
        % Since the majority of these works are verification approaches, we follow the logic line of verification approaches, and certifiably robust defenses are mainly introduced alongside their closely-related verification approaches.

 \subsection{Complete Verification}
    \label{sec:complete-verification}
 
    In this subsection, we introduce complete robustness verification approaches, which is a branch of \textit{deterministic verification}.
    These approaches usually consider $\cL_\infty$ adversary and mainly support feed-forward ReLU networks~(see \Cref{def:feed-forward-nn}).
    % So, 
    % by default, 
    % we assume $\cL_\infty$ adversary hereafter unless noted otherwise.
    % \linyi{Delete ``by default'' to save some space.}
    % Furthermore, they mainly support feed-forward ReLU networks, so we start from investigating this specific neural network class.
    
    \para{Neuron Classification.}
        Many complete verification approaches rely on the activation patterns within neural networks, so we provide a classification of neurons for later use.
        \begin{definition}[Neuron Classification for Feed-Forward ReLU Networks]
            % For any given input $x$, the input to any neuron $n$ in the feed-forward ReLU network is either $< 0$ or $\ge 0$.
            % If the input to $n$ is $< 0$, the neuron $n$ is \emph{inactive}.
            % If the input is $\ge 0$, the neuron $n$ is \emph{active}.
            Let $n$ be a neuron in a feed-forward ReLU network.
            For given input $x$, if the input to $n$ is $< 0$, we call $n$  \emph{inactive}, otherwise \emph{active}. %if the input to $n$ is $\ge 0$, we call $n$ is \emph{active}.
            Let $\cS$ be an input region, for any $x \in \cS \subseteq \cX$, if we can certify that input to $n$ is always $> 0$ or $\le 0$, we call neuron $n$ \emph{stable}
            % ~(always active or inactive) 
            with respect to region $\cS$; otherwise we call $n$ \emph{unstable}.
            % with respect to region $\cS$.
            \label{def:active-inactive-relu-neuron}
        \end{definition}
        \begin{remark*}
            When a neuron $n$ is stable, it serves as a constant linear mapping as $y = 0$ or $y = x$ for the network.
            % for any input in region $\cS$.
        \end{remark*}
    
    \para{Piecewise-Linear Property.}
    % 
    % \para{Properties of Feed-Forward ReLU Networks.}
    %     We first investigate some properties of feed-forward ReLU networks.
    %     For given input, we can classify their neurons according to their activation patterns.
        % 
    %     % \begin{remark*}
    %         % The stable neurons correspond to linear mappings in the whole input region $\cS$; while unstable neurons correspond to only pointwise or piecewise linear mappings.
    %     % \end{remark*}
    %     % No matter whether the neuron is active or not, it is linear to the input locally.
        % 
        Since each ReLU neuron outputs $\relu(x) = \max\{x,\,0\}$, it is always locally linear within some region around input $x$.
        Since feed-forward ReLU networks are the composition of these piecewise linear neurons and (linear) affine mappings, \emph{the output is locally linear w.r.t input $x$.}
        This property is formally stated and proved in \cite{jordan2019provable}.
        It serves as the foundation for many verification approaches.
        
        Next we will introduce different type of complete verification approaches in detail.
        
        % Concretely, we have \Cref{thm:piecewise-linear-theorem}, which is formally stated and proved in \cite{jordan2019provable}.
        % % though has been widely exploited before.
        % The theorem serves as the foundation for many verification approaches.
        % \begin{theorem}
        %     \label{thm:piecewise-linear-theorem}
        %     Feed-forward ReLU Networks are \emph{piecewise linear}.
        % \end{theorem}
        % % A formal proof and extensions of this theorem can be found in 
        % % For example, we can enumerate all piecewise linear regions in $B_{p,r}(x_0)$ by enumerating every combination of neuron state and solve the corresponding linear programming problems to completely verify robustness with respect to input $x_0$.
    % 
    \subsubsection{\textbf{Branch-and-Bound}\texorpdfstring{~\cite{ehlers2017formal,katz2017reluplex,bunel2018unified,gehr2018ai2,wang2018formal,wang2018efficient}}{}}\hfill\\
    % 
         To solve the verification on feed-forward ReLU networks (\Cref{def:feed-forward-nn}), some work~\cite{pulina2010abstraction,pulina2012challenging} directly models it as an SMT problem, so that a complete verification could be directly performed via an off-the-shelf SMT solver such as Z3~\cite{de2008z3}. However such verification is usually too slow to be practical~\cite{katz2017reluplex}.%The SMT formula for ReLU directly
        %\begin{equation}
        %    \left( (\hz_{i,j} \ge 0)\,\wedge\, (z_{i,j} = \hz_{i,j}) \right) 
        %    \vee 
        %    \left( (\hz_{i,j} < 0)\,\wedge\, (z_{i,j} = 0) \right)
        %    \label{eq:relu-smt-formula}
        %\end{equation}
        %enables complete robustness verification using off-the-shelf SMT solver such as Z3~\cite{de2008z3}.
        %However such verification is normally too slow to be practical~\cite{katz2017reluplex}.
        
        % Let the data input be $(x_0,\,y_0)$ where $x_0 \in \cX$ is the original input and $y_0 \in [C]$ is the true label.
        % Knowing from the optimization problem formulation~(\Cref{eq:verification-optimization-problem}), we only need to check whether there exists a point~(adversarial example) $x \in B_{p,\epsilon}(x_0)$ such that $f(x)_{y_0} < \underset{{y\in[C]:y\neq y_0}}{\max} f(x)_y$.
        % % Inspired from the above brute-force search, 
        % We can express each ReLU constraint 
        % $
        %     z_{i,j} = \relu(\hz_{i,j})
        % $ 
        % where $2 \le i \le l$ and $1 \le j \le n_i$ as a SMT formula:
        % \begin{equation}
        %     \left( (\hz_{i,j} \ge 0)\,\wedge\, (z_{i,j} = \hz_{i,j}) \right) 
        %     \vee 
        %     \left( (\hz_{i,j} < 0)\,\wedge\, (z_{i,j} = 0) \right).
        %     \label{eq:relu-smt-formula}
        % \end{equation}
        % Since the norm type $p=\infty$, the input constraint $x\in B_{p,r}(x_0)$ can be expressed by linear constraints $x_0 - r \le x \le x_0 + r$.
        % In addition, the affine constraints $\hz_{i+1} = \bW_iz_i+ b_i$ and the adversarial condition $f(x)_{y_0} < \max_{y\in[C]:y\neq y_0} f(x)_y = \bigvee_{y\in[C]:y\neq y_0} f(x)_{y_0} < f(x)_y$ are also linear.
        % Thus, with only linear constraints, the overall verificaiton problem is a SMT formula and we can leverage existing SMT solvers such as Z3~\cite{de2008z3} or Gurobi to do complete verification.
        % However, such verification is usually too slow to be practical.
        
        As a more practical approach, \t{Planet}~\cite{ehlers2017formal} adopts the branch-and-bound strategy. 
        % The key idea can be summarized as: first relax then tighten the  by divide-and-conquer. 
        The verification problem is essentially a non-linear optimization problem  (\Cref{prob:verification-optimization-problem}), where the main non-linearity comes from the non-linear activation functions. Thus, they propose to first use the linear polytope (\Cref{def:tightest-linear-polytope}) to replace the ReLU activation's non-linear constraints at the cost of looseness, and provide a lower bound of $\cM(y_0,y_t)$. If the lower bound is already non-negative, then the certification could be made. If not, we can always tighten the relaxation by splitting an unstable (\Cref{def:active-inactive-relu-neuron}) ReLU neuron into two versions --- always active and always inactive, i.e. splitting the original one optimization problem into two sub-problems by adding specific conditions and solve them respectively. Then they will repeatedly follow this strategy in a divide-and-conquer way, constantly tighten the relaxation until the certification is made or all of the unstable neurons are already split where the relaxation is totally removed.
        
       % l\textcolor{green}{As an improvement,} Planet~\cite{ehlers2017formal} adopts branch-and-bound strategy for verification \textcolor{green}{so that faster? but at cost of ? link up with the 1-st para.}.
        %At high level, it starts from an over-approximated region for output $\cS_o \supseteq \cS := \{f(x):\,x\in B_{p,\epsilon}(x_0)\}$ which is easy to compute but loose.
        %If no adversarial example could be found \textcolor{green}{what is relationship between adv examples and the relaxed output region... Not clear.}, we choose an unstable neuron to split and work on the resulting regions: $\cS_o \cap \{x:\,z_{i,j}\text{ is always active}\}$ and $\cS_o \cap \{x:\,z_{i,j}\text{ is always inactive}\}$. \textcolor{green}{(where is $x$ from? $x\in ...$)}
        %In Planet, a random neuron is chosen to split.
        %After all neurons are split, the resulting regions can all be described by linear constraints. Thus, the verification problem is reduced to a linear programming~(LP).
        %Thus, we can solve linear programming~(LP) problems for verification.
        
        %The over-approximated region used in Planet is the tightest polytope for ReLU as defined in \Cref{def:tightest-linear-polytope}, which can be expressed by linear constraints.
        %Thus, again, we can verify the robustness in this over-approximated region using LP.
        % In \cite{ehlers2017formal}, Planet is proposed, which is later summarized~\cite{bunel2018unified} as a type of the branch-and-bound approach.
        % In high level, branch-and-bound approach starts from an over-approximation region $\cS_o \supseteq \cS := \{f(x):\,x\in B_{p,\epsilon}(x_0)\}$.
        % The $\cS_o$ should be easy to compute, for example, bounded by only linear constraints, but may be too loose.
        % If there may be adversarial example in over-approximated region, we adopt a policy to choose a neuron $z_{i,j}$ to split the region, i.e., consider when $z_{i,j}$ is active and when $z_{i,j}$ is inactive.
        % As the result, we try to certify whether there is adversarial example in $\cS_o \cap \{x:\,z_{i,j}\text{ is active}\}$ and $\cS_o \cap \{x:\,z_{i,j}\text{ is inactive}\}$.
        % When all neurons are split, the resulting region can be expressed by linear constraints thus we only need to solve a linear programming problem for robustness verification.
        % % Among them, the region certified to have no adversarial example is crossed off, the region with adversarial example suggests we have verified the input is non-robust, and the region fail to certify and find adversarial examples is split recursively.
        % % The algorithm can terminate since when all neurons are split, where the resulting region is a linear-bounded region which is easy to completely certify~(just by solving a linear programming problem)
        
        % Planet~\cite{ehlers2017formal} over-approximate the region by outer linear constraints.
        % Concretely, Planet proposes the polytope constraints as shown in \Cref{def:tightest-linear-polytope}.
        % Thus, the over-approximation region is bounded by linear constraints, and we can completely certify the existence of adversarial examples using linear programming.
        % Planet chooses \emph{random} neuron to split.
        % % when there is adversarial example in the over-approximation region.
        % After splitting, the new constraint that the neuron is active or not corresponds to $z_{i,j} \lessgtr 0$, which is an another linear constraints capable of linear programming-based certification.
        % % In addition, Planet supports max-pooling layers.
        
        \begin{definition}[ReLU Polytope]
            For neuron $z_{i,j} = \relu(\hz_{i,j})$, let $l_{i,j}$ and $u_{i,j}$ be the lower bound and upper bound of its output when the input region is $B_{p,\epsilon}(x_0)$:
            \begin{equation}
                l_{i,j} \le \min_{x\in B_{p,\epsilon}(x_0)} \hz_{i,j}(x) \le
                \max_{x\in B_{p,\epsilon}(x_0)} \hz_{i,j}(x) \le u_{i,j}.
                \label{eq:l-u-bound-for-relu}
            \end{equation}
            Then, if $l_{i,j} < 0 < u_{i,j}$, neuron $z_{i,j} = \relu(\hz_{i,j})$ can be bounded by linear constraints:
            \begin{equation}
                z_{i,j} \ge 0,\, z_{i,j} \ge \hz_{i,j},\, z_{i,j} \le \dfrac{u_{i,j}}{u_{i,j} - l_{i,j}} (\hz_{i,j} - l_{i,j}).
                \label{eq:linear-relu-0}
            \end{equation}
            We call this set of constraints \emph{the polytope for ReLU}.
            \label{def:tightest-linear-polytope}
        \end{definition}
        
        % The polytope is the bounded intersection of finitely many half-spaces.
        We show a polytope for ReLU in \Cref{fig:tightest-linear-polytope}.
        We can see that when both $l_{i,j}$ and $u_{i,j}$ are tight, 
        % i.e., $l_{i,j} = \min_{x\in B_{p,\epsilon}(x_0)}$ and $\max_{x\in B_{p,\epsilon}(x_0)} \hz_{i,j}(x) = u_{i,j}$, 
        the polytope is the tightest convex hull for this ReLU neuron.
        This polytope is widely used \cite{wong2018provable,wong2018scaling,tjeng2018evaluating}.
        % 
        An important issue regarding using this polytope comes from computing $l$ and $u$.
        The computation of tight $l$ and $u$ is $\NP$-complete.
        A practical solution is to compute the $l$ and $u$ from linear relaxation of previous layers, which yields an iterative algorithm.
        % , since the previous layers already have linear relaxation by then.
        More discussion is in \Cref{sec:lp-relaxation-intro}.
        Once the relaxation is used for all unstable neurons, the constraints for the verification problem are linear.
        Thus, we can use linear programming~(LP) to derive the certification.

        
        Several improvements of \t{Planet}~\cite{ehlers2017formal} come from better neuron split heuristics, and tighter $l$ and $u$ bounds, such as \t{BaB}~\cite{bunel2018unified} and \t{BaBSR}~\cite{bunel2019branch}.
        % BaB~\cite{bunel2018unified} improves Planet by splitting over input range which produces more stabilized neurons, and improving its $l$ and $u$ bound.
        % BaBSR~\cite{bunel2019branch} further improves BaB by better branching strategy and also provides an in-depth comparision of complete verification approaches, though not on common datasets like MNIST or CIFAR-10.
        We note that \t{Reluval}~\cite{wang2018formal} and \t{Neurify}~\cite{wang2018efficient}, though derived from different perspectives, are similar to \t{Planet}, where the differences lie in the forms of over-approximation and the split policies.
        %  Reluval~\cite{wang2018formal} is a verification approach proposed at early stage.
        % In Reluval, we maintain the tight linear bound for stable neurons layer by layer.
        % % Since the neuron is stable, the local behavior of neural network is also linear and the bound is tight.
        % However, when it confronts unstable neurons, the linear bound can no longer be maintained.
        % % since we do not know whether $z_{i,j} = \relu(\hz_{i,j})$ equals to $z_{i,j} = \hz_{i,j}$ or $z_{i,j} = 0$.
        % In this case, Reluval concretizes the linear bound to numerical bound, i.e., compute $l$ and $u$, then proceeds.
        % The process can be viewed as an improvement on IBP-based verification, since it maintains tighter linear bound instead of just numerical interval when possible.
        % Reluval further introduces splitting operation to do complete verification, which shares similar ideas with branch-and-bound approaches~(\Cref{sec:complete-verification}).
        % % The original goal of Reluval is for complete verification.
        % % To do so, it produces the split operation: 1)~choose the numerical interval of an unstable neuron, namely $[l_x,\,u_x]$; 
        % % 2)~split it evenly, namely $[l_x,\,(l_x+u_x)/2]$ and $[(l_x+u_x)/2,\,u_x]$;
        % % 3)~check if there is adversarial in each resulting interval heuristically, and propagate the interval if not find.
        % % Reluval selects the neuron to split based on a few heuristics such as influence analysis, gradient magnitude, etc.
        % % The idea can be categorized to BaB framework discussed in \cref{sec:complete-verification}.
        % Reluval is evaluated on ACAS Xu and MNIST dataset, and has significant improvement over Reluplex when used for complete verification.
        % % - the state-of-the-art at that time.
        % % 
        % Neurify~\cite{wang2018efficient} further improves Reluval by combining it with linear relaxations the same as Fast-Lin.
        % In Neurify, when the linear relaxation fails to certify, the interval of some heuristically chosen neuron is split.
        % % $[l_x,\,u_x]$ is split to $[l_x,\,0]$ and $[0,\,u_x]$ similar as Reluval.
        % % The neuron choosing is choosing the neuron with larger gradient.
        % Neurify significantly improves the results of Reluval and Reluplex.
        % % Though the direct comparison with other approaches is lacked.
        % We can view Reluval as combining interval bound propagation with branching, and Neurify as combining linear inequality propagation with branching.
        
        Similarly, \t{AI$^2$}~\cite{gehr2018ai2} and \t{Reluplex}~\cite{katz2017reluplex} also partially use the branch-and-bound strategy. \t{AI$^2$}~\cite{gehr2018ai2} maintains a limited number of polyhedrons, which is called a type of abstract interpretations in the paper. The polyhedrons are propagated through the neural network layer by layer. When there are unstable neurons, relevant polyhedrons are split.
        % 
        % In essence, due to the piecewise linear nature, the input domain of feed-forward neural network $f$ can be divided to finite set of polyhedra domains where $f$ is linear in each domain.
        % Concretely, when confronting a ReLU neuron, it checks whether the neuron could be unstable.
        % If so, it splits the domains.
        % 
        \t{Reluplex}~\cite{katz2017reluplex} extends the simplex method which is widely used to solve LP to robustness verification.
        % In each iteration, the simplex method finds ascending edges to ``climb'' until it reaches global optima via updating variables with loose constraints.
        Comparing with classical simplex method, \t{Reluplex} additionally takes ReLU constraints into account.
        \t{Reluplex} permits temporary violation of ReLU specifications.
        In each iteration, it either fixes such violation, or performs normal operation as in simplex method for optimization.
        After a certain ReLU neuron is fixed too many times, the neuron is split and the resulting subproblems are solved in parallel.
        % which is its so-called branching strategy or split strategy.
        
        
        All the approaches above are complete and would need exponential time in the worst-case.
        As for practical performance, all approaches are evaluated and performed  on small models with small datasets like ACAS~\cite{julian2016policy}.
        % Reluplex is inferior than Planet and BaB.
        % According to the evaluation in \cite{ehlers2017formal}, the actual efficiency of Planet and BaB are comparable.
        % Even though BaB requires significantly fewer splits, due to the complex strategy, the certification process for each region is slower.
        On larger datasets such as MNIST with larger network, 
        \t{Planet} takes several hours per input, while \t{Reluval}, \t{Neurify}, and \t{AI$^2$} can solve in reasonable time only when the model size is strictly controlled.
        % Planet takes several hours per input for non-trivial radius $\epsilon$ and BaB does not report.
        % Reluval and Neurify can work on MNIST if the neural network size is small, and these two both outperform Reluplex significantly.
        % Moreover, from our evaluation, AI2 also performs well on MNIST when the neural network size is relative small.
        
        % the branching strategy of Planet by splitting over input range.
        % Also 
        % In BaB~\cite{bunel2018unified}, a few new branching and over-approximation computation strategies are proposed.
        % The new branching strategy is to split the input features, i.e., the $x_i \in [l_i,\,u_i]$ in previous over-approximation is replaced by two regions $x_i \in [l_i,\,(l_i + u_i)/2]$ and $x_i \in [(l_i + u_i)/2,\,u_i]$, which encourages more stabilized neurons after each split.
        % The over-approximation computation in Planet is improved by tighter $l$ and $u$.
        % BaBSR~\cite{bunel2019branch} further improves BaB by better branching strategy and also provides an in-depth comparision of complete verification approaches, though not on common datasets like MNIST or CIFAR-10.
        
        % AI2~\cite{gehr2018ai2} maintains bounded powerset domains for neural network verification, which is called a type of abstract interpretation in their work.
        % In essence, due to the piecewise linear nature~(\cref{thm:piecewise-linear-theorem}), the input domain of feed-forward neural network $f$ can be divided to finite set of polyhedra domains where $f$ is linear in each domain.
        % Each ReLU neuron split or branching corresponds to a split towards this, and when all neurons are split, we can yield the final set.
        % A variant of AI2 maintains such set of polyhedra domains through the neural network layer by layer to do complete verification.
        % Concretely, when confronting a ReLU neuron, it checks whether the neuron could be unstable.
        % If so, it splits the domains.
        % For acceleration, AI2 can limit the number of polyhedra domains it maintains, and heuristically merges domains with closest distance when the number exceeds.
        % When two polyhedra domains are merged, the resulting domain may not be a polyhedra, therefore an over-approximation is introduced, which drives the verification to be incomplete in this case.
        
        % All these approaches are complete thus has worst-case exponential time complexity.
        % In term of evaluation, all approaches are evaluated and perform well on small models for datasets like ACAS~\cite{julian2016policy}.
        % Reluplex is inferior than Planet and BaB.
        % According to the evaluation in \cite{ehlers2017formal}, the actual efficiency of Planet and BaB are comparable.
        % Even though BaB requires significantly fewer splits, due to the complex strategy, the certification process for each region is slower.
        % On larger datasets like MNIST, however, Planet takes several hours per input for non-trivial radius $\epsilon$ and BaB does not report.
        % AI2 does not present evaluation using polyhedra domain, so it is not comparable with others.
    
    \subsubsection{\textbf{MILP-Based Approaches}\texorpdfstring{~\cite{ehlers2017formal,cheng2017maximum,lomuscio2017approach,tjeng2018evaluating,xiao2018training}}{}}\hfill\\
        Several approaches model robustness verification as a mixed integer linear programming~(MILP) problem.
        %The mixed integer linear programming~(MILP) problem is extended from LP problem: MILP permits integer constraints on some variables.
        %This extension enables the robustness verification of feed-forward ReLU neural networks to be exactly encoded as MILP problem.
        Unlike LP, the MILP problem is able to model the verification without relaxation.
        % There are off-the-shelf MILP solvers such as Gurobi~\cite{gurobi}.
        % Coincidentally, branch and bound~\cite{clausen1999branch} is also widely used for this general class of optimization problems.
        
        \t{Sherlock}~\cite{dutta2017output} leverages MILP solver to find the tightest lower and upper bound of neuron outputs, i.e., $l$ and $u$.
        % The finding process is an interation of local search and global search where local search uses PGD and global search uses MILP solver.
        % % In Sherlock~\cite{dutta2017output}, the goal is to find the tightest lower and upper bound, i.e., $l$ and $u$.
        % The finding process is an iteration of local search and global search.
        % In local search, the projected gradient descent is used.
        % When the local search reaches local optima, Sherlock formulates the search of better solution as an MILP problem and leverage MILP solver to find it out.
        % If no solution is found, the global optima is found, otherwise the solution serves as another starting point of local search.
        The $l$ and $u$ can be leveraged to improve the tightness of existing verification approaches.
        % such as \Cref{def:tightest-linear-polytope}.
        % \cite{bunel2018unified} improves Planet~\cite{ehlers2017formal} in this fusion.
        
        In \t{Reachability}~\cite{lomuscio2017approach} and \t{ChengMIP}~\cite{cheng2017maximum}, for unstable neuron $z_{i,j}$~(the neuron could be both active or inactive), the constraint of $z_{i,j} = \relu(\hz_{i,j})$ is encoded by the following constraints:
        \begin{equation}
            \small
            \left\{
            \begin{aligned}
                & z_{i,j} \ge 0, \quad z_{i,j} \ge \hz_{i,j}, \\
                % & z_{i,j} \le \hz_{i,j} + M_{i,j}(1-a_{i,j}), \\
                & z_{i,j} \le Ma_{i,j}, \quad z_{i,j} \le \hz_{i,j} + M_{i,j}(1-a_{i,j}), \\
            \end{aligned}
            \right.
            \label{eq:milp-relu-form-1}
        \end{equation}
        where $M_{i,j} = \max \{ |l_{i,j}|, |u_{i,j}| \}$, and $a_{i,j} \in \{0,\,1\}$ is the newly introduced binary decision variable.
        When $a_{i,j} = 0$, $z_{i,j}$ is inactive; otherwise it is active.
        Thus the encoding precisely expresses ReLU.
        % In Bounded MILP~\cite{tjeng2018evaluating}, the encoding is further improved to: 
        % \begin{equation}
        %     \left\{
        %     \begin{aligned}
        %         & z_{i,j} \ge 0, \quad z_{i,j} \ge \hz_{i,j}, \\
        %         & z_{i,j} \le \hz_{i,j} - l_{i,j}(1-a_{i,j}), \\
        %         & z_{i,j} \le u_{i,j}a_{i,j}.
        %     \end{aligned}
        %     \right.
        %     \label{eq:milp-relu-form-2}
        % \end{equation}
        In \t{Bounded MILP}~\cite{tjeng2018evaluating}, the encoding is further improved by using the lower bound $l_{i,j}$ and upper bound $u_{i,j}$ separately instead of just $M_{i,j}$, which boosts the solving process significantly in practice.
        Recently, \citeauthor{anderson2020strong}~\cite{anderson2020strong} provide rigorous analysis and a novel and efficient approach on modeling robustness verification using MILP.
        % and generalization on modeling using MILP efficiently.
        % It also proposes efficient verificaiton approach which claims to be more efficient than all others.
        % 
        % Using linear relaxation propagation~\ref{sec:lp-relaxation-intro}, we can compute imprecise but usable $l_{i,j}$ and $u_{i,j}$.
        % Comparing with \cref{eq:milp-relu-form-1}, it substitutes the general bound $M_{i,j}$ to more precise $l_{i,j}$ and $u_{i,j}$, which accelerates the branch and bound in MILP solvers in practice.
        % 
        % ChengMIP additionally supports $\cL_1$ robustness verification by encoding the constraint that $\|x - x_0\|_1 = \sum_{i=1}^n |x - x_0| \le \epsilon$, which could also be supported by Reachability and Bounded MILP if we compute $l$ and $u$ using $B_{\infty,\epsilon}(x_0)$ since $B_{1,\epsilon}(x_0) \subseteq B_{\infty,\epsilon}(x_0)$.
        
        By leveraging MILP solvers such as \t{Gurobi}~\cite{gurobi}, complete robustness verification can be done efficiently for many robustly trained neural networks even on large datasets such as CIFAR-10 with models specifically trained by different approaches \cite{wong2018scaling,gowal2019scalable,zhang2020towards}.
        However, the naturally trained neural networks are still hard to be verified by these verification approaches even on MNIST.
        % And the worst case time complexity is still exponential.
        % We note that Bounded MILP~\cite{tjeng2018evaluating} is normally the most efficient exact robustness verification approach when used in practice.
        % And these MILP approaches also introduce an encoding for max-pooling layers and thus supports neural networks with them.
        
        % \para{Robust training.} 
        % Following the observation~\cite{tjeng2018evaluating} that unstable ReLU neurons significantly slow down the verification, Stability~\cite{xiao2018training} uses a regularization term to encourage ReLU neurons' stability, thus accelerating MILP-based verification.
        % % On a majority of test set samples on MNIST and CIFAR-10,
        % On neural networks trained by Stability on MNIST and CIFAR-10, most samples can be completely verified, and the certified robustness is comparable to other robust training approaches.
        % \linyi{Robust training approach moved.}
    
    \subsubsection{\textbf{Other Approaches}\texorpdfstring{~\cite{10.1007/978-3-319-63387-9_1,jordan2019provable}}{}}\hfill\\
        \t{DLV}~\cite{10.1007/978-3-319-63387-9_1} is a complex approach which propagates and back-propagates the certified robust region layer by layer.
        % In each layer, we enlarge the safe region by leveraging an SMT solver.
        \t{DLV} can search adversarial examples in hidden layers, however, it fails to verify $\cL_p$-bounded robustness.
        % Besides feed-forward ReLU networks, DLV can also support activation functions other than ReLU and other types of layers such as pooling layer and zero-padding layer.
        % 
        \t{GeoCert}~\cite{jordan2019provable} enlarges the certified robust region iteratively
        by consistently adding new linear regions overlapping $B_{p,\epsilon}(x_0)$ and verifying their robustness.
        Though it runs slightly slower than MILP-based approaches, it provides good intermediate verification results if stopped early.
        % Concretely, it starts from the local linear region centered at input $x_0$, then it iteratively chooses the closest boundary and adds the neighboring linear regions to the set until all linear regions overlapping $B_{p,\epsilon}(x_0)$ are added.
        % When a new linear region is added, GeoCert performs robustness verification on it.
        % % The approach terminates when the closest boundary has larger than $\epsilon$ distance with original input $x_0$, thus the robustness with respect to $B_{p,\epsilon}(x_0)$ is verified.
        % The actual performance is slightly slower than MILP-based approaches such as \cite{tjeng2018evaluating} but it provides acceptable intermediate results if stopped early.
    
    {\noindent\textbf{Summary:}}
        More details about complete verification approaches are discussed in ~\cite{liu2019algorithms}.
        Current complete verification approaches cannot scale up to common DNNs even on MNIST unless the DNN model is specially trained.
        On the other hand, these approaches are useful and important when the DNN models are small such as those for aircraft control system~\cite{julian2016policy}.
        
        % All complete verification approaches have exponential time complexity in the worst case~\cite{katz2017reluplex,weng2018towards}, and cannot scale up to common neural networks even on MNIST unless the model is specially trained.
        % On the other hand, in some safety-critical scenarios like aircraft control system, the neural networks are usually small.
        % Thus, these complete verification approaches become effective and important.
 
    \begin{figure}
        \centering
        \begin{subfigure}{.2\linewidth}
             \centering
             \includegraphics[width=\linewidth]{figures/relu-activations_0.pdf}
             \vspace{-0.75em}
             \caption{\,}
             \label{fig:tightest-linear-polytope}
         \end{subfigure}
        \begin{subfigure}{.2\linewidth}
             \centering
             \includegraphics[width=\linewidth]{figures/relu-activations_1.pdf}
             \vspace{-0.75em}
             \caption{\,}
             \label{fig:relu-lower-bound-1}
         \end{subfigure}
         \begin{subfigure}{.2\linewidth}
             \centering
             \includegraphics[width=\linewidth]{figures/relu-activations_2.pdf}
             \vspace{-0.75em}
             \caption{\,}
             \label{fig:relu-lower-bound-2}
         \end{subfigure}
         \begin{subfigure}{.2\linewidth}
             \centering
             \includegraphics[width=\linewidth]{figures/relu-activations_3.pdf}
             \vspace{-0.75em}
             \caption{\,}
             \label{fig:relu-lower-bound-3}
         \end{subfigure}
        \vspace{-1.1em}
        \caption{Different linear relaxations for ReLU. 
        (a) shows the tightest polytope~(the blue region) for ReLU which is used in \cite{ehlers2017formal,wong2018provable,wong2018scaling,tjeng2018evaluating};
        (b) is used in \t{Fast-Lin}~\cite{weng2018towards}, \t{CROWN}~\cite{zhang2018efficient} and \t{DeepPoly}~\cite{singh2019abstract}; 
        (c) is used in \t{CROWN} and \t{DeepPoly}; 
        (d) shows that \t{CROWN} and \t{DeepPoly} can adjust the slope of lower bound. }
        \vspace{-1.5em}
        \label{fig:different-relu-lower-bounds}
    \end{figure}
 
 \subsection{Robustness Verification Based on Linear Relaxation}
 
    \label{sec:lp-relaxation-intro}
    Due to the scalability barrier of complete robustness verification, many incomplete verification approaches based on relaxations are proposed.
    Among them, linear relaxations are well studied.
    This category of verification approaches run much faster and many can scale up to state-of-the-art models on CIFAR-10 dataset, which contain $10,000 - 100,000$ neurons.
    
    In general, all linear relaxation-based approaches require computing $l_{i,j}$ and $u_{i,j}$~(see \Cref{def:tightest-linear-polytope}) for each neuron $z_{i,j}$, then compute an over-approximation bound $\cS$ for the region $f_\theta \left(B_{p,\epsilon}(x_0)\right) := \{ f_\theta(x):\, x\in B_{p,\epsilon}(x_0) \}$, i.e., $\cS \supseteq f_\theta \left( B_{p,\epsilon}(x_0) \right)$.
    $\cS$ is specially chosen so that it is easy to verify whether all points in $\cS$ correspond to the true class $y_0$.
    % The $\cS$ can be easily computed and completely verified, i.e., we can compute the predicate $P = \left[\forall s \in \cS, \argmax_{i\in[C]} s_i = y_0\right]$ easily.
    % If $P$ is true, we successfully verify the robustness of model $f_\theta$ for original input $x_0$ and true label $y_0$ in $B_{p,\epsilon}$ ball.
    % Otherwise, the verification fails.
    If it is true, the original region $f_\theta \left(B_{p,\epsilon}(x_0)\right)$ is robust.
    % 
    Though these approaches may compute $l$ and $u$ differently, or choose different $\cS$'s, they all describe $\cS$ by linear constraints.
    % These approaches propose different techniques for $l$ and $u$ computation, and different techniques for computation and robustness verification of the over-approximation $\cS$.
    % The commonalities of them is that, $\cS$ are expressed by linear constraints, or linear bounds, or the union of them.
    
    % For convenient, for given $B_{p,\epsilon}(x_0)$, we denote $\cI_i, \cI_i^+, \cI_i^-$ to unstable, active, and inactive neurons in layer $i$ respectively:
    % % \cref{def:neuron-partitioning} gives the formal definition.
    % \begin{definition}[Neuron Partitioning]
    %     On layer $i \in \{2, \dots, l\}$,
    %     \begin{equation}
    %         \begin{aligned}
    %             & \cI_i = \{j:\, l_{i,j} < 0 < u_{i,j}\} \text{ is the unstable neuron set},\\
    %             & \cI_i^+ = \{j:\, 0 \le l_{i,j} \le u_{i,j}\} \text{ is the active neuron set},\\
    %             & \cI_i^- = \{j:\, l_{i,j} \le u_{i,j} \le 0\} \text{ is the inactive neruon set},
    %         \end{aligned}
    %     \end{equation}
    %     where $l_{i,j}$ and $u_{i,j}$ are as defined in \Cref{eq:l-u-bound-for-relu}.
    %     \label{def:neuron-partitioning}
    % \end{definition}
 
    \subsubsection{\textbf{Linear Programming}\texorpdfstring{~\cite{weng2018towards,salman2019convex,tjandraatmadja2020convex}}{}}\hfill\\
    \label{sec:linear-programming-intro}
        In \cite{weng2018towards}, \t{LP-full} is proposed, and is further studied in \cite{salman2019convex}.
        \t{LP-full} is the theoretically tightest verification approach if only using $l_{i,j}$ and $u_{i,j}$ derived from single neuron linear relaxations.
    
        In \t{LP-full}, we compute $l$ and $u$ layer by layer, apply the polytope relaxation (\Cref{def:tightest-linear-polytope}) for each ReLU neuron, and finally solve the resulting LP problem. %On layer $k+1$, we have already known $l_i$ and $u_i$ for all previous layers, i.e., for all $i \le k$, then we apply the tightest polytope relaxation for ReLU as in \Cref{def:tightest-linear-polytope} and solve the resulting LP problem.
        Due to the relaxation, we obtain a lower bound of $\cM(y_0,y)$ in \Cref{prob:verification-optimization-problem}.%, i.e., LP-full is an incomplete robustness verification approach.
        
        Even though LPs can be solved in polynomial time, in practice, solving LP is still expensive.
        Using LP-full on a typical model on CIFAR-10 for single instance takes several hours to several days~\cite{salman2019convex}.
        % This algorithm needs to solve $O(n)$ LP problems, and each problem has $O(n)$ constraints, where $n$ is the number of neural neurons.
        % Even the overall complexity is polynomial, in practice, solving a typical model on CIFAR-10 for single instance takes several hours to several days~\cite{salman2019convex}.
        Moreover, although \texttt{LP-full} is the tightest verification approach using single neuron linear relaxations, comparing with complete verification, the certifiable robust radius is usually $1.5 - 5$ times smaller, which indicates the intrinsic tightness barrier of linear relaxations.
        % , though they may be more scalable than complete verification.
        
        Recently, \t{C2V}~\cite{tjandraatmadja2020convex} is proposed to improve upon \t{LP-full} by leveraging linear relaxations on linear combinations of neurons instead of single neuron.
        Its two variants try to heuristically find good linear combinations for relaxations, which improve either scalability or tightness, but no better at order of magnitude.
        
        % % Furthermore, since $z_1 = x$, we have $l_1 = \min x = x_0 - \epsilon$ and $u_1 = \max x = x_0 + \epsilon$.
        % % Then, we apply the tightest polytope relaxation for ReLU as defined in \cref{def:tightest-linear-polytope}, which yields the following linear constraints:
        % % \begin{equation}
        % %     \left\{
        % %     \begin{aligned}
        % %         & z_1 \ge l_1, z_1 \le u_1, \\
        % %         & \hz_{i+1} = \bW_i z_i + b_i, \quad \text{for } i = 2, \dots, k \\
        % %         & z_{i,j} \ge 0,\, z_{i,j} \ge \hz_{i,j},\, z_{i,j} \le \dfrac{u_{i,j}}{u_{i,j} - l_{i,j}} (\hz_{i,j} - l_{i,j}), \\
        % %         & \quad\quad \text{for } i = 2, \dots, k-1;\, j \in \cI_i \\
        % %         & z_{i,j} = \hz_{i,j}, \quad \text{for } i = 2, \dots, k-1;\, j \in \cI_i^+ \\
        % %         & z_{i,j} = 0. \quad \text{for } i = 2, \dots, k-1;\, j \in \cI_i^- \\
        % %     \end{aligned}
        % %     \right.
        % %     \label{eq:lp-full-polytope}
        % % \end{equation}
        % % In \cref{eq:lp-full-polytope}, $l_i, u_i$ are constants and $z_i, \hz_i$ are variables.
        % % It defines the over-approximation for $\{\hz_{k+1}(x):\, x\in B_{\infty, \epsilon}(x_0)\}$.
        % % Thus, we can set the objective function to $\maximize \hz_{k+1,j}$ and $\minimize \hz_{k+1,j}$ for each $j \in [n_{k+1}]$ to obtain $l_{k+1}$ and $u_{k+1}$ from linear programming.
        
        % % After all $l_k$ and $u_k$ are computed out, we formulate the over-approximation $\cS = \{f(x) = \hz_l(x):\, x\in B_{\infty, \epsilon}(x_0)\}$ in the same manner and optimize over 
        % % $$
        % %     \minimize_{\hz_l \in \cS}\quad (\hz_l)_y - \max_{y' \in [C]: y'\neq y} (\hz_l)_{y'}.
        % % $$
        % % According to \cref{thm:verification-optimization-problem} we get an lower bound of $OPT$.
        % % Thus, the procedure is an (in)complete robustness verification.
        
        % This algorithm needs to solve $O(n)$ number of linear programming problems, where $n$ is the number of neural neurons.
        % Popular methods for solving linear programming problems like simplex-based methods and interior point methods are all quite expensive.
        % Therefore, even solving a typical model on CIFAR-10 for single input instance takes several hours to several days~\cite{salman2019convex}.
        % Moreover, although LP-full provides the tightest verificaiton using layerwise linear relaxations, comparing with complete verification, the certified radius is usually $1.5 - 5$ times smaller, which indicates the intrinsic tightest barrier of linear relaxations, though they could be scalable.
    
    \subsubsection{\textbf{Linear Inequality Propagation}\texorpdfstring{~\cite{weng2018towards,zhang2018efficient,singh2019abstract}}{}}\hfill\\
        \label{sec:linear-inequality-propagation-intro}
        % The main performance bottleneck of LP-full is solving linear programming problems.
        To circumvent solving LPs,
        \t{Fast-Lin}~\cite{weng2018towards}, \t{CROWN}~\cite{zhang2018efficient}, and \t{DeepPoly}~\cite{singh2019abstract}
        % \citeauthor{weng2018towards,zhang2018efficient,singh2019abstract}~\cite{weng2018towards,zhang2018efficient,singh2019abstract} 
        replace the two lower bounds in tightest polytope by a single lower bound.
        The idea is illustrated in \Cref{fig:relu-lower-bound-1,fig:relu-lower-bound-2,fig:relu-lower-bound-3}.
        The advantage of single linear lower bound is that, the linear bounds can be propagated through the layers efficiently instead of solving LP problem.
        
        \t{Fast-Lin}~\cite{weng2018towards} uses a parallel line as the lower bound as shown in \Cref{fig:relu-lower-bound-1}.
        \t{CROWN}~\cite{zhang2018efficient} and \t{DeepPoly}~\cite{singh2019abstract} both support adjustable lower bound.
        They use $y = \lambda x$ with adjustable $\lambda \in [0,1]$ as the lower bound, while their policies of determining $\lambda$ are slightly different.
        % :
        % when $|u_{i,j}| \ge |l_{i,j}|$, CROWN sets $\lambda = 1$, otherwise it sets $\lambda = 0$;
        % DeepPoly calculates the $\lambda$ which minimizes the over-approximated area per neuron.
        
        As an overview, we maintain the linear bound for each layer~$k$: $\bL_k x + b_{L,k} \le z_k(x) \le \bU_k x + b_{U,k}$ for any $x \in B_{p,\epsilon}(x_0)$.
        From the bound for layer $k$, we can deduct the bound after affine mapping $\hz_{k+1} = \bW_k z_k + b_k$:
        \begin{equation}
            \small
            \begin{aligned}
                & (\bW_k^+ \bL_k + \bW_k^- \bU_k)x + \bW_k^+ b_{L,k} + \bW_k^- b_{U,k} + b_k \\
                \le & \hz_{k+1}(x) \\
                \le & (\bW_k^+ \bU_k + \bW_k^- \bL_k)x + \bW_k^+ b_{U,k} + \bW_k^- b_{L,k} + b_k.
            \end{aligned}
            \label{eq:affine-linear-bound}
        \end{equation}
        Then, we can compute the activation value bound $l_{k+1}$ and $u_{k+1}$ for $\hz_{k+1}$, and compute the linear bound for $z_{k+1}(x) = \relu(\hz_{k+1}(x))$ using the ReLU polytope relaxation.
        By repeating the process, we can finally bound the last layer $\hz_l$, i.e., the model $f$ itself.
        Due to computing matrices $\bL_k$ and $\bU_k$, the time complexity is $\Theta(ln_i^3)$ if the number of neurons in each layer is $n_i$.
        This method scales up to normal models on MNIST and CIFAR-10, though is still too expensive for~ImageNet.
        
        \t{DeepPoly}~\cite{singh2019abstract} is also based on the linear inequality propagation described above, though it formally describes the deduction semantics of the method to provide more flexibility.
        
        % \linyi{Shortened.}
        % \textcolor{green}{condense or delete ((((}The single linear lower bound and upper bound can be propagated as such.
        % We view $z_i$ as a function with respect to input $x$.
        % We maintain $\bL_i, b_{L,i}$ and $\bU_i, b_{U,i}$ for each layer $i$ such that for any $x \in B_{p,\epsilon}(x_0)$, we have $\bL_i x + b_{L,i} \le z_i(x) \le \bU_i x + b_{U,i}$.
        % Suppose now we have such bound for $z_k$, namely, $\bL_k x + b_{L,k} \le z_k(x) \le \bU_k x + b_{U,k}$.
        % From $\hz_{k+1} = \bW_k z_k + b_k$, we have
        % \begin{equation}
        %     \small
        %     \begin{aligned}
        %         & (\bW_k^+ \bL_k + \bW_k^- \bU_k)x + \bW_k^+ b_{L,k} + \bW_k^- b_{U,k} + b_k \\
        %         \le & \hz_{k+1}(x) \\
        %         \le & (\bW_k^+ \bU_k + \bW_k^- \bL_k)x + \bW_k^+ b_{U,k} + \bW_k^- b_{L,k} + b_k.
        %     \end{aligned}
        %     \label{eq:affine-linear-bound}
        % \end{equation}
        % From \Cref{eq:affine-linear-bound}, we can compute $l_{k+1}$ and $u_{k+1}$ and derive the linear bound for $z_{k+1}(x) = \relu(\hz_{k+1}(x))$ using aforementioned ReLU relaxation.
        % % 
        % % from the fact that
        % % $$
        % % \begin{aligned}
        % %     \min_{x \in B(p,\epsilon)(x_0)} (\bW x + b)_i = \bW_{i,:} x_0 + b_i + \epsilon\|\bW_{i,:}\|_q, \\
        % %     \max_{x \in B(p,\epsilon)(x_0)} (\bW x + b)_i = \bW_{i,:} x_0 + b_i + \epsilon\|\bW_{i,:}\|_q.
        % % \end{aligned}
        % % $$
        % % Here $q$ is the dual norm of $q$.
        % % 
        % % 
        % % $$
        % % \begin{aligned}
        % %     & \hz_{k+1}(x)_i  \\
        % %     = &   \sum_{j=1}^{n_k} (\bW_k)_{ij} (z_k)_j + (b_k)_i \\
        % %     \ge & \sum_{j=1:\,(\bW_k)_{ij} \ge 0}^{n_k} (\bW_k)_{ij}(\bL_{k} x + b_{L,k})_j + \\
        % %     & \quad \sum_{j=1:\,(\bW_k)_{ij} < 0}^{n_k} (\bW_k)_{ij}(\bU_{k} x + b_{U,k})_j + (b_k)_i \\
        % %     = & \left( (\bW_k^+ \bL_k + \bW_k^- \bU_k) x + (\bW_k^+ b_{L,k} + \bW_k^- b_{U,k}) + b_k \right)_i,
        % % \end{aligned}
        % % $$
        % % % where $\bM^+ := \max\{ \bM ,\,\bzero \}$ and $\bM^- := \min\{ \bM ,\,\bzero \}$ elementwise.
        % % Similarly, we can obtain the upper bound, and compactly they are written as
        % % \begin{equation}
        % %     \begin{aligned}
        % %         & (\bW_k^+ \bL_k + \bW_k^- \bU_k)x + \bW_k^+ b_{L,k} + \bW_k^- b_{U,k} + b_k \\
        % %         \le & \hz_{k+1}(x) \\
        % %         \le & (\bW_k^+ \bU_k + \bW_k^- \bL_k)x + \bW_k^+ b_{U,k} + \bW_k^- b_{L,k} + b_k.
        % %     \end{aligned}
        % %     \label{eq:affine-linear-bound}
        % % \end{equation}
        % % Now we can directly compute $l_{k+1}$ and $u_{k+1}$ from the fact that
        % % $$
        % % \begin{aligned}
        % %     \min_{x \in B(p,\epsilon)(x_0)} (\bW x + b)_i = \bW_{i,:} x_0 + b_i + \epsilon\|\bW_{i,:}\|_q, \\
        % %     \max_{x \in B(p,\epsilon)(x_0)} (\bW x + b)_i = \bW_{i,:} x_0 + b_i + \epsilon\|\bW_{i,:}\|_q.
        % % \end{aligned}
        % % $$
        % % Here $q$ is the dual norm of $q$.
        % % For $p = \infty$, $q = 1$; for $p = 2$, $q = 2$; for $p = 1$, $q = \infty$.
        % % With $l_{k+1}$ and $u_{k+1}$, for unstable neurons, we can apply the lower bound and upper bound of ReLU neuron accordingly to the LHS and RHS of \cref{eq:affine-linear-bound} respectively.
        % % As the result, we can obtain the lower and upper bound for $z_{k+1} = \relu(\hz_{k+1})$ expressed as linear function.
        % By repeating the process, we can finally bound the last layer $\hz_l$, i.e., model $f$ itself.
        % % namely, $\bL_f x + b_{L,f} \le f(x) \le \bU_f x + b_{U,f}$.
        % The objective in \Cref{prob:verification-optimization-problem} can thus be lower bounded.
        % % from
        % % $$
        % % \begin{aligned}
        % %     & f(x)_y - f(x)_y' \\
        % %     \ge & (\bL_f)_{y,:} x + (b_{L,f})_y - (\bU_f)_{y':} x - (b_{U,f})_{y'} \\
        % %     \ge & \left( (\bL_f)_{y,:} - (\bU_f)_{y':} \right) x_0 - \epsilon \| (\bL_f)_{y,:} - (\bU_f)_{y':} \|_q + \\
        % %     & \quad \quad (b_{L,f})_y - (b_{U,f})_{y'}.
        % % \end{aligned}
        % % $$
        % As we can see, by using linear inequality upper and lower bounds in this manner, the expensive LP solving is greatly simplified to matrix multiplications and propagation.
        % As the result, the approach can verify common fully-connected neural networks on MNIST and CIFAR-10 dataset.
        % What prevents it from larger dataset is that, in each layer, in order to compute $l_k$ and $u_k$, we must compute the matrix norm of $\bL_k$ and $\bU_k$.
        % It is of time complexity $\cO(n_0 n_k n_{k+1})$ per layer.
        % So the overall time complexity is $\cO(\sum_{i=1}^{l-1} n_0n_in_{i+1}) = \cO(ln_i^3)$ if all $n_i$'s are equal,
        % which is still too expensive for normal-sized models on ImageNet or large models on MNIST and CIFAR-10.
        
        % % Note that CROWN additionally proposes linear bounds for other activations such as sigmoid and arctan, and derived the form for quadratic bounds.
        % % In evaluation, they have similar performance, as shown in detail in \cref{sec:evaluation}.
        
        % % DeepPoly~\cite{singh2019abstract} chooses the lower bound slope flexibly to minimize the over-approximated area, as shown in \cref{fig:different-relu-lower-bounds}(c).
        % In DeepPoly~\cite{singh2019abstract}, the linear inequality propagation is not explicitly stated as the form shown here.
        % Instead, it is expressed as a sequence of linear inequalities, and it defines semantics to deduct the final linear inequalities relating model output to the input from the inequality sequence.
        % These semantics are just an alternative way to express this approach.\textcolor{green}{))))}
        % % This formulation fosters further exploition of linear bounds and inspired k-ReLU~\cite{singh2019beyond}~(see \Cref{sec:hybrid-approach-intro}).
    
    \subsubsection{\textbf{Zonotopes}\texorpdfstring{~\cite{gehr2018ai2,mirman2018differentiable,singh2018fast,anderson2019optimization}}{}}\hfill \\
        Besides linear inequalities, zonotope is another type of over-approximation that can be propagated layer by layer efficiently.
        \t{AI$^2$}~\cite{gehr2018ai2}, \t{Diffai}~\cite{mirman2018differentiable}, \t{DeepZ}~\cite{singh2018fast}, \t{Charon}~\cite{anderson2019optimization}, and \t{RefineZono}~\cite{singh2018robustness} use zonotopes.
        Zonotope is a special form of polytope whose shape can be expressed efficiently.
        After affine transformation, the resulting region of zonotope is still a zonotope which can be easily computed.
        After ReLU $z \mapsto \relu(\hz)$, the resulting region can be over-approximated by parallelogram~(a type of zonotope) as shown in \Cref{fig:relu-parallelograms}.
        % \begin{definition}[Hybrid Zonotope, restated from \cite{mirman2018differentiable}]
        %     The hybrid zonotope is a triple $h = \langle h_C,\,h_B,\,\bH_E \rangle$ which represents region
        %     $$
        %     \resizebox{0.495\textwidth}{!}{
        %         $
        %             \gamma_H(h) = \left\{ h_C + \diag(h_B) \beta + \bH_E e: 
        %             \beta \in [-1,\,1]^p, e \in [-1,\,1]^m \right\}.
        %         $
        %     }
        %     $$
        %     Here $h_C \in \bbR^p$ is the center, $\bH_E \in \bbR^{p \times m}$ describes the error coefficient, and $h_B \in \bbR^m_{\ge 0}$ is non-negative deviations.
        %     \label{def:hybrid-zonotope}
        % \end{definition}
        % 
        % % \begin{definition}[Zonotope, restated from \cite{gehr2018ai2,mirman2018differentiable}]
        % %     A zonotope is a tuple $z = \langle z_C,\,\bZ_E \rangle$ which represents the region
        % %     $$
        % %         \gamma_Z(z) = \{ z_C + \bZ_E \cdot e : \, e \in [-1,\,1]^m \} \subseteq \bbR^p.
        % %     $$
        % %     Here $z_C \in \bbR^p$ is the center of the zonotope, and $\bZ_E \in \bbR^{p \times m}$ describes a linear relationship between the error vector $e \in [-1,\,1]^m$ and the output components.
        % %     \label{def:zonotope}
        % % \end{definition}
        % % % The application of Zonotope dates back from \cite{ghorbal2009zonotope}.
        % As we can seen, the zonotope is a special form of polytope whose shape be expressed succinctly using $z_C$, $h_B$ and $\bH_E$.
        % For affine transformation $z \mapsto \bW z + b$, the resulting region of hybrid zonotope $\langle h_C,\,h_B,\,\bH_E \rangle$ is exactly $\langle \bM h_C + b,\, |\bM| h_B,\, \bM h_E \rangle$, where $|\bM|$ calculates the absolute value of $\bM$ elementwise.
        % For ReLU activation function, given $l$ and $u$, the zonotope can over-approximate the ReLU by a parallelogram as shown in \Cref{fig:relu-parallelograms}.
        % % Some possibles over-approximations are shown in \Cref{fig:relu-parallelograms}.
        Among them, \t{Diffai}~\cite{mirman2018differentiable} uses \Cref{fig:relu-parallelograms-a}~(zBox) and \Cref{fig:relu-parallelograms-b}~(zDiag) as the base shapes, and heuristically combine them to form certain shapes of \Cref{fig:relu-parallelograms-c}.
        \t{DeepZ}~\cite{singh2018fast} minimizes the over-approximation area by selecting appropriate slope of \Cref{fig:relu-parallelograms-c}.
        It also supports activation functions other than ReLU.
        \t{AI$^2$}~\cite{gehr2018ai2} also supports zonotope as one type of its abstract interpretation.
        To improve tightness, \t{AI$^2$} maintains a set of zonotopes instead of just one.
        \t{Charon}~\cite{anderson2019optimization} improves \t{AI$^2$} by leveraging Bayesian optimization to learn ReLU splitting policy and the shape of over-approximation for a given input.
        These approaches have the same time complexity as linear inequality propagation, thus similar scalability.
        % 
        % All these works can scale up to models on CIFAR-10 dataset.
        % 
        % A more important property of zonotope is that, after affine transformation, the resulting region is still a zonotope and can be efficiently computed.
        % In practice, hybrid zonotope is used, which expresses the same class of regions as zonotope but is more convenient for computation.
        % % \begin{definition}[Hybrid Zonotope, restated from \cite{mirman2018differentiable}]
        % %     The hybrid zonotope is a triple $h = \langle h_C,\,h_B,\,\bH_E \rangle$ which represents the region
        % %     $$
        % %     \begin{aligned}
        % %         \gamma_H(h) = & \left\{ h_C + \diag(h_B) \cdot \beta + \bH_E \cdot e: \right. \\
        % %         & \quad \left. \beta \in [-1,\,1]^p, e \in [-1,\,1]^m \right\}.
        % %     \end{aligned}
        % %     $$
        % %     Here $h_C \in \bbR^p$ is the center, $\bH_E \in \bbR^{p \times m}$ describes the error coefficient, and $h_B \in \bbR^m_{\ge 0}$ is non-negative deviations.
        % %     \label{def:hybrid-zonotope}
        % % \end{definition}
        % 
        
        \begin{figure}
            \centering
            \begin{subfigure}{.22\linewidth}
                 \centering
                 \includegraphics[width=\textwidth]{figures/relu-activations_6.pdf}
                 \vspace{-1.5em}
                 \caption{}
                 \label{fig:relu-parallelograms-a}
             \end{subfigure}
             \begin{subfigure}{.22\linewidth}
                 \centering
                 \includegraphics[width=\textwidth]{figures/relu-activations_5.pdf}
                 \vspace{-1.5em}
                 \caption{}
                 \label{fig:relu-parallelograms-b}
             \end{subfigure}
             \begin{subfigure}{.22\linewidth}
                 \centering
                 \includegraphics[width=\textwidth]{figures/relu-activations_4.pdf}
                 \vspace{-1.5em}
                 \caption{}
                 \label{fig:relu-parallelograms-c}
             \end{subfigure}
             \vspace{-0.75em}
            \caption{(a) and (b) are used in \cite{mirman2018differentiable}; (c) shows that \t{DeepZ}~\cite{singh2018fast} adjusts the slope to minimize the over-approximation area.
                %  The concrete type of ReLU approximation used is not recorded in \cite{gehr2018ai2} and \cite{anderson2019optimization}.
            }
            \vspace{-1.5em}
            \label{fig:relu-parallelograms}
        \end{figure}
        % We remark that to compute the resulting zonotope after ReLU, we still need to compute $l$ and $u$, which requires the exact computation of $\bH_E$.
        % So it has the same time complexity order as linear inequality propagation.
        % To derive the over-approximation shown in \cref{fig:relu-parallelograms}, the last thing we need to solve is to compute $l$ and $u$.
        % Luckily, for hybrid zonotope $z = \langle z_C,\,z_B,\,\bH_E \rangle$, the bounds have closed form:
        % $$
        % \resizebox{0.48\textwidth}{!}{$
        %     z_i \in \left[ (h_C)_i - (h_B)_i - \sum_{j=1}^m |(\bH_E)_{ij}|,\, (h_C)_i + (h_B)_i + \sum_{j=1}^m |(\bH_E)_{ij}| \right].
        % $}
        % $$
        % However, from the bounds, the exact computation of $\bH_E$ is still unavoidable, which results in same order of time complexity as linear inequality propagation.
        % Though these approaches may be marginally faster, the larger over-approximation also causes marginal tightness loss.
        % 
        % DeepZ~\cite{singh2018fast} directly uses Zonotope as the over-approximation.
        % It adjusts the slope for each ReLU over-approximation to minimize the over-approximated area.
        % It also derives the zonotope over-approximation for sigmoid and tanh.
        % Fast-Lin and DeepZ have similar tightness while DeepZ runs slightly faster. 
        
        % \linyi{Robust training approach moved.}
        
        % \para{Robust training.}
        % Diffai~\cite{mirman2018differentiable} notices that zonotope shape parameters are all differentiable.
        % By directly injecting the lower bound of \Cref{prob:verification-optimization-problem} obtained from zonotope relaxation to adversarial training~\cite{madry2017towards}, it can train neural networks which have non-trivial certified robustness on MNIST and CIFAR-10 dataset, i.e., it is an effective robust training approach.
    
    \subsubsection{\textbf{Interval Bound Propagation}\texorpdfstring{~\cite{gehr2018ai2,gowal2019scalable}}{}}\hfill \\
        \label{sec:ibp-intro}
        A more straightforward and efficient but much looser approach comes from directly propagating $l$ and $u$ through the layers of the neural networks.
        Instead of maintaining linear bounds or zonotopes as the over-approximation, we directly use the numerical interval $[l_i,\,u_i]$, and derive $[l_{i+1},\,u_{i+1}]$ from $[l_i,\,u_i]$.
        In short, if $l_k \le z_k \le u_k$, based on $\hz_{k+1} = \bW_k z_k + b_k$, $\hz_{k+1}$ can be bounded by $l_{k+1} \le \hz_{k+1} \le u_{k+1}$ where
        $$
            \small
            l_{k+1} = \bW_k^+ l_k + \bW_k^- u_k + b_k,
            \, 
            u_{k+1} = \bW_k^+ u_k + \bW_k^- l_k + b_k.
            % \begin{aligned}
            %     & (\hz_{k+1})_i = \sum_{j=1}^{n_k} (\bW_k)_{ij} (z_k)_j + (b_k)_i \ge \left(\bW_k^+ l_k + \bW_k^- u_k + b_k\right)_i,\\
            %     & (\hz_{k+1})_i = \sum_{j=1}^{n_k} (\bW_k)_{ij} (z_k)_j + (b_k)_i \le \left(\bW_k^+ u_k + \bW_k^- l_k + b_k\right)_i.
            % \end{aligned}
        $$
        And $z_{k+1} = \relu(\hz_{k+1})$ can be bounded by $\max\{l_{k+1},\,0\} \le z_{k+1} \le \max\{u_{k+1},\,0\}$.
        
        % Here we consider $\cL_\infty$ bounded verification.
        % Given $l_k$ and $u_k$.
        % From \cref{eq:l-u-bound-for-relu}, we know:
        % $$
        %     l_k \le \min_{x \in B_{\infty,\epsilon}(x_0)} \hz_{k} 
        %     \text{ and }
        %     \max_{x \in B_{\infty,\epsilon}(x_0)} \hz_{k} \le u_k.
        % $$
        % Because $z_k = \relu(\hz_k)$,
        % $$
        % \begin{aligned}
        %     & l_k' := \max\{l_k,\,0\} & \le & \min_{x \in B_{\infty,\epsilon}(x_0)} z_k \\
        %     \text{ and } & u'_k := \max\{u_k,\,0\} & \ge & \max_{x \in B_{\infty,\epsilon}(x_0)} z_k.
        % \end{aligned}
        % $$
        % From $\hz_{k+1} = \bW_k z_k + b_k$, we thus have
        % $$
        % \resizebox{0.48\textwidth}{!}{$
        % \begin{aligned}
        %     & (\hz_{k+1})_i = \sum_{j=1}^{n_k} (\bW_k)_{ij} (z_k)_j + (b_k)_i \ge \left(\bW_k^+ l_k + \bW_k^- u_k + b_k\right)_i,\\
        %     & (\hz_{k+1})_i = \sum_{j=1}^{n_k} (\bW_k)_{ij} (z_k)_j + (b_k)_i \le \left(\bW_k^+ u_k + \bW_k^- l_k + b_k\right)_i.
        % \end{aligned}
        % $}
        % $$
        % In other words,
        % $$
        % \begin{aligned}
        %     l_{k+1} := \bW_k^+ l_k + \bW_k^- u_k + b_k,\\
        %     u_{k+1} := \bW_k^+ u_k + \bW_k^+ l_k + b_k
        % \end{aligned}
        % $$
        % are the valid lower bound and upper bound for $\hz_{k+1}$ .
        % The base case is $z_1 = x \Rightarrow l_1 = x - \epsilon,\, u_1 = x + \epsilon$.
        % Similarly, we can bound the lower bound of OPT in \cref{eq:verification-optimization-problem} from:
        % $$
        % \begin{aligned}
        %     & f_\theta(x)_y - f_\theta(x)_{y'} \\
        %     = & (\bW_{k-1}z_{k-1} + b_{k-1})_y - (\bW_{k-1}z_{k-1} + b_{k-1})_{y'} \\
        %     = & \left((\bW_{k-1})_{y,:} - (\bW_{k-1})_{y',:}\right) z_{k-1} + (b_{k-1})_y - (b_{k-1})_{y'} \\
        %     = &  \left((\bW_{k-1})_{y,:} - (\bW_{k-1})_{y',:}\right)^+ l_{k-1} \\
        %     & \quad + \left((\bW_{k-1})_{y,:} - (\bW_{k-1})_{y',:}\right)^- u_{k-1} \\
        %     & \quad + (b_{k-1})_y - (b_{k-1})_{y'}. \\
        % \end{aligned}
        % $$
        
        This bound propagation through each layer just performs $4$ matrix-vector products, which is at the same order of model inference.
        As the result, the approach is scalable for verifying models on ImageNet.
        The approach is named interval bound propagation~(\t{IBP}) in \cite{gowal2019scalable}, and is also named interval arithmetic in the literature.
        It is equivalent to \t{AI$^2$} with ``Box'' domain~\cite{gehr2018ai2}.
        % In the taxonomy tree~(\Cref{fig:tree-categorization}), we view interval bound propagation as a special form of linear inequality propagation.
        
        % \linyi{Shortened.}
        % \para{Robust training.}
        % In \cite{gowal2019scalable}, a training approach is proposed by integrating the differentiable lower bound into the training objective of adversarial training~\cite{madry2017towards}.
        % It can train models with higher certified robustness than Diffai~\cite{mirman2018differentiable}, WK~\cite{wong2018provable}, etc,
        % % though the bound is much more coarse, 
        % so it is an effective robust training approach.
        % % Though the training requires much more computation resources and dedicated tuning than these defenses.
    
    \subsubsection{\textbf{Linear Dual}\texorpdfstring{~\cite{wong2018provable,wong2018scaling,dvijotham2018dual,dvijotham2018training}}{}}\hfill \\
        \label{sec:dual-intro}
        Since the robustness verification can be viewed as an optimization problem~(\Cref{prob:verification-optimization-problem}), we can consider the Lagrangian dual.
        Especially, since \Cref{prob:verification-optimization-problem} is a minimization problem, any feasible dual solution provides a valid lower bound of the primal problem.
        Moreover, the dual problem is always convex~\cite{boyd2004convex}.
        These characteristics meet the needs for robustness verification.
        
        In \t{WK}~\cite{wong2018provable}, $l$ and $u$ are computed using an approach the same as \t{Fast-Lin}~\cite{weng2018towards}, then the ReLU polytope is used for over-approximation, which yields an LP problem.
        \t{WK} considers its dual problem, and by
         fixing some dual variables, the authors find that a solution could be derived from layerwise propagation over a new network, which is called dual network.
        Thus, once the dual network is formed, the verification can be done from its layerwise propagation.
        % Benefited from the dual network structure, once the network is formed~(with computed $l$ and $u$), the verification can be done.
        % In particular, in dual network, the convolutional layer becomes transposed convolutional layer whose computation can be benefited from GPU acceleration.
        % Whereas, even though the optimal solution of the dual problem is exactly the optimal of primal linear programming problem.
        % At the expense of fixing some dual variables, the resulting conditional optimal solution is suboptimal.
        According to \cite{salman2019convex}, the fixing of the selected dual variables results in the ReLU polytope shown in \Cref{fig:relu-lower-bound-1} which is used by \t{Fast-Lin}.
        Therefore, the tightness of \t{WK} should be close or equivalent to \t{Fast-Lin}.
        
        % % Because back-propagating over the dual network directly computes the lower bound of \Cref{eq:verification-optimization-problem}, it is straightforward to apply the adversarial training idea here, which results in a strong certifiably robust training approach.
        % \para{Robust training.}
        % The lower bound from WK can be put into the training objective of adversarial training, which results in an effective robust training approach.
        % Observing that the lower bound for training need not be precise, in WK+~\cite{wong2018scaling}, $l$ and $u$ are approximately computed from Cauchy projection, which improves scalability and enables large ResNet~\cite{he2016deep} network training on CIFAR-10.
        % % Additionally, WK+ extends the verification of WK to skip-connection neural networks~(including ResNet), other activation functions, and batch normalization layers.
        % \vspace{1em}
        % \linyi{Robust training approach moved.}
        
        \citeauthor{dvijotham2018training} also propose several verification and training approaches in dual space, such as \t{D-LP}~\cite{dvijotham2018dual} and \t{PVT}~\cite{dvijotham2018training}.
        Recently, a new dual approach called \t{Lagrangian decomposition} is proposed, which is claimed to be tighter and faster~\cite{bunel2020lagrangian}.
        
        % Dvijotham et al. also propose several verification and training approaches in dual space~\cite{dvijotham2018training,dvijotham2018dual,dvijotham2019efficient}.
        % % Instead of doing linear relaxation first, \citeauthor{dvijotham2018training} directly consider the dual problem for the general problem.
        % Due to the difficulty of solving the general dual problem, additional constraints are applied.
        % In D-LP~\cite{dvijotham2018dual}, the $l$ and $u$ bound constraints are added and PGD~(projected gradient descent) is used to derive the solution.
        % In PVT~\cite{dvijotham2018training}, the dual variables come from a neural network based predictor instead of PGD for acceleration.
        % The predictor and the original model can be trained jointly, which improves the certified robustness of the original model, so it is also a robust training approach.
        % % In PGD-SDP~\cite{dvijotham2019efficient}, the additional SDP constraints are added.
        % % After fixing some dual variables, it uses PGD to derive the solution.
        % Recently, a new dual form called Lagrangian decomposition is proposed, which is claimed to be tighter and faster~\cite{bunel2020lagrangian}.
        
        % To ease the 
        % In D-LP~\cite{dvijotham2018training}, the $l$ and $u$ bound constraints are added to ease the difficulty of solving the dual problem.
        % Then, subgradient method such as PGD is applied to the outer maximization over dual variables.
        % If the optimal solution can be found, the verification result is equivalent to those of verification approaches using tightest ReLU polytope in the primal space such as LP-All.
        % % Note that since the general problem is non-convex, weak duality implies that the dual problem optimal may be not tight, but is a valid lower bound.
        % % The original dual problem is a max-min problem, where the outer maximization is over dual variables, and the inner minimization is over $x \in B_{\infty,\epsilon}(x_0)$ and other $z_i, \hz_i$.
        % % Without additional constraints on $x$, the authors find the inter minimization produces vacuous bound.
        % % Therefore, the $l$ and $u$ bound constraints are added to tighten, i.e., we compute $l$ and $u$ use linear inequality propagation or interval bound propagation, then additionally constrain each inner $\hz_i$ and $z_i$ by corresponding $l$ and $u$.
        % % With such constraint, the author finds the inner minimization has closed form solution.
        % % Then, subgradient method such as PGD is applied to the outer maximization over dual variables.
        % % In D-LP~\cite{dvijotham2018training}, the author proves that when $l$ and $u$ are produced from linear inequality propagation, the optimal solution is equivalent to using tightest ReLU polytope in the primal space~(though $l$ and $u$ is looser).
        % % 
        % In PVT~\cite{dvijotham2018dual}, to improve the scalability, $l$ and $u$ are computed from faster interval bound propagation, and the dual variables come from a neural network predictor instead of from subgradient method.
        % Moreover, PVT can train the original model to fit it better for the predictor, i.e., make it easier to be verified by the predictor.
        % % , which forms an elegant confronting structure.
        % The resulting model achieves good certifiable robustness.
        % Thus, PVT is also a \textbf{certifiable defense}.
        % % 
        % Following this line, PGD-SDP~\cite{dvijotham2019efficient} considers the dual problem of SDP~(will introduce in \cref{sec:sdp-intro}).
        % Here, to avoid expensive solving, in spirit, it does something similar to WK~\cite{wong2018provable} - fixing some dual variables.
        % Then the other variables can be optimized using subgradient method as in D-LP.
        % % 
        % Recently, \cite{bunel2020lagrangian} proposes a new dual form called Lagrangian decomposition which claims to have tighter dual bounds along with a tighter and faster verification approach.
    
    \subsubsection{\textbf{Hybrid Approaches}\texorpdfstring{~\cite{singh2019beyond,singh2018robustness,zhang2020towards}}{}}\hfill \\
        \label{sec:hybrid-approach-intro}
        There are several works combining interval bound propagation and linear inequality propagation~(such as \cite{zhang2020towards}), or linear relaxations and complete verification approaches~(such as \cite{wang2018formal,wang2018efficient,singh2018robustness,singh2019beyond}).
        The ultimate goal of these works is to achieve a better trade-off between scalability and tightness by standing in the midpoint of the combined approaches.
        
        \t{CROWN-IBP}~\cite{zhang2020towards} combines \t{CROWN}~\cite{zhang2018efficient} and \t{IBP}~(\cref{sec:ibp-intro}).
        At high level, \t{CROWN-IBP} firstly computes $l$ and $u$ quickly using \t{IBP}.
        Then, it derives the linear bound from \t{CROWN} using $l$ and $u$.
        %, which optimizes the lower bound slope heuristically.
        % The linear bound is computed in backward manner for efficiency, and finally we can get a linear function as the lower bound of $f$.
        It achieves scalability comparable to \t{IBP}, but improves the tightness of \t{IBP} benefited from \t{CROWN}.
        % Since $l$ and $u$ are computed from IBP, they can break the efficiency barrier of other linear relaxation approaches.
        % And the linear bound built upon $l$ and $u$ using CROWN makes it tighter than purely relying on $l$ and $u$ like IBP.
        % Thus, it results in an efficient verification approach whose tightness is between linear bounds and IBP, and scalability is comparable to IBP.
        % 
        % Moreover, the high efficiency permits CROWN-IBP to be used as a training objective in adversarial training.
        % \linyi{Robust training approach omitted.}
        % When combined with regular training loss and IBP bound loss, the training can achieve or comparable to state-of-the-art certifiable robustness.
        % Therefore, it is a very effective \textbf{robust training approach}.
        % % The trained neural network can be easily certified to be robust by CROWN-IBP.
        
        \t{RefineZono}~\cite{singh2018robustness} is extended from zonotope over-approximation of \t{DeepZ}~\cite{singh2018fast}.
        % Due to the looseness of zonotope over-approximaiton, in RefineZono, the first few layers use MILP to refine more precise bounds for $l$ and $u$; the subsequent middle layers use linear programming~(\cref{sec:linear-programming-intro}) to improve tightness; and the last several layers return back to zonotope as used in DeepZ.
        It uses MILP to refine the $l$ and $u$ bound.
        The approach is slower but tighter than \t{DeepZ}.
        % 
        \t{k-ReLU}~\cite{singh2019beyond} is inspired by \t{DeepPoly}~\cite{singh2018fast}.
        In \t{k-ReLU}, in each layer, they further applying ReLU over-approximations shown in \Cref{fig:different-relu-lower-bounds} to neuron's linear combinations, e.g., $\sum_{j=1}^{n_k} z_{k,j}$ or $-\sum_{j=1}^{n_k} z_{k,j}$, to tighten the verification.
        % use linear inequalities $\sum_{j=1}^{n_k} z_{k,j}$ or $-\sum_{j=1}^{n_k} z_{k,j}$. for linear combinations of neurons.
        % For example, applying ReLU over-approximations shown in \Cref{fig:different-relu-lower-bounds} to the quantity $\sum_{j=1}^{n_k} z_{k,j}$ or $-\sum_{j=1}^{n_k} z_{k,j}$.
        % % besides each single neuron $z_{k,j}$.
        % % The number of such linear combinations is infinite.
        % % Therefore, k-ReLU partitions neurons in considered layers to $3-5$ per group.
        % % Then adding new linear inequalities in fixed pattern to each group.
        % % This could limit the number of linear inequalities from explosion, but also limit the tightness.
        \t{k-ReLU} is slower but moderately tighter than \t{DeepPoly}.
        \t{k-ReLU} also shares some similarities with \t{C2V}~\cite{tjandraatmadja2020convex} introduced in \Cref{sec:linear-programming-intro}.
    
    \subsubsection{\textbf{Beyond Feed-Forward ReLU Networks}\texorpdfstring{~\cite{wong2018scaling,boopathy2019cnn}}{}}\hfill \\
        \label{sec:beyond-ff-relu-networks}
        In practice, more complex layers or structures such as convolutional layers, max-pooling layers, or residual blocks~\cite{he2016deep} are commonly used.
        Many aforementioned approaches also support them, such as \t{IBP}~\cite{gowal2019scalable}, \t{WK+}~\cite{wong2018scaling}.
        \t{CNNCert}~\cite{boopathy2019cnn} extends \t{Fast-Lin} and \t{CROWN} to support them.
        Moreover, many approaches~\cite{wong2018provable,zhang2018efficient,singh2018fast,gowal2019scalable} support other activation functions besides ReLU.
        Though tighter relaxations for these activation functions are still open.
        
        % % For practical dataset such as MNIST, CIFAR-10, and ImageNet, since their inputs are images, more complex layers such as convolutional layers, max-pooling layers, or residual blocks~\cite{he2016deep} are commonly used in their neural networks.
        % % In this section we discuss the extensions to support these structures.
        % In practice, more complex layers or structures such as convolutional layers, max-pooling layers, or residual blocks~\cite{he2016deep} are commonly used.
        % % 
        % Interval bound propagation~(IBP) can be easily extended to support these structures since IBP encodes its bound propagation almost directly into forward computation of neural networks.
        % % where the computation of these complex structures are efficiently implemented.
        % % 
        % However, supporting them for other verification approaches seems to be non-trivial.
        % For example, although convolutional layer is essentially a type of affine transformation, unfolding it to affine layer is intractable in practice, due to the large amounts of input and output neurons.
        % % 
        % In WK+~\cite{wong2018scaling}, convolutional layers and skip connections are supported.
        % % For convolutional layers, WK+ defines $l$ and $u$ at the kernel level as the minimum and maximum of those in the reception field.
        % % Thus, the relaxation has the same slope for each output neuron and the computation can be written as convolution, though induces some degree of over-approximation.
        % % For skip connections, WK+ generalize the dual neural network to support them by further analysis for the dual problem.
        % % Thus, it can support complex network structures like ResNet.
        % % 
        % More contributions on this come from CNNCert~\cite{boopathy2019cnn}, which equips Fast-Lin and CROWN
        % % , i.e., general linear inequality propagation-based verification approaches, 
        % with support of convolutional layers, pooling layers, and skip connections.
        % The general approach is similar to WK+, but some finer-grain analysis is proposed, especially for pooling layers and skip connections.
        % % As the result, it also supports ResNet.
        
        % % NonlinearSpec~\cite{qin2018verification} extends the verification approaches from a different angle.
        % % It considers other robustness definitions or other properties that could be verified, beyond $\cL_p$ perturbation based ones.
        % % Theoretically, NonlinearSpec shows that any convex specification could be verified using linear inequality propagation based approaches since it is an convex optimization problem.
        % % Then, it showcases two specifications, one defines metric of misclassification based on inter-class distance, and the another one defines distance to a general physics law for a simulation system.
        % % Note that complex properties are well-studied by complete robustness verification approaches such as Reluplex~\cite{katz2017reluplex} and BaB~\cite{bunel2018unified}, and ACAS dataset defines many properties.
        % % Further extension of them on relaxation-based verification approaches could be benefited from this work.
        
        % In practice, besides ReLU, other functions like tanh and sigmoid are also used in neural networks.
        % % The activation functions are also where extensions can come from.
        % % Besides ReLU, tanh, sigmoid, etc are also used in neural networks.
        % Many of approaches discussed before, such as \cite{wong2018provable,zhang2018efficient,singh2018fast,gowal2019scalable} support them.
        % The general flow is to find out the linear relaxation based on the geometry shapes of these activation functions.
        % A tighter relaxation of them is still worth exploring.
     
    \subsubsection{\textbf{Robust Training}}\hfill \\
        % \linyi{omit references since it takes too much space.}
    % \subsubsection{\textbf{Robust Training}\texorpdfstring{~\cite{xiao2018generating,wong2018provable,wong2018scaling,dvijotham2018training,mirman2018differentiable,gowal2019scalable,wang2018mixtrain,li2019robustra,pmlr-v89-croce19a,Croce2020Provable,Balunovic2020Adversarial,zhang2020towards}}{}}\hfill \\
        % \xiangyu{redundant to the discussion on robust training in each separate subsec from 1) to 7)} 
        % \linyi{fixed the redundancy, and moved some key contents from above to here.}
        The robust training approaches aim to train neural networks to be certified with non-trivial robustness guarantees.
        In this subsection we summarize the major techniques used in robust training based on or inspired by linear relaxation-based robustness verification.
        \footnote{
        Some work proposes both verification and robust training approach, such as \t{IBP}~\cite{gowal2019scalable} and \t{CROWN-IBP}~\cite{zhang2020towards}.
        In this case, we use the same approach name to refer to both verification and robust training.
        }
        
        \para{Certified adversarial training.}
        The robust training approaches are usually extended from adversarial training  \cite{wong2018provable,wong2018scaling,mirman2018differentiable,gowal2019scalable,Balunovic2020Adversarial,zhang2020towards}.
        % Adversarial training~\cite{madry2017towards}, which approximately solves min-max problem:
        % $$
        %     \min_\theta \max_{x \in B_{p,\epsilon}(x_0)} l(f_\theta(x),\,y_0),
        % $$
        % where $l$ is the regular loss function such as cross-entropy loss.
        % % measuring distance of model prediction $f_\theta(x)$ from the correct label $y_0$ such as cross-entropy loss.
        % The inner maximization is instrinsically hard to solve due to non-convexity, and is usually approximated by heuristic attacks such as PGD attack. 
        % The outer minimization optimizes model parameters. % using common optimizers.
        % % such as stochastic gradient descent or Adam optimizer~\cite{kingma2014adam}.
        % Many certifiably robust defenses use this framework, but substitute the inner maximization by the upper bound found by verification approaches.
        % % ~(as shown by \cref{thm:verification-optimization-problem}).
        Adversarial training~\cite{madry2017towards} is a powerful~\cite{Dong_2020_CVPR} defense which approximately solves the min-max problem:
        $$
            \min_\theta \max_{x \in B_{p,\epsilon}(x_0)} l(f_\theta(x),\,y_0),
        $$
        where $l$ is the regular loss function such as cross-entropy loss.
        % % measuring distance of model prediction $f_\theta(x)$ from the correct label $y_0$ such as cross-entropy loss.
        The inner maximization is hard to solve due to non-convexity, and is usually approximated by empirical attacks such as PGD~(projected gradient descent) attack~\cite{madry2017towards}. 
        The outer minimization optimizes model parameters based on gradients as normal training. % using common optimizers.
        % % such as stochastic gradient descent or Adam optimizer~\cite{kingma2014adam}.
        Though adversarially trained models are robust against existing attacks, it cannot be certified with high robustness guarantees~\cite{tjeng2018evaluating}.
        In counter to this, many robust training approaches substitute the inner maximization by the certified bounds for \Cref{prob:verification-optimization-problem} found by verification approaches.
        The certified bounds derived from linear inequalities, relaxed dual linear problem, and interval bounds are differentiable, so they can be efficiently optimized by gradient descent during training.
        % % ~(as shown by \cref{thm:verification-optimization-problem}).
        % This is because verification approaches can provide an upper bound for the inner maximization of adversarial training objective.
        % In adversarial training, the inner maximization in the training objective is approximated by heuristic attacks which find adversarial examples.
        % Whereas in certifiable adversarial training, the inner maximization is the upper bound provided by the verification approach.
        % By training over such over-approximation, the neural network achieves non-trivial robustness in the exact region $\{f_\theta(x'):\, x' \in B_{p,\epsilon}(x)\}$, and is easily verified by the corresponding verification approach.
        Note that the training only uses training set, but the non-trivial certified robustness is obtained from the test set, which indicates that \emph{certified adversarial training generalizes}, as first concluded in \cite{wong2018provable}.
        % , just like regular training, and heuristic adversarial training.
        
        % , i.e., certifiable defenses, are usually achieved by optimizing a min-max problem, where the inner max problem seeks the ``most adversarial examples'' and the outer minimization seeks the best model parameter $\theta$~\cite{wong2018scaling,mirman2018differentiable,gowal2019scalable}.
        % The ``most adversarial example'' is normally measured by a loss function to facilitate back-propagation.
        % The idea is a direct extension of adversarial training which is one of state-of-the-art defenses against heuristic attacks~\cite{madry2017towards}, so we call it \emph{certifiable adversarial training}.
        % In adversarial training, a heuristic attack is applied to seek the adversarial example.
        % Due to the lack of certification, the heuristic attack may not find the adversarial example out even though it exists.
        % While in these certifiable defenses, the ``most adversarial example'' in the over-approximation region is guaranteed to be used.
        % By training over such over-approximation, the neural network achieves non-trivial robustness in the exact region $\{f_\theta(x'):\, x' \in B_{p,\epsilon}(x)\}$, and is easily verified by the corresponding verification approach.
        % Note that the training only uses training set, and the non-trivial certifiable robustness is evaluated on the unseen test set, which means that the certifiable robust training generalizes, just like regular training, and heuristic adversarial training.
        
        % Besides this certifiable adversarial training scheme, there are several works proposing novel certifiable training approaches.
        % A useful technique is to add additional terms, i.e., regularizer, either to improve the accuracy on original input, or to further improve certifiable robustness.
        
        \para{Combine adversarial training with regular training loss.}
        The regular training loss is aimed at improving model accuracy under normal input~(i.e., improving clean accuracy).
        It can be combined to the (certified) adversarial training loss to improve both certified robustness and clean accuracy, which is utilized by
        \t{Mixtrain}~\cite{wang2018mixtrain}, \t{IBP}~\cite{gowal2019scalable}, and \t{CROWN-IBP}~\cite{zhang2020towards}.

        % Mixtrain~\cite{wang2018mixtrain} combines regular training loss to the robust training loss of \cite{wong2018provable}, then by weighing between regular training and robust training differently at different phases, it yields slightly better certifiable robustness than \cite{wong2018provable} and better clean accuracy.
        % IBP~\cite{gowal2019scalable} also exploits this idea and combines it with robust training loss derived from interval bound propagation, which in turn gets much better certifiable robustness than \cite{wong2018provable,wang2018mixtrain} but inferior than CROWN-IBP~\cite{zhang2020towards}.
        % % Note that better certifiable robustness of trained model could be obtained from other verification approaches such as Bounded MILP~\cite{tjeng2018evaluating} instead of the verification approach from which the defense is derived.
        
        \para{Penalize over-approximation or unstable neurons.}
        Adding regularizer to the training objective which encourages tight verification could help to improve the certified robustness.
        Examples are \t{IBP}~\cite{gowal2019scalable}, \t{Stability}~\cite{xiao2018generating}, and \t{MMR}~\cite{pmlr-v89-croce19a}.
        % IBP training~\cite{gowal2019scalable} can be marginally improved by adding regularization term $\sum \|u_k - l_k\|^2$ to penalize over-approximation~\cite{morawiecki2019fast}.
        % Stability~\cite{xiao2018training}, as discussed before, adds regularizer to enhance ReLU stability.
        % MMR~\cite{pmlr-v89-croce19a} proposes regularizer to directly maximize the linear region along with the lower bound of that linear region.
        % % The certifiable robustness of trained model is comparable to WK+~ \cite{wong2018scaling}.
        \t{MMR-Universal}~\cite{Croce2020Provable} further improves \t{MMR} to certifiably defend against any $\cL_p$ adversary for $p \ge 1$.
        % It is based on the $\cL_p$ norm analysis which shows that proper combination of $\cL_1$ and $\cL_\infty$ defenses can yield the defense against any $\cL_p$.
        
        \para{Transferability-based training.}
        An intriguing property of adversarial examples is that, they usually transfer from one model to another, though these models are trained independently~\cite{szegedy2013intriguing,tramer2017space}.
        In \t{Robustra}~\cite{li2019robustra}, a proxy of transferable adversarial space is used to boost the robustness of robust training in \t{WK}~\cite{wong2018provable}.
        % combined with WK~\cite{wong2018provable} to work as a certifiable defense, which improves the certifiable robustness of WK.
        % Though due to the over-approximation nature, precise computation of such space is intractable, a proxy space is used based on the dual space relaxation of WK~\cite{wong2018provable}.
        % Training over such proxy space gives rise to a novel training approach which not only reduces transferability but also improves certifiable robustness.
        % Note that the certifiable robustness here is generally inferior then IBP~\cite{gowal2019scalable} or CROWN-IBP~\cite{zhang2020towards}, mainly because the training objective based on WK is too expensive to train the model well.
        
        % \para{Train from hidden layer over-approximation.}
        % COLT~\cite{Balunovic2020Adversarial} computes the over-approximation up to some intermediate layer, then use a heuristic attack to find adversarial examples from that over-approximated layer.
        % The adversarial examples are put into the adversarial training objective.
        % %as the proxy of inner maximization.
        % % The motivation is to ``cancel out'' the over-approximation from verification which poses difficulty on training.
        % % Its actual performance is comparable to CROWN-IBP~\cite{zhang2020towards} but slightly inferior.
        
        % COLT~\cite{Balunovic2020Adversarial} analyzes the difference between heuristic adversarial training and certifiable adversarial training.
        % Concretely, it views the training examples of heuristic adversarial training as from heuristic attacks on the input layer; 
        % while it views the training examples of certifiable adversarial training as from strongest attacks on the over-approximated output layer.
        % As the result, a new training scheme comes at the midpoint, which is training by adversarial examples from over-approximated intermediate layers.
        % Firstly, an over-approximation is computed up to that intermediate layer, then, heuristic attack is applied to that layer.
        % Though this training objective has no guarantee such as being lower bound, the sub-optimality of heuristic attack in some degree ``cancels out'' the difficulty posed by over-approximation, thus yields good certifiable robustness.
        % Its actual performance is comparable to CROWN-IBP~\cite{zhang2020towards} but slightly inferior.
    
    % \vspace{0.1em}

    
    {\noindent\underline{\textbf{Summary:}}}
    % \linyi{I prefer keep it. Since this is the tool for high-level recap of these verification approaches. Otherwise we just introduce the approaches and don't have systematization.}
        Except the linear dual approaches, all other linear relaxation-based approaches can be viewed as propagating the over-approximation layer by layer, and the main difference is based on different types of over-approximation.
        % In AI2~\cite{gehr2018ai2}, the concept of \emph{abstract interpretation} is exploited.
        % %, which can summarize these approaches.
        % The abstract interpretation is used to verify program properties by saving and operating on compact state representation in program static analysis~\cite{cousot1977abstract}.
        % All these over-approximations such as interval bounds, linear inequalities and zonotopes are effective abstract interpretations for neural networks.
        Future improvements of verification could come from tighter and more efficient over-approximations~(a.k.a. abstract interpretations~\cite{gehr2018ai2}).
        % \linyi{Saved some space here.}
        
        From the optimization point of view,
        \citeauthor{salman2019convex}~\cite{salman2019convex} connect all these linear relaxation based verification approaches and compare their tightness theoretically:
        \t{IBP} is the loosest.
        \t{Fast-Lin}~\cite{weng2018towards}, \t{DeepZ}~\cite{singh2018fast}, \t{Diffai}~\cite{mirman2018differentiable}, and the dual approach \t{WK}~\cite{wong2018provable} have equivalent tightness and time complexity.
        \t{CROWN}~\cite{zhang2018efficient} and \t{DeepPoly}~\cite{singh2018robustness} are tighter than these with similar time complexity.
        \t{LP-Full}~\cite{salman2019convex} is the tightest using only single neuron linear relaxations.
        Theoretically, \t{k-ReLU}~\cite{singh2019beyond} can be tighter than \t{LP-Full} given that it uses relaxations based on multiple neurons, if it leverages LP during computing each $l$ and $u$.
        Finally, \t{C2V}~\cite{tjandraatmadja2020convex} is tighter than \t{k-ReLU} empirically and theoretically.
        Generally, tighter verification approaches are less efficient, as reflected by the tightness and scalability trade-off.
        
        A pessimistic result is that, even using relatively tight \t{LP-All}, the certified robustness still has large gap compared with the complete verification.
        % , which is called ``convex barrier'' and could be more precisely deemed as single neuron linear relaxation barrier.
        To circumvent this barrier, we need to turn to hybrid techniques or approaches other than linear relaxation-based ones.
      
        
        % Viewing from optimization, \citeauthor{salman2019convex}~\cite{salman2019convex} connect all these linear relaxation based verification approaches
        % % , including both primal and dual space ones, 
        % and compare their tightness theoretically.
        % According to the analysis, 
        % % among these linear relaxations based approaches, 
        % interval bound should be the loosest.
        % % and zonotopes should be the loosest.
        % Fast-Lin~\cite{weng2018towards} is equivalent to zonotope-based approach like DeepZ~\cite{singh2018fast} and Diffai~\cite{mirman2018differentiable}.
        % Linear inequalities such as CROWN~\cite{zhang2018efficient} and DeepPoly~\cite{singh2018robustness} are tighter than these.
        % On the other hand, the dual approaches, if without dual variable fixing, should be tighter than linear inequalities and be equivalent to the tightest LP-All~\cite{salman2019convex}.
        % A pessimistic result is that, even using the tightest LP-All, the certifiable robust radius still has large gap from complete verification, which is called ``convex barrier'' and could be more precisely deemed as linear relaxation barrier.
        % To circumvent this barrier, we could use hybrid techniques or use approaches in other categories.
 
 \subsection{Certified Robustness Based on Semidefinite Programming}
    \label{sec:sdp-intro}
    
    Semidefinite programming~(SDP) is a convex optimization problem which can be solved in polynomial time.
    Its decision variable is a matrix which is constrained to be symmetric, semi-positive, and the elements can be linearly constrained~\cite{boyd2004convex}.
    % SDP can be solved in polynomial time.
    
    \t{SDP Verify}~\cite{raghunathan2018semidefinite} formulates the robustness verification as a SDP problem.
    It constrains the outer product matrix of neuron activations, namely $\bP$, to be semi-definite and imposes ReLU or affine mapping constraints on $\bP$.
    The relaxation comes from removing the rank constraint of $\bP$.
    \t{SDP Verify} is usually much tighter than linear relaxation-based verification.
    Moreover, even for neural networks which are not robustly trained~(e.g., trained via empirical defense), \t{SDP Verify} still provides reasonably good robustness certification.
    However, \t{SDP Verify} only scales up to small size models on MNIST.
    
    \t{PGD-SDP}~\cite{dvijotham2019efficient} introduces several additional relaxations to \t{SDP Verify} from the dual space to significantly improve scalability, though at the expense of tightness.
    \t{LMIVerify}~\cite{fazlyab2019efficient} supports scalability/tightness trade-off adjustments via directly analyzing the SDP dual problem, i.e., LMI problem.
    % considers the SDP dual problem --- linear matrix inequality~(LMI) constrained problem.
    % It enables scalability/tightness adjustments.
    However, in practice, \t{LMI Verify} is either too slow or too loose.
    
    On the training side, \t{SDPTrain}~\cite{raghunathan2018certified} is an early-stage robust training approach which uses SDP relaxation to lower bound the verification problem~(\Cref{prob:verification-optimization-problem}).
    However, the approach is limited to only two-layer networks, and it achieves non-trivial certified robustness only on MNIST dataset.
    
    Though SDP-based approaches are tighter than linear relaxations, they usually fail to scale up to large models even on MNIST due to the high time complexity of solving SDP.
    
    % Semidefinite programming~(SDP) is a class of convex optimization problems, where the decision variable is a matrix which is constrained to be symmetric and semi-positive and whose elements can be linearly constrained.
    % Its formal definition can be found in \cite{boyd2004convex}.
    % SDP can be solved in polynomial time.
    % % Its formal definition can be found in \cref{def:sdp}.
    % % 
    % % \begin{definition}[SDP Standard Form~\cite{boyd2004convex}]
    % %     With decision variable $\bX \in \bbS^n$, and constant matrices $\bC,\,\bA_1, \dots, \bA_p \in \bbS^n$, i.e., they are all symmetric $n \times n$ matrices, the standard form of semidefinite programming~(SDP) problem is:
    % %     \begin{equation}
    % %         \begin{aligned}
    % %             \minimize_{\bX \in \bbS^n} \quad & \tr(\bC \bX) \\
    % %             \text{s.t.} \quad & \tr(\bA_i \bX) = b_i, \quad i = 1,\dots,p \\
    % %             & \bX \succeq 0.
    % %         \end{aligned}
    % %         \label{eq:sdp-std-form}
    % %     \end{equation}
    % %     \label{def:sdp}
    % % \end{definition}
    % % In above definition, $\tr(\cdot)$ stands for matrix trace.
    % % For symmetric matrix $\bA,\,\bB \in \bbS^n$, we can easily see $\tr(\bA\bB) = \sum_{i=1}^n \sum_{j=1}^n \bA_{i,j} \bB_{i,j}$.
    % % The SDP problem is a convex problem, where gradient-based methods and existing optimization approaches such as internal-point methods can find the global minima.
    % % In practice, off-the-shelf solvers can solve SDP in practical time for $n \times n$ matrix decision variable when $n$ is smaller than roughly $1,000$.
    
    % SDP Verify~\cite{raghunathan2018semidefinite} formulates the robustness verification as a SDP problem.
    % The main reformulation used in SDP Verify is:
    % \begin{equation}
    %     z_{ij} = \relu(\hz_{ij}) \Longleftrightarrow
    %     \left\{
    %     \begin{aligned}
    %         & z_{ij} \ge 0, \quad z_{ij} \ge \hz_{ij}, \\
    %         & z_{ij}z_{ij}^\T = z_{ij} \hz_{ij}^\T. \\
    %     \end{aligned}
    %     \right.
    %     \label{eq:relu-sdp-formulation}
    % \end{equation}
    % To handle the quadratic constraint, we define the vector $v := (1,\,z_1,\,\dots,\,z_l)^\T$ which encodes all ReLU activations, and consider the matrix $\bP = vv^\T$ as the SDP decision variable. 
    % Since we discard the constraint $\rank(\bP)=1$ which comes from $\bP = vv^\T$, it is a relaxation.
    % % 
    % % \para{SDP Verify.} SDP Verify~\cite{raghunathan2018semidefinite} formulates the robustness verification as a SDP problem.
    % % The main reformulation used in SDP Verify is:
    % % \begin{equation}
    % %     z_{ij} = \relu(\hz_{ij}) \Longleftrightarrow
    % %     \left\{
    % %     \begin{aligned}
    % %         & z_{ij} \ge 0, \quad z_{ij} \ge \hz_{ij}, \\
    % %         & z_{ij}z_{ij}^\T = z_{ij} \hz_{ij}^\T. \\
    % %     \end{aligned}
    % %     \right.
    % %     \label{eq:relu-sdp-formulation}
    % % \end{equation}
    % % The reformulation is equivalent to ReLU constraint with no relaxation, but introduces a quadratic constraint $z_i^2 = z_i^\T \hz_i$.
    % % In order to deal with this quadratic constraint, SDP Verify imposes constraints over the outer product.
    % % 
    % % Specifically, on feed-forward ReLU neural network, we define the vector $v := (1,\,z_1,\,\dots,\,z_l)^\T$ which encodes all ReLU activations, and consider the matrix $\bP = vv^\T$ as the SDP decision variable.
    % % The ReLU constraints as shown in \Cref{eq:relu-sdp-formulation}, the affine transformation constraints $\hz_k = \bW_{k-1}z_{k-1}+b_{k-1}$, and input constraints can all be encoded as linear constraints on this symmetric semi-positive matrix $\bP$.
    % % The objective function $f(x)_{y_0} - f(x)_y$ is a linear combination of $\bP$'s elements.
    % % Therefore, the verification problem can be formulated as an SDP.
    % % 
    % % Since we discard the constraint $\rank(\bP)=1$ which comes from the fact that $\bP = vv^\T$, it is a relaxation, i.e., SDP Verify is an incomplete verification approach. 
    % % 
    % % % To start with, consider single layer constraints 
    % % % $
    % % % \left\{
    % % %     \begin{aligned}
    % % %         & \hz_{k} = \bW_{k-1} z_{k-1} + b_{k-1} \\
    % % %         & z_{k} = \relu(\hz_{k})
    % % %     \end{aligned}
    % % % \right.
    % % % $,
    % % % we introduce the decision variable $\bP \in \bbS^{1 + n_{k-1} + n_k}$, and try to bound it to be $vv^\T$ where $v = (1,\,z_{k-1},\,z_k)^\T$.
    % % % Define the partition 
    % % % $$
    % % %     \bP := \left[
    % % %     \begin{matrix}
    % % %         \bP[1] & \bP[z_{k-1}]^\T & \bP[z_k]^\T \\
    % % %         \bP[z_{k-1}] & \bP[z_{k-1} z_{k-1}^\T] & \bP[z_{k-1} z_k^\T] \\
    % % %         \bP[z_k] & \bP[z_k z_{k-1}^\T] & \bP[z_k z_k^\T] \\
    % % %     \end{matrix}
    % % %     \right]
    % % % $$
    % % % Then, derived from \cref{eq:relu-sdp-formulation}, we can write down the following constraints:
    % % % \begin{subequations}
    % % %     % \small
    % % %     \begin{align}
    % % %         & \bP[z_k] \ge 0,\label{eq:percy-sdp-a} \\
    % % %         & \bP[z_k] \ge \bW_{k-1}\bP[z_{k-1}] + b_{k-1},\label{eq:percy-sdp-b} \\
    % % %         & \diag(\bP[z_k z_k^\T]) = \diag(\bW_{k-1}\bP[z_{k-1}z_k^\T]) + b_{k-1} \odot \bP[z_k^\T],\label{eq:percy-sdp-c}\\
    % % %         & \bP[1] = 1, \, \bP \succeq 0.\label{eq:percy-sdp-d}
    % % %     \end{align}
    % % %     \label{eq:percy-sdp-abcd}
    % % % \end{subequations}
    % % % In \cref{eq:percy-sdp-c}, the operator $\odot$ stands for element-wise product.
    % % % The \cref{eq:percy-sdp-a,eq:percy-sdp-b,eq:percy-sdp-c} correspond to $z_{ij} \ge 0$, $z_{ij} \ge \hz_{ij}$ and $z_{ij}z_{ij}^\T = z_{ij}\hz_{ij}^\T$ in \cref{eq:relu-sdp-formulation} respectively.
    % % % The \cref{eq:percy-sdp-d} tries to constrain $\bP$ to be the outer product $vv^\T$.
    % % % Here comes the relaxation, as another constraint $\rank(\bP) = 1$ is required to fulfill such constraint, but is discarded for ease of solving.
    % % 
    % % % When it comes to multiple layers, we construct $\bP \in \bbS^{1 + \sum_{i=1}^{l-1} n_i}$ to express all neurons in all but last layers.
    % % % And construct ReLU constraints similar to \cref{eq:percy-sdp-abcd}.
    % % % Here we deal with $\cL_\infty$-bounded perturbations, thus, $z_1 = x \ge x_0 - \epsilon$ and $z_1 = x \le x_0 + \epsilon$ exactly express the input constraints of $x \in B_{\infty,\epsilon}(x_0)$.
    % % % The objective function is $f(x)_y - f(x)_{y'} = \left(\bW_{l-1})_{y,:} - (\bW_{l-1})_{y',:}\right) \bP[z_{l-1}] + b_{l-1}$, which is a linear constraint and brings a lower bound for \cref{eq:verification-optimization-problem}.
    % % % So SDP Verify is a verification approach.
    % % 
    % SDP Verify usually gives much tighter bound than linear relaxations, both shown experimentally and theoretically in \cite{raghunathan2018semidefinite}, and it flees from the ``linear relaxation barrier'' discussed in \cite{salman2019convex}.
    % Moreover, unlike linear relaxations, SDP Verify behaves well for ``external networks'':
    % for neural networks which are not robustly trained~(e.g., only empirically defensed), SDP Verify still provides reasonably good robustness radius, unlike linear relaxation-based verification approaches.
    % % When the network is not certifiably defenses using linear relaxations, the verification approaches based on linear relaxations usually provides vacuous robustness radius, while SDP Verify still provides reasonbly good robustness radius.
    % However, the number of decision variables, as we can see, is of quadratic order to number of neurons, making it not scalable even to moderate size models on MNIST.
    
    % PGD-SDP~\cite{dvijotham2019efficient} exploits \Cref{eq:relu-sdp-formulation} and introduces several SDP-based relaxations from Lagrangian dual space, which results in a much scalable approach than SDP Verify, but loses tightness in some degree and the ability to verify ``external networks''.
    % LMIVerify~\cite{fazlyab2019efficient} considers the dual problem of SDP - optimization with linear matrix inequality constraints~(LMI).
    % It enables scalability/tightness adjustments from relaxation mode adjustments. However, in practice, LMI Verify is either too slow or too loose comparing to other approaches.
    % SDPTrain~\cite{raghunathan2018certified} is an early-stage work.
    % % towards certifiable robustness verification and training.
    % It uses a SDP relaxation to lower bound $\max_{x \in B_{\infty,\epsilon}(x_0)} \|f(x)\|_1$, which can derive the overall optimization problem lower bound.
    % However, the approach is limited to only two-layer networks, and it obtains non-trivial verifiable robustness on only MNIST dataset with small radius.
    
    % % % \para{PGD-SDP.} 
    % % PGD-SDP~\cite{dvijotham2019efficient} exploits \Cref{eq:relu-sdp-formulation} and turn to its Lagrangian dual.
    % % It introduces additional semi-definite constraint to turn the inner maximization to convex problem, fixes some dual variables and decouples some variable dependencies, though at the cost of tightness loss.
    % % Then, PGD-SDP uses PGD to optimize the remaining variables.
    % % As the result, the verification is significantly scalable than SDP Verify~\cite{raghunathan2018semidefinite}, and reaches the tightness level between SDP Verify and linear relaxation based approaches.
    % % However, it loses the ability to verify ``external networks''.
    % % 
    % % Then, just as many previous \citeauthor{dvijotham2019efficient}'s work, it directly turns to its Lagrangian dual problem, with the ReLU constraint being replaced by \Cref{eq:relu-sdp-formulation}.
    % % In the dual min-max problem, though the overall problem is convex, the inner maximization with respect to $x$ is still non-convex.
    % % PGD-SDP introduces the additional semi-definite constraint to turn it to convex problem, though at the cost of verification tightness.
    % % Furthermore, PGD-SDP fixes some dual variables and decouples some variable dependencies.
    % % Then, PGD-SDP uses PGD to iteratively optimize the remaining variables.
    % % As the result, the verification is significantly scalable than SDP Verify~\cite{raghunathan2018semidefinite}, and reaches the tightness level between SDP Verify and linear relaxation based approaches.
    % % However, it loses the ability to verify ``external networks''.
    % % 
    % % LMIVerify~\cite{fazlyab2019safety} formulates the verification problem as optimization where the constraints are linear matrix inequalities~(LMI).
    % % LMI is the dual problem of SDP.
    % % The LMI formulation allows us to adjust number of free variables and thus adjust the scalability/tightness easily.
    % % However, in practice, LMIVerify is typically too slow or too loose comparing to other approaches.
    % % However, from experiments we find that, when the number of free variables is reduced to an solvable level, the tightness drops drastically and becomes much inferior than SDP Verify.
    
    % % \para{LMIVerify.} LMIVerify~\cite{fazlyab2019safety} formulates the verification problem as optimization where the constraints are linear matrix inequalities~(LMI).
    % % LMI is the dual problem of SDP.
    % % % The linear matrix inequalities can be viewed as a linearly parameterized matrix.
    % % The approach stems from control theory and partitions the constraints to three components: input specification, ReLU specification, and safety specification.
    % % % The input specification matrix determines a quadratic form where all legal inputs induces $\ge 0$ value.
    % % % The ReLU specification matrix determines a quadratic form where all legal input-output for ReLUs induce $\ge 0$ value.
    % % % While the sefety specification matrix determines a quadratic form where any correct predictions induce $\le 0$ value.
    % % % As the result, by summing these matrices up, if the summation is a semi-negative matrix, the model is provable robustness.
    % % % Easily seen, the relaxations could come from the semi-negative condition, and the summation.
    % % % Since LMI is the dual problem of SDP~(strong duality is satisfied when Slater's condition holds~\cite{slater2014lagrange}), it can be as efficiently solved as SDP.
    % % The LMI formulation allows us to adjust number of free variables and thus adjust the scalability/tightness easily.
    % % % by adjusting the specification matrix form, thus we can adjust the scalability easily.
    % % However, from experiments we find that, when the number of free variables is reduced to an solvable level, the tightness drops drastically and becomes much inferior than SDP Verify.
    
    % % SDPTrain~\cite{raghunathan2018certified} is an early-stage work towards certifiable robustness verification and training.
    % % It uses a SDP relaxation to lower bound $\max_{x \in B_{\infty,\epsilon}(x_0)} \|f(x)\|_1$, which can derive the overall optimization problem lower bound.
    % % However, the approach is limited to only two-layer networks, and it obtains non-trivial certifiable robustness on only MNIST dataset with small radius.
    % % % and the radius used for training is small.
    % % % However, it inspired the aforementioned SDP Verify~\cite{raghunathan2018semidefinite}.
    
    % % \para{SDP Train.} SDPTrain~\cite{raghunathan2018certified} is an early-stage work towards certifiable robustness verification and training.
    % % SDPTrain uses two-step relaxation: 
    % % (1)~relate $f(x)$ lower bound to $\max_{x \in B_{\infty,\epsilon}(x_0)} \|f(x)\|_1$; 
    % % (2)~use a SDP relaxation to compute $\max_{x \in B_{\infty,\epsilon}(x_0)} \|f(x)\|_1$.
    % % The dual of the relaxed SDP is injected to the training objective as a \textbf{certifiable defense}.
    % % % since it provides a valid lower bound.
    % % % Due to the excessive over-approximation, 
    % % The approach is limited to only two-layer networks.
    % % Furthermore, it obtains non-trivial certifiable robustness on only MNIST dataset with small radius.
    % % % and the radius used for training is small.
    % % However, it inspired the aforementioned SDP Verify~\cite{raghunathan2018semidefinite}.
    
    % Comparing to linear relaxations, using SDP seems to be less popular, even though its potential to achieve much tighter verification than linear relaxations.
    % We think the main reason is its scalability.
    % Using common solvers, the raw SDP problem can only be practically solved when the matrix size $n$ is less than $1,000$. 
    % However, the input dimension of CIFAR-10 images is over $2,000$.
    % Further relaxations based on SDP is hard technically, and such relaxations make SDP much looser, i.e., lose its main advantage.
    % In \Cref{sec:scaling-up-sdp-approaches}, we discuss a potential direction for scaling up SDP-based verification approaches.

 \subsection{Certified Robustness Based on Lipschitz and Curvature}
    \label{sec:lipschitz-intro}
    If we know $f(x_0)$, the lower bound value of $f(x)$ for $x \in B_{p,r}(x_0)$ can be easily computed given the local Lipschitz constant $L$ for $x \in B_{p,r}(x_0)$.
    % The definition of Lipchitz constant is in \Cref{def:lipschitz-constant}.
    % , and the formal theorem is in \cref{thm:lipschitz-based-theorem}.
    A few work performs verification along this line, mainly targeting at providing a tighter estimation of local Lipschitz constant $L$.
    
    \t{Op-Norm}~\cite{szegedy2013intriguing} simply multiples the norm of all weight matrices $\bW_i$ to obtain the global Lipschitz constant of the model.
    \t{CL}~\cite{hein2017formal} computes local Lipschitz constant for one-hidden-layer neural networks using differentiable proxy $\sigma_\alpha(x) = \alpha^{-1} \log(1 + \exp(-\alpha x))$ of ReLU as the activation function, and it proposes a training regularizer to reduce such Lipschitz constant, i.e., it is also a robust training approach.
    \t{FastLip}~\cite{weng2018towards} and \t{RecurJac}~\cite{zhang2019recurjac} compute local Lipschitz constant in a similar way as \t{FastLip} and \t{CROWN}.
    SDP based approaches can also be used for local Lipschitz constant computation~\cite{fazlyab2019efficient}, however, the low scalability impedes it from practical usage.
    In general, both local and global Lipschitz constant are too loose to be used in practice.
    % for robustness verification.
    
    Recently, \t{CRC/CRT}~\cite{singla2020second} is proposed to leverage the second-order derivative bound, i.e., curvature bound, for robustness verification and robust training.
    The results on MNIST is promising.
    However, the approach only supports smooth activation functions~(excluding ReLU), small fully-connected neural networks on MNIST, and $\cL_2$ adversary.
    
    
    % % 
    % \begin{definition}[Lipschitz Constant]
    %     \label{def:lipschitz-constant}
    %     We say scalar function $g: \bbR^n \supseteq \cX \mapsto \bbR^C$ has local Lipschitz constant $L$ with respect to $\cL_q$ norm, in region $B_{p,r}(x_0)$ if $\forall x,y \in B_{p,r}(x_0)$ and $\forall c \in [C],$
    %     \begin{equation}
    %         \dfrac{|g_c(x) - g_c(y)|}{\|x - y\|_q} \le L.
    %     \end{equation}
    % \end{definition}
    % % 
    % % \begin{theorem}[Lipschitz-Based Lower Bound]
    % %     Let $x_0 \in \cX$ be the original input and $y_0 \in [C]$ be its label.
    % %     Suppose $L$ is the local Lipschitz constant with respect to $\cL_q$ norm of function $(f_\theta)_{y_0} - (f_\theta)_{y}$ for $x \in B_{p,r}(x_0)$ and for any $y \in [C]$ such that $y \neq y_0$.
    % %     Then, within region $B_{p,r}(x_0)$,
    % %     \begin{equation}
    % %         \begin{aligned}
    % %         & f_\theta(x)_{y_0} - \max_{y\in [C]: y\neq y_0} f_\theta(x)_y \\
    % %         \ge &
    % %         \min_{y\in [C]: y\neq y_0} (f_\theta(x_0)_{y_0} - f_\theta(x_0)_y) - rL.
    % %         \end{aligned}
    % %         \label{eq:lipschitz-based-lower-bound}
    % %     \end{equation}
    % %     Here, $p$ and $q$ are dual norms.
    % %     \label{thm:lipschitz-based-theorem}
    % % \end{theorem}
    % % In particular, when $g$ is continuous and diffentiable almost everywhere, any $L \ge \max_{x \in B_{p,r}(x_0)} \| \nabla g(x) \|_q$ is a valid local Lipschitz constant.
    % % 
    % % \begin{proof}
    % %     From \cref{def:lipschitz-constant}, we know that $g(x) \in [g(x_0) - L\|x - x_0\|_p,\, g(x_0) + L\|x - x_0\|_p]$ given that $g$ is locally $L$-Lipschitz with respect to $\cL_p$'s dual norm $\cL_q$.
    % %     The \cref{eq:lipschitz-based-lower-bound} directly follows from this observation.
    % % \end{proof}
    % % 
    % % As we can see, the \cref{eq:lipschitz-based-lower-bound} provides a lower bound for \cref{eq:verification-optimization-problem}.
    % % Therefore, 
    % Easily seen, given that we know $f(x_0)$~(the model output for the clean input $(x_0,\,y_0)$), once we know $L$ for function $x \mapsto f_{y_0}(x) - f(x)$, the lower bound for \Cref{prob:verification-optimization-problem} can be easily computed, and the robustness can be thus verified.
    % Note that even we could obtain a tight $L$, the bound may still be loose, because the model may only have gradient as large as $L$ in small region.
    
    % % \para{Op-norm.}
    % Op-norm~\cite{szegedy2013intriguing} is firstly proposed to analyze the neural network properties, and is used as a verification approach in \cite{weng2018towards}.
    % It is the global Lipschitz constant of model $f_\theta$.
    % The Op-norm simply computes the product of $\cL_p$-induced norm of all weight matrices $\bW_i,\,1\le i \le l-1$. 
    % According to \cite{szegedy2013intriguing}, this is the $\cL_q$ global Lipschitz constant of the model $f_\theta$, i.e., $L = \prod_{i=1}^{l-1} \|\bW_i\|_p$, because ReLU function is a contractive mapping~\cite{szegedy2013intriguing}.
    % The approach is effective and scalable due to simple matrix norm computation, but gives very loose bound.
    % It is also called spectral norm, e.g., in \cite{zhang2019recurjac}.
    % % In some other literature, such as \cite{zhang2019recurjac}, this simple approach is also called spectral norm, as it directly uses the product of spectral norms of weight matrices.
    
    % % \para{CL.}
    % CL~\cite{hein2017formal} considers neural networks with only one hidden layer using the differentiable proxy $\sigma_\alpha(x) = \alpha^{-1} \log(1 + \exp(-\alpha x))$ of ReLU as the activation function.
    % Under this condition, it derives an approach for computing local Lipschitz constant for each $(f_\theta)_{y_0} - (f_\theta)_y$, which is significantly tighter than the global Lipschitz constant used on Op-norm.
    % Also, it proposes a training regularizer to reduce such Lipschitz constant in a heuristic way.
    % The experiment shows the effectiveness of both local Lipschitz computation, and the robust training approach.
    % However, the approach is hard to scale up when the number of hidden layers is larger than just one, and when the activation function is ReLU.
    
    % % \para{FastLip.}
    % FastLip~\cite{weng2018towards} computes the local Lipschitz constant for any feedforward ReLU neural networks.
    % It borrows the ideas from linear relaxations - computes $l$ and $u$ and decides which neurons are stable.
    % The $l$ and $u$ can be computed using linear relaxations, MILP, etc.
    % With $l$ and $u$, FastLip derives Lipschitz constant by discussing the lower bound and upper bound induced by the unstable neurons in a similar way as Fast-Lin~\cite{weng2018towards}.
    % % Then, FastLip unfolds the neural network expression.
    % % Since the slope of each ReLU neuron for a given input is either $0$ and $1$, FastLip bounds the maximum gradients by considering the worst case slopes of unstable neurons which maximizes the overall gradients.
    % % The bound is computed elementwise.
    % % In this way, the lower and upper gradient bound for each neuron in current layer could be obtained.
    % % When it comes to multiple layers, FastLip derives the new bound with the last layer added when the bound of previous layers is present, thus the bound could be iteratively computed similar as Fast-Lin.
    % % From these elementwise gradient bound, we can easily derive the end-to-end local Lipschitz bound for any $\cL_p$.
    % The approach is more scalable and tighter than Op-norm.
    % Its efficiency is similar to Fast-Lin, however, the tightness is much worse than these linear relaxation based verification approaches introduced in \Cref{sec:lp-relaxation-intro}.
    
    % % \para{RecurJac.}
    % RecurJac~\cite{zhang2019recurjac} further improves FastLip by exploiting stable neurons better to tighten the Lipschitz bound.
    % Moreover, RecurJac supports any gradient bounded activations functions, while in FastLip except ReLU only LeakyReLU is supported.
    % % RecurJac~\cite{zhang2019recurjac} improves FastLip by making better use of stable neuron information.
    % % For stable neurons, it jumps out of the layer-by-layer bounding scheme and eagerly extends the corresponding entries.
    % % In this way, the worst case analysis in FastLip becomes tighter in RecurJac.
    % % In practice, RecurJac has significantly tighter bound than FastLip, and thus induces a tighter verification approach.
    % % Moreover, RecurJac supports any gradient bounded activations functions, while in FastLip except ReLU only LeakyReLU is supported.
    
    % SDP based approaches can also be used for local Lipschitz constant computation~\cite{fazlyab2019efficient}, however, the low scalability and the inherent looseness of Lipschitz-based verification prevent it from practical use.
    % In fact, both local and global Lipschitz constant are too loose to be used practically for robustness verification.
    % % However, it has many other applications such as neural network analysis.

 \subsection{Probabilistic Robustness Verification}
 \label{sec:probabilistic-robustness-verification-root}
%  \subsection{Certified Robustness Inspired by Random Noise}

%  before change-------
% Besides the deterministic verification approaches, one recently emerging branch of studies propose to exert random noise to the classifiers, randomizing the predictions. The final prediction is the label with the highest probability under the probabilistic setting. (See \Cref{def:smoothing_measure}, \Cref{def:randomized_classifier}) We call this line of works the \emph{probabilistic robustness verification} approaches in our context.
% after change--------
Besides the deterministic verification approaches, one recently emerging branch of studies propose to add random noise to smooth the models and derive the  certified robustness for these smoothed models~(See \Cref{def:randomized_classifier}). We call this line of work \emph{probabilistic robustness verification} approaches or \emph{randomized-smoothing based} approaches,
since they provide probabilistic robustness guarantees for these randomized models smoothed by noise.
% in our context.
% (See definition \ref{def:base_classifier}, \ref{def:smoothing_measure}, \ref{def:randomized_classifier})

% Moreover, state-of-the-art certification results on real world datasets like Cifar-10 and ImageNet are achieved under this setting.

% We will outline this set of verification approaches in the following subsections:
% \Cref{sec:rand-smooth-intro-1} presents necessary preliminaries and notations;
% \Cref{sec:rand-smooth-intro-2} discusses early ideas like \emph{differential privacy}~\cite{lecuyer2019certified} and \emph{divergence based bounding}~\cite{li2019certified};
% \Cref{sec:rand-smooth-intro-3} introduces \emph{Neyman-Pearson based certification} approaches for various noise types and distance metrics~(\cite{cohen2019certified,lee2019tight,teng2020ell,Zhang2020BlackBoxCW,levine2019robustness});
% \Cref{sec:rand-smooth-intro-4} shows more general frameworks from \cite{Dvijotham2020A,yang2020randomized};
% \Cref{sec:rand-smooth-intro-5} discusses several certifiable defenses~(\cite{salman2019provably,Zhai2020MACER:,feng2020regularized});
% and \Cref{sec:rand-smooth-intro-6} analyzes theoretical limitations~(\cite{yang2020randomized,kumar2020curse,mohapatra2020rethinking}).

% Necessary preliminaries and notations are covered in \Cref{sec:rand-smooth-intro-1}. Early ideas like \emph{differential privacy} \cite{lecuyer2019certified} and \emph{divergence based bounding} \cite{li2019certified} are reviewed in \Cref{sec:rand-smooth-intro-2}. Then, in \Cref{sec:rand-smooth-intro-3}, we will introduce \emph{Neyman-Pearson based certification} which includes a special family of certification approaches (\cite{cohen2019certified,lee2019tight,teng2020ell,Zhang2020BlackBoxCW,levine2019robustness}) for various noise types and distance metrics. \Cref{sec:rand-smooth-intro-4} covers two works (\cite{Dvijotham2020A,yang2020randomized}) that aim at building more general frameworks.
% % 
% Besides the robustness certification, in \Cref{sec:rand-smooth-intro-5}, we will review various techniques (\cite{salman2019provably,Zhai2020MACER:,feng2020regularized}) that help to enhance the robustness of randomized models. Analysis of theoretical limitations of the probabilistic robustness verification methods (\cite{yang2020randomized,kumar2020curse,mohapatra2020rethinking}) are covered in \cref{sec:rand-smooth-intro-6}.


%\begin{definition}[Base Classifier]
%\label{def:base_classifier}
%Base classifier is the deterministic model built on standard setting. A soft classifier is defined as $f$ : $\cX \mapsto \cP $. Given any input $x\in \cX$, the output $f(x)\in \cP$ is a \emph{probability} vector on candidate labels set : $\cK=[C]$, denoted as $f(x) := (f_1(x),\dots,f_C(x)) $. Based on a corresponding soft classifier, a hard classifier could be defined as $F$ : $\cX\mapsto \cK$,  $F(x):=\argmax_i{f_i(x)} $.
%\end{definition}

% \begin{definition}[Smoothing Mechanism]
% \label{def:smoothing_measure}
% Given an input $x\in \mathcal{X}$, a smoothing mechanism $\mu$ computes $\mu(x,x')$ to denote the probability density at $x'\in \cX$ where $x'  = x+\epsilon$ and $\epsilon$ is sampled from the smoothing distribution $\mu_x$.
% \end{definition}

\begin{definition}[Randomized Classifier]
\label{def:randomized_classifier}
Given a smoothing distribution $\mu$, we use $\mu(\delta)$ to denote the density at $\delta$. 
% The randomized counterpart of any given function $f$ on input space $\mathcal{X}$ is defined as:
% \begin{small}
% \begin{equation}
%     h_{\smooth}(x)=\int_{\epsilon\in \supp(\mu)}{f(x+\epsilon)\mu(\epsilon)} \dif \epsilon.
%     \label{eq:h-smooth}
% \end{equation}
% \end{small}
% \linyi{Propose to change the above definition to below.}
For a given classifier $F$,  we define the \emph{randomized classifier} $F_{\smooth}$ as: 
% \begin{small}
$$
    \small
    F_{\smooth}(x)
    % = \argmax_{i\in [C]} \1\left[F(\cdot)=i\right]_{\smooth} 
    = \argmax_{i \in [C]} \int_{\delta\in \supp(\mu)} \1\left[F(x + \delta)=i\right]\mu(\delta) \dif \delta.
$$
\label{eq:h-smooth}
% \end{small}
% Specifically, we define \emph{soft randomized classifier}: $g(x)=\bbE_{\epsilon \sim \mu}[f(x+\epsilon)]$ and \emph{hard randomized classifier}: $g(x)=\argmax_{i\in [C]}{\Pr_{\epsilon \sim\mu}}[F(x+\epsilon)=i]$, where $F(x):=\argmax_{i\in [C]}{f(x)_i}$ as defined in \Cref{sec:sec_notations}.
\end{definition}

In probabilistic verification, the integral in \Cref{eq:h-smooth} cannot be exactly solved. Thus, instead, Monte Carlo estimation and hypothesis test from
\cite{hung2019rank} are used to approximate the exact solution. As a result, the verification result only holds with certain probability as mentioned in \Cref{def:verification-approach}. Specifically, most of existing work follows the approximation algorithm \sc{Certify} in \cite{cohen2019certified}. 

To our best knowledge, all existing probabilistic verification approaches keep agnosticism about model architectures. This relaxation makes probabilistic approaches scalable to large neural network models such as those on ImageNet dataset. However, due to the relaxations, all the probabilistic verification approaches are incomplete. Among the existing methodologies, the Neyman-Pearson based approaches (\Cref{sec:rand-smooth-intro-3}) achieve the tightest certification under the probabilistic setting.





% \subsubsection{\textbf{ Motivation Based on Differential Privacy}\texorpdfstring{~\cite{lecuyer2019certified, li2019certified}}{}}\hfill \\
\subsubsection{\textbf{ Motivation from Differential Privacy}\texorpdfstring{~\cite{lecuyer2019certified, li2019certified}}{}}\hfill \\
\label{sec:rand-smooth-intro-2}
Differential privacy \cite{dwork2006calibrating} aims at securing sensitive information while releasing statistical quantities from a database. The core idea is --- if the absence of an individual would nearly not influence the statistics, no privacy of this individual could be leaked by comparing the difference of statistics.
% 
% The differential privacy theory \cite{dwork2006calibrating} is originally aiming at securing individual information while releasing statistics quantity from a database. The threat scenario is: while releasing the statistics from a database, an individual sample's information may be included in one statistics while may not in another statistics, then by comparing the difference, one may conclude this specific individual's private information. Differential privacy theory 
% solves this problem based on a straightforward idea: if the absence of an individual would nearly not influence the statistics, then, no privacy of this individual could be leaked by comparing the difference. This idea can be naively formalized as: $\Pr [h(x)=t] \approx \Pr [h(\hat{x})=t]$, where $h$ is the statistics function, and both $x$, $\hat{x}$ are databases and only differ in one instance (we can call this absent instance $I$). When we get a statistics $t$ from a database, we cannot conclude whether $I$ is in the database, if the probability that we get statistics $t$ from the two databases are almost the same. 
% 
Analogously, if the change or absence of a few pixels cannot be concluded by comparing the difference of statistics~(e.g., the model prediction), the model itself should be robust. 
Based on this connection, \cite{lecuyer2019certified} first proves the effectiveness of the randomized smoothing technique as a defense mechanism and provides rigorous robustness verification under probabilistic setting. Gaussian and Laplacian mechanisms from \cite{dwork2006calibrating} are directly adopted for randomization and robustness verification.
% Later, \fullcite{cohen2019certified} rewrite this robustness condition for $\cL_2$ metric with Gaussian noise in a more compact form, and derive the robustness condition for $\cL_1$ metric with Laplacian noise.

% :
% $$
% R = \sup_{0\textless \epsilon \le \min{(1,\frac{1}{2}\log{\frac{P_A}{P_B}}})} {\frac{\sigma\epsilon}{\sqrt{2\log{(\frac{1.25(1+exp(\epsilon))}{P_A-exp(2\epsilon)p_B})}}}},
% $$
% where R is the robustness radius and $P_A,P_B$ are probabilities of top-1 and runner-up classes.

% Similarly, the radius under $L_1$ metric and Laplacian noise is derived as:
% $$
% R = \frac{\sigma}{2\sqrt{2}}\log{\frac{P_A}{P_B}} =\frac{\lambda}{2}\log{\frac{P_A}{P_B}}
% $$


Later, the robustness radius (recall the definition in \Cref{sec:sec_notations}) derived in \cite{lecuyer2019certified} are shown to be loose. \citeauthor{li2019certified}~\cite{li2019certified} derive tighter robustness radius by bounding the variation of the output based on R\'enyi Divergence.
% Empirically, the certification made by differential privacy based method is shown to be loose. Therefore, in \cite{li2019certified}, the concept of differential privacy is totally abandoned. Instead, they derive the certification radius through bounding the variation of the output under the metric of R\'enyi Divergence.
% % 
% The key idea is: for any two probability predictions which lead to different top-1 labels, there is a lower bound for the R\'enyi Divergence between the two predictions. Then, as long as we could bound the R\'enyi divergence of the predictions within the lower bound, the top-1 class corresponding to the prediction would remain constant. Based on this idea, tighter robustness radii are derived. 
% 
Specifically, with the smoothing distribution as Gaussian $\cN(0,\sigma^2I)$, the $\cL_2$ certified robustness radius $r$ is derived as:
$$
\resizebox{0.49\textwidth}{!}{
$
 r = \sup_{\alpha > 1}{-\dfrac{2\sigma^2}{\alpha}\log\left(1-P_{A}-P_{B}+2\left(\frac{1}{2}(P_{A}^{1-\alpha}+P_{B}^{1-\alpha})\right)^{\frac{1}{1-\alpha}}\right)},
$
}
$$
where $P_A,P_B$ are the 
% lower and upper bounds for 
probabilities of top-1 and runner-up classes respectively, $\alpha$ is the parameter of R\'enyi Divergence. 
Similarly, $r = -\lambda\ \log(1-P_A+P_B)$ is derived for $\cL_1$ metric under Laplacian noise $\mathrm{Laplace}(0,\lambda)$.
% \linyi{change $p_{(1)}, p_{(2)}$ to $p_A, p_B$, check if it is correct}



\subsubsection{\textbf{Neyman-Pearson Based approaches}~\texorpdfstring{\cite{cohen2019certified,teng2020ell,lee2019tight,levine2019robustness,Zhang2020BlackBoxCW}}{}} \hfill \\
\label{sec:rand-smooth-intro-3}
\para{Geometry perspective.} Suppose we choose uniform distribution on a bounded ball $B_{p,\epsilon}$ as the smoothing distribution.
For any input $x_0$, the randomized classifier queries all points in $B_{p,\epsilon}(x_0)$ uniformly and picks the label $c$ which has the largest mass $P_A$.
Likewise, for its neighboring point $x_0'$, the randomized classifier queries all points in $B_{p,\epsilon}(x_0')$ uniformly.
To lower bound the mass of label $c$ in $B_{p,\epsilon}(x_0')$, namely $P_A'$, the information we can use is the volume of intersection $B_{p,\epsilon}(x_0) \cap B_{p,\epsilon}(x_0')$ which is represented by $\beta$. 
% $B_{p,\epsilon}(x_0) \cap B_{p,\epsilon}(x_0')$ w.r.t $B_{p,\epsilon}(x_0)$.
Then, we can lower bound $P_A'$ as $P_A' \ge \max\{ P_A - (1 - \beta),\,0 \}$ by considering the worst case that all the points in the non-intersection region have the label $c$.
If the lower bound of $P_A'$ $\ge 0.5$, we can certify that the predicted label at point $x_0'$ is still $c$.
Unlike the uniform distribution, if we choose other noise distributions such as Gaussian or Laplace, which has non-zero support for the whole data space, lower bounding $P_A'$ involves more analysis. Intuitively, the concepts of ``intersection'' and ``non-intersection'' can be generalized to ``likelihood ratio''.
% 
% Let's consider a simple case where the random noise are sampled from a cubic uniform distribution. When we input $x$ to the randomized model, instead of merely querying the single point $x$, all the surrounding points in the cube $M$ centered at $x$ will be queried. We call the surrounding cube the ``sampling region''. The top-1 label $c$ that takes the highest ratio $P_A$ of the sampling region is eventually returned as the prediction. Likewise, for the point $x'$, which is the close neighbor of $x$, the randomized model will also query the whole sampling region $N$ around it. 
% 
% Given the sampling probability $P_A$ of class $c$ in $M$, the only secrete that enables us to bound the probability $P_A'$ for $c$ in $N$ is the rich information residing in the intersection between $M$ and $N$ --- suppose the intersection region takes a ratio of $P_I$ of $M$, then, for label $c$ in $M$, there is at least a ratio of $max\{P_A - (1-P_I),0\}$ is from the intersection region (in the worst situation, all the points in the non-intersection region have the label $c$), thus, the probability of $c$ at $x'$ is at least $max\{P_A - (1-P_I),0\}$. And in this simple case, if we do not have any other knowledge about the labels' distribution in the sampling region, that is already the best bound we could certify. %%Thus, then second question is also answered under this simple setting.
% 
% 
% For noise types that have nonzero support for the whole data space, like Gaussian or Laplacian noise, the story is much more complex, because we can not simply use the concepts like intersection and non-intersection for sampling regions under these scenarios. Instead, the concepts of `intersection' and `non-intersection' are generalized as `likelihood ratio' in definition \ref{def:likelihood_ratio}.
% 
\begin{definition}[Likelihood Ratio]
\label{def:likelihood_ratio}
The likelihood ratio on $z$ under two sampling centers $x$ and $\bar{x}$ is defined as follow:
% $$
% \eta_{x,\bar{x}}(z) := \dfrac{\Pr_{X\sim \mu(x)} [X=z]}{\Pr_{X\sim \mu(\bar{x})} [X=z]}.
% $$
% \linyi{The above is the probability of continuous random value equals to some value, which is $0$... Propose change to below}\bo{agree, please change it}
$$
\eta_{x,\bar{x}}(z) := \dfrac{\mu(z - x)}{\mu(z - \bar{x})}.
$$
\end{definition}

%=============== previous version =================
% Given \Cref{def:likelihood_ratio}, one intuition is: the region where the likelihood ratio is very close to 1 could be deemed as the general form of intersection region, and otherwise the non-intersection region. 
% % 
% Analogously, given the mass $P_A$ of label $c$ under $\mu(x_0)$, we could try to find the lower bound of the mass $P_A'$ for label $c$ under $\mu(x_0')$ by greedily supposing all the points with high likelihood ratio have label $c$ under $\mu(x)$~(similar to supposing all points in ``non-intersection'' region has label $c$). To be more concrete, we need to find a threshold $k$, such that the set~(called Neyman-Pearson set later) $S=\{z:\,\eta_{x_0,x_0'}(z)\ge k\}$ exactly has a mass of $P_A$ under the measure $\mu(x_0)$, then the mass of $S$ under measure $\mu(x_0')$ is the tightest lower bound we can achieve for $P_A'$ without additional information other than label statistics. \bo{Linyi, please read this section} 
% % we do not have additional knowledge about the label's distribution. 
% % Likewise, we could also derive the upper bound of $P_A'$ in similar manner (greedily suppose all the points in $\bar{S}$ has the label $c$). 
% % 
% This intuition is theoretically justified in \cite{cohen2019certified} by applying the Neyman-Pearson lemma \cite{neyman1933ix}.
%=============== new version =================
Given \Cref{def:likelihood_ratio}, one intuition is: the region where the likelihood ratio is very close to 1 could be deemed as the general form of intersection region, and otherwise the non-intersection region. 
% 
Analogously, given the mass $P_A$ of label $c$ under shifted distribution $x + \mu$~(meaning distribution $\mu$ shifted by vector $x$), we could try to find the lower bound of the mass $P_A'$ for label $c$ under shifted distribution $x' + \mu$ by greedily supposing all the points with high likelihood ratio have label $c$~(similar to supposing all points in ``non-intersection'' region have label $c$). To be more concrete, we need to find a threshold $k$, such that the set~(called Neyman-Pearson set later) $S=\{z:\,\eta_{x_0,x_0'}(z)\ge k\}$ exactly has a mass of $P_A$ under the distribution $x_0 + \mu$, then the mass of $S$ under distribution $x_0' + \mu$ is the tightest lower bound we can achieve for $P_A'$ without additional information other than label statistics. 
% \bo{Linyi, please read this section} 
% we do not have additional knowledge about the label's distribution. 
% Likewise, we could also derive the upper bound of $P_A'$ in similar manner (greedily suppose all the points in $\bar{S}$ has the label $c$). 
% 
This intuition is theoretically justified in \cite{cohen2019certified} by applying the Neyman-Pearson lemma \cite{neyman1933ix}.
%=============== end =================


\para{Optimization perspective.} Despite additional uncertainty in randomized classifiers, the verification could still be modeled as an optimization problem similar to the discussion in \Cref{prob:verification-optimization-problem}. %So far, we have explained the principle of Neyman-Pearson based verification mainly from a geometrical perspective. Interestingly,
\citeauthor{Zhang2020BlackBoxCW}~\cite{Zhang2020BlackBoxCW} proposed a verification framework purely~from~optimization~perspective.% --- functional optimization, which essentially could also be attributed to the Neyman-Pearson family.

%Consider the verification problem under binary setting:
%$$
%    \min_{x':\|x-x'\|_p \le r} \Pr_{X\sim \mu(x')}[F(X)=c]>0.5,
%$$
Since we keep agnosticism about the base classifier $F$ and the only knowledge we have is $\Pr_{\delta \sim \mu}[F(x+\delta)=c]=P_A$, the key idea of \cite{Zhang2020BlackBoxCW} is to compute the lower bound of $\min_{x':\|x-x'\|_p \le r} \Pr_{\delta \sim \mu}[F(x'+\delta)=c]$ by performing relaxation on the base classifier $F$. More concretely, they allow $F$ to be any function from $\mathcal{H} := \{H: H(z)\in [C], \forall z \in \bbR^n \}$, as long as the condition $\Pr_{\delta\sim\mu}[F(x+\delta)=c]=P_A$ holds. Through Lagrange duality, this relaxed optimization problem could be efficiently solved using the proposed algorithm. 
Essentially, this methodology is still based on Neyman-Pearson, since a Neyman-Pearson set is implicitly constructed during the optimization process. 
% \textbf{Interested readers could refer to Appendix for rigorous justification of this claim.}

We observe that a considerable amount of probabilistic verification approaches~\cite{cohen2019certified,lee2019tight,teng2020ell,Zhang2020BlackBoxCW,levine2019robustness} could be attributed to this family, and they either explicitly or implicitly construct the Neyman-Pearson set $S$. We outline these approaches as follow.
% We will list them out in the rest of this subsection. 


\para{Verification under $\cL_2$ metric.}  Under Gaussian smoothing distribution $\mu$, given $\Pr_{\delta\sim\mu}[F(x+\delta)=c]=p$, \citeauthor{cohen2019certified}~\cite{cohen2019certified} construct the corresponding Neyman-Pearson set for $\cL_2$ metric:
$$
S := \left\{z\in \mathbb{R}^d:v^\T(z-x)\ge\sigma \|v\|_2\Phi^{-1}(p)\right\},
$$
and the $\cL_2$ robustness radius is derived as:
$r=\frac{\sigma}{2}\left(\Phi^{-1}(P_A)-\Phi^{-1}(P_B)\right),$
where $\sigma$ is the standard deviation of Gaussian noise and $\Phi$ is the standard Gaussian CDF.

\para{Verification under $\cL_1$ metric.} Similarly, \citeauthor{teng2020ell}~\cite{teng2020ell} derive the closed form for $\cL_1$ robust radius under Laplacian noise:
$R=\max \left\{ \frac{\lambda}{2}\log(P_A/P_B),\,-\lambda\log(1-P_A+P_B)\right\}.$
% 
\cite{teng2020ell} is very similar to \cite{li2019certified} in that they both derive the term $-\lambda\log(1-P_A+P_B)$, although from different perspectives.
% \cite{teng2020ell} claims that, their result is tighter, because they derive another bound $\frac{\lambda}{2}\log(P_A/P_B)$ and their final result is obtained by taking maximum from the two bounds. However, when we reimplement the two methods, we find that the final certification results do not have too much difference. Because, in real implementation, where $P_B$ is usually set as $1-P_A$, $-\lambda\log(1-P_A+P_B)$ is almost always greater than $\frac{\lambda}{2}\log(P_A/P_B)$. This is not surprising, because the additional bound $\frac{\lambda}{2}\log(P_A/P_B)$ is also exactly the result derived through differential privacy method, which is loose.



\para{Verification under $\cL_0$ metric.}
\citeauthor{lee2019tight}~\cite{lee2019tight} consider the discrete setting, where the smoothing distribution is on discrete space (values of pixels are randomly sampled from a small discrete set) and the distance metric is $\cL_0$. They propose to partition the data space $\mathcal{X}$ into $n$ regions $\{\cX_i:\, 1\le i \le n\}$ such that $\dot \cup_{i=1}^n \cX_i = \cX$,
%   $$
%   \mathcal{L}_1,\mathcal{L}_2,...,\mathcal{L}_n: \bigcup_{i=1}^n \mathcal{L}_i = \mathcal{X},
%   $$
 and the likelihood ratio within each region $\cX_i$ is a constant $\eta_i \in [0,\infty]$. Based on this partition, the Neyman-Pearson set could be constructed, and the certification could be effectively computed.
%  with the numerical algorithm they propose.

  
%   Besides \cite{lee2019tight}, 
  Recently, \citeauthor{levine2019robustness}~\cite{levine2019robustness}  also propose to certify $\mathcal{L}_0$ robustness. They adopt a different smoothing technique --- randomized ablation, where the randomly smoothed input $x'$ is generated by randomly ablating pixels from the original input $x$. Empirically, the randomized ablation strategy suits the $\mathcal{L}_0$ metric well and achieves better certified robustness. 
%   \xiangyu{After thinking again, I agree to delete it. Because essentially, both of \cite{lee2019tight} and \cite{levine2019robustness} derive the robustness radius based on building a Neyman-Pearson set, although they do not explicitly mention that.}




% \linyi{omit references in title to save space}
\subsubsection{\textbf{General Verification Frameworks for Various Settings}}
\label{sec:rand-smooth-intro-4}
% \hfill \\
% \subsubsection{\textbf{General Verification Frameworks for Various Settings}~\texorpdfstring{\cite{Dvijotham2020A,yang2020randomized}}{}}
% \label{sec:rand-smooth-intro-4}\hfill \\
\citeauthor{Dvijotham2020A}~\cite{Dvijotham2020A} and \citeauthor{yang2020randomized}~\cite{yang2020randomized} attempt to devise more general verification frameworks that could be easily extended to various distance norms.

\citeauthor{Dvijotham2020A}~\cite{Dvijotham2020A} propose to compute the lower bound of the non-convex optimization problem $\min_{x':\rho(x,x')\le r}{\Pr_{\delta\sim\mu} [F(x'+\mu)=c]}$ by relaxing the norm bound of perturbation to a divergence bound. The high level idea is: with $\rho(x',x)\le r$, there should be a bound $\eta $ for the distribution divergence as $D\left((x + \mu)\|(x' + \mu)\right) \le \eta$,
% \linyi{Changed from $D\left(\mu(x+v)\|\mu(x)\right) \le \eta$, is it correct?}
where $D$ denotes certain divergence. Thus, the relaxation is derived as:
$\min_{\mathcal{U'}:D(\mathcal{U'}\|(x + \mu))\le \eta}{\Pr_{X\sim \mathcal{U'}}[f(X)=c]}$.
% \linyi{Changed from $\min_{\mathcal{U'}:D(\mathcal{U'}\|\mu(x))\le \eta}{\Pr_{X\sim \mathcal{U'}}[f(X)=c]}$, is it correct?} 
However, in real implementation, the certified robustness radius computed via this framework is usually too loose comparing with other approaches. Similar result is also reported by \cite{yang2020randomized}.
% \cite{Dvijotham2020A} claims that this relaxation leads to a general framework which could handle any noise type and distance metric, as long as the divergence bound could be computed. However, computing a tight divergence bound based on the original distance bound and noise type is not a trivial work --- they just transferred the difficulty to the computation of divergence bound, instead of addressing the generality issue. Moreover, the robustness radius certified by this framework is too loose compared with the results produced by state-of-the-art methods in real implementation. Similar result is also reported by \cite{yang2020randomized}.


\citeauthor{yang2020randomized}~\cite{yang2020randomized} propose a pair of complementary verification approaches --- level set method and differential method. The former one is generalized from the Neyman-Pearson based approaches and offers favorable certification results for spherical noise. The latter  offers support for non-spherical noise, and is based on a worst-case path integral $ R := \int_{1-P_A}^{1/2} \dif t / \Psi(t)$, where $P_A$ is the probability of the top class and $\Psi(p) := \sup_{\|v\|=1}{\sup_{U\subseteq\mathbb{R}^d:q(U)=p}{\lim_{r\rightarrow 0}{\left(q(U-rv)-p\right) / {r}}}}.$
% 
By applying the differential method, the authors have derived the closed form of certified robustness under different settings.
% , which is quite impressive.

\subsubsection{\textbf{Robust Training for Randomized Models}\texorpdfstring{~\cite{cohen2019certified,lecuyer2019certified,salman2019provably,carmon2019unlabeled,li2019certified,jeong2020consistency,Zhai2020MACER:,feng2020regularized,awasthi2020adversarial,Zhang2020BlackBoxCW,yang2020randomized}}{}} \hfill \\
\label{sec:rand-smooth-intro-5}
This subsection mainly summarizes \emph{robust training} approaches for randomized models, along with other efforts towards robust randomized models. 

% In previous subsections, we focus on the certification methods for randomized models. However, these certification methods fail to give us any insight about how to obtain an accurate and robust randomized models. In this subsection, we will review techniques that help to build accurate and robust models under probabilistic setting.

\para{Data augmentation.} 
% The probabilistic verification does not pose any requirement on the base model. However, for standard trained classifier, the discrepancy between standard training data and noise corrupted testing data will severely hurt the prediction accuracy of the smoothed model.
Empirically, \cite{cohen2019certified} and \cite{lecuyer2019certified} suggest that we could augment the training data with the noised corrupted ones.
% % , which would bridge the gap between the training and inference. 
% This augmentation technique works very well in real implementation and is also formally justified by \cite{cohen2019certified}. 
% Due to the efficiency and practical effectiveness, this technique is still the most popular training practice under probabilistic setting. 
This augmentation technique works well in practice and is also formally justified by \cite{cohen2019certified}.
Currently, this is still the most widely-used training approach under probabilistic setting.
% 
Besides leveraging the noise corrupted data, several work also utilize additional unlabeled data to pretrain the models to enhance the robustness~\cite{salman2019provably,carmon2019unlabeled}.
% , which could also effectively enhance the robustness.

% \linyi{Summarize ``Stability training'' and ``Training to maximize certified radius'' as Regularization.}
\para{Regularization.}
Robust training of randomized models can be achieved by regularizing the models to be stable or consistent under noise perturbations.
For example, \citeauthor{li2019certified}~\cite{li2019certified} train randomized models by adding a regularization term into the training objective which minimizes the cross-entropy loss of models outputs between original samples and noise samples.
\citeauthor{jeong2020consistency}~\cite{jeong2020consistency} further improve it by only minimizing the cross-entropy loss among noised samples.
\t{MACER}~\cite{Zhai2020MACER:} derives a regularization term which directly maximizes the certified robustness.
% To make the term differentiable for training, it utilizes soft randomized classifier~(see \Cref{def:randomized_classifier}) as the proxy.
\t{ADRE}~\cite{feng2020regularized} proposes another regularizer to penalize the misclassified samples and improve the certified robustness of the correctly predicted samples.

% \para{Stability training.} Different from the augmentation methodology, \cite{li2019certified} proposes to add a regularization term into the training target to encourage the stability of the base classifier's output under noise perturbation. A suggested regularizer is based on cross-entropy: $L_{\mathrm{stability}}=-\sum_j{\Pr(y_j|x)\log{\Pr(y_j|x')}}$. Empirically, this training technique is also very effective.
% ADRE~\cite{feng2020regularized} proposes another regularizer to penalize the misclassified samples and improve the certified radius of the correctly predicted examples.
% Consistency~\cite{jeong2020consistency} enhances the stability of the base classifier's output under noise perturbation via a simpler but more effective regularizer.

\para{Adversarial training.} 
Adversarial training framework is widely used in empirical defenses and deterministic verification based defenses.
\citeauthor{salman2019provably}~\cite{salman2019provably} propose to combine  adversarial training  with the probabilistic verification framework.
This combination exhibits a promising complementary property:  adversarial training boosts the certified robustness of randomized models by a significant margin.
\t{Low Rank enforcement}~\cite{awasthi2020adversarial} further improves \cite{salman2019provably} by projecting the noised data to low-dimension space then applying adversarial training.

% The well-studied adversarial training framework (\cite{madry2017towards}; \cite{kurakin2016adversarial}) is empirically shown to be very effective for training robust models. However, one major limitation of adversarial training is the lacking of theoretical guarantee. \cite{salman2019provably} proposes to combine the adversarial training framework with the probabilistic verification framework.

% This combination exhibits a very promising complementary property: the adversarial training helps to boost the robustness of randomized models by a significant margin, while the probabilistic setting offers the theoretical guarantee the standard adversarial training framework lacks of.

% \para{Training to maximize certified radius.} \citeauthor{Zhai2020MACER:}~\cite{Zhai2020MACER:} propose to train robust smoothed classifiers via MAximizing the CErtified Radius (MACER), which obtains considerable robustness gain comparable to the adversarial training method on ImageNet. The core idea is: directly incorporating the differentiable version of certified radius into training objective.
% % so that the training procedure will try to output a better model that could achieve larger certified radius. 

% \para{ADRE.} An important observation is: when the top class is correctly predicted, a big radius is desirable, while a misclassified point with large radius would greatly hurt the model's accuracy. Based on this observation, \cite{feng2020regularized} proposes the ADaptive Radius Enhancing (ADRE) regularizer:
% $$
% L_{\mathrm{ADRE}}=CE(h(x),\argmax_{c \ne y}{h_c(x)}),
% $$
% where $h_i(x)=\Pr_{X\sim \mu(x)}{\left[F(X)=i\right]}$, $y$ is the ground truth and $CE$ is the cross-entropy function. Intuitively, this regularizer penalizes the misclassified examples and encourages the certified robustness of correctly predicted examples. 


\para{Choice of smoothing distribution.} Besides the training approaches, the choice of smoothing distribution is also an important factor that affects the certified robustness. 

Most existing approaches adopt Gaussian noise and Laplacian noise as the default choices for $\cL_2$ and $\cL_1$ distance metrics respectively. However, \citeauthor{Zhang2020BlackBoxCW}~\cite{Zhang2020BlackBoxCW} point out that in high dimensional space, under Gaussian and Laplacian distributions, most mass concentrates on a thin shell far from the center.
% , which is a commonly known conclusion from high dimensional statistics. 
They argue that this decentralization makes these two noises sub-optimal and propose several substitutes. 

\citeauthor{yang2020randomized}~\cite{yang2020randomized} also studied the optimal choice of smoothing distribution. They show that against $\cL_p$ adversary the optimal smoothing distributions have level sets that are their respective Wulff Crystals --- a kind of crystal structure studied in physics. Specifically, uniform noise is shown to be much better than Laplacian noise against $\cL_1$ adversary. 


%\subsubsection{\textbf{Theoretical Limitations}}\hfill \\
%\label{sec:rand-smooth-intro-6}
%Despite of the promising features of randomized smoothing framework, several theoretical limitations of this framework are shown by recent works, posing great challenge to its further development. In this subsection, we will briefly review two critical limitations of randomized smoothing.
%-----------------------------------------------------------------------
%\para{Trade-off between robustness and accuracy.} Trade-off between robustness and accuracy has been widely observed~\cite{fawzi2018analysis,tsipras2018robustness,raghunathan2020understanding} in many workflows that aim at building robust models. Similar trade-off in randomized smoothing framework is also observed since its birth. \cite{yang2020randomized} and \cite{Zhang2020BlackBoxCW} discuss this trade-off mainly from intuitive perspectives.
% have attempted to formalize this trade-off in randomized smoothing with several illustrative mathematical expressions, however these discussions are still mainly from intuitive perspectives and give little insight into the reason why this trade-off exists.
% 
%More recently, \cite{mohapatra2020rethinking} gives out the first rigorous formalization and proof of this trade-off issue from the perspective of decision region shrinkage.
%The decision region of certain label $c$ is defined as the input region which are predicted as label $c$ by the classifier.
%As the intensity of random noise becomes large, compared with the original deterministic classifier, the randomized classifier will have a shrunk decision region and it may even disappear.
% and in extreme cases, the decision region may disappear. 
%This shrinkage theory explains why probabilistic setting hurt the standard accuracy and theoretically reveals a fundamental limitation of probabilistic verification workflow: we have to apply a large enough noise variance to be robust, however also have to keep the variance small enough to avoid severe shrinkage of the decision region.
%---------------------------------------------------------

% \begin{definition}[Decision Region]
% \label{def:decision_region}
% Given a classifier $h$, the decision region of label $c$ determined by $h$ is defined as the set of points that are assigned the label $c$ by $h$. 
% \end{definition}


%------------------------------------------------------------------------
%\para{Curse of dimensionality.} 
% Besides the shrinkage of decision regions, 
%Recent works also reveal another severe limitation of randomized smoothing: curse of dimensioanlity. \citeauthor{yang2020randomized}~\cite{yang2020randomized} prove that without more information than label statistics, under randomized smoothing framework, the models cannot achieve nontrivial certified robustness against perturbations of $\cL_p$-norm $\Omega(\min(1,n^{\frac{1}{p}-\frac{1}{2}}))$. \citeauthor{kumar2020curse}~\cite{kumar2020curse} also show similar conclusion: for a vast class of i.i.d smoothing distributions, the largest $\cL_p$-radius that can be certified decreases as $O(1/d^{\frac{1}{2}-\frac{1}{n}})$ with dimension $n$ for $n> 2$.
% 
%This means, under $p$-norm metric with large $p$, especially like the popular $\cL_{\infty}$ metric, it would be very hard to certify a nontrivial robustness radius for randomized smoothing framework, when the dimension of input data is very high. This result poses severe challenge to the randomized smoothing methodology: since the randomized smoothing framework cannot even give out a non-trivial certified result for the common $\cL_{\infty}$ attack, whether the seemly promising feature of randomized smoothing is yet another illusion?
% ---------------------------------------------------------------

%\noindent{\textbf{Remarks:}}
%\label{sec:rand-smooth-intro-7}
% \textbf{1. Probabilistic setting helps to simplify the robustness verification.} 
% Under deterministic setting, given input $x_0$, the prediction is only based on this single point.
% Any counter-example within its perturbation ball implies non-robustness.
% Thus, the verification approach must capture counter-example if it exists.
% % from the data space, which makes the robustness condition very strong --- merely one counter-example within the perturbation ball could break the certification. 
% However, under probabilistic setting, we only need to check whether the probability is above a certain level against perturbations.
% % we do not care specific single point, we only need to check whether the probability of a specific label $c$ still remains above a certain level against the perturbation.
% \textbf{2. Probabilistic setting helps to improve the robustness.} 
% Intuitively, under deterministic setting, even one adversarial point would break the robustness.
% However, under probabilistic setting, as long as the density of the adversarial points is kept low, the robustness would not get affected.
%\underline{Probabilistic verification is incomplete:} 
%To our best knowledge, all existing probabilistic verification approaches are agnostic to model architectures. This relaxation makes such probabilistic approaches scalable; however, incomplete. Among existing methodologies, the Neyman-Pearson based approaches achieve the tightest certification result under this assumption.
%\underline{Smoothed Prediction can be computed:}
%In probabilistic verification framework, the integral in \Cref{eq:h-smooth} cannot be exactly solved. Thus, instead, Monte Carlo estimate and the theories from confidence interval are used to approximate the exact solution. Specifically, most of existing works follow the approximation algorithm CERTIFY proposed in \cite{cohen2019certified}. 
% \subsection{Summary}

    % In this section, we overview major neural network verification and certifiably robust training approaches.
    % In \cref{tab:approach-taxonogy}, we present an taxonogy of these approaches.
    
    

% \subsection{Theoretical Findings}

%     In \cref{tab:theory-taxonogy} we categorize approaches which presents theoretical findings or theoretical/empirical analysis about certifiable robustness training and verification.

%     \begin{table*}[!t]
%         \centering
%         \caption{Works providing additional discoveries.}
%         \begin{tabular}{c|c|l}
%             \toprule
%             Paper & Category & Main Conclusion \\
%             \hline \hline
%             \cite{weng2018towards} & Hardness & Impossibility for constant ratio $\ell_\infty$ radii certify \\
%             \cite{salman2019convex} & Connection & Show connection of almost all LP and LP-Dual approaches \\
%             \cite{kumar2020curse} & Hardness & Barrier for randomized smoothing against $\ell_\infty$ adversary \\
%             \cite{yang2020randomized} & Hardness & Barrier for randomized smoothing against $\ell_\infty$ adversary \\
%             \cite{Ghiasi2020BREAKING} & Questioning & Questioning the value of certified robustness \\
%             \cite{Baader2020Universal} & Strength & Universal approximation by certified neural network \\
%             \cite{mohapatra2020rethinking} & Hardness & Empirical study shows randomized smoothing training limitation \\
%             \bottomrule
%         \end{tabular}
%         \label{tab:theory-taxonogy}
%     \end{table*}
    
\section{Evaluation and Comparison}

    \label{sec:evaluation}

    We evaluate and compare the robustness verification and training approaches by two sets of experiments:
    (1)~for major deterministic verification approaches, we compare their certified robustness over a diverse set of trained models of different scales;
    (2)~for major probabilistic verification approaches and their corresponding robust training approaches, we compare the best certified robustness they jointly achieve since the verification and training approaches are usually coupled.
    We do such separation mainly because in deterministic and probabilistic settings, the model inference methods are different and cannot be directly compared.
    % provide different degrees of robustness guarantees~(see \Cref{def:verification-approach}).
    % We provide the state-of-the-art table of best verifiable robustness for common settings considering both deterministic and probabilistic approaches in \Cref{sec:adx-state-of-the-art-on-cert-robust}.
    % the ultimate goal of both verification approaches and defenses is to provide better certifiable robustness, either by increase the tightness under affordable running time, or by increase the model robustness itself, or by better inference schemes.
    % Among them, for those verification approaches based on single point prediction~(i.e., deterministic verification approaches), their \emph{practical tightness}, i.e., the tightness it can achieve under practical running time, can be fairly compared by setting a uniform benchmark.
    
    We provide the first open-sourced unified evaluation platform --- a toolkit integrating a wide range of verification approaches by succinct and uniform interface based on \texttt{PyTorch}~\cite{pytorch}~(see \Cref{sec:intro} for URL).
    In the toolkit, we tend to integrate the original implementations released by the authors when it is available;
    otherwise, we implement and optimize them to match the reported performance.
    
    \para{Experiment Environment.} We run the evaluation on $24$-core Intel Xeon Platinum 8259CL CPU running at \SI{2.50}{GHz} with single NVIDIA Tesla T4 GPU.
    
    \subsection{Comparison of Deterministic Verification Approaches}
        \label{sec:exp-A}
        
        % ---- 2 tables for deterministic verification comparison ----
        \begin{table}[!t]
            \caption{Deterministic verification approaches benchmarked in our evaluation.}
            % In the table, ``Complete'' means whether the verification approach is complete or incomplete.}
            \vspace{-1em}
            \centering
            \resizebox{0.80\linewidth}{!}{
            \begin{tabular}{c|c|l}
                \toprule
                Category & Approach & Implementation \\
                \hline \hline
                MILP & \t{Bounded MILP}~\cite{tjeng2018evaluating} & Reimplementation \\
                \hline
                Branch and Bound & \t{AI$^2$}~\cite{gehr2018ai2} & From \cite{singh2019abstract} \\
                \hline
                 & \t{LP-Full}~\cite{weng2018towards,salman2019convex} & From \cite{boopathy2019cnn} \\
                % \hline
                  & \t{DeepPoly}~\cite{singh2019abstract} & From \cite{singh2019abstract} \\
                & \t{Fast-Lin}~\cite{weng2018towards} & From \cite{boopathy2019cnn} \\
                Linear & \t{CROWN}~\cite{zhang2018efficient} & From \cite{zhang2020towards} \\
                Relaxation & \t{CNN-Cert}~\cite{boopathy2019cnn}  & From \cite{boopathy2019cnn} \\
                 & \t{CROWN-IBP}~\cite{zhang2020towards} & From \cite{zhang2020towards} \\
                & \t{IBP}~\cite{gowal2019scalable} & Reimplementation \\
                % \hline
                & \t{WK}~\cite{wong2018provable,wong2018scaling} & From \cite{wong2018scaling} \\
                \hline
                \multirow{2}{*}{Hybrid}  & \t{k-ReLU}~\cite{singh2019beyond} & From \cite{singh2019abstract} \\
                 & \t{RefineZono}~\cite{singh2019beyond} & From \cite{singh2019abstract} \\
                \hline
                \multirow{2}{*}{SDP} & \t{SDPVerify}~\cite{raghunathan2018semidefinite} & Reimplementation \\
                & \t{LMIVerify}~\cite{fazlyab2019safety} & Reimplementation \\
                \hline
                \multirow{3}{*}{Lipschitz} & \t{Op-norm}~\cite{szegedy2013intriguing} & From \cite{zhang2019recurjac} \\
                & \t{Fast-Lip}~\cite{weng2018towards} & From \cite{zhang2019recurjac} \\
                & \t{RecurJac}~\cite{zhang2019recurjac} & From \cite{zhang2019recurjac} \\
                \bottomrule
            \end{tabular}
            }
            % \vspace{-2em}
            \label{table:exp-A-evaluated-verification-approaches}
        \end{table}
        
        \input{tables/exp-A-cifar10-verify-robust-acc}
        % ------------------------------------------------------------
        
        We present a thorough comparison of major \emph{deterministic verification approaches} as listed in \Cref{table:exp-A-evaluated-verification-approaches}.
        % The list covers major branches of deterministic verification approaches.
        % on a diverse set of trained neural networks of different scales in order to compare the verifiable robustness each approach can provide.
    
        \subsubsection{\textbf{Experimental Setup}}\hfill \\
            % We build an integrated toolkit and use it as the test platform.
            % \para{Verification approaches.}
            % We run the experiments with the toolkit, which integrates the approaches to compare.
            % In the tool, we integrate and implement various major verification approaches 
            % Our selection covers major branches of deterministic verification approaches.
            % % according to the classification in \cref{fig:tree-categorization}.
            % 
            % to have similar performance as the original implementations.
            % When the verification approach is complex but publicly available implementation is available, we directly integrate such implementation into our tool.
            % If multiple implementations are available, we tend to use the latest one with at least one developer is the paper author.
            % When the verification approach is rather simple, or no publicly available implementation, we implement it on our own.
            % 
            \para{Dataset.}
            We evaluate these verification approaches on image classification datasets MNIST~\cite{lecuyer2019certified} and CIFAR-10~\cite{krizhevsky2009learning}.
            % Both MNIST and CIFAR-10 are widely used datasets for image classification task.
            % The MNIST dataset contains $50,000$ train set samples and $10,000$ test set samples.
            % Each sample is a $28 \times 28$ gray-scale image with pixel color normalized to range $[0,\,1]$, and contains a handwritten digit ranging from $0$ to $9$.
            % The CIFAR-10 dataset contains $60,000$ train set samples and $10,000$ test set samples.
            % Each sample is a $32 \times 32$ colored image with pixel color normalized to range $[0,\,1]$, and contains a object.
            % Both datasets have $10$ classes.
            % \ifnum\arxiv=0
            % We defer the experiment settings and results on MNIST to the platform website~(see \Cref{sec:intro} for URL) due to page limit.
            % \fi
            % \ifnum\arxiv=1
            We deter the experiment settings and results on MNIST to \Cref{sec:adx-full-exp-deterministic}.
            % \fi
            
            \para{Models.}
            We include $7$ different neural network structures from the literature.
            % and adapt them for each dataset.
            Among them, $3$~(\sc{FCNNa} - \sc{FCNNc}) are fully-connected neural networks, and $4$~(\sc{CNNa} - \sc{CNNd}) are convolutional neural networks.
            They are all feed-forward ReLU neural networks.
            % supported by these verification approaches.
            The number of neurons ranges from $50$~(\sc{FCNNa}) to about $200,000$~(\sc{CNNd}).
            For each neural network structure, we train $5$ sets of weights: 
            \begin{itemize}
                \item \texttt{clean}: regular training; 
                \item \texttt{adv2}: PGD adversarial training with $\epsilon = 2/255$; 
                \item \texttt{adv8}: PGD adversarial training with $\epsilon = 8/255$;
                \item \texttt{cadv2}: \t{CROWN-IBP} training with $\epsilon = 2/255$;
                \item \texttt{cadv8}: \t{CROWN-IBP} training with $\epsilon = 8/255$.
            \end{itemize}
            
            Here, $\epsilon$ is the $\cL_\infty$ radius of the adversarial examples.
            % The regular training only aims for high accuracy on clean inputs.
            The PGD adversarial training~\cite{madry2017towards} is a strong empirical defense.
            % ====== BELOW IS WRONG ======
            % so here we leverage its robust accuracy to serve as the potential upper bound of the certified robustness.
            % \linyi{Omitted a wrong sentence which someone added somehow.}
            % % , and it aims for high robust accuracy against adversarial examples within $\cL_\infty$ ball with $\epsilon$ radius.
            The \t{CROWN-IBP}~\cite{zhang2020towards} is a strong robust training approach, which achieves state-of-the-art certified robustness on CIFAR-10 against $(\cL_\infty, 8/255)$ adversary.
            % % which aims for certifiable high robust accuracy against adversarial example within $\cL_\infty$ ball with $\epsilon$ radius.
            We choose these training configurations to reflect $3$ common types of models on which  verification approaches are used: normal models; empirical defense models; and robustly trained models.
            % 
            % We defer the model statistics and their structures to 
            All models are trained to reach their expected accuracy or robustness.
            % \ifnum\arxiv=0
            % We defer the model structure and statistics to the website. 
            % \fi
            % \ifnum\arxiv=1
            We defer the model structure and statistics to \Cref{sec:adx-full-exp-deterministic}. 
            % \fi
            % detail statistics and accuracy of these models to \Cref{sec:adx-full-exp-deterministic}.
            % Furthermore, for each set of weights we report the clean accuracy and empirical robustness~(measured by robust accuracy under PGD attack) in \Cref{sec:adx-full-exp-deterministic}.
            
            \para{Evaluation protocol.}
            We present the performance of verification approaches by their \emph{robust accuracy} with respect to $\cL_\infty$ radius $\epsilon$.
            The chosen radius $\epsilon$ for verification corresponds to the radius trained for defense.
            The robust accuracy is defined as $$\mathrm{robacc} := \dfrac{\text{\# samples verified to be robust}}{\text{\# number of all samples}}.$$
            On each dataset, we uniformly sample $100$ test set samples as the fixed set for evaluation.
            % The samples are uniformly sampled.
            We further limit the running time to \SI{60}{s} per instance and count timeout instances as ``non-robust''.
            
            We also report the robust accuracy under empirical attack~(PGD attack), which gives an upper bound of robust accuracy, so we can estimate the gap between certified robust accuracy and accuracy of existing attack.
            
            For verification approaches with hyperparameters, we use their default hyperparameters as described in the papers or original implementations.
            We remark that due to hyperparameter tuning, limited running time~(\SI{60}{s}), and different neural network models used in evaluation, the robust accuracy of some approaches differs much with the reported numbers, such as \t{k-ReLU}~\cite{singh2019beyond}, \t{RefineZono}~\cite{singh2018robustness}, \t{SDPVerify}~\cite{raghunathan2018semidefinite}, and \t{LMIVerify}~\cite{fazlyab2019safety}.
            % 
            We also evaluate the verification approaches by measuring their average certified robustness radius.
            % \ifnum\arxiv=0
            % The results are available on the project website.
            % \fi
            % \ifnum\arxiv=1
            The results are in \Cref{sec:adx-full-exp-deterministic}.
            % \fi
            % The full experiment results are deferred to \Cref{sec:adx-full-exp-deterministic}.
            
            % % 
            % % We measure the performance of verification approaches by two measures: robust accuracy with respect to certain radius~($\mathrm{robacc}$); and average robust radius it can certify~($\bar{r}$).
            % % 
            % The \emph{robust accuracy}~($\mathrm{robacc}$) stands for the verified accuracy we can obtain from the verification approach.
            % We select a subset from the test set samples, then for each sample, we compute whether the verification approach could verify its robustness in $\cL_\infty$ ball with given radius $\epsilon$.
            % The robust accuracy is defined as $\mathrm{robacc} := \dfrac{\text{\# samples verified to be robust}}{\text{\# number of all samples}}$.
            % For each set of trained weight, we select the radius $\epsilon$ accordingly, which is recorded in the upperleft corner of the result tables.
            
            % We select $100$ samples from the test set as the fixed subset for evaluation.
            % The samples chosen have numbers being the multiplier of $100$, i.e., $\#0, \#100, \#200, \dots$.
            % % 
            % We limit the running time to \SI{60}{s} and count timeout instances as ``non-robust'' since verification on it fails.
            
            % Note that due to the incompleteness and over-time running, the robust accuracy reported is the valid lower bound of actual robust accuracy of the model.
            % For reference, we also report the corresponding numbers obtained from an empirical attack~(PGD attack) which gives a valid upper bound.
            % Therefore, we can directly compare the tightness of these verification approaches under time limit, and notice its heuristic gap by viewing PGD upper bound as the proxy of exact robust accuracy.
            
            % We also evaluate these verification approaches by measuring their average robust radius.
            % The full experiment results are deferred to \Cref{sec:adx-full-exp-deterministic}.
            
            % We remark that due to limited running time per sample~(\SI{60}{s}) and different neural network models used in evaluation, the robust accuracy of some approaches differs much with the reported numbers in their original papers, such as k-ReLU~\cite{singh2019beyond}, RefineZono~\cite{singh2018robustness}, SDPVerify~\cite{raghunathan2018semidefinite}, and LMIVerify~\cite{fazlyab2019safety}.
            
            % \para{Implementation and Running environment.}
            % We defer the details to \Cref{sec:adx-full-exp-deterministic}.
        
        \subsubsection{\textbf{Results and Discussions}}\hfill \\
            \label{sec:expA-rob-acc}
            % 
            \Cref{tab:exp-A-cifar10-verify-robust-acc} shows robust accuracy on CIFAR-10 dataset.
            % The results on MNIST dataset is deferred to \Cref{tab:exp-A-mnist-verify-robust-acc} in \Cref{sec:adx-full-exp-deterministic}.
            Each row corresponds to a verification approach, PGD attack, or clean accuracy.
            % along with the robust accuracy upper bound found by PGD attacks and the clean accuracy on the same test set samples for reference.
            Each column corresponds to a DNN model.
            % where the detail information could be found in \Cref{table:expA-models-stats} and \Cref{table:expA-models-originalacc}.
            % Higher robust accuracy in the table implies tighter verification~(under practical time).
            % \ifnum\arxiv=1
            \Cref{sec:adx-full-exp-deterministic} contains full experiment results and additional findings.
            % \fi
            
            \para{Remarks.}
            % higher tightness and better verification result.
            % The performance of these verification approaches varies across different model size and different training mode.
            % For regular trained neural networks~(\texttt{clean}), when model size is small, the complete verification approaches~(Bounded MILP and AI2) have similar or slightly better performance than others; however, when model size becomes larger, they usually time out and LP-relaxation based approaches are better.
            % For heuristically defensed models~(\texttt{adv2} and \texttt{adv8}), similarly, on small models, complete verification approaches are better, especially AI2.
            % On larger models, linear relaxation based approaches are better.
            % For certifiably defensed models~(\texttt{cadv2} and \texttt{cadv8}),
            % usually, IBP and CROWN-IBP are the best among them.
            % We have the following observations:
            (1)~On relatively small models, complete verification approaches can effectively compute the exact robust accuracy, thus they are the best choice.
            (2)~On larger models, if the model is normally trained or heuristically defensed, usually linear inequality propagation or zonotope based verification approaches~(including \t{DeepPoly}, \t{Fast-Lin}, \t{CROWN}, \t{CNN-Cert}, \t{CROWN-IBP}, \t{WK}) are the best.
            Since the complete verification approaches are too slow and other approaches are too loose.
            However, they cannot handle large DNNs and they are still too loose comparing with the PGD upper bound of robust accuracy.
            (3)~On robustly trained models, if the robust training approach is \t{CROWN-IBP}, the verification approach \t{IBP} and \t{CROWN-IBP} perform the best.
            Both of them can scale up to large DNNs and the gap with PGD upper bound is small.
            Similar observations can be found on MNIST and consistent with the literature~\cite{wong2018provable,zhang2020towards}.
            (4)~Hybrid approaches, SDP-based approaches, and Lipschitz-based approaches are typically inferior than linear relaxation-based approaches and complete verification approaches under most settings.
           
    
    \subsection{Comparison of Probabilistic Approaches}
    
        \begin{table}[!t]
            \caption{Probabilistic approaches used in evaluation.}
            \vspace{-1em}
            \centering
            \resizebox{0.80\linewidth}{!}{
            \begin{tabular}{l|l|l}
                \toprule
                \multicolumn{2}{c|}{Approaches} & Adversaries in Evaluation \\
                \hline \hline
                Verification & Differential Privacy Based~\cite{lecuyer2019certified} & $\cL_1, \cL_2$ \\
                Approaches & Neyman-Pearson Based~\cite{cohen2019certified,yang2020randomized,Zhang2020BlackBoxCW,teng2020ell} & $\cL_1,\cL_2,\cL_\infty$ \\
                & $f$-Divergence~\cite{Dvijotham2020A} & $\cL_2$ \\
                & R\'enyi divergence Based~\cite{li2019certified} & $\cL_1$ \\
                \hline
                Robust Training & Data Augmentation~\cite{cohen2019certified,yang2020randomized} & $\cL_1, \cL_2, \cL_\infty$ \\
                Approaches & Adversarial Training~\cite{salman2019provably} & $\cL_2$ \\
                & Adversarial + Pretraining~\cite{salman2019provably,carmon2019unlabeled} & $\cL_2$ \\
                & \t{MACER}~\cite{Zhai2020MACER:} & $\cL_2$ \\
                & \t{ADRE}~\cite{feng2020regularized} & $\cL_2$ \\
                \bottomrule
            \end{tabular}
            }
            \vspace{-1.75em}
            \label{tab:probabilistic-approach-benchmarked}
        \end{table}
    
        \input{tables/exp-B-main-table}
        
        We present a through comparison of major \emph{probabilistic approaches} including both \emph{verification approaches}~(include different smoothing distributions) and \emph{robust training approaches}.
        
        \subsubsection{\textbf{Experimental Setup}}\hfill \\
        We implement various major verification approaches and integrate representative robust training approaches.
        In our evaluation, we either fix the robust training part and vary the verification approaches, or the other way around.
        
        \para{Dataset.}
        Our evaluation is on CIFAR-10 and ImageNet~\cite{russakovsky2015imagenet}.
        
        \para{Models.}
        Following common practice in  literature~\cite{cohen2019certified,yang2020randomized}, we use ResNet-110 and Wide ResNet 40-2  on CIFAR-10; and ResNet-50  on ImageNet.
        
        \para{Number of Samples and failure probability.}
        Following common practice, on both datasets, $n=1,000$ samples are used for selecting the top label; $N = 100,000$ samples are used for certification.
        The failure probability is set to $1 - \alpha = .001$.
        % , i.e., the probabilistic verfication is $.999$-confident.
        % \linyi{Trimmed for space...}
        
        \para{Evaluation Protocol.}
        For both datasets, we evaluate on a subset of $500$ samples uniformly drawn from the test set.
        We report and compare the robust accuracy~(see definition in \Cref{sec:exp-A}) at given radius $r$ under $\cL_p$ for $p = 1,\, 2,\, \infty$.
        
        \para{Evaluated approaches.}
        We list the evaluated approaches in \Cref{tab:probabilistic-approach-benchmarked}.
        We tune the hyper-parameters to achieve the best performance for each approach.
        To evaluate the $\cL_\infty$ robustness, we use the following norm conversion rule:
        given input dimension $d$, since $\|x\|_2 \le \|x\|_\infty \sqrt d$, the model with certified robust radius $r$ in $\cL_2$ norm at point $x_0$ is also certified robust with radius $r / \sqrt d$ in $\cL_\infty$ norm.
        The above conversion gives $\cL_\infty$ robustness certification from existing $\cL_{2}$-based certification, which is empirically shown to achieve the highest certified robustness for probabilistic approaches under $\mathcal{L}_{\infty}$ adversary.
        
        % To our best knowledge, all state-of-the art $\mathcal{L}_\infty$ certification results under probabilistic settings are obtained based on conversions from other norm metrics. 
        % For example, given input dimension $d$, since $\|x\|_2 \le \|x\|_\infty \sqrt d$, the model with certified robust radius $r$ in $\cL_2$ norm at point $x_0$ is also certified robust with radius $r / \sqrt d$ in $\cL_\infty$ norm.
        % % The core idea is one robustness radius derived under a certain $\cL_p$ norm metric could be directly converted to a robustness radius for another norm metric $\cL_k$. So, the $\cL_\infty$ robustness could be directly derived from other metrics (e.g. $\cL_2$).
        % % The conversion rule and theoretical foundations are deferred to \Cref{sec:adx-full-exp-probabilistic}.
        % Based on the conversion rule, we could directly obtain the $\cL_{\infty}$ robustness from state-of-the-art results under $\cL_{2}$ adversary with Gaussian smoothing
        % \linyi{In experiments it seems that we are not deriving from the state-of-the-art result. May be incorrect.}
        % % $$
        % %     r = \frac{\sigma\Phi^{-1}(\underline{P_A})}{\sqrt{d}},
        % % $$
        % which is empirically shown to be the best probabilistic setting for $\mathcal{L}_{\infty}$ \cite{yang2020randomized}.
        % % 
        % We evaluate the $\mathcal{L}_{\infty}$ robustness with this Gaussian setting on both CIFAR-10 and ImageNet, the result is reported in \Cref{table:L_inf+uniform}.
        
        \subsubsection{\textbf{Results and Discussions}}\hfill \\
        \Cref{tab:exp-B-main-table} shows the results.
        Each ``Group \#'' labels a variable-controlled comparable group.

        \para{Remarks.} 
        (1)~For both $\cL_1$ and $\cL_2$ adversaries, Neyman-Pearson based verification achieves the tightest results compared to other verification approaches.
        (2)~The robust training approaches effectively enhances the models' certified robustness. Among these existing robust training approaches, adversarial training usually achieves the best performance. 
        (3)~The choice of smoothing distribution can greatly affect the robustness of randomized models. One evidence is that, under $\cL_1$ adversary, the superior result is achieved by uniform smoothing distribution.
        (4)~For probabilistic verification approaches, certifying robustness under $\mathcal{L}_\infty$ adversary is hard, and would become harder when the data dimension increases.
        
        % \linyi{==== above is new, below is old ===(((}
        
        
        % In this subsection, we present the certified robustness comparison of probabilistic approaches, including both verification approaches and robust training approaches.
        
        % % ~\\
        
        % \subsubsection{\textbf{Experiment Setup}}\hfill \\ 
        % In our study, we integrate various major verification approaches under probabilistic setting (most of them could be reduced to close forms of the robustness radius) and reimplement the verification process. 
        % We evaluate these verification approaches on CIFAR-10 and ImageNet.
        % For both datasets, we certified a subsample of $500$ samples from the test set. All of the test examples are uniformly sampled from each class. 
        % We adopt ResNet-50 as the base classifier for ImageNet, following the fashion of all existing works. As for CIFAR-10, both Wide ResNet~(used by \cite{cohen2019certified}) and ResNet-110~(used by \cite{yang2020randomized}) are evaluated. 
        % We mainly report and compare the robust accuracy at given radius $r$ under $\cL_p$ norm. Specifically, we evaluate the cases where $p=1,2,\infty$.
        % % which is defined as the fraction of the test set for which the smoothed classifier correctly classifies and certifies robustness at an $l_p$ radius at least $r$. 
        
        % We follow the experimental procedure described by \cite{cohen2019certified} and \cite{yang2020randomized}. On both datasets, $n=1000$ samples are used for selecting the top label, $N=100,000$ samples are used for certification, and the failure probability is set to $1-\alpha=.001$, i.e., the probabilistic verification is $.999$-confident.
        % % 
        
        % % As the main motivation of our study is to validate the effectiveness of existing works and make a fair comparison, 
        % We mainly report the best robust accuracy of the most common settings.
        % The robust accuracy for each setting is shown in \Cref{tab:exp-B-main-table}.
        % % We encourage interested readers to refer the original papers of these frameworks to get a more thorough view.
        
        % % ~\\
        
        % \subsubsection{\textbf{\texorpdfstring{$\cL_2$}{L2} adversary}}\hfill \\
        % % 
        % In this part, we evaluate the robust accuracy on $\cL_2$ adversary.
        % % 
        % We mainly evaluate three verification approaches for $\cL_2$ adversary under Gaussian noise:
        % \begin{itemize}
        %     \item Differential privacy based method~\cite{lecuyer2019certified}; 
            
        %     \item Neyman-Pearson based method~\cite{cohen2019certified,yang2020randomized,Zhang2020BlackBoxCW};
            
        %     \item $f$-Divergence framework~\cite{Dvijotham2020A}.
        % \end{itemize}
        
        % The base classifier models are trained with different certifiable defenses: 
        % (1)~Adversarial training~\cite{salman2019provably};
        % (2)~Pretraining~\cite{salman2019provably,carmon2019unlabeled}: incorporating additional labeled and unlabeled data for supervised/semi-supervised pretraining. We directly follow the settings in \cite{salman2019provably};
        % (3)~MACER~\cite{Zhai2020MACER:};
        % (4)~ADRE~\cite{feng2020regularized}.
        
        % On CIFAR-10, We adopt Wide ResNet 40-2 with the common Gaussian noise data augmentation training~(recommended by \cite{yang2020randomized}) to evaluate the robust accuracy of the three verification approaches.
        % % the verification results are in \Cref{table:L2+augmentation+cifar}.
        % % 
        % To validate the effectiveness of recently proposed robust training approaches. We also train a set of ResNet-110 models with different robust training approaches. For fair comparison, The verification results are obtained via Neyman-Pearson method. 
        % % The results are in \Cref{table:L2+training+cifar}.
        
        % % \begin{itemize}
        % %     \item We adopt Wide ResNet 40-2 with the common gaussian noise data augmentation training (recommended by \cite{yang2020randomized}) to evaluate the certified accuracy of the three certification procedures. (See table \ref{table:L2+augmentation+cifar})
        % %     \item To validate the effectiveness of recently proposed training techniques. We also train a set of ResNet-110 models with different training techniques. For fair comparison, The certification results are obtained via Neyman-Pearson method. (See \Cref{table:L2+training+cifar})
        % % \end{itemize}
        
        
        % On ImageNet, All the evaluations are performed on ResNet-50 model. We train the model with Gaussian noise data augmentation training and other robust training approaches respectively. The comparison among the three verification approaches we listed above are conducted on noise data augmentation based model.
        % % The verification results are in \Cref{table:L2+augmentation+imagenet}. 
        % Neyman-Pearson method is adopted to evaluate and compare different robust training approaches.
        % % The results are in \Cref{table:L2+training+imagenet}.
        
        % All results on $\cL_2$ adversary are shown in \Cref{tab:L2-probability-synthesized}.
        
        % \begin{table}
        %     \caption{Robust accuracy against $\cL_2$ adversary on CIFAR-10 and ImageNet with different radius $r$.
        %     When evaluating probabilistic verification approaches, the model is trained under noise augmentation.
        %     When evaluating robust training approaches, the model is verified by Neyman-Pearson.
        %     On CIFAR-10, we adopt Wide ResNet 40-2 model for verification approaches and ResNet-110 model for robust training approaches.
        %     On ImageNet, we adopt ResNet-50 model.
        %     }
        %     \label{tab:L2-probability-synthesized}
        %     \centering
        %     \resizebox{0.49\textwidth}{!}{
        %     \begin{tabular}{c|c|c|c|c|c|c}
        %         \toprule
        %         \multirow{2}{*}{CIFAR-10} &  \multicolumn{6}{c}{$r$} \\
        %         \cline{2-7}
        %          & $0.25$ & $0.5$ & $0.75$ & $1.0$ & $1.25$ & $1.5$ \\
        %         \hline
        %         \multicolumn{7}{l}{\textbf{Verification Approach}} \\
        %         \hline
        %         Differential Privacy & $34.2\%$ & $14.8\%$ & $6.8\%$ & $2.2\%$ & $0\%$ & $0\%$\\
        %         \hline
        %         Neyman-Pearson & $\mb{68.8\%}$ & $\mb{46.8\%}$ & $\mb{36.0\%}$ & $\mb{25.4\%}$ & $\mb{19.8\%}$ & $\mb{15.6\%}$\\
        %         \hline
        %         $f$-Divergence & $62.2\%$ & $41.8\%$ & $27.2\%$ & $19.2\%$ & $14.2\%$ & $11.4\%$\\
        %         \hline
        %         \multicolumn{7}{l}{\textbf{Robust Training Approach}} \\
        %         \hline
        %         Noise augmentation & $61.2\%$ & $43.2\%$ & $32.0\%$ & $22.4\%$ & $17.2\%$ & $14.0\%$ \\
        %         \hline
        %         Adversarial training & $73.0\%$ & $57.8\%$ & $48.2\%$ & $\mb{37.2\%}$ & $33.6\%$ & $\mb{28.2\%}$ \\
        %         \hline
        %         Adversarial + pretraining & $\mb{81.8\%}$ & $\mb{62.6\%}$ & $\mb{52.4\%}$ & $37.2\%$ & $\mb{34.0\%}$ & $30.2\%$ \\
        %         \hline
        %         MACER & $68.8\%$ & $52.6\%$ & $40.4\%$ & $33.0\%$ & $27.8\%$ & $25.0\%$ \\
        %         \hline
        %         ADRE & $68.0\%$ & $50.2\%$ & $37.8\%$ & $30.2\%$ & $23.0\%$ & $17.0\%$ \\
        %         \hline\hline
        %         \multirow{2}{*}{ImageNet} &  \multicolumn{6}{c}{$r$} \\
        %         \cline{2-7}
        %          & $0.5$ & $1.0$ & $1.5$ & $2.0$ & $2.5$ & $3.0$ \\
        %         \hline
        %         \multicolumn{7}{l}{\textbf{Verification Approach}} \\
        %         \hline
        %         Differential Privacy & $26.0\%$ & $12.2\%$ & $4.4\%$ & $0\%$ & $0\%$ & $0\%$ \\
        %         \hline
        %         Neyman-Pearson & $\mb{49.2\%}$ & $\mb{37.4\%}$ & $\mb{29.0\%}$ & $\mb{19.2\%}$ & $\mb{14.8\%}$ & $\mb{12.0\%}$\\
        %         \hline
        %         $f$-Divergence & $43.4\%$ & $30.4\%$ & $13.6\%$ & $3.2\%$ & $0\%$ & $0\%$\\
        %         \hline
        %         \multicolumn{7}{l}{\textbf{Robust Training Approach}} \\
        %         \hline
        %         Noise augmentation & $49.2\%$ & $37.4\%$ & $29.0\%$ & $19.2\%$ & $14.8\%$ & $12.0\%$\\
        %         \hline
        %         Adversarial training & $56.4\%$ & $\mb{44.8\%}$ & $\mb{38.2\%}$ & $\mb{28.0\%}$ & $\mb{25.6\%}$ & $\mb{20.0\%}$ \\
        %         \hline
        %         MACER & $\mb{57.0\%}$ & $43.2\%$ & $31.4\%$ & $24.8\%$ & $17.6\%$ & $14.0\%$ \\
        %         \hline
        %         ADRE & $\mb{57.0\%}$ & $41.8\%$ & $30.0\%$ & $23.6\%$ & $17.8\%$ & $14.2\%$ \\
        %         \bottomrule
        %     \end{tabular}
        %     }
        % \end{table}
        
        % % \begin{table}
        % %         \centering
        % %         \caption{Robust accuracy under $\cL_2$ adversary on CIFAR-10 with different radius $r$ for different probabilistic verification approaches. 
        % %         Wide ResNet 40-2 is adopted as the base classifier and the model is trained under common noise data augmentation.
        % %         }
        % %         \resizebox{0.49\textwidth}{!}{
        % %         \begin{tabular}{c|c|c|c|c|c|c}
        % %             \toprule
        % %             Verification & \multicolumn{6}{c}{$r$} \\
        % %              \cline{2-7}
        % %             Approach & $0.25$ & $0.5$ & $0.75$ & $1.0$ & $1.25$ & $1.5$  \\
        % %             \hline
        % %             Differential Privacy & $34.2\%$ & $14.8\%$ & $6.8\%$ & $2.2\%$ & $0\%$ & $0\%$\\
        % %             \hline
        % %             Neyman-Pearson & $68.8\%$ & $46.8\%$ & $36.0\%$ & $25.4\%$ & $19.8\%$ & $15.6\%$\\
        % %             \hline
        % %             $f$-Divergence & $62.2\%$ & $41.8\%$ & $27.2\%$ & $19.2\%$ & $14.2\%$ & $11.4\%$\\
        % %             \bottomrule
        % %         \end{tabular}
        % %         }
        % %         \label{table:L2+augmentation+cifar}
        % %     \end{table}
            
        % %     \begin{table}
        % %         \centering
        % %         \caption{Robust accuracy under $\mathcal{L}_2$ adversary on CIFAR-10 with different radius $r$. ResNet-110 is adopted as the base classifier and the models are trained with various robust training approaches. The verification is made by Neyman-Pearson method.}
        % %         \resizebox{0.49\textwidth}{!}{
        % %         \begin{tabular}{c|c|c|c|c|c|c}
        % %             \toprule
        % %             Robust Training & \multicolumn{6}{c}{$r$} \\
        % %             \cline{2-7}
        % %             Approach & $0.25$ & $0.5$ & $0.75$ & $1.0$ & $1.25$ & $1.5$  \\
        % %             \hline
        % %             Noise augmentation & $61.2\%$ & $43.2\%$ & $32.0\%$ & $22.4\%$ & $17.2\%$ & $14.0\%$ \\
        % %             \hline
        % %             Adversarial training & $80.5\%$ & $62.2\%$ & $52.1\%$ & $38.1\%$ & $33.9\%$ & $30.4\%$ \\
        % %             \hline
        % %             Adversarial + pretraining & $81.8\%$ & $62.6\%$ & $52.4\%$ & $37.2\%$ & $34.0\%$ & $30.2\%$ \\
        % %             \hline
        % %             MACER & $68.8\%$ & $52.6\%$ & $40.4\%$ & $33.0\%$ & $27.8\%$ & $25.0\%$ \\
        % %             \hline
        % %             ADRE & $68.0\%$ & $50.2\%$ & $37.8\%$ & $30.2\%$ & $23.0\%$ & $17.0\%$ \\
        % %             \bottomrule
        % %         \end{tabular}
        % %         }
        % %         \label{table:L2+training+cifar}
        % %     \end{table}
            
        % %      \begin{table}
        % %         \centering
        % %         \caption{Robust accuracy under $\mathcal{L}_2$ adversary on ImageNet with different radius $r$ for different probabilistic verification approaches. ResNet-50 is adopted as the base classifier and the model is trained under common noise data augmentation.}
        % %         \resizebox{0.49\textwidth}{!}{
        % %         \begin{tabular}{c|c|c|c|c|c|c}
        % %             \toprule
        % %             Verification & \multicolumn{6}{c}{$r$} \\
        % %             \cline{2-7}
        % %             Approach & $0.5$ & $1.0$ & $1.5$ & $2.0$ & $2.5$ & $3.0$  \\
        % %             \hline
        % %             Differential Privacy & $26\%$ & $12\%$ & $4\%$ & $0\%$ & $0\%$ & $0\%$\\
        % %             \hline
        % %             Neyman-Pearson & $49\%$ & $37\%$ & $29\%$ & $19\%$ & $15\%$ & $12\%$\\
        % %             \hline
        % %             $f$-Divergence & $43\%$ & $30\%$ & $14\%$ & $3\%$ & $0\%$ & $0\%$\\
        % %             \bottomrule
        % %         \end{tabular}
        % %         }
        % %         \label{table:L2+augmentation+imagenet}
        % %     \end{table}
            
        % %     \begin{table}
        % %         \centering
        % %         \caption{Robust accuracy under $\mathcal{L}_2$ adversary for ImageNet with different radius $r$. ResNet-50 is adopted as the base classifier and the models are trained with various robust training approaches. Verification is made by Neyman-Pearson method.}
        % %         \resizebox{0.49\textwidth}{!}{
        % %         \begin{tabular}{c|c|c|c|c|c|c}
        % %             \toprule
        % %             Robust Training & \multicolumn{6}{c}{$r$} \\
        % %             \cline{2-7}
        % %             Approach & $0.5$ & $1.0$ & $1.5$ & $2.0$ & $2.5$ & $3.0$  \\
        % %             \hline
        % %             Noise augmentation & $49\%$ & $37\%$ & $29\%$ & $19\%$ & $15\%$ & $12\%$ \\
        % %             \hline
        % %             Adversarial training & $56\%$ & $45\%$ & $38\%$ & $28\%$ & $26\%$ & $20\%$ \\
        % %             \hline
        % %             MACER & $57\%$ & $43\%$ & $31\%$ & $25\%$ & $18\%$ & $14\%$ \\
        % %             \hline
        % %             ADRE & $57\%$ & $42\%$ & $30\%$ & $24\%$ & $18\%$ & $14\%$ \\
        % %             \bottomrule
        % %         \end{tabular}
        % %         }
        % %         \label{table:L2+training+imagenet}
        % %     \end{table}
        
        % % ~\\
        
        % \subsubsection{\textbf{\texorpdfstring{$\mathcal{L}_1$}{L1} adversary}}\hfill \\
        % % 
        % % In this part, we mainly evaluate the certified accuracy on $\mathcal{L}_1$ adversary. 
        % There are mainly two popular choices of smoothing noise for $\mathcal{L}_1$ adversary: Laplacian noise and Uniform noise. Note that all the noises are i.i.d..
        
        % For Laplacian noise, we mainly evaluate three verification approaches:
        % \begin{itemize}
        %     \item Differential privacy based method~\cite{lecuyer2019certified}:
        %     % $$
        %     %     \frac{\lambda}{2}\log(\frac{P_A}{1-P_A})
        %     % $$
            
        %     \item R\'enyi divergence based method~\cite{li2019certified}:
        %     % $$
        %     %     r = -\lambda\log(2(1-p_A))
        %     % $$
            
        %     \item Neyman-Pearson based method~\cite{teng2020ell,yang2020randomized}:
        %     % $$
        %     %     r=\max{\{\frac{\lambda}{2}\log(\frac{P_A}{1-P_A}),-\lambda\log(2(1-P_A))\}}
        %     % $$
        % \end{itemize}
        % For Uniform noise, we use the closed form derived by \cite{yang2020randomized}.
        % % via differential method:
        % % $$
        % %     r = 2\lambda(p_A-\frac{1}{2}).
        % % $$
        % % 
        % We adopt Wide ResNet 40-2 as the base classifier on CIFAR-10 and ResNet-50 on ImageNet.
        
        % All results are shown in \Cref{tab:L1-probability-synthesized}.
        
        % % The experiment results under Laplace noise on CIFAR-10 and ImageNet are shown in \Cref{table:L1+laplace+cifar} and \Cref{table:L1+laplace+imagenet} respectively. 
        % One can easily find that \cite{teng2020ell} and \cite{li2019certified} have almost the same performance. That is because the extra bound in \cite{teng2020ell} is exactly the loose bound in \cite{lecuyer2019certified} which is almost always less than the other bound.
        % \linyi{Do you mean \cite{teng2020ell} is worse than \cite{lecuyer2019certified}? But experiment numbers seem to show the opposite...}
        % % (see figure \ref{fig:bounds_teng}). 
        % % 
        % % The experiment results under uniform noise on CIFAR-10 and ImageNet are shown in \Cref{table:L1+uniform+cifar} and \Cref{table:L1+uniform+imagenet}.
        
        
        % \begin{table}
        %     \caption{Robust accuracy against $\cL_1$ adversary on CIFAR-10 and ImageNet with different radius $r$.
        %     When evaluating probabilistic verification approaches, the model is trained under Laplacian noise.
        %     When evaluating smoothing noises, the model is verified by Neyman-Pearson.
        %     We adopt Wide ResNet 40-2 model on CIFAR-10 and ResNet-50 model on ImageNet.}
        %     \label{tab:L1-probability-synthesized}
        %     \centering
        %     \resizebox{0.49\textwidth}{!}{
        %     \begin{tabular}{c|c|c|c|c|c|c|c|c}
        %         \toprule
        %         \multirow{2}{*}{CIFAR-10} & \multicolumn{8}{c}{$r$} \\
        %         \cline{2-9}
        %         & $0.5$ & $1.0$ & $1.5$ & $2.0$ & $2.5$ & $3.0$ & $3.5$ & $4.0$  \\
        %         \hline
        %         \multicolumn{9}{l}{\textbf{Verification Approach}} \\
        %         \hline
        %         Differential privacy & $43.0\%$ & $20.8\%$ & $12.2\%$ & $7.2\%$ & $3.4\%$ & $1.4\%$ & $0.4\%$ & $0\%$ \\
        %         \hline
        %         R\'enyi divergence & $58.2\%$ & $39.4\%$ & $\mb{27.0\%}$ & $16.8\%$ & $\mb{12.2\%}$ & $\mb{9.2\%}$ & $\mb{6.4\%}$ & $4.0\%$ \\
        %         \hline
        %         Neyman-Pearson & $\mb{58.4\%}$ & $\mb{39.6\%}$ & $\mb{27.0\%}$ & $\mb{17.2\%}$ & $\mb{12.2\%}$ & $\mb{9.2\%}$ & $\mb{6.4\%}$ & $\mb{4.2\%}$ \\
        %         \hline
        %         \multicolumn{9}{l}{\textbf{Smoothing Noise}} \\
        %         \hline
        %         Laplace & $58.4\%$ & $39.6\%$ & $27.0\%$ & $17.2\%$ & $12.2\%$ & $9.2\%$ & $6.4\%$ & $4.2\%$ \\
        %         \hline
        %         Uniform & $\mb{69.2\%}$ & $\mb{56.6\%}$ & $\mb{48.0\%}$ & $\mb{39.4\%}$ & $\mb{32.0\%}$ & $\mb{26.0\%}$ & $\mb{23.4\%}$ & $\mb{20.4\%}$ \\
        %         \hline\hline
        %         \multirow{2}{*}{ImageNet} & \multicolumn{8}{c}{$r$} \\
        %         \cline{2-9}
        %         & $0.5$ & $1.0$ & $1.5$ & $2.0$ & $2.5$ & $3.0$ & $3.5$ & $4.0$  \\
        %         \hline
        %         \multicolumn{9}{l}{\textbf{Verification Approach}} \\
        %         \hline
        %         Differential privacy & $39.0\%$ & $26.2\%$ & $17.8\%$ & $13.0\%$ & $8.2\%$ & $6.8\%$ & $0\%$ & $0\%$ \\
        %         \hline
        %         R\'enyi divergence & $48.2\%$ & $40.4\%$ & $31.0\%$ & $25.8\%$ & $\mb{22.2\%}$ & $\mb{19.0\%}$ & $\mb{17.4\%}$ & $\mb{13.6\%}$ \\
        %         \hline
        %         Neyman-Pearson & $\mb{49.0\%}$ & $\mb{40.8\%}$ & $\mb{31.2\%}$ & $\mb{26.0\%}$ & $\mb{22.2\%}$ & $\mb{19.0\%}$ & $\mb{17.4\%}$ & $\mb{13.6\%}$ \\
        %         \hline
        %         \multicolumn{9}{l}{\textbf{Smoothing Noise}} \\
        %         \hline
        %         Laplace & $49.0\%$ & $40.8\%$ & $31.2\%$ & $26.0\%$ & $22.2\%$ & $19.0\%$ & $17.4\%$ & $13.6\%$ \\
        %         \hline
        %         Uniform & $\mb{55.2\%}$ & $\mb{49.0\%}$ & $\mb{45.6\%}$ & $\mb{42.0\%}$ & $\mb{37.4\%}$ & $\mb{32.8\%}$ & $\mb{28.0\%}$ & $\mb{24.8\%}$ \\
        %         \bottomrule
        %     \end{tabular}
        %     }
        % \end{table}
        
        % % \begin{table}
        % %         \centering
        % %         \caption{Robust accuracy on CIFAR-10 under $\mathcal{L}_1$ adversary and Laplacian noise using different verification approaches with different radius $r$. Wide ResNet 40-2 is adopted as the base classifier.}
        % %         \resizebox{0.49\textwidth}{!}{
        % %         \begin{tabular}{c|c|c|c|c|c|c|c|c}
        % %             \toprule
        % %             Verification & \multicolumn{8}{c}{$r$} \\
        % %             \cline{2-9}
        % %             Approach & $0.5$ & $1.0$ & $1.5$ & $2.0$ & $2.5$ & $3.0$ & $3.5$ & $4.0$  \\
        % %             \hline
        % %             Differential privacy & $43.0\%$ & $20.8\%$ & $12.2\%$ & $7.2\%$ & $3.4\%$ & $1.4\%$ & $0.4\%$ & $0\%$ \\
        % %             \hline
        % %             R\'enyi divergence & $58.2\%$ & $39.4\%$ & $27.0\%$ & $16.8\%$ & $12.2\%$ & $9.2\%$ & $6.4\%$ & $4.0\%$ \\
        % %             \hline
        % %             Neyman-Pearson & $58.4\%$ & $39.6\%$ & $27.0\%$ & $17.2\%$ & $12.2\%$ & $9.2\%$ & $6.4\%$ & $4.2\%$ \\
        % %             \bottomrule
        % %         \end{tabular}
        % %         }
        % %         \label{table:L1+laplace+cifar}
        % %     \end{table}
            
        % %     \begin{table}
        % %         \centering
        % %         \caption{Robust accuracy on CIFAR-10 under $\mathcal{L}_1$ adversary and Uniform noise with different radius $r$. Wide ResNet 40-2 is adopted as the base classifier.}
        % %         \resizebox{0.49\textwidth}{!}{
        % %         \begin{tabular}{c|c|c|c|c|c|c|c|c}
        % %             \toprule
        % %             & \multicolumn{8}{c}{$r$} \\
        % %             \cline{2-9}
        % %             \multirow{1}{*}{ } & $0.5$ & $1.0$ & $1.5$ & $2.0$ & $2.5$ & $3.0$ & $3.5$ & $4.0$  \\ 
        % %             \hline
        % %             Uniform & $69.2\%$ & $56.6\%$ & $48.0\%$ & $39.4\%$ & $32.0\%$ & $26.0\%$ & $23.4\%$ & $20.4\%$ \\
        % %             \bottomrule
        % %         \end{tabular}
        % %         }
        % %         \label{table:L1+uniform+cifar}
        % %     \end{table}
            
        % %     \begin{table}
        % %         \centering
        % %         \caption{Robust accuracy on ImageNet under $\mathcal{L}_1$ adversary and Laplace noise using different verification approaches with different radius $r$. ResNet-50 is adopted as the base classifier.}
        % %         \resizebox{0.49\textwidth}{!}{
        % %         \begin{tabular}{c|c|c|c|c|c|c|c|c}
        % %             \toprule
        % %             Verification & \multicolumn{8}{c}{$r$} \\
        % %             \cline{2-9}
        % %             Approach & $0.5$ & $1.0$ & $1.5$ & $2.0$ & $2.5$ & $3.0$ & $3.5$ & $4.0$  \\
        % %             \hline
        % %             \sc{Differential privacy} & $39\%$ & $26\%$ & $18\%$ & $13\%$ & $8\%$ & $7\%$ & $0\%$ & $0\%$ \\
        % %             \hline
        % %             \sc{R\'enyi divergence} & $48\%$ & $40\%$ & $31\%$ & $26\%$ & $22\%$ & $19\%$ & $17\%$ & $14\%$ \\
        % %             \hline
        % %             \sc{Neyman-Pearson} & $49\%$ & $41\%$ & $31\%$ & $26\%$ & $22\%$ & $19\%$ & $17\%$ & $14\%$ \\
        % %             \bottomrule
        % %         \end{tabular}
        % %         }
        % %         \label{table:L1+laplace+imagenet}
        % %     \end{table}
            
        % %     \begin{table}
        % %         \centering
        % %         \caption{Robust accuracy on CIFAR-10 under $\mathcal{L}_1$ adversary and Uniform noise with different radius $r$. Wide ResNet 40-2 is adopted as the base classifier.}
        % %         \resizebox{0.49\textwidth}{!}{
        % %         \begin{tabular}{c|c|c|c|c|c|c|c|c}
        % %             \toprule
        % %             & \multicolumn{8}{c}{$r$} \\
        % %             \cline{2-9}
        % %             & $0.5$ & $1.0$ & $1.5$ & $2.0$ & $2.5$ & $3.0$ & $3.5$ & $4.0$  \\ 
        % %             \hline
        % %             Uniform & $55\%$ & $49\%$ & $46\%$ & $42\%$ & $37\%$ & $33\%$ & $28\%$ & $25\%$ \\
        % %             \bottomrule
        % %         \end{tabular}
        % %         }
        % %         \label{table:L1+uniform+imagenet}
        % %     \end{table}
        
        % % ~\\
        
        % \subsubsection{\textbf{\texorpdfstring{$\mathcal{L}_\infty$}{Linfty} adversary}}\hfill \\
        % To our best knowledge, all state-of-the art $\mathcal{L}_\infty$ certification results under probabilistic settings are obtained based on conversions from other norm metrics. 
        % For example, given input dimension $d$, since $\|x\|_2 \le \|x\|_\infty \sqrt d$, the model with certified robust radius $r$ in $\cL_2$ norm at point $x_0$ is also certified robust with radius $r / \sqrt d$ in $\cL_\infty$ norm.
        % % The core idea is one robustness radius derived under a certain $\cL_p$ norm metric could be directly converted to a robustness radius for another norm metric $\cL_k$. So, the $\cL_\infty$ robustness could be directly derived from other metrics (e.g. $\cL_2$).
        % % The conversion rule and theoretical foundations are deferred to \Cref{sec:adx-full-exp-probabilistic}.
        % Based on the conversion rule, we could directly obtain the $\cL_{\infty}$ robustness from state-of-the-art results under $\cL_{2}$ adversary with Gaussian smoothing
        % \linyi{In experiments it seems that we are not deriving from the state-of-the-art result. May be incorrect.}
        % % $$
        % %     r = \frac{\sigma\Phi^{-1}(\underline{P_A})}{\sqrt{d}},
        % % $$
        % which is empirically shown to be the best probabilistic setting for $\mathcal{L}_{\infty}$ \cite{yang2020randomized}.
        % % 
        % We evaluate the $\mathcal{L}_{\infty}$ robustness with this Gaussian setting on both CIFAR-10 and ImageNet, the result is reported in \Cref{table:L_inf+uniform}.
        
        %  \begin{table}
        %         \centering
        %         \caption{Robust accuracy under $\cL_\infty$ adversary and Gaussian noise under varous raidus $r$. Wide ResNet 40-2 is adopted for CIFAR-10 and ResNet-50 for ImageNet.}
        %         % \resizebox{0.49\textwidth}{!}{
        %         \small
        %         \begin{tabular}{c|c|c|c|c}
        %             \toprule
        %             & \multicolumn{4}{c}{$r$} \\
        %             \cline{2-5}
        %             & $1/255$ & $2/255$ & $4/255$ & $8/255$ \\ 
        %             \hline
        %             CIFAR-10 & $71.4\%$ & $52.0\%$ & $29.0\%$ & $12.8\%$ \\
        %             \hline
        %             ImageNet & $28.2\%$ & $11.4\%$ & $0\%$ & $0\%$ \\
        %             \bottomrule
        %         \end{tabular}
        %         % }
        %         \label{table:L_inf+uniform}
        %     \end{table}
        
        % % ~\\
        
        % % \linyi{Maybe we need a discussion about the results here?}
        % \subsubsection{\textbf{Discussions}}\hfill \\
        % According to the experiment results, several key conclusions are as follow:
        % \begin{itemize}
        %     \item For both $\mathcal{L}_1$ and $\mathcal{L}_2$ metrics, Neyman-Pearson based verification achieves the tightest results compared to other methodologies.
        %     \item The robust training techniques effectively enhance the models' certified robustness. Among these existing techniques, adversarial training methodology achieves the state-of-the-art performance. 
        %     \item The choice of smoothing measure can greatly affect the robustness of randomized models. The superior result achieved by uniform noise smoothing under $\mathcal{L}_1$ metric is one prominent evidence.
        %     \item Certifying robustness radius for $\mathcal{L}_\infty$ metric is hard would become harder when the data dimension increases. 
        % \end{itemize}
        % \linyi{)))}
        
        
        % \subsubsection{\textbf{Discussion}}\hfill \\
        %     \TODO
        

\section{Related Applications and Extensions}

    The methodologies derived from neural network certified robustness have recently been applied to much boarder areas.
    In this section we exemplify the representatives.
    
    \para{Beyond $\cL_p$ adversary.}
        There are several beyond $\cL_p$ adversarial attacks proposed recently.
        The semantic transformations such as rotation or scaling with small angles or ratios can generate adversarial examples~\cite{engstrom2017rotation,xiao2018spatially}.
        Linear-relaxation based approaches~\cite{singh2019abstract,balunovic2019certifying,Mohapatra_2020_CVPR} or probabilistic approaches~\cite{fischer2020certification,li2020provable} can provide robustness verification against these attacks.
        Moreover, if the input image space is discrete, the robustness verification against these attacks can be achieved by enumeration~\cite{pei2017towards}.
        The patch adversary will add a small patch to the input image with random pattern.
        Robustness verification against patch adversary is subsumed by verification against $\cL_0$ adversary~\cite{lee2019tight,levine2019robustness}.
        There are also other better-tailored verification approaches~\cite{Chiang*2020Certified,alex2020derandomized} based on linear relaxations or probabilistic approaches.
        \citeauthor{levine2019wasserstein}~\cite{levine2019wasserstein} propose verification against Wasserstein adversary~\cite{pmlr-v97-wong19a}.
        A few verification approaches can verify predefined linear safety properties.
        These approaches can be either complete~\cite{ehlers2017formal,katz2017reluplex,10.1007/978-3-319-63387-9_1} or incomplete~\cite{qin2018verification}.
        % 
        Recently, probabilistic verification approaches are extended to verify top-$k$ prediction robustness~\cite{jia2020certified}, and robustness against label-flipping attack~\cite{rosenfeld2020certified} and back-door attack~\cite{weber2020rab,levine2020deep}.

    % In previous sections we limited the scoop to neural network verifiable robustness against $\cL_p$ adversary.
    % Here, we enlarge our scoop ---
    % we briefly introduce robustness verification approaches for: (1)~adversaries other than $\cL_p$ adversary; 
    % (2)~models other than classical neural networks; 
    % and (3)~tasks other than classification.
    % % \linyi{Plan to draw a branch figure to visualize all these various extensions.}
    
    % \subsection{Beyond \texorpdfstring{$\cL_p$}{Lp} Adversary}
    %     \label{sec:beyond-lp-adversary}
        
    %     Adversarial example can be generated by many other types of adversaries besides $\cL_p$ bounded perturbations, such as spatial transformations and noise patches.
    %     Examples generated in these ways are imperceptible to human but can still deteriorate the model accuracy significantly~\cite{brown2017adversarial,karmon2018lavan,xiao2018spatially}.
    %     We briefly overview the robust verification approaches against these adversaries.
        
    %     \subsubsection{Verifying Against Semantic-Based Attacks}
    %         \bo{1. additional challenges compare with norm based; 2. summarize existing work+table. 3. comparison. 4. potential other ways}
                
    %             Besides $\cL_p$ adversary, 
    %             in \Cref{tab:semantic-taxonogy} we categorize verification approaches against semantic transformations.
            
    %             \begin{table}[!t]
    %                 \centering
    %                 \label{tab:semantic-taxonogy}
    %                 \caption{robustness verification approaches against semantic-based attacks.}
    %                 % \resizebox{0.49\textwidth}{!}{
    %                 \begin{tabular}{c|c|c}
    %                     \toprule
    %                     Approach & Category  & Scalability \\
    %                     \hline \hline
    %                     DeepPoly~\cite{singh2019abstract} & IBP &  Toy MNIST \\
    %                     DeepG~\cite{balunovic2019certifying} & LP, relax & CIFAR-10 \\
    %                     Semantify-NN~\cite{Mohapatra_2020_CVPR} & LP, relax & CIFAR-10 \\
    %                     \citeauthor{fischer2020certification}~\cite{fischer2020certification} & Rand. Smooth & ImageNet \\
    %                     \citeauthor{li2020provable}~\cite{li2020provable} & Rand. Smooth & ImageNet \\
    %                     \bottomrule
    %                 \end{tabular}
    %                 % }
    %             \end{table}
    %         The semantic transformations refer to geometric transformations which do not change the image semantics, such as rotation with small angles or translation with small displacement.
    %         The semantic-based attacks exert semantic transformations to the image input to mislead the model.
    %         These attackes can produce quite difference images measured by $\cL_p$ norm, which poses challenges to existing verification approaches.
            
    %         DeepPoly~\cite{singh2019abstract} firstly show how to verify against rotation transformation by splitting the interval to be verified, and computing per-pixel color interval in each split interval.
    %         Then, standard linear relaxation based verification approaches can be applied.
    %         DeepG~\cite{balunovic2019certifying} extends DeepPoly by using symbolic computation to get the Lipschitz bound with respect to transformation parameters, then, it does splitting and generates linear constraints for verification.
    %         It supports much more types of semantic transformations.
    %         % and the composition of them.
    %         Semantify-NN~\cite{Mohapatra_2020_CVPR} encodes the transformations as computation on neural networks so traditional verification approaches against $\cL_p$ adversary can be directly applied.
    %         However, the transformations which cannot be precisely encoded require finer and more complex analysis.
            
    %         Recently, \citeauthor{fischer2020certification}~\cite{fischer2020certification} and \citeauthor{li2020provable}~\cite{li2020provable} propose randomized smoothing based verification approaches for semantic verifications.
    %         A major threat for extending randomized smoothing to semantic transformation is that, the noise is usually not additive with respect to transformation parameters such as rotation angles or scaling ratios.
    %         % In \cite{li2020provable}, this characteristic is discussed in detail.
    %         To mitigate this, \cite{fischer2020certification} use probabilistic sampling to estimate the non-additive error and step back to only defend against randomized adversary.
    %         % , so the probabilistic sampling based error bound is valid.
    %         In \cite{li2020provable}, the rigorous error upper bound is computed from local Lipschitz constant, so it can defend any adversary, and it achieved good verifiable robust accuracy.
        
    %     % \subsubsection{Certifying Against Wasserstein Adversarial Examples}
        
    %     \subsubsection{Verifying Against Patch Attacks}
    %         Another popular adversary definition is the patch adversary, where the adversary can add a small random patch to the image.
    %         Both semantic transformations and patches have valid implication in real-world applications such as autonomous driving, where the attacker can rotate the camera or attach a sticker to the camera.
            
    %         The verification against $\cL_0$ adversary~\cite{lee2019tight,levine2019robustness} can be directly applied to certify patch attacks.
    %         % They are all based on randomized smoothing.
    %         Furthermore, \citeauthor{Chiang*2020Certified}~\cite{Chiang*2020Certified} build patch attack robustness verification from interval bound propagation, and \citeauthor{alex2020derandomized}~\cite{alex2020derandomized} improves \cite{levine2019robustness} by improving the robust accuracy and eliminating the randomness.
        
    %     \subsubsection{Verifying Against Wassterstein Adversary}
    %         \citeauthor{pmlr-v97-wong19a}~\cite{pmlr-v97-wong19a} proposes to bound the adversary power by Wasserstein distance.
    %         Based on randomized smoothing, \citeauthor{levine2019wasserstein}~\cite{levine2019wasserstein} verifies model robustness against this adversary.
        
    %     \subsubsection{Others}
    %         A few complete verification approaches verify predefined safety specifications~\cite{ehlers2017formal,katz2017reluplex,10.1007/978-3-319-63387-9_1}.
    %         \citeauthor{qin2018verification}~\cite{qin2018verification} propose an approach to verify any convex specification using linear inequality propagation.
    %         From randomized smoothing, the verification for top-$k$ prediction can also be achieved~\cite{jia2020certified}.
        
    %     % Recently, randomized smoothing is shown to be able to extend to certifiably defend black-box pretrained model, as shown by \cite{salman2020blackbox}.
        
    %     % \subsubsection{Certifying \texorpdfstring{Top-$k$}{Top-k} Predictions}
        
    \para{Beyond classical neural network models.}
    % 
        The methodologies derived from DNN robustness verification have inspired robustness verification approaches for: tree models~\cite{chen2019robustness,andriushchenko2019provably}; model ensemble~\cite{zhang2019enhancing}, probabilistic models~\cite{dvijotham2018verification}, and generative models~\cite{mirman2020robustness}.
        We note that the certified robustness on boosted trees is comparable to DNNs on MNIST and CIFAR-10~\cite{andriushchenko2019provably}.
    
        % There is rich literature regarding robustness verification of other machine learning models except classical neural networks.
        % % Recent new approaches are mainly on tree models and the models using neural networks as the building blocks.
        
        % \subsubsection{Tree Models}
        %     In \cite{chen2019robustness}, a verification approach for tree-based models is proposed.
        %     Their novel verification approach exploits the tree structure efficiently.
        %     Recently, \citeauthor{andriushchenko2019provably}~\cite{andriushchenko2019provably} proposes a novel verification approach for boosted trees.
        %     The accompanied robust training approach pushes boosted trees to a comparable verifiable robust level as neural networks on both MNIST and CIFAR-10.
        
        % \subsubsection{Model Ensemble}
        %     To achieve higher robustness, a natural direction to follow is model ensemble, by aggregating a group of models together.
        %     In WK+~\cite{wong2018scaling}, ``cascade ensemble'' is proposed, where new model of the ensemble is trained only on samples that are failed to being robustly verified by previous models.
        %     This ensemble outperforms single model in terms of verifiable robustness.
        %     \citeauthor{zhang2019enhancing}~\cite{zhang2019enhancing} propose verification and training approaches for model ensemble by assigning different weights to each model.
        
        % % \subsubsection{\texorpdfstring{$k$-NN}{k-NN}}
        
        % % \subsubsection{Probabilistic Models}
        
        % \subsubsection{Others}
        %     There are also verification approaches for probabilistic models~\cite{dvijotham2018verification} and generative models~\cite{mirman2020robustness}.
        %     % Since these models use neural networks as the building blocks, existing verification approaches can be extended to them.

    \para{Beyond image based classification.}
    % 
        In natural language processing, the linear relaxations have been adopted to certify robustness against word substitutions~\cite{Jia2019CertifiedRT}, word transformations~\cite{zhang2020robustness}, and robustness of transformers with self-attention and cross-position dependency~\cite{Shi2020Robustness}.
        % 
        In graph neural networks, recent robustness verification approaches are motivated from either linear relaxations~\cite{bojchevski2019certifiable,zugner2019certifiable} or randomized smoothing~\cite{jia2020community}.
        % 
        The relaxation-based approaches can also verify the reinforcement learning robustness~\cite{wang2019verification,lutjens2019certified}.
    
        % \subsubsection{Natural Language Processing}
        %     Using the similar idea as linear relaxations, some work deals with popular natural language processing models.
        %     \citeauthor{Jia2019CertifiedRT}~\cite{Jia2019CertifiedRT} verify robustness against word substitutions by applying interval bound propagation to word embedding models.
        %     \citeauthor{zhang2020robustness}~\cite{zhang2020robustness} combine interval bound propagation into the training objective to train robust models against word transformation, and their verification is done by exhaustive search benefited from the finite space.
        %     \citeauthor{Shi2020Robustness}~\cite{Shi2020Robustness} extend linear relaxation based approaches to transformers for robustness verification.
        %     They handle self-attention and cross-position dependency efficiently.
        
        % \subsubsection{Graph Neural Networks}
        %     The graph neural networks are widely used in data mining and their robustness is of concern~\cite{jin2020adversarial}.
        %     The robustness verification and robust training on graph neural networks can be derived from optimization and linear relaxation~\cite{bojchevski2019certifiable,zugner2019certifiable}, or from randomized smoothing~\cite{jia2020community}.
        
        % \subsubsection{Reinforcement Learning}
        %     The robustness verification in reinforcement learning can be achieved from relaxation-based approaches~\cite{wang2019verification,lutjens2019certified},
        %     or program synthesis~\cite{zhu2019inductive}.
    
    % \subsection{Defense Existing Models}
    
    %     \linyi{Black-box defense existing models using randomized smoothing.}
        

% \section{Verification approaches for different Applications}

%     In \cref{tab:related-taxonogy} we list a few relevant application of verification techniques in concrete applications or other relevant models.
    
    % \begin{table*}[!t]
    %     \centering
    %     \caption{Certified robustness for different applications and models.}
    %     \begin{tabular}{c|c|c|l}
    %         \toprule
    %         Domain & Paper & Category & Main Contribution \\
    %         \hline \hline
    %         NLP & \cite{Jia2019CertifiedRT} & IBP, training & Robust to word substitutions  \\
    %         & \cite{zhang2020robustness} & IP, training & Robust to word transformations \\
    %         & \cite{Shi2020Robustness} & LP, relax & Verification for transformers \\
    %         \hline
    %         RL & \cite{wang2019verification} & LP, relax & Control policy \\
    %         \hline
    %         Tree Model & \cite{chen2019robustness} & D\&C, relax & Verification of tree model \\
    %         & \cite{andriushchenko2019provably} & exact & Verification and training of boosted trees \\
    %         $k$-NN & \cite{wang2019evaluating} & CQP, dual & Verification of $k$-NN model \\
    %         Ensemble & \cite{wong2018scaling} & LP, relax & Train of ensemble \\
    %         & \cite{zhang2019enhancing} & LP, relax & Train and verification of ensemble \\
    %         \hline
    %         Image Patch Adversary & \cite{Chiang*2020Certified} & IBP & Defense and verification \\
    %         & \cite{alex2020derandomized} & Rand. Smooth & Defense and verification \\
    %         \hline
    %         Randomized Smoothing & \cite{jia2020certified} & Rand. Smooth & Top-$k$ prediction certification \\
    %         & \cite{jia2020community} & Rand. Smooth & Community detection on graph \\
    %         & \cite{wang2020backdoor} & Rand. Smooth & Backdoor attack certification \\
    %         & \cite{salman2020blackbox} & Rand. Smooth & Defense built upon pretrained models \\
    %         \bottomrule
    %     \end{tabular}
    %     \label{tab:related-taxonogy}
    % \end{table*}


\section{Discussion}
    
    \para{Where are we?}
    After the booming in recent years, the certified robustness on DNNs have had significant progresses in practice.
    On MNIST, the certified robust accuracy against $\cL_\infty$ adversary with $0.3$ radius has reached over $92\%$; with $0.4$ radius has reached about $88\%$~\cite{gowal2019scalable,zhang2020towards}.
    This is remarkable since the limit is $0.5$ radius where any input image can be perturbed to indistinguishable half-gray.
    This is achieved by \t{CROWN-IBP} and \t{IBP} robust training, which is derived from the time efficient but loose verification approach.
    On more challenging CIFAR-10 and ImageNet dataset, however, current certified robust accuracy is still vacuous.
    On CIFAR-10, against $\cL_\infty$ adversary with $2/255$ radius, it is only about $68\%$ certified robust accuracy~\cite{salman2019provably}; with $8/255$ radius, it is only about $33\%$ certified robust accuracy~\cite{zhang2020towards}.
    Both numbers are too far from the over $90\%$ accuracy on clean inputs achieved by common CIFAR-10 models.
    On ImageNet, currently, only probabilistic approaches, e.g., \cite{cohen2019certified,yang2020randomized,salman2019provably}, can provide non-trivial robustness bound: $28\%$ under $\cL_2$ radius $2.0$; and about $38\%$ under $\cL_\infty$ radius $1/255$~\cite{zhang2020towards}.
    They are achieved by pre-training, self-training, then adversarial training of the randomized models. The Neyman-Pearson based approach provides the robustness certification for such trained model.
    
    As we can see, deterministic approaches perform well on small dataset like MNIST.
    On slightly larger CIFAR-10, deterministic approaches are better with large radius while probabilistic approaches are better with small radius.
    On large dataset ImageNet, the probabilistic approaches outperforms deterministic ones significantly.
    
    \para{Challenges.}
    From above results, one may think about improving probabilistic approaches to achieve better certified robustness on large datasets.
    % \xiangyu{higher certified robustness $\rightarrow$ better certified robustness.}
    However, current probabilistic approaches suffer from great challenges both theoretically and practically.
    % \xiangyu{approach $\rightarrow$ approaches, related usage is also modified.}
    Theoretically, they suffer from \emph{curse of dimensionality}:
    without more information than label statistics, no smoothing techniques can certify non-trivial robust accuracy at $\cL_\infty$ radius $\Omega\left(\min(1,\,d^{\frac{1}{p} - \frac{1}{2}})\right)$~\cite{yang2020randomized,kumar2020curse}.
    This conclusion implies that current probabilistic approaches cannot certify large $\cL_\infty$ radius intrinsically.
    Empirically, to certify large radius using probabilistic approach, we have to exert large noise to the input, which significantly hurt the prediction accuracy~\cite{cohen2019certified}.
    
    Now we present a novel barrier for randomized classifiers.
    %\para{Shrinkage of verifiable robustness.}
        %We present the following theorem.
    \begin{theorem}
        \label{thm:bar}
        For binary classification task, for any $\cL_p$ norm,
        assume the base classifier $F$'s decision region for label $y_0$ is centered at $x_0$ with radius $r$, i.e., $F(x) = y_0 \iff x \in B_{p,r}(x_0)$.
        % 
        Define the randomized classifier $G^\mu(x) := \argmax_i \bbE_{\delta\sim\mu} \left[F(x+\delta)=i\right]$ where $\delta$ is drawn from any continuous distribution $\mu$.
        Its robust radius at point $x_0$ satisfies
        $r' < r$,
        i.e., there exists $x$ such that $\|x - x_0\|_p \le r$ and $G^\mu(x) \neq y_0$.
    \end{theorem}
    The proof is deferred to \Cref{sec:adx-omit-proof-barrier-rand-smooth}.
    % \ifnum\arxiv=1
    % \linyi{Add one sentence to explain the theorem better. Available only for ArXiv version due to page limit.}
    Intuitively, the theorem implies that, if a base classifier $F$'s decision region for some label $y_0$ is exactly the ball $B_{p,r}(x_0)$, then, after smoothing by any continuous distribution $\mu$, the resulting decision region for $y_0$ in the randomized classifier $G^\mu$ does not contain any $r$-radius ball under $\cL_p$ metric.
    % \fi
    It implies that when the base classifier is robust within an $\cL_p$ ball, then \emph{any} randomized classifier cannot enlarge the robust ball's radius anymore for \emph{any} $\cL_p$ metric.
    % It is possible to extend the theorem for other decision region shapes or noise distributions.
    Such decision region shrinkage is also utilized for a theoretical explanation of trade-off between accuracy and certified robustness in Gaussian-smoothing based probabilistic verification approaches under $\cL_2$ adversary~\cite{mohapatra2020rethinking}.
    Before \cite{mohapatra2020rethinking}, such trade-off is widely observed~\cite{fawzi2018analysis,tsipras2018robustness,raghunathan2020understanding} and just intuitively explained for probabilistic verification ~\cite{yang2020randomized,Zhang2020BlackBoxCW}.
    
    On the other hand, the deterministic verification approaches suffer from strong trade-off between tightness and scalability.
    Comparing to probabilistic approaches, since they require complex computation within the model, they usually have much poorer scalability and can hardly support typically large models on ImageNet.
    Though further improvements for linear relaxations and SDP approaches should be possible, the \NP-completeness barrier blocks substantial advance or rigorous tightness/efficiency guarantee.
    For deterministic verification-based robust training, the trade-off between accuracy and certified robustness is also observed~\cite{wang2018mixtrain,wong2018provable}. 
    
    \para{Future Directions.}
    We believe major improvements of certified robustness could come from the following aspects:
    (1)~\underline{Tighter and more efficient verification}:
    just as MILP-based approaches have satisfactory efficiency for verifying robustly trained models even given its worst-case exponential complexity, 
    it is quite possible to improve other verification approaches to perform well in practice.
    In fact, \citeauthor{Baader2020Universal}~\cite{Baader2020Universal} prove the universal approximation power of IBP-certifiable neural networks.
    (2)~\underline{More effective robust training approaches}:
    though the trade-off between accuracy and certified robustness exists, it does not filter out further improvements from either accuracy or certified robustness.
    Actually, more effective robust training approaches are proposed consistently.
    (3)~\underline{Better inference scheme}:
    jumping out of using DNNs, we have seen that boosted trees have comparable certified robustness on MNIST and CIFAR-10.
    One future direction could be leveraging more structured machine learning models to improve the certified robustness, in which DNNs could serve as a component.

\section{Conclusions}
    In this paper we present the systematization of knowledge for certifiably robust approaches for DNNs, including both robustness verification approaches and corresponding robust training approaches.
    The comprehensive study shows that, there have been a remarkable research progress in certified robustness for DNNs, both practically and theoretically.
    Our discussion reveals current research status, limitations, and future directions in this emerging and promising field.    

% \begin{acks}
%     We thank Sasa Misailovic and Gagandeep Singh for their thoughtful feedback.
%     We are also thankful to the support of AWS Machine Learning Research Awards.
% \end{acks}

% \section*{Acknowledgement}


==> tables/exp-A-cifar10-radius-robust-acc.tex <==
% This file is automatically generated by experiments/model_summary.py



\begin{table*}
    \caption{
    \emph{Average certified robustness radius divided by $255$} on CIFAR-10 models certified by different \emph{deterministic verification approaches}. The verification is under $\cL_\infty$ adversary. 
    We include radius of adversarial example found by PGD attack to serve as the upper bound.
    The \textbf{bolded} numbers mark the highest ones among verification approaches.
    }
    \centering
    \vspace{-0.5em}
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &    \emc{2}{\texttt{clean}}\\
\midrule
 \t{Bounded MILP} &       \mc{2}{$\mb{5.053}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\rowcolor{tabgray}
       \t{AI$^2$} &            \mc{2}{$5.047$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
      \t{LP-Full} &            \mc{2}{$3.966$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\rowcolor{tabgray}
     \t{DeepPoly} &            \mc{2}{$3.984$} &       \mc{2}{$\mb{2.888}$} &      \mc{2}{$\tle{0.000}$} &       \mc{2}{$\mb{1.669}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
     \t{Fast-Lin} &            \mc{2}{$3.723$} &            \mc{2}{$2.596$} &            \mc{2}{$0.812$} &            \mc{2}{$1.503$} &            \mc{2}{$0.637$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\rowcolor{tabgray}
        \t{CROWN} &            \mc{2}{$3.984$} &       \mc{2}{$\mb{2.888}$} &       \mc{2}{$\mb{1.065}$} &       \mc{2}{$\mb{1.669}$} &       \mc{2}{$\mb{0.765}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
     \t{CNN-Cert} &            \mc{2}{$3.893$} &            \mc{2}{$2.819$} &      \mc{2}{$\tle{0.000}$} &            \mc{2}{$1.625$} &            \mc{2}{$0.699$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &            \mc{2}{$2.187$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
          \t{IBP} &            \mc{2}{$1.026$} &            \mc{2}{$0.011$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\rowcolor{tabgray}
           \t{WK} &            \mc{2}{$2.818$} &            \mc{2}{$1.738$} &      \mc{2}{$\tle{0.000}$} &            \mc{2}{$0.734$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
       \t{k-ReLU} &            \mc{2}{$4.203$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\rowcolor{tabgray}
   \t{RefineZono} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
    \t{SDPVerify} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\rowcolor{tabgray}
    \t{LMIVerify} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
      \t{Op-norm} &            \mc{2}{$0.183$} &            \mc{2}{$0.071$} &      \mc{2}{$\tle{0.000}$} &            \mc{2}{$0.002$} &            \mc{2}{$0.001$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\rowcolor{tabgray}
      \t{FastLip} &            \mc{2}{$2.988$} &            \mc{2}{$1.256$} &      \mc{2}{$\tle{0.000}$} &            \mc{2}{$0.599$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
     \t{RecurJac} &            \mc{2}{$3.596$} &            \mc{2}{$2.400$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\hline
\rowcolor{tabgray}
PGD Upper Bound &            \mc{2}{$5.679$} &            \mc{2}{$5.521$} &            \mc{2}{$6.037$} &            \mc{2}{$3.482$} &            \mc{2}{$2.560$} &            \mc{2}{$4.187$} &           \emc{2}{$1.819$} \\
\hline\hline
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2}\\
\midrule
 \t{Bounded MILP} &  $\mb{6.429}$ &  $\mb{9.301}$ & $\tle{0.000}$ &       $5.229$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
       \t{AI$^2$} &       $6.033$ &  $\mb{9.301}$ & $\tle{0.000}$ &       $0.185$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
      \t{LP-Full} &       $4.930$ &       $8.747$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
     \t{DeepPoly} &       $5.009$ &       $7.408$ &  $\mb{3.683}$ &       $4.720$ & $\tle{0.000}$ &       $0.173$ &  $\mb{2.601}$ &       $4.682$ & $\tle{0.000}$ &       $0.498$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
     \t{Fast-Lin} &       $4.714$ &       $7.103$ &       $3.211$ &       $4.036$ &       $0.655$ &       $3.080$ &       $2.269$ &       $4.079$ &       $1.294$ &       $2.486$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
        \t{CROWN} &       $5.009$ &       $7.408$ &  $\mb{3.683}$ &       $4.720$ &  $\mb{0.847}$ &  $\mb{4.071}$ &  $\mb{2.601}$ &       $4.682$ &  $\mb{1.551}$ &       $3.030$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
     \t{CNN-Cert} &       $4.856$ &       $7.321$ &       $3.575$ &       $4.911$ & $\tle{0.000}$ & $\tle{0.000}$ &       $2.532$ &       $4.578$ &       $1.339$ &       $2.702$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &       $2.717$ &       $7.863$ & $\tle{0.000}$ &       $5.004$ & $\tle{0.000}$ &       $3.936$ & $\tle{0.000}$ &       $5.415$ & $\tle{0.000}$ &       $3.889$ & $\tle{0.000}$ &       $3.909$ & $\tle{0.000}$ &       $3.551$ \\
          \t{IBP} &       $0.826$ &       $8.324$ &       $0.016$ &  $\mb{5.027}$ & $\tle{0.000}$ &       $3.508$ &       $0.028$ &  $\mb{5.958}$ & $\tle{0.000}$ &  $\mb{4.611}$ & $\tle{0.000}$ &  $\mb{4.411}$ & $\tle{0.000}$ &  $\mb{4.233}$ \\
\rowcolor{tabgray}
           \t{WK} &       $3.939$ &       $7.103$ &       $2.407$ &       $4.036$ & $\tle{0.000}$ &       $3.080$ &       $1.476$ &       $4.079$ &       $0.423$ &       $2.486$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
       \t{k-ReLU} &       $5.184$ &       $8.871$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
   \t{RefineZono} & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
    \t{SDPVerify} & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
    \t{LMIVerify} & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
      \t{Op-norm} &       $0.174$ &       $0.011$ &       $0.068$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ &       $0.002$ & $\tle{0.000}$ &       $0.001$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
      \t{FastLip} &       $3.696$ &       $6.319$ &       $1.359$ &       $3.399$ & $\tle{0.000}$ &       $2.404$ &       $0.742$ &       $3.523$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
     \t{RecurJac} &       $4.550$ &       $6.375$ &       $2.765$ &       $3.509$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\hline
\rowcolor{tabgray}
PGD Upper Bound &       $7.856$ &      $13.485$ &       $8.581$ &      $10.864$ &       $9.292$ &       $9.181$ &       $7.185$ &      $11.432$ &       $6.629$ &      $10.301$ &       $7.901$ &       $9.578$ &       $5.472$ &       $9.981$ \\
\hline\hline
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8}\\
\midrule
 \t{Bounded MILP} & $\mb{12.134}$ & $\mb{22.428}$ & $\tle{0.000}$ & $\mb{23.259}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ &      $18.953$ & $\tle{0.000}$ &       $1.328$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
       \t{AI$^2$} &      $10.972$ &      $22.364$ & $\tle{0.000}$ &      $13.613$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
      \t{LP-Full} &       $8.542$ &      $21.593$ & $\tle{0.000}$ &      $10.625$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
     \t{DeepPoly} &       $8.882$ &      $20.870$ &  $\mb{5.398}$ &      $15.780$ & $\tle{0.000}$ &       $6.411$ &  $\mb{5.156}$ &      $11.617$ & $\tle{0.000}$ &       $7.294$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
     \t{Fast-Lin} &       $7.825$ &      $17.946$ &       $4.637$ &      $11.422$ &       $0.881$ &       $9.259$ &       $4.471$ &       $9.171$ &       $2.396$ &       $6.469$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
        \t{CROWN} &       $8.882$ &      $20.870$ &  $\mb{5.398}$ &      $15.780$ &  $\mb{1.226}$ &      $11.615$ &  $\mb{5.156}$ &      $11.617$ &  $\mb{2.890}$ &       $8.093$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
     \t{CNN-Cert} &       $8.444$ &      $20.163$ &       $5.169$ &      $14.900$ & $\tle{0.000}$ &       $2.452$ &       $4.952$ &      $11.601$ &       $2.523$ &       $7.019$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &       $5.614$ &      $21.014$ &       $0.108$ &      $20.603$ & $\tle{0.000}$ &      $14.852$ &       $0.589$ &      $15.012$ & $\tle{0.000}$ &      $14.604$ & $\tle{0.000}$ &      $13.934$ & $\tle{0.000}$ &      $11.710$ \\
          \t{IBP} &       $1.517$ &      $22.276$ &       $0.074$ &      $22.271$ & $\tle{0.000}$ & $\mb{15.880}$ &       $0.277$ & $\mb{19.115}$ & $\tle{0.000}$ & $\mb{18.770}$ & $\tle{0.000}$ & $\mb{18.920}$ & $\tle{0.000}$ & $\mb{15.553}$ \\
\rowcolor{tabgray}
           \t{WK} &       $7.003$ &      $17.946$ &       $3.877$ &      $11.422$ & $\tle{0.000}$ &       $9.259$ &       $3.577$ &       $9.171$ &       $1.541$ &       $6.469$ & $\tle{0.000}$ &       $5.137$ & $\tle{0.000}$ & $\tle{0.000}$ \\
       \t{k-ReLU} &       $9.304$ &      $22.300$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
   \t{RefineZono} & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
    \t{SDPVerify} & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
    \t{LMIVerify} & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
      \t{Op-norm} &       $0.117$ &       $0.020$ &       $0.052$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ &       $0.002$ & $\tle{0.000}$ &       $0.001$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
      \t{FastLip} &       $6.309$ &      $18.002$ &       $1.992$ &      $10.019$ & $\tle{0.000}$ &       $8.799$ &       $2.173$ &       $8.147$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
     \t{RecurJac} &       $7.539$ &      $18.002$ &       $3.971$ &      $10.027$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\hline
\rowcolor{tabgray}
PGD Upper Bound &      $15.500$ &      $35.723$ &      $15.783$ &      $35.278$ &      $19.558$ &      $25.796$ &      $15.219$ &      $31.399$ &      $13.128$ &      $34.687$ &      $14.913$ &      $37.088$ &      $12.040$ &      $28.578$ \\
\bottomrule

    \end{tabular}
    }
    % \vspace{-1.25em}
    \vspace{5em}
    \label{tab:exp-A-cifar10-radius-robust-acc}
\end{table*}



==> tables/exp-A-cifar10-radius-time.tex <==
% This file is automatically generated by experiments/model_summary.py



\begin{table*}
    \caption{
    \emph{Average running time for robustness radius computation} in seconds per correctly-predicted instance on CIFAR-10 models of different verification approaches. The verification is on $\cL_\infty$ ball. We stop the execution when time exceeds $\SI{120}{s}$ per instance. We include running time of PGD attack as the reference.}
    \centering
    \vspace{-0.5em}
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &    \emc{2}{\texttt{clean}}\\
\midrule
 \t{Bounded MILP} &            \mc{2}{$23.76$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
\rowcolor{tabgray}
       \t{AI$^2$} &            \mc{2}{$40.75$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
      \t{LP-Full} &             \mc{2}{$8.96$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
\rowcolor{tabgray}
     \t{DeepPoly} &             \mc{2}{$0.40$} &             \mc{2}{$5.26$} &     \mc{2}{$\tle{120.00}$} &            \mc{2}{$24.44$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
     \t{Fast-Lin} &             \mc{2}{$0.05$} &             \mc{2}{$0.22$} &            \mc{2}{$12.19$} &            \mc{2}{$13.14$} &           \mc{2}{$112.11$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
\rowcolor{tabgray}
        \t{CROWN} &             \mc{2}{$0.03$} &             \mc{2}{$0.05$} &             \mc{2}{$0.43$} &             \mc{2}{$0.20$} &             \mc{2}{$2.96$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
     \t{CNN-Cert} &             \mc{2}{$0.24$} &             \mc{2}{$3.05$} &     \mc{2}{$\tle{120.00}$} &             \mc{2}{$5.03$} &           \mc{2}{$102.79$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &             \mc{2}{$0.02$} &             \mc{2}{$0.02$} &             \mc{2}{$0.04$} &             \mc{2}{$0.03$} &             \mc{2}{$0.04$} &             \mc{2}{$0.05$} &            \emc{2}{$0.06$} \\
          \t{IBP} &             \mc{2}{$0.02$} &             \mc{2}{$0.02$} &             \mc{2}{$0.04$} &             \mc{2}{$0.02$} &             \mc{2}{$0.04$} &             \mc{2}{$0.05$} &            \emc{2}{$0.08$} \\
\rowcolor{tabgray}
           \t{WK} &             \mc{2}{$0.03$} &             \mc{2}{$0.05$} &             \mc{2}{$0.25$} &             \mc{2}{$0.11$} &             \mc{2}{$0.70$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
       \t{k-ReLU} &           \mc{2}{$100.18$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
\rowcolor{tabgray}
   \t{RefineZono} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
    \t{SDPVerify} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
\rowcolor{tabgray}
    \t{LMIVerify} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
      \t{Op-norm} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.01$} &             \mc{2}{$0.01$} &             \mc{2}{$0.03$} &    \emc{2}{$\tle{120.00}$} \\
\rowcolor{tabgray}
      \t{FastLip} &             \mc{2}{$0.41$} &             \mc{2}{$1.98$} &            \mc{2}{$13.48$} &            \mc{2}{$77.41$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
     \t{RecurJac} &             \mc{2}{$5.72$} &            \mc{2}{$26.99$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
\hline
\rowcolor{tabgray}
PGD Attack &             \mc{2}{$2.54$} &             \mc{2}{$2.87$} &             \mc{2}{$3.68$} &             \mc{2}{$2.89$} &             \mc{2}{$3.48$} &             \mc{2}{$3.69$} &            \emc{2}{$4.81$} \\
\hline\hline
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2}\\
\midrule
 \t{Bounded MILP} &       $26.48$ &       $16.01$ &$\tle{120.00}$ &      $117.08$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
       \t{AI$^2$} &       $59.12$ &       $48.56$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
      \t{LP-Full} &        $8.89$ &        $8.65$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
     \t{DeepPoly} &        $0.41$ &        $0.36$ &        $5.07$ &        $3.91$ &$\tle{120.00}$ &$\tle{120.00}$ &       $22.75$ &       $11.02$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
     \t{Fast-Lin} &        $0.05$ &        $0.08$ &        $0.22$ &        $0.27$ &       $12.10$ &       $14.38$ &       $13.27$ &       $13.08$ &      $108.53$ &       $96.77$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
        \t{CROWN} &        $0.03$ &        $0.03$ &        $0.05$ &        $0.05$ &        $0.43$ &        $0.41$ &        $0.20$ &        $0.20$ &        $3.00$ &        $4.26$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
     \t{CNN-Cert} &        $0.25$ &        $0.34$ &        $3.17$ &        $2.66$ &$\tle{120.00}$ &$\tle{120.00}$ &        $5.60$ &        $5.75$ &      $113.73$ &      $116.81$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &        $0.02$ &        $0.03$ &        $0.02$ &        $0.03$ &        $0.05$ &        $0.06$ &        $0.03$ &        $0.04$ &        $0.04$ &        $0.10$ &        $0.05$ &        $0.07$ &        $0.06$ &        $0.08$ \\
          \t{IBP} &        $0.02$ &        $0.02$ &        $0.02$ &        $0.03$ &        $0.04$ &        $0.05$ &        $0.03$ &        $0.04$ &        $0.04$ &        $0.05$ &        $0.04$ &        $0.05$ &        $0.08$ &        $0.10$ \\
\rowcolor{tabgray}
           \t{WK} &        $0.03$ &        $0.04$ &        $0.05$ &        $0.07$ &        $0.25$ &        $0.28$ &        $0.11$ &        $0.13$ &        $0.79$ &        $1.35$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
       \t{k-ReLU} &       $91.47$ &       $93.79$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
   \t{RefineZono} &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
    \t{SDPVerify} &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
    \t{LMIVerify} &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
      \t{Op-norm} &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.03$ &        $0.03$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
      \t{FastLip} &        $0.42$ &        $0.40$ &        $1.88$ &        $1.74$ &       $16.78$ &       $65.67$ &       $99.47$ &       $65.69$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
     \t{RecurJac} &        $5.83$ &        $6.41$ &       $27.72$ &       $28.83$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\hline
\rowcolor{tabgray}
PGD Attack &        $2.79$ &        $3.64$ &        $3.04$ &        $3.60$ &        $4.15$ &        $4.26$ &        $3.19$ &        $4.13$ &        $3.79$ &        $4.57$ &        $4.01$ &        $4.73$ &        $5.05$ &        $6.63$ \\
\hline\hline
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8}\\
\midrule
 \t{Bounded MILP} &       $36.26$ &       $19.76$ &$\tle{120.00}$ &       $89.66$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &      $106.38$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
       \t{AI$^2$} &       $89.11$ &       $68.36$ &$\tle{120.00}$ &      $117.86$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
      \t{LP-Full} &        $9.56$ &        $8.43$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
     \t{DeepPoly} &        $0.47$ &        $0.38$ &        $5.10$ &        $2.87$ &$\tle{120.00}$ &$\tle{120.00}$ &       $18.33$ &        $9.65$ &$\tle{120.00}$ &      $119.79$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
     \t{Fast-Lin} &        $0.05$ &        $0.06$ &        $0.23$ &        $0.23$ &       $12.23$ &       $12.47$ &       $12.97$ &       $13.05$ &      $106.36$ &       $92.09$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
        \t{CROWN} &        $0.03$ &        $0.03$ &        $0.05$ &        $0.05$ &        $0.43$ &        $0.41$ &        $0.20$ &        $0.20$ &        $3.00$ &        $4.15$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
     \t{CNN-Cert} &        $0.28$ &        $0.27$ &        $3.56$ &        $3.52$ &$\tle{120.00}$ &$\tle{120.00}$ &        $6.38$ &        $6.27$ &      $112.92$ &      $118.42$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &        $0.02$ &        $0.03$ &        $0.02$ &        $0.03$ &        $0.05$ &        $0.06$ &        $0.03$ &        $0.04$ &        $0.04$ &        $0.09$ &        $0.05$ &        $0.06$ &        $0.06$ &        $0.08$ \\
          \t{IBP} &        $0.02$ &        $0.03$ &        $0.03$ &        $0.03$ &        $0.04$ &        $0.05$ &        $0.03$ &        $0.03$ &        $0.04$ &        $0.05$ &        $0.05$ &        $0.06$ &        $0.08$ &        $0.09$ \\
\rowcolor{tabgray}
           \t{WK} &        $0.03$ &        $0.04$ &        $0.05$ &        $0.07$ &        $0.24$ &        $0.27$ &        $0.10$ &        $0.13$ &        $0.74$ &        $1.19$ &$\tle{120.00}$ &        $1.61$ &$\tle{120.00}$ &$\tle{120.00}$ \\
       \t{k-ReLU} &       $96.06$ &      $101.99$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
   \t{RefineZono} &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
    \t{SDPVerify} &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
    \t{LMIVerify} &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
      \t{Op-norm} &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.03$ &        $0.03$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
      \t{FastLip} &        $0.45$ &        $0.45$ &        $2.05$ &        $1.79$ &       $17.55$ &       $86.96$ &      $102.45$ &       $70.16$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
     \t{RecurJac} &        $6.91$ &        $7.11$ &       $30.71$ &       $34.06$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\hline
\rowcolor{tabgray}
PGD Attack &        $3.41$ &        $4.58$ &        $3.80$ &        $5.17$ &        $4.95$ &        $5.52$ &        $4.04$ &        $5.66$ &        $4.48$ &        $6.73$ &        $4.58$ &        $6.66$ &        $5.67$ &        $8.05$ \\
\bottomrule

    \end{tabular}
    }
    % \vspace{-1.25em}
    \vspace{5em}
    \label{tab:exp-A-cifar10-radius-time}
\end{table*}



==> tables/exp-A-cifar10-verify-robust-acc.tex <==
% This file is automatically generated by experiments/model_summary.py



\begin{table*}
    \caption{\emph{Robust accuracy} on CIFAR-10 models certified by different \emph{deterministic verification approaches}. The verification is under $\cL_\infty$ adversary with radius $\epsilon$~(specified in table). We include accuracy under PGD attack to serve as the upper bound of robust accuracy, and the clean accuracy. 
    % \linyi{Here it is ``PGD attack'' instead of ``PGD adversarial training''! We used the correct term but someone changed it to the wrong one. Please confirm with others before changing the terms or make comments for us to check it...
    % In our submitted version we used the wrong term...}
    The \textbf{bolded} numbers mark the highest ones among verification approaches.}
    \centering
    \vspace{-0.5em}
    % \ifnum\arxiv=1
        \newcommand{\mytabwidth}{0.95}
    % \fi
    % \ifnum\arxiv=0
    %     \newcommand{\mytabwidth}{0.85}
    % \fi
    \resizebox{\mytabwidth\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
$\epsilon=0.5/255$ &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &    \emc{2}{\texttt{clean}}\\
\midrule
 \t{Bounded MILP} &             \mc{2}{$\mb{40\%}$} &             \mc{2}{$\mb{43\%}$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$23\%$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
 \rowcolor{tabgray}
          \t{AI$^2$} &             \mc{2}{$\mb{40\%}$} &             \mc{2}{$\mb{43\%}$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$\mb{51\%}$} &              \mc{2}{$9\%$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
      \t{LP-Full} &             \mc{2}{$\mb{40\%}$} &             \mc{2}{$\mb{43\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
 \rowcolor{tabgray}
     \t{DeepPoly} &             \mc{2}{$\mb{40\%}$} &             \mc{2}{$\mb{43\%}$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$\mb{51\%}$} &             \mc{2}{$\mb{52\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
     \t{Fast-Lin} &             \mc{2}{$\mb{40\%}$} &             \mc{2}{$42\%$} &             \mc{2}{$49\%$} &             \mc{2}{$\mb{51\%}$} &             \mc{2}{$49\%$} &             \mc{2}{$\mb{45\%}$} &       \emc{2}{$\tle{0\%}$} \\
 \rowcolor{tabgray}
        \t{CROWN} &             \mc{2}{$\mb{40\%}$} &             \mc{2}{$\mb{43\%}$} &             \mc{2}{$\mb{51\%}$} &             \mc{2}{$\mb{51\%}$} &             \mc{2}{$\mb{52\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
     \t{CNN-Cert} &             \mc{2}{$\mb{40\%}$} &             \mc{2}{$\mb{43\%}$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$\mb{51\%}$} &             \mc{2}{$\mb{52\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
 \rowcolor{tabgray}
    \t{CROWN-IBP} &             \mc{2}{$\mb{40\%}$} &             \mc{2}{$24\%$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$13\%$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
          \t{IBP} &             \mc{2}{$29\%$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
 \rowcolor{tabgray}
           \t{WK}  &             \mc{2}{$\mb{40\%}$} &             \mc{2}{$42\%$} &             \mc{2}{$49\%$} &             \mc{2}{$\mb{51\%}$} &             \mc{2}{$49\%$} &             \mc{2}{$\mb{45\%}$} &             \emc{2}{$\mb{3\%}$} \\
       \t{k-ReLU} &             \mc{2}{$\mb{40\%}$} &             \mc{2}{$\mb{43\%}$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$48\%$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
 \rowcolor{tabgray}
   \t{RefineZono} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
    \t{SDPVerify} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
 \rowcolor{tabgray}
    \t{LMIVerify} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
      \t{Op-norm} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
 \rowcolor{tabgray}
      \t{FastLip} &             \mc{2}{$\mb{40\%}$} &             \mc{2}{$40\%$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$36\%$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
     \t{RecurJac} &             \mc{2}{$\mb{40\%}$} &             \mc{2}{$42\%$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
\hline
  \rowcolor{tabgray}
PGD Upper Bound &             \mc{2}{$40\%$} &             \mc{2}{$43\%$} &             \mc{2}{$53\%$} &             \mc{2}{$51\%$} &             \mc{2}{$61\%$} &             \mc{2}{$49\%$} &            \emc{2}{$76\%$} \\
\hline
   Clean Acc. &             \mc{2}{$41\%$} &             \mc{2}{$47\%$} &             \mc{2}{$54\%$} &             \mc{2}{$57\%$} &             \mc{2}{$68\%$} &             \mc{2}{$54\%$} &            \emc{2}{$85\%$} \\
\hline\hline
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
$\epsilon=2/255$ & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2}\\
\midrule
 \t{Bounded MILP} &   $\mb{35\%}$ &   $\mb{33\%}$ &        $30\%$ &   $\mb{37\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\mb{47\%}$ &   $\tle{0\%}$ &        $49\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
          \t{AI$^2$} &   $\mb{35\%}$ &   $\mb{33\%}$ &   $\mb{39\%}$ &   $\mb{37\%}$ &   $\tle{0\%}$ &        $20\%$ &   $\mb{34\%}$ &   $\mb{47\%}$ &   $\mb{19\%}$ &        $45\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
      \t{LP-Full} &   $\mb{35\%}$ &   $\mb{33\%}$ &        $36\%$ &   $\mb{37\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
     \t{DeepPoly} &   $\mb{35\%}$ &   $\mb{33\%}$ &        $36\%$ &        $35\%$ &   $\tle{0\%}$ &        $17\%$ &   $\mb{34\%}$ &        $46\%$ &   $\mb{19\%}$ &        $45\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
     \t{Fast-Lin} &   $\mb{35\%}$ &   $\mb{33\%}$ &        $35\%$ &        $34\%$ &   $\tle{0\%}$ &        $30\%$ &        $33\%$ &        $45\%$ &        $14\%$ &        $43\%$ &   $\mb{13\%}$ &        $46\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
        \t{CROWN} &   $\mb{35\%}$ &   $\mb{33\%}$ &        $36\%$ &        $35\%$ &    $\mb{1\%}$ &   $\mb{32\%}$ &   $\mb{34\%}$ &        $46\%$ &   $\mb{19\%}$ &        $45\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
     \t{CNN-Cert} &   $\mb{35\%}$ &   $\mb{33\%}$ &        $35\%$ &        $35\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\mb{34\%}$ &        $46\%$ &   $\mb{19\%}$ &        $45\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
    \t{CROWN-IBP} &        $30\%$ &   $\mb{33\%}$ &   $\tle{0\%}$ &        $34\%$ &   $\tle{0\%}$ &   $\mb{32\%}$ &   $\tle{0\%}$ &        $46\%$ &   $\tle{0\%}$ &        $46\%$ &   $\tle{0\%}$ &        $50\%$ &   $\tle{0\%}$ &        $47\%$ \\
          \t{IBP} &         $6\%$ &   $\mb{33\%}$ &   $\tle{0\%}$ &        $35\%$ &   $\tle{0\%}$ &   $\mb{32\%}$ &   $\tle{0\%}$ &        $45\%$ &   $\tle{0\%}$ &   $\mb{49\%}$ &   $\tle{0\%}$ &   $\mb{51\%}$ &   $\tle{0\%}$ &   $\mb{51\%}$ \\
 \rowcolor{tabgray}
           \t{WK}  &   $\mb{35\%}$ &   $\mb{33\%}$ &        $35\%$ &        $34\%$ &   $\tle{0\%}$ &        $30\%$ &        $33\%$ &        $45\%$ &        $14\%$ &        $43\%$ &   $\mb{13\%}$ &        $46\%$ &   $\tle{0\%}$ &        $23\%$ \\
       \t{k-ReLU} &   $\mb{35\%}$ &   $\mb{33\%}$ &        $35\%$ &   $\mb{37\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &        $44\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
   \t{RefineZono} &   $\tle{0\%}$ &   $\mb{33\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
    \t{SDPVerify} &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
    \t{LMIVerify} &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
      \t{Op-norm} &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
      \t{FastLip} &        $33\%$ &        $32\%$ &        $15\%$ &        $32\%$ &   $\tle{0\%}$ &        $25\%$ &         $3\%$ &        $40\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
     \t{RecurJac} &        $34\%$ &        $32\%$ &        $33\%$ &        $32\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
\hline
 \rowcolor{tabgray}
PGD Upper Bound &        $36\%$ &        $35\%$ &        $41\%$ &        $39\%$ &        $26\%$ &        $38\%$ &        $43\%$ &        $49\%$ &        $52\%$ &        $50\%$ &        $49\%$ &        $53\%$ &        $62\%$ &        $54\%$ \\
\hline
   Clean Acc. &        $44\%$ &        $40\%$ &        $48\%$ &        $43\%$ &        $35\%$ &        $46\%$ &        $54\%$ &        $55\%$ &        $66\%$ &        $60\%$ &        $59\%$ &        $63\%$ &        $81\%$ &        $62\%$ \\
\hline\hline
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
$\epsilon=8/255$ & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8}\\
\midrule
 \t{Bounded MILP} &   $\mb{19\%}$ &   $\mb{27\%}$ &         $1\%$ &   $\mb{25\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\mb{34\%}$ &   $\tle{0\%}$ &   $\mb{36\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
          \t{AI$^2$} &   $\mb{19\%}$ &   $\mb{27\%}$ &    $\mb{7\%}$ &        $23\%$ &   $\tle{0\%}$ &        $22\%$ &    $\mb{8\%}$ &   $\mb{34\%}$ &   $\tle{0\%}$ &        $20\%$ &   $\tle{0\%}$ &        $14\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
      \t{LP-Full} &        $15\%$ &   $\mb{27\%}$ &         $6\%$ &   $\mb{25\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
     \t{DeepPoly} &        $15\%$ &   $\mb{27\%}$ &         $6\%$ &        $20\%$ &   $\tle{0\%}$ &        $22\%$ &    $\mb{8\%}$ &        $33\%$ &    $\mb{1\%}$ &        $20\%$ &   $\tle{0\%}$ &         $7\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
     \t{Fast-Lin} &        $15\%$ &        $25\%$ &         $4\%$ &        $18\%$ &   $\tle{0\%}$ &        $19\%$ &         $3\%$ &        $26\%$ &   $\tle{0\%}$ &        $15\%$ &   $\tle{0\%}$ &         $7\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
        \t{CROWN} &        $15\%$ &   $\mb{27\%}$ &         $6\%$ &        $20\%$ &   $\tle{0\%}$ &        $22\%$ &    $\mb{8\%}$ &        $33\%$ &    $\mb{1\%}$ &        $20\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
     \t{CNN-Cert} &        $15\%$ &   $\mb{27\%}$ &         $5\%$ &        $20\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &         $7\%$ &        $33\%$ &   $\tle{0\%}$ &        $20\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
    \t{CROWN-IBP} &         $9\%$ &   $\mb{27\%}$ &   $\tle{0\%}$ &        $22\%$ &   $\tle{0\%}$ &        $28\%$ &   $\tle{0\%}$ &   $\mb{34\%}$ &   $\tle{0\%}$ &        $31\%$ &   $\tle{0\%}$ &        $32\%$ &   $\tle{0\%}$ &        $25\%$ \\
          \t{IBP} &   $\tle{0\%}$ &   $\mb{27\%}$ &   $\tle{0\%}$ &   $\mb{25\%}$ &   $\tle{0\%}$ &   $\mb{30\%}$ &   $\tle{0\%}$ &   $\mb{34\%}$ &   $\tle{0\%}$ &        $35\%$ &   $\tle{0\%}$ &   $\mb{38\%}$ &   $\tle{0\%}$ &   $\mb{28\%}$ \\
 \rowcolor{tabgray}
           \t{WK}  &        $15\%$ &        $25\%$ &         $4\%$ &        $18\%$ &   $\tle{0\%}$ &        $19\%$ &         $3\%$ &        $26\%$ &   $\tle{0\%}$ &        $15\%$ &   $\tle{0\%}$ &         $7\%$ &   $\tle{0\%}$ &         $5\%$ \\
       \t{k-ReLU} &        $15\%$ &   $\mb{27\%}$ &         $2\%$ &        $23\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &        $32\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
   \t{RefineZono} &   $\tle{0\%}$ &   $\mb{27\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
    \t{SDPVerify} &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
    \t{LMIVerify} &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
      \t{Op-norm} &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
      \t{FastLip} &        $12\%$ &   $\mb{27\%}$ &   $\tle{0\%}$ &        $17\%$ &   $\tle{0\%}$ &        $17\%$ &   $\tle{0\%}$ &        $24\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
     \t{RecurJac} &        $14\%$ &   $\mb{27\%}$ &         $2\%$ &        $17\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
\hline
 \rowcolor{tabgray}
PGD Upper Bound &        $22\%$ &        $28\%$ &        $23\%$ &        $26\%$ &        $19\%$ &        $34\%$ &        $34\%$ &        $34\%$ &        $33\%$ &        $39\%$ &        $36\%$ &        $40\%$ &        $41\%$ &        $31\%$ \\
\hline
   Clean Acc. &        $33\%$ &        $31\%$ &        $37\%$ &        $30\%$ &        $26\%$ &        $39\%$ &        $44\%$ &        $46\%$ &        $53\%$ &        $48\%$ &        $52\%$ &        $46\%$ &        $66\%$ &        $46\%$ \\
\bottomrule

    \end{tabular}
    }
    \vspace{-1.25em}
    \label{tab:exp-A-cifar10-verify-robust-acc}
\end{table*}



==> tables/exp-A-cifar10-verify-time.tex <==
% This file is automatically generated by experiments/model_summary.py



\begin{table*}
    \caption{
    \emph{Average running time for single-instance robustness verification} in seconds per correctly-predicted instance on CIFAR-10 models of different verification approaches. The verification is under $\cL_\infty$ adversary with $\epsilon$~(specified in table) radius. We stop the execution when time exceeds $\SI{60}{s}$ per instance. We include running time of PGD attack and normal inference as the reference.}
    \centering
    \vspace{-0.5em}
    \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &    \emc{2}{\texttt{clean}}\\
\midrule
 \t{Bounded MILP} &             \mc{2}{$0.93$} &            \mc{2}{$10.70$} &      \mc{2}{$\tle{60.00}$} &            \mc{2}{$50.60$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
\rowcolor{tabgray}
       \t{AI$^2$} &             \mc{2}{$0.07$} &             \mc{2}{$2.09$} &      \mc{2}{$\tle{60.00}$} &             \mc{2}{$7.69$} &            \mc{2}{$57.57$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
      \t{LP-Full} &             \mc{2}{$0.71$} &            \mc{2}{$33.68$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
\rowcolor{tabgray}
     \t{DeepPoly} &             \mc{2}{$0.05$} &             \mc{2}{$0.53$} &      \mc{2}{$\tle{60.00}$} &             \mc{2}{$2.55$} &            \mc{2}{$41.52$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
     \t{Fast-Lin} &             \mc{2}{$0.03$} &             \mc{2}{$0.02$} &             \mc{2}{$1.03$} &             \mc{2}{$1.49$} &            \mc{2}{$11.07$} &            \mc{2}{$32.62$} &     \emc{2}{$\tle{60.00}$} \\
\rowcolor{tabgray}
        \t{CROWN} &             \mc{2}{$0.00$} &             \mc{2}{$0.01$} &             \mc{2}{$0.08$} &             \mc{2}{$0.03$} &             \mc{2}{$0.32$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
     \t{CNN-Cert} &             \mc{2}{$0.19$} &             \mc{2}{$0.71$} &      \mc{2}{$\tle{60.00}$} &             \mc{2}{$1.43$} &            \mc{2}{$35.36$} &            \mc{2}{$59.69$} &     \emc{2}{$\tle{60.00}$} \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.01$} &             \mc{2}{$0.01$} &             \mc{2}{$0.01$} &             \mc{2}{$0.01$} &            \emc{2}{$0.01$} \\
          \t{IBP} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.01$} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.01$} &            \emc{2}{$0.01$} \\
\rowcolor{tabgray}
           \t{WK} &             \mc{2}{$0.00$} &             \mc{2}{$0.01$} &             \mc{2}{$0.05$} &             \mc{2}{$0.01$} &             \mc{2}{$0.06$} &             \mc{2}{$0.10$} &           \emc{2}{$54.42$} \\
       \t{k-ReLU} &             \mc{2}{$5.83$} &            \mc{2}{$20.91$} &      \mc{2}{$\tle{60.00}$} &            \mc{2}{$31.63$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
\rowcolor{tabgray}
   \t{RefineZono} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
    \t{SDPVerify} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
\rowcolor{tabgray}
    \t{LMIVerify} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
      \t{Op-norm} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.01$} &             \mc{2}{$0.01$} &             \mc{2}{$0.03$} &     \emc{2}{$\tle{60.00}$} \\
\rowcolor{tabgray}
      \t{FastLip} &             \mc{2}{$0.09$} &             \mc{2}{$0.43$} &             \mc{2}{$1.35$} &            \mc{2}{$21.28$} &            \mc{2}{$49.81$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
     \t{RecurJac} &             \mc{2}{$1.56$} &             \mc{2}{$5.67$} &      \mc{2}{$\tle{60.00}$} &            \mc{2}{$57.99$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
\hline
\rowcolor{tabgray}
PGD Attack &             \mc{2}{$0.23$} &             \mc{2}{$0.27$} &             \mc{2}{$0.35$} &             \mc{2}{$0.30$} &             \mc{2}{$0.35$} &             \mc{2}{$0.39$} &            \emc{2}{$0.54$} \\
\hline
   Normal Inference &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &            \emc{2}{$0.00$} \\
\hline\hline
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2}\\
\midrule
 \t{Bounded MILP} &        $1.24$ &        $1.05$ &       $32.64$ &        $4.87$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ &        $4.70$ & $\tle{60.00}$ &       $30.27$ & $\tle{60.00}$ &       $59.55$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
       \t{AI$^2$} &        $1.99$ &        $1.06$ &        $5.16$ &        $7.01$ & $\tle{60.00}$ &       $45.69$ &       $23.65$ &        $4.81$ &       $54.19$ &       $27.01$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
      \t{LP-Full} &        $0.74$ &        $0.77$ &       $34.64$ &       $26.08$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
     \t{DeepPoly} &        $0.05$ &        $0.04$ &        $0.56$ &        $0.45$ & $\tle{60.00}$ &       $41.60$ &        $2.49$ &        $1.10$ &       $43.68$ &       $17.67$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
     \t{Fast-Lin} &        $0.01$ &        $0.03$ &        $0.02$ &        $0.05$ &        $1.36$ &        $1.36$ &        $1.48$ &        $1.45$ &       $11.77$ &       $10.92$ &       $33.87$ &       $34.73$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
        \t{CROWN} &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.07$ &        $0.04$ &        $0.03$ &        $0.03$ &        $0.33$ &        $0.47$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
     \t{CNN-Cert} &        $0.05$ &        $0.17$ &        $0.67$ &        $0.70$ &       $10.71$ &       $55.88$ &        $1.18$ &        $1.26$ &       $18.84$ &       $33.65$ &       $42.77$ &       $58.12$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ \\
          \t{IBP} &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ \\
\rowcolor{tabgray}
           \t{WK} &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.06$ &        $0.03$ &        $0.02$ &        $0.01$ &        $0.08$ &        $0.10$ &        $0.15$ &        $0.09$ & $\tle{60.00}$ &        $0.40$ \\
       \t{k-ReLU} &        $7.08$ &        $7.33$ &       $34.73$ &       $25.81$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ &       $26.78$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
   \t{RefineZono} & $\tle{60.00}$ &       $26.05$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
    \t{SDPVerify} & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
    \t{LMIVerify} & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
      \t{Op-norm} &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.03$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
      \t{FastLip} &        $0.06$ &        $0.09$ &        $0.30$ &        $0.30$ &        $1.30$ &       $11.06$ &       $11.90$ &       $11.24$ &       $37.44$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
     \t{RecurJac} &        $0.90$ &        $1.43$ &        $4.83$ &        $5.14$ & $\tle{60.00}$ & $\tle{60.00}$ &       $59.51$ &       $59.17$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\hline
\rowcolor{tabgray}
PGD Attack &        $0.24$ &        $0.27$ &        $0.28$ &        $0.30$ &        $0.37$ &        $0.40$ &        $0.30$ &        $0.37$ &        $0.36$ &        $0.45$ &        $0.37$ &        $0.46$ &        $0.55$ &        $0.64$ \\
\hline
   Normal Inference &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ \\
\hline\hline
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8}\\
\midrule
 \t{Bounded MILP} &        $3.34$ &        $0.95$ &       $59.44$ &        $3.85$ & $\tle{60.00}$ &       $58.94$ & $\tle{60.00}$ &        $4.55$ & $\tle{60.00}$ &       $27.30$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
       \t{AI$^2$} &        $3.68$ &        $1.72$ &       $47.08$ &       $10.74$ & $\tle{60.00}$ &       $36.69$ &       $49.39$ &        $4.29$ & $\tle{60.00}$ &       $37.84$ & $\tle{60.00}$ &       $57.95$ & $\tle{60.00}$ & $\tle{60.00}$ \\
      \t{LP-Full} &        $1.02$ &        $0.82$ &       $51.35$ &       $20.84$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
     \t{DeepPoly} &        $0.05$ &        $0.04$ &        $0.57$ &        $0.29$ & $\tle{60.00}$ &       $25.26$ &        $1.95$ &        $0.97$ &       $38.23$ &       $15.16$ & $\tle{60.00}$ &       $57.25$ & $\tle{60.00}$ & $\tle{60.00}$ \\
     \t{Fast-Lin} &        $0.01$ &        $0.01$ &        $0.03$ &        $0.02$ &        $1.44$ &        $1.58$ &        $1.49$ &        $1.24$ &       $11.77$ &       $10.14$ &       $38.27$ &       $34.86$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
        \t{CROWN} &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.07$ &        $0.04$ &        $0.03$ &        $0.03$ &        $0.33$ &        $0.46$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
     \t{CNN-Cert} &        $0.04$ &        $0.05$ &        $0.25$ &        $0.50$ &       $10.94$ &       $42.49$ &        $0.48$ &        $1.03$ &        $4.11$ &       $21.88$ &       $14.79$ &       $41.58$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ \\
          \t{IBP} &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ \\
\rowcolor{tabgray}
           \t{WK} &        $0.01$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.06$ &        $0.03$ &        $0.02$ &        $0.01$ &        $0.09$ &        $0.11$ &        $0.40$ &        $0.10$ & $\tle{60.00}$ &        $5.71$ \\
       \t{k-ReLU} &       $10.14$ &        $7.66$ &       $57.61$ &       $34.26$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ &       $32.65$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
   \t{RefineZono} & $\tle{60.00}$ &        $7.77$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
    \t{SDPVerify} & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
    \t{LMIVerify} & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
      \t{Op-norm} &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.03$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
      \t{FastLip} &        $0.05$ &        $0.06$ &        $0.12$ &        $0.19$ &        $1.44$ &        $9.25$ &        $8.40$ &        $8.36$ &       $28.66$ &       $59.01$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
     \t{RecurJac} &        $0.74$ &        $0.90$ &        $2.81$ &        $4.04$ &       $48.90$ &       $59.14$ &       $57.64$ &       $58.93$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\hline
\rowcolor{tabgray}
PGD Attack &        $0.23$ &        $0.27$ &        $0.27$ &        $0.32$ &        $0.38$ &        $0.39$ &        $0.29$ &        $0.37$ &        $0.38$ &        $0.43$ &        $0.39$ &        $0.47$ &        $0.55$ &        $0.65$ \\
\hline
   Normal Inference &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ \\
\bottomrule

    \end{tabular}
    }
    % \vspace{-1.25em}
    \label{tab:exp-A-cifar10-verify-time}
\end{table*}



==> tables/exp-A-mnist-radius-robust-acc.tex <==
% This file is automatically generated by experiments/model_summary.py



\begin{table*}
    \caption{
    \emph{Average certified robustness radius} on MNIST models certified by different \emph{deterministic verification approaches}. The verification is under $\cL_\infty$ adversary. 
    We include radius of adversarial example found by PGD attack to serve as the upper bound.
    The \textbf{bolded} numbers mark the highest ones among verification approaches.
    }
    \centering
    \vspace{-0.5em}
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &    \emc{2}{\texttt{clean}}\\
\midrule
 \t{Bounded MILP} &       \mc{2}{$\mb{0.054}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\rowcolor{tabgray}
       \t{AI$^2$} &       \mc{2}{$\mb{0.054}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
      \t{LP-Full} &            \mc{2}{$0.027$} &            \mc{2}{$0.019$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\rowcolor{tabgray}
     \t{DeepPoly} &            \mc{2}{$0.045$} &       \mc{2}{$\mb{0.035}$} &      \mc{2}{$\tle{0.000}$} &       \mc{2}{$\mb{0.039}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
     \t{Fast-Lin} &            \mc{2}{$0.026$} &            \mc{2}{$0.018$} &      \mc{2}{$\tle{0.000}$} &            \mc{2}{$0.021$} &            \mc{2}{$0.014$} &       \mc{2}{$\mb{0.009}$} &     \emc{2}{$\tle{0.000}$} \\
\rowcolor{tabgray}
        \t{CROWN} &            \mc{2}{$0.045$} &       \mc{2}{$\mb{0.035}$} &       \mc{2}{$\mb{0.005}$} &       \mc{2}{$\mb{0.039}$} &       \mc{2}{$\mb{0.030}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
     \t{CNN-Cert} &            \mc{2}{$0.027$} &            \mc{2}{$0.020$} &      \mc{2}{$\tle{0.000}$} &            \mc{2}{$0.022$} &            \mc{2}{$0.015$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &            \mc{2}{$0.033$} &            \mc{2}{$0.006$} &      \mc{2}{$\tle{0.000}$} &            \mc{2}{$0.011$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
          \t{IBP} &            \mc{2}{$0.006$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\rowcolor{tabgray}
           \t{WK} &            \mc{2}{$0.026$} &            \mc{2}{$0.018$} &      \mc{2}{$\tle{0.000}$} &            \mc{2}{$0.021$} &            \mc{2}{$0.014$} &       \mc{2}{$\mb{0.009}$} &     \emc{2}{$\tle{0.000}$} \\
       \t{k-ReLU} &            \mc{2}{$0.046$} &            \mc{2}{$0.001$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\rowcolor{tabgray}
   \t{RefineZono} &            \mc{2}{$0.045$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
    \t{SDPVerify} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\rowcolor{tabgray}
    \t{LMIVerify} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
      \t{Op-norm} &            \mc{2}{$0.003$} &            \mc{2}{$0.001$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\rowcolor{tabgray}
      \t{FastLip} &            \mc{2}{$0.020$} &            \mc{2}{$0.008$} &      \mc{2}{$\tle{0.000}$} &            \mc{2}{$0.009$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
     \t{RecurJac} &            \mc{2}{$0.030$} &            \mc{2}{$0.021$} &      \mc{2}{$\tle{0.000}$} &            \mc{2}{$0.009$} &      \mc{2}{$\tle{0.000}$} &      \mc{2}{$\tle{0.000}$} &     \emc{2}{$\tle{0.000}$} \\
\hline
\rowcolor{tabgray}
PGD Upper Bound &            \mc{2}{$0.057$} &            \mc{2}{$0.060$} &            \mc{2}{$0.046$} &            \mc{2}{$0.073$} &            \mc{2}{$0.087$} &            \mc{2}{$0.090$} &           \emc{2}{$0.103$} \\
\hline\hline
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1}\\
\midrule
 \t{Bounded MILP} &  $\mb{0.135}$ &  $\mb{0.131}$ & $\tle{0.000}$ &  $\mb{0.150}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ &       $0.122$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
          \t{AI$^2$} &  $\mb{0.135}$ &  $\mb{0.131}$ & $\tle{0.000}$ &  $\mb{0.150}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
      \t{LP-Full} &       $0.063$ &       $0.097$ &       $0.040$ &       $0.102$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
     \t{DeepPoly} &       $0.095$ &       $0.120$ &  $\mb{0.064}$ &       $0.118$ & $\tle{0.000}$ &       $0.096$ &  $\mb{0.086}$ &       $0.152$ &       $0.008$ &       $0.160$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
     \t{Fast-Lin} &       $0.060$ &       $0.083$ &       $0.036$ &       $0.080$ &       $0.007$ &       $0.056$ &       $0.061$ &       $0.142$ &       $0.051$ &       $0.149$ &  $\mb{0.041}$ &       $0.138$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
        \t{CROWN} &       $0.095$ &       $0.120$ &  $\mb{0.064}$ &       $0.118$ &  $\mb{0.019}$ &       $0.096$ &  $\mb{0.086}$ &       $0.152$ &  $\mb{0.075}$ &       $0.168$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
     \t{CNN-Cert} &       $0.062$ &       $0.084$ &       $0.039$ &       $0.085$ & $\tle{0.000}$ & $\tle{0.000}$ &       $0.066$ &       $0.150$ &       $0.056$ &       $0.161$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &       $0.055$ &       $0.123$ &       $0.009$ &       $0.135$ & $\tle{0.000}$ &       $0.133$ &       $0.030$ &  $\mb{0.154}$ &       $0.001$ &  $\mb{0.176}$ & $\tle{0.000}$ &  $\mb{0.179}$ & $\tle{0.000}$ &  $\mb{0.174}$ \\
          \t{IBP} &       $0.011$ &       $0.128$ & $\tle{0.000}$ &       $0.142$ & $\tle{0.000}$ &  $\mb{0.143}$ &       $0.005$ &  $\mb{0.154}$ & $\tle{0.000}$ &       $0.174$ & $\tle{0.000}$ &       $0.175$ & $\tle{0.000}$ &       $0.168$ \\
\rowcolor{tabgray}
           \t{WK} &       $0.060$ &       $0.083$ &       $0.036$ &       $0.080$ &       $0.007$ &       $0.056$ &       $0.061$ &       $0.142$ &       $0.051$ &       $0.149$ &  $\mb{0.041}$ &       $0.139$ & $\tle{0.000}$ & $\tle{0.000}$ \\
       \t{k-ReLU} &       $0.100$ &       $0.129$ &       $0.014$ &       $0.097$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
   \t{RefineZono} &       $0.097$ &       $0.120$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
    \t{SDPVerify} & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
    \t{LMIVerify} & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
      \t{Op-norm} &       $0.002$ &       $0.002$ &       $0.001$ &       $0.002$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
      \t{FastLip} &       $0.041$ &       $0.078$ &       $0.016$ &       $0.074$ & $\tle{0.000}$ &       $0.052$ &       $0.032$ &       $0.131$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
     \t{RecurJac} &       $0.060$ &       $0.081$ &       $0.035$ &       $0.078$ & $\tle{0.000}$ & $\tle{0.000}$ &       $0.032$ &       $0.107$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\hline
\rowcolor{tabgray}
PGD Upper Bound &       $0.145$ &       $0.157$ &       $0.155$ &       $0.190$ &       $0.151$ &       $0.213$ &       $0.163$ &       $0.194$ &       $0.168$ &       $0.233$ &       $0.169$ &       $0.278$ &       $0.181$ &       $0.320$ \\
\hline\hline
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3}\\
\midrule
 \t{Bounded MILP} &  $\mb{0.157}$ &  $\mb{0.256}$ & $\tle{0.000}$ &  $\mb{0.278}$ & $\tle{0.000}$ &       $0.230$ & $\tle{0.000}$ &       $0.255$ & $\tle{0.000}$ &       $0.233$ & $\tle{0.000}$ &       $0.018$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
          \t{AI$^2$} &  $\mb{0.157}$ &  $\mb{0.256}$ & $\tle{0.000}$ &  $\mb{0.278}$ & $\tle{0.000}$ &       $0.232$ & $\tle{0.000}$ &       $0.240$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
      \t{LP-Full} &       $0.079$ &       $0.229$ &       $0.049$ &       $0.217$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
     \t{DeepPoly} &       $0.119$ &       $0.239$ &  $\mb{0.076}$ &       $0.224$ & $\tle{0.000}$ &       $0.228$ &  $\mb{0.174}$ &       $0.254$ &       $0.105$ &       $0.188$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
     \t{Fast-Lin} &       $0.074$ &       $0.202$ &       $0.043$ &       $0.151$ &       $0.008$ &       $0.033$ &       $0.117$ &       $0.221$ &       $0.106$ &       $0.174$ &       $0.083$ &       $0.143$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
        \t{CROWN} &       $0.119$ &       $0.239$ &  $\mb{0.076}$ &       $0.224$ &  $\mb{0.021}$ &       $0.228$ &  $\mb{0.174}$ &       $0.254$ &  $\mb{0.141}$ &       $0.204$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
     \t{CNN-Cert} &       $0.078$ &       $0.210$ &       $0.048$ &       $0.189$ & $\tle{0.000}$ & $\tle{0.000}$ &       $0.130$ &       $0.253$ &       $0.120$ &       $0.179$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &       $0.069$ &       $0.239$ &       $0.005$ &       $0.256$ & $\tle{0.000}$ &       $0.288$ &       $0.074$ &       $0.283$ & $\tle{0.000}$ &       $0.272$ & $\tle{0.000}$ &       $0.277$ & $\tle{0.000}$ &       $0.272$ \\
          \t{IBP} &       $0.008$ &  $\mb{0.256}$ & $\tle{0.000}$ &       $0.275$ & $\tle{0.000}$ &  $\mb{0.295}$ &       $0.018$ &  $\mb{0.294}$ & $\tle{0.000}$ &  $\mb{0.296}$ & $\tle{0.000}$ &  $\mb{0.292}$ & $\tle{0.000}$ &  $\mb{0.299}$ \\
\rowcolor{tabgray}
           \t{WK} &       $0.074$ &       $0.202$ &       $0.043$ &       $0.151$ &       $0.008$ &       $0.033$ &       $0.117$ &       $0.221$ &       $0.106$ &       $0.174$ &  $\mb{0.085}$ &       $0.143$ & $\tle{0.000}$ & $\tle{0.000}$ \\
       \t{k-ReLU} &       $0.125$ &  $\mb{0.256}$ &       $0.002$ &       $0.209$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ &       $0.227$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
   \t{RefineZono} &       $0.120$ &       $0.237$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
    \t{SDPVerify} & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
    \t{LMIVerify} & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
      \t{Op-norm} &       $0.001$ & $\tle{0.000}$ & $\tle{0.000}$ &       $0.001$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\rowcolor{tabgray}
      \t{FastLip} &       $0.053$ &       $0.189$ &       $0.015$ &       $0.153$ & $\tle{0.000}$ &       $0.043$ &       $0.067$ &       $0.199$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
     \t{RecurJac} &       $0.072$ &       $0.193$ &       $0.039$ &       $0.157$ & $\tle{0.000}$ & $\tle{0.000}$ &       $0.058$ &       $0.146$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ & $\tle{0.000}$ \\
\hline
\rowcolor{tabgray}
PGD Upper Bound &       $0.199$ &       $0.309$ &       $0.216$ &       $0.331$ &       $0.231$ &       $0.427$ &       $0.308$ &       $0.302$ &       $0.313$ &       $0.318$ &       $0.328$ &       $0.316$ &       $0.366$ &       $0.325$ \\
\bottomrule

    \end{tabular}
    }
    % \vspace{-1.25em}
    % \vspace{5em}
    \label{tab:exp-A-mnist-radius-robust-acc}
\end{table*}



==> tables/exp-A-mnist-radius-time.tex <==
% This file is automatically generated by experiments/model_summary.py



\begin{table*}
    \caption{\emph{Average running time for robustness radius computation} in seconds per correctly-predicted instance on MNIST models of different verification approaches. The verification is on $\cL_\infty$ ball. We stop the execution when time exceeds $\SI{120}{s}$ per instance. We include running time of PGD attack as the reference.}
    \centering
    \vspace{-0.5em}
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &    \emc{2}{\texttt{clean}}\\
\midrule
 \t{Bounded MILP} &             \mc{2}{$3.14$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
\rowcolor{tabgray}
       \t{AI$^2$} &             \mc{2}{$3.95$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
      \t{LP-Full} &             \mc{2}{$2.63$} &           \mc{2}{$113.84$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
\rowcolor{tabgray}
     \t{DeepPoly} &             \mc{2}{$0.17$} &             \mc{2}{$1.50$} &     \mc{2}{$\tle{120.00}$} &            \mc{2}{$13.42$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
     \t{Fast-Lin} &             \mc{2}{$0.04$} &             \mc{2}{$0.17$} &            \mc{2}{$12.30$} &             \mc{2}{$2.04$} &            \mc{2}{$32.25$} &           \mc{2}{$103.94$} &    \emc{2}{$\tle{120.00}$} \\
\rowcolor{tabgray}
        \t{CROWN} &             \mc{2}{$0.03$} &             \mc{2}{$0.05$} &             \mc{2}{$0.17$} &             \mc{2}{$0.09$} &             \mc{2}{$0.80$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
     \t{CNN-Cert} &             \mc{2}{$0.11$} &             \mc{2}{$1.19$} &     \mc{2}{$\tle{120.00}$} &             \mc{2}{$3.23$} &            \mc{2}{$75.62$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &             \mc{2}{$0.03$} &             \mc{2}{$0.03$} &             \mc{2}{$0.07$} &             \mc{2}{$0.04$} &             \mc{2}{$0.06$} &             \mc{2}{$0.08$} &            \emc{2}{$0.08$} \\
          \t{IBP} &             \mc{2}{$0.02$} &             \mc{2}{$0.02$} &             \mc{2}{$0.03$} &             \mc{2}{$0.02$} &             \mc{2}{$0.03$} &             \mc{2}{$0.04$} &            \emc{2}{$0.05$} \\
\rowcolor{tabgray}
           \t{WK} &             \mc{2}{$0.04$} &             \mc{2}{$0.06$} &             \mc{2}{$0.22$} &             \mc{2}{$0.08$} &             \mc{2}{$0.32$} &             \mc{2}{$1.06$} &    \emc{2}{$\tle{120.00}$} \\
       \t{k-ReLU} &            \mc{2}{$70.72$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
\rowcolor{tabgray}
   \t{RefineZono} &            \mc{2}{$32.98$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
    \t{SDPVerify} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
\rowcolor{tabgray}
    \t{LMIVerify} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
      \t{Op-norm} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.01$} &    \emc{2}{$\tle{120.00}$} \\
\rowcolor{tabgray}
      \t{FastLip} &             \mc{2}{$0.15$} &             \mc{2}{$0.57$} &             \mc{2}{$9.95$} &            \mc{2}{$19.23$} &           \mc{2}{$111.50$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
     \t{RecurJac} &             \mc{2}{$6.81$} &            \mc{2}{$29.75$} &     \mc{2}{$\tle{120.00}$} &           \mc{2}{$114.36$} &     \mc{2}{$\tle{120.00}$} &     \mc{2}{$\tle{120.00}$} &    \emc{2}{$\tle{120.00}$} \\
\hline
\rowcolor{tabgray}
PGD Attack &             \mc{2}{$1.61$} &             \mc{2}{$1.81$} &             \mc{2}{$2.59$} &             \mc{2}{$2.03$} &             \mc{2}{$2.68$} &             \mc{2}{$2.85$} &            \emc{2}{$3.13$} \\
\hline\hline
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1}\\
\midrule
 \t{Bounded MILP} &        $4.97$ &        $2.39$ &$\tle{120.00}$ &       $14.06$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &      $118.88$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
       \t{AI$^2$} &        $5.28$ &        $6.44$ &$\tle{120.00}$ &       $39.72$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
      \t{LP-Full} &        $2.77$ &        $2.33$ &      $107.16$ &       $73.58$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
     \t{DeepPoly} &        $0.16$ &        $0.12$ &        $1.50$ &        $0.99$ &$\tle{120.00}$ &       $65.62$ &        $9.55$ &        $8.65$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
     \t{Fast-Lin} &        $0.03$ &        $0.04$ &        $0.16$ &        $0.17$ &       $11.18$ &        $9.15$ &        $2.11$ &        $2.62$ &       $32.73$ &       $28.51$ &       $96.23$ &      $119.36$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
        \t{CROWN} &        $0.03$ &        $0.03$ &        $0.05$ &        $0.05$ &        $0.17$ &        $0.18$ &        $0.09$ &        $0.09$ &        $0.80$ &        $0.80$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
     \t{CNN-Cert} &        $0.16$ &        $0.16$ &        $1.48$ &        $1.70$ &$\tle{120.00}$ &$\tle{120.00}$ &        $4.09$ &        $4.69$ &       $94.97$ &      $115.68$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &        $0.03$ &        $0.03$ &        $0.03$ &        $0.03$ &        $0.10$ &        $0.07$ &        $0.04$ &        $0.04$ &        $0.06$ &        $0.07$ &        $0.08$ &        $0.08$ &        $0.08$ &        $0.08$ \\
          \t{IBP} &        $0.02$ &        $0.02$ &        $0.02$ &        $0.03$ &        $0.03$ &        $0.04$ &        $0.02$ &        $0.03$ &        $0.03$ &        $0.04$ &        $0.04$ &        $0.05$ &        $0.05$ &        $0.06$ \\
\rowcolor{tabgray}
           \t{WK} &        $0.04$ &        $0.04$ &        $0.06$ &        $0.06$ &        $0.21$ &        $0.20$ &        $0.08$ &        $0.08$ &        $0.33$ &        $0.23$ &        $1.03$ &        $0.77$ &$\tle{120.00}$ &$\tle{120.00}$ \\
       \t{k-ReLU} &       $65.10$ &       $69.00$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
   \t{RefineZono} &       $56.38$ &      $100.87$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
    \t{SDPVerify} &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
    \t{LMIVerify} &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
      \t{Op-norm} &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
      \t{FastLip} &        $0.16$ &        $0.16$ &        $0.67$ &        $0.69$ &        $8.59$ &       $46.72$ &       $20.61$ &       $25.84$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
     \t{RecurJac} &        $5.87$ &        $5.62$ &       $29.77$ &       $28.10$ &$\tle{120.00}$ &$\tle{120.00}$ &      $119.21$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\hline
\rowcolor{tabgray}
PGD Attack &        $1.70$ &        $2.04$ &        $1.91$ &        $2.25$ &        $2.67$ &        $2.96$ &        $2.11$ &        $2.33$ &        $2.74$ &        $2.97$ &        $2.85$ &        $3.21$ &        $3.16$ &        $3.40$ \\
\hline\hline
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3}\\
\midrule
 \t{Bounded MILP} &        $4.75$ &        $2.53$ &$\tle{120.00}$ &        $7.77$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &      $116.93$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
       \t{AI$^2$} &        $4.96$ &        $3.74$ &$\tle{120.00}$ &       $12.73$ &$\tle{120.00}$ &      $117.14$ &$\tle{120.00}$ &      $118.62$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
      \t{LP-Full} &        $2.51$ &        $2.39$ &      $104.91$ &       $63.49$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
     \t{DeepPoly} &        $0.16$ &        $0.13$ &        $1.76$ &        $0.94$ &$\tle{120.00}$ &       $32.34$ &       $10.85$ &        $8.12$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
     \t{Fast-Lin} &        $0.03$ &        $0.04$ &        $0.17$ &        $0.15$ &       $11.21$ &        $8.92$ &        $1.78$ &        $2.40$ &       $29.16$ &       $28.74$ &      $115.24$ &      $106.29$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
        \t{CROWN} &        $0.03$ &        $0.03$ &        $0.05$ &        $0.05$ &        $0.17$ &        $0.18$ &        $0.09$ &        $0.09$ &        $0.80$ &        $0.80$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
     \t{CNN-Cert} &        $0.16$ &        $0.16$ &        $1.41$ &        $1.95$ &$\tle{120.00}$ &$\tle{120.00}$ &        $4.71$ &        $5.14$ &      $112.83$ &      $117.19$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &        $0.03$ &        $0.03$ &        $0.03$ &        $0.03$ &        $0.07$ &        $0.08$ &        $0.04$ &        $0.04$ &        $0.10$ &        $0.07$ &        $0.08$ &        $0.08$ &        $0.08$ &        $0.08$ \\
          \t{IBP} &        $0.02$ &        $0.02$ &        $0.02$ &        $0.03$ &        $0.03$ &        $0.04$ &        $0.02$ &        $0.03$ &        $0.03$ &        $0.04$ &        $0.04$ &        $0.05$ &        $0.05$ &        $0.06$ \\
\rowcolor{tabgray}
           \t{WK} &        $0.04$ &        $0.04$ &        $0.06$ &        $0.06$ &        $0.21$ &        $0.18$ &        $0.07$ &        $0.08$ &        $0.18$ &        $0.21$ &        $0.57$ &        $0.78$ &$\tle{120.00}$ &$\tle{120.00}$ \\
       \t{k-ReLU} &       $64.68$ &       $63.76$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
   \t{RefineZono} &       $79.13$ &       $21.92$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
    \t{SDPVerify} &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
    \t{LMIVerify} &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
      \t{Op-norm} &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.00$ &        $0.01$ &        $0.01$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\rowcolor{tabgray}
      \t{FastLip} &        $0.16$ &        $0.19$ &        $0.62$ &        $0.74$ &        $9.15$ &       $38.31$ &       $31.29$ &       $25.23$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
     \t{RecurJac} &        $5.37$ &        $5.92$ &       $29.40$ &       $30.22$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ &$\tle{120.00}$ \\
\hline
\rowcolor{tabgray}
PGD Attack &        $1.81$ &        $2.38$ &        $2.00$ &        $2.23$ &        $2.79$ &        $3.08$ &        $2.10$ &        $2.24$ &        $2.71$ &        $2.82$ &        $2.92$ &        $3.10$ &        $3.25$ &        $3.32$ \\
\bottomrule

    \end{tabular}
    }
    \vspace{5em}
    % \vspace{-1.25em}
    \label{tab:exp-A-mnist-radius-time}
\end{table*}



==> tables/exp-A-mnist-verify-robust-acc.tex <==
% This file is automatically generated by experiments/model_summary.py



\begin{table*}
    \caption{
    \emph{Robust accuracy} on MNIST models certified by different \emph{deterministic verification approaches}. The verification is under $\cL_\infty$ adversary with radius $\epsilon$~(specified in table). We include accuracy under PGD attack to serve as the upper bound of robust accuracy, and the clean accuracy. 
    The \textbf{bolded} numbers mark the highest ones among verification approaches.
    }
    \centering
    \vspace{-0.5em}
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
$\epsilon=0.02$ &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &    \emc{2}{\texttt{clean}}\\
\midrule
 \t{Bounded MILP} &             \mc{2}{$\mb{80\%}$} &             \mc{2}{$84\%$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$44\%$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
 \rowcolor{tabgray}
       \t{AI$^2$} &             \mc{2}{$\mb{80\%}$} &             \mc{2}{$\mb{86\%}$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$\mb{89\%}$} &            \mc{2}{$\mb{90\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
      \t{LP-Full} &             \mc{2}{$70\%$} &             \mc{2}{$68\%$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
 \rowcolor{tabgray}
     \t{DeepPoly} &             \mc{2}{$79\%$} &             \mc{2}{$85\%$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$\mb{89\%}$} &             \mc{2}{$\mb{90\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
     \t{Fast-Lin} &             \mc{2}{$68\%$} &             \mc{2}{$56\%$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$72\%$} &             \mc{2}{$28\%$} &              \mc{2}{$\mb{5\%}$} &       \emc{2}{$\tle{0\%}$} \\
 \rowcolor{tabgray}
        \t{CROWN} &             \mc{2}{$79\%$} &             \mc{2}{$85\%$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$\mb{89\%}$} &             \mc{2}{$\mb{90\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
     \t{CNN-Cert} &             \mc{2}{$70\%$} &             \mc{2}{$67\%$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$73\%$} &             \mc{2}{$44\%$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
 \rowcolor{tabgray}
    \t{CROWN-IBP} &             \mc{2}{$77\%$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$13\%$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
          \t{IBP} &              \mc{2}{$3\%$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
 \rowcolor{tabgray}
           \t{WK} &             \mc{2}{$68\%$} &             \mc{2}{$56\%$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$72\%$} &             \mc{2}{$28\%$} &              \mc{2}{$\mb{5\%}$} &       \emc{2}{$\tle{0\%}$} \\
       \t{k-ReLU} &             \mc{2}{$79\%$} &             \mc{2}{$85\%$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$\mb{89\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
 \rowcolor{tabgray}
   \t{RefineZono} &             \mc{2}{$79\%$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
    \t{SDPVerify} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
 \rowcolor{tabgray}
    \t{LMIVerify} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
      \t{Op-norm} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
 \rowcolor{tabgray}
      \t{FastLip} &             \mc{2}{$60\%$} &              \mc{2}{$4\%$} &        \mc{2}{$\tle{0\%}$} &              \mc{2}{$6\%$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
     \t{RecurJac} &             \mc{2}{$70\%$} &             \mc{2}{$52\%$} &        \mc{2}{$\tle{0\%}$} &             \mc{2}{$33\%$} &        \mc{2}{$\tle{0\%}$} &        \mc{2}{$\tle{0\%}$} &       \emc{2}{$\tle{0\%}$} \\
\hline
 \rowcolor{tabgray}
PGD Upper Bound &             \mc{2}{$80\%$} &             \mc{2}{$86\%$} &             \mc{2}{$85\%$} &             \mc{2}{$92\%$} &             \mc{2}{$95\%$} &             \mc{2}{$93\%$} &            \emc{2}{$97\%$} \\
\hline
   Clean Acc. &             \mc{2}{$89\%$} &             \mc{2}{$92\%$} &             \mc{2}{$95\%$} &             \mc{2}{$99\%$} &            \mc{2}{$100\%$} &            \mc{2}{$100\%$} &           \emc{2}{$100\%$} \\
\hline\hline
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
$\epsilon=0.1$ & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1}\\
\midrule
 \t{Bounded MILP} &     $\mb{70\%}$ & $\mb{68\%}$ &   $\tle{0\%}$ &   $\mb{85\%}$ &   $\tle{0\%}$ &        $67\%$ &   $\tle{0\%}$ &   $\mb{95\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
       \t{AI$^2$} &     $\mb{70\%}$ & $\mb{68\%}$ &         $1\%$ &   $\mb{85\%}$ &   $\tle{0\%}$ &        $52\%$ &         $6\%$ &   $\mb{95\%}$ &         $1\%$ &        $93\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
      \t{LP-Full} &         $8\%$ &        $46\%$ &   $\tle{0\%}$ &        $57\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
     \t{DeepPoly} &        $47\%$ &        $64\%$ &    $\mb{4\%}$ &        $72\%$ &   $\tle{0\%}$ &        $52\%$ &   $\mb{32\%}$ &        $93\%$ &    $\mb{2\%}$ &        $93\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
     \t{Fast-Lin} &         $5\%$ &        $35\%$ &   $\tle{0\%}$ &        $36\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &        $90\%$ &   $\tle{0\%}$ &        $89\%$ &   $\tle{0\%}$ &        $86\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
        \t{CROWN} &        $47\%$ &        $64\%$ &    $\mb{4\%}$ &        $72\%$ &   $\tle{0\%}$ &        $52\%$ &   $\mb{32\%}$ &        $93\%$ &    $\mb{2\%}$ &        $93\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
     \t{CNN-Cert} &         $5\%$ &        $36\%$ &   $\tle{0\%}$ &        $44\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &        $92\%$ &   $\tle{0\%}$ &        $93\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
    \t{CROWN-IBP} &         $2\%$ &        $67\%$ &   $\tle{0\%}$ &        $76\%$ &   $\tle{0\%}$ &        $73\%$ &   $\tle{0\%}$ &        $93\%$ &   $\tle{0\%}$ &   $\mb{94\%}$ &   $\tle{0\%}$ &        $88\%$ &   $\tle{0\%}$ &   $\mb{94\%}$ \\
          \t{IBP} &   $\tle{0\%}$ &   $\mb{68\%}$ &   $\tle{0\%}$ &   $\mb{85\%}$ &   $\tle{0\%}$ &   $\mb{80\%}$ &   $\tle{0\%}$ &   $\mb{95\%}$ &   $\tle{0\%}$ &        $91\%$ &   $\tle{0\%}$ &   $\mb{89\%}$ &   $\tle{0\%}$ &        $90\%$ \\
 \rowcolor{tabgray}
           \t{WK} &         $5\%$ &        $35\%$ &   $\tle{0\%}$ &        $36\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &        $90\%$ &   $\tle{0\%}$ &        $89\%$ &   $\tle{0\%}$ &        $86\%$ &   $\tle{0\%}$ &         $1\%$ \\
       \t{k-ReLU} &        $51\%$ &   $\mb{68\%}$ &    $\mb{4\%}$ &   $\mb{85\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &         $3\%$ &   $\mb{95\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
   \t{RefineZono} &        $49\%$ &        $63\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
    \t{SDPVerify} &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
    \t{LMIVerify} &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
      \t{Op-norm} &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
      \t{FastLip} &   $\tle{0\%}$ &        $30\%$ &   $\tle{0\%}$ &        $31\%$ &   $\tle{0\%}$ &         $2\%$ &   $\tle{0\%}$ &        $86\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
     \t{RecurJac} &         $2\%$ &        $30\%$ &   $\tle{0\%}$ &        $31\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &        $85\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
\hline
 \rowcolor{tabgray}
PGD Upper Bound &        $71\%$ &        $69\%$ &        $80\%$ &        $85\%$ &        $82\%$ &        $89\%$ &        $94\%$ &        $95\%$ &        $95\%$ &        $97\%$ &        $95\%$ &        $96\%$ &        $97\%$ &        $99\%$ \\
\hline
   Clean Acc. &        $92\%$ &        $88\%$ &        $97\%$ &        $97\%$ &        $98\%$ &        $96\%$ &       $100\%$ &        $99\%$ &       $100\%$ &        $99\%$ &       $100\%$ &       $100\%$ &       $100\%$ &       $100\%$ \\
\hline\hline
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
$\epsilon=0.3$ & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3}\\
\midrule
 \t{Bounded MILP} &         $6\%$ &   $\mb{25\%}$ &   $\tle{0\%}$ &   $\mb{54\%}$ &   $\tle{0\%}$ &         $7\%$ &   $\tle{0\%}$ &   $\mb{88\%}$ &   $\tle{0\%}$ &        $84\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
       \t{AI$^2$} &         $6\%$ &   $\mb{25\%}$ &   $\tle{0\%}$ &   $\mb{54\%}$ &   $\tle{0\%}$ &        $16\%$ &   $\tle{0\%}$ &        $73\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
      \t{LP-Full} &   $\tle{0\%}$ &        $15\%$ &   $\tle{0\%}$ &         $8\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
     \t{DeepPoly} &   $\tle{0\%}$ &        $23\%$ &   $\tle{0\%}$ &        $27\%$ &   $\tle{0\%}$ &        $16\%$ &   $\tle{0\%}$ &        $40\%$ &   $\tle{0\%}$ &         $7\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
     \t{Fast-Lin} &   $\tle{0\%}$ &         $4\%$ &   $\tle{0\%}$ &         $1\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &         $6\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
        \t{CROWN} &   $\tle{0\%}$ &        $23\%$ &   $\tle{0\%}$ &        $27\%$ &   $\tle{0\%}$ &        $16\%$ &   $\tle{0\%}$ &        $40\%$ &   $\tle{0\%}$ &         $7\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
     \t{CNN-Cert} &   $\tle{0\%}$ &        $13\%$ &   $\tle{0\%}$ &         $5\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &        $39\%$ &   $\tle{0\%}$ &         $1\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
    \t{CROWN-IBP} &   $\tle{0\%}$ &        $23\%$ &   $\tle{0\%}$ &        $45\%$ &   $\tle{0\%}$ &        $20\%$ &   $\tle{0\%}$ &        $76\%$ &   $\tle{0\%}$ &        $71\%$ &   $\tle{0\%}$ &        $75\%$ &   $\tle{0\%}$ &        $65\%$ \\
          \t{IBP} &   $\tle{0\%}$ &   $\mb{25\%}$ &   $\tle{0\%}$ &   $\mb{54\%}$ &   $\tle{0\%}$ &   $\mb{22\%}$ &   $\tle{0\%}$ &   $\mb{88\%}$ &   $\tle{0\%}$ &   $\mb{85\%}$ &   $\tle{0\%}$ &   $\mb{87\%}$ &   $\tle{0\%}$ &   $\mb{89\%}$ \\
 \rowcolor{tabgray}
           \t{WK} &   $\tle{0\%}$ &         $4\%$ &   $\tle{0\%}$ &         $1\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &         $6\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
       \t{k-ReLU} &   $\tle{0\%}$ &   $\mb{25\%}$ &   $\tle{0\%}$ &   $\mb{54\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &        $57\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
   \t{RefineZono} &   $\tle{0\%}$ &        $21\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
    \t{SDPVerify} &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
    \t{LMIVerify} &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
      \t{Op-norm} &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
 \rowcolor{tabgray}
      \t{FastLip} &   $\tle{0\%}$ &         $1\%$ &   $\tle{0\%}$ &         $2\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &         $2\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
     \t{RecurJac} &   $\tle{0\%}$ &         $1\%$ &   $\tle{0\%}$ &         $2\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &         $2\%$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ &   $\tle{0\%}$ \\
\hline
 \rowcolor{tabgray}
PGD Upper Bound &        $19\%$ &        $26\%$ &        $26\%$ &        $64\%$ &        $26\%$ &        $26\%$ &        $81\%$ &        $90\%$ &        $91\%$ &        $94\%$ &        $90\%$ &        $93\%$ &        $92\%$ &        $94\%$ \\
\hline
   Clean Acc. &        $75\%$ &        $37\%$ &        $88\%$ &        $76\%$ &        $78\%$ &        $28\%$ &        $97\%$ &        $95\%$ &       $100\%$ &        $98\%$ &        $99\%$ &        $98\%$ &       $100\%$ &        $98\%$ \\
\bottomrule

    \end{tabular}
    }
    \vspace{-1.25em}
    \label{tab:exp-A-mnist-verify-robust-acc}
\end{table*}



==> tables/exp-A-mnist-verify-time.tex <==
% This file is automatically generated by experiments/model_summary.py



\begin{table*}
    \caption{\emph{Average running time for single-instance robustness verification} in seconds per correctly-predicted instance on MNIST models of different verification approaches. The verification is under $\cL_\infty$ adversary with $\epsilon$~(specified in table) radius. We stop the execution when time exceeds $\SI{60}{s}$ per instance. We include running time of PGD attack and normal inference as the reference.}
    \centering
    \vspace{-0.5em}
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &     \mc{2}{\texttt{clean}} &    \emc{2}{\texttt{clean}}\\
\midrule
 \t{Bounded MILP} &             \mc{2}{$0.37$} &            \mc{2}{$12.67$} &      \mc{2}{$\tle{60.00}$} &            \mc{2}{$54.28$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
\rowcolor{tabgray}
       \t{AI$^2$} &             \mc{2}{$0.09$} &             \mc{2}{$1.09$} &      \mc{2}{$\tle{60.00}$} &             \mc{2}{$7.92$} &            \mc{2}{$48.89$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
      \t{LP-Full} &             \mc{2}{$0.41$} &            \mc{2}{$15.22$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
\rowcolor{tabgray}
     \t{DeepPoly} &             \mc{2}{$0.03$} &             \mc{2}{$0.25$} &      \mc{2}{$\tle{60.00}$} &             \mc{2}{$2.45$} &            \mc{2}{$49.04$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
     \t{Fast-Lin} &             \mc{2}{$0.03$} &             \mc{2}{$0.03$} &             \mc{2}{$1.71$} &             \mc{2}{$0.35$} &             \mc{2}{$4.70$} &            \mc{2}{$15.95$} &     \emc{2}{$\tle{60.00}$} \\
\rowcolor{tabgray}
        \t{CROWN} &             \mc{2}{$0.01$} &             \mc{2}{$0.01$} &             \mc{2}{$0.03$} &             \mc{2}{$0.02$} &             \mc{2}{$0.13$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
     \t{CNN-Cert} &             \mc{2}{$0.12$} &             \mc{2}{$0.43$} &      \mc{2}{$\tle{60.00}$} &             \mc{2}{$1.13$} &            \mc{2}{$28.40$} &            \mc{2}{$59.67$} &     \emc{2}{$\tle{60.00}$} \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &             \mc{2}{$0.01$} &             \mc{2}{$0.01$} &             \mc{2}{$0.01$} &             \mc{2}{$0.01$} &             \mc{2}{$0.01$} &             \mc{2}{$0.01$} &            \emc{2}{$0.01$} \\
          \t{IBP} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.01$} &             \mc{2}{$0.00$} &             \mc{2}{$0.01$} &             \mc{2}{$0.01$} &            \emc{2}{$0.01$} \\
\rowcolor{tabgray}
           \t{WK} &             \mc{2}{$0.01$} &             \mc{2}{$0.01$} &             \mc{2}{$0.04$} &             \mc{2}{$0.01$} &             \mc{2}{$0.03$} &             \mc{2}{$0.08$} &     \emc{2}{$\tle{60.00}$} \\
       \t{k-ReLU} &            \mc{2}{$12.49$} &            \mc{2}{$26.05$} &      \mc{2}{$\tle{60.00}$} &            \mc{2}{$30.49$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
\rowcolor{tabgray}
   \t{RefineZono} &             \mc{2}{$3.40$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
    \t{SDPVerify} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
\rowcolor{tabgray}
    \t{LMIVerify} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
      \t{Op-norm} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.01$} &             \mc{2}{$0.01$} &     \emc{2}{$\tle{60.00}$} \\
\rowcolor{tabgray}
      \t{FastLip} &             \mc{2}{$0.20$} &             \mc{2}{$0.20$} &             \mc{2}{$1.68$} &             \mc{2}{$5.81$} &            \mc{2}{$25.47$} &            \mc{2}{$54.26$} &     \emc{2}{$\tle{60.00}$} \\
     \t{RecurJac} &             \mc{2}{$0.81$} &             \mc{2}{$2.25$} &            \mc{2}{$43.29$} &            \mc{2}{$50.35$} &      \mc{2}{$\tle{60.00}$} &      \mc{2}{$\tle{60.00}$} &     \emc{2}{$\tle{60.00}$} \\
\hline
\rowcolor{tabgray}
PGD Attack &             \mc{2}{$0.26$} &             \mc{2}{$0.30$} &             \mc{2}{$0.42$} &             \mc{2}{$0.33$} &             \mc{2}{$0.43$} &             \mc{2}{$0.46$} &            \emc{2}{$0.51$} \\
\hline
   Normal Inference &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &             \mc{2}{$0.00$} &            \emc{2}{$0.00$} \\
\hline\hline
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1}\\
\midrule
 \t{Bounded MILP} &        $0.73$ &        $0.28$ & $\tle{60.00}$ &        $1.32$ & $\tle{60.00}$ &       $53.35$ & $\tle{60.00}$ &        $6.86$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
       \t{AI$^2$} &        $0.52$ &        $0.23$ &       $59.38$ &        $1.12$ & $\tle{60.00}$ &       $31.50$ &       $56.49$ &        $2.61$ &       $59.80$ &       $25.03$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
      \t{LP-Full} &        $0.43$ &        $0.35$ &       $23.59$ &        $9.57$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
     \t{DeepPoly} &        $0.03$ &        $0.02$ &        $0.24$ &        $0.15$ & $\tle{60.00}$ &        $7.97$ &        $1.61$ &        $1.34$ &       $41.59$ &       $23.53$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
     \t{Fast-Lin} &        $0.01$ &        $0.01$ &        $0.03$ &        $0.02$ &        $2.06$ &        $1.71$ &        $0.39$ &        $0.41$ &        $5.63$ &        $4.80$ &       $17.31$ &       $19.13$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
        \t{CROWN} &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.03$ &        $0.03$ &        $0.02$ &        $0.02$ &        $0.13$ &        $0.13$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
     \t{CNN-Cert} &        $0.02$ &        $0.03$ &        $0.05$ &        $0.31$ & $\tle{60.00}$ & $\tle{60.00}$ &        $0.21$ &        $1.35$ &        $4.18$ &       $36.00$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ \\
          \t{IBP} &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ \\
\rowcolor{tabgray}
           \t{WK} &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.04$ &        $0.04$ &        $0.01$ &        $0.01$ &        $0.07$ &        $0.03$ &        $0.21$ &        $0.09$ & $\tle{60.00}$ &       $59.41$ \\
       \t{k-ReLU} &       $12.87$ &       $11.92$ &       $34.56$ &       $38.43$ & $\tle{60.00}$ & $\tle{60.00}$ &       $59.35$ &       $34.48$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
   \t{RefineZono} &        $7.27$ &       $14.51$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
    \t{SDPVerify} & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
    \t{LMIVerify} & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
      \t{Op-norm} &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
      \t{FastLip} &        $0.02$ &        $0.03$ &        $0.05$ &        $0.12$ &        $1.17$ &        $6.04$ &        $2.52$ &        $5.51$ &       $20.05$ & $\tle{60.00}$ &       $46.69$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
     \t{RecurJac} &        $0.36$ &        $0.35$ &        $0.88$ &        $1.77$ &       $24.96$ &       $57.75$ &       $28.61$ &       $49.91$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\hline
\rowcolor{tabgray}
PGD Attack &        $0.26$ &        $0.30$ &        $0.30$ &        $0.33$ &        $0.42$ &        $0.48$ &        $0.33$ &        $0.37$ &        $0.44$ &        $0.48$ &        $0.47$ &        $0.50$ &        $0.52$ &        $0.54$ \\
\hline
   Normal Inference &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ \\
\hline\hline
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3}\\
\midrule
 \t{Bounded MILP} &        $0.63$ &        $0.30$ & $\tle{60.00}$ &        $1.39$ & $\tle{60.00}$ &       $52.52$ & $\tle{60.00}$ &        $5.61$ & $\tle{60.00}$ &       $50.35$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
       \t{AI$^2$} &        $0.72$ &        $0.29$ & $\tle{60.00}$ &        $1.72$ & $\tle{60.00}$ &       $23.66$ & $\tle{60.00}$ &       $27.46$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
      \t{LP-Full} &        $0.49$ &        $0.39$ &       $22.97$ &       $12.75$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
     \t{DeepPoly} &        $0.02$ &        $0.02$ &        $0.29$ &        $0.15$ & $\tle{60.00}$ &        $5.14$ &        $1.75$ &        $1.28$ &       $40.27$ &       $27.57$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
     \t{Fast-Lin} &        $0.01$ &        $0.01$ &        $0.03$ &        $0.03$ &        $2.14$ &        $1.96$ &        $0.34$ &        $0.44$ &        $5.66$ &        $5.28$ &       $18.63$ &       $20.04$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
        \t{CROWN} &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.03$ &        $0.03$ &        $0.02$ &        $0.02$ &        $0.13$ &        $0.13$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
     \t{CNN-Cert} &        $0.01$ &        $0.02$ &        $0.06$ &        $0.12$ & $\tle{60.00}$ & $\tle{60.00}$ &        $0.17$ &        $0.89$ &        $4.20$ &        $5.91$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
    \t{CROWN-IBP} &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.02$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.02$ &        $0.01$ \\
          \t{IBP} &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ \\
\rowcolor{tabgray}
           \t{WK} &        $0.01$ &        $0.01$ &        $0.01$ &        $0.01$ &        $0.04$ &        $0.04$ &        $0.01$ &        $0.01$ &        $0.07$ &        $0.06$ &        $0.38$ &        $0.19$ & $\tle{60.00}$ & $\tle{60.00}$ \\
       \t{k-ReLU} &       $12.37$ &       $12.78$ &       $45.15$ &       $44.37$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ &       $48.59$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
   \t{RefineZono} &       $12.08$ &       $18.52$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
    \t{SDPVerify} & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
    \t{LMIVerify} & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
      \t{Op-norm} &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.01$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\rowcolor{tabgray}
      \t{FastLip} &        $0.01$ &        $0.03$ &        $0.02$ &        $0.07$ &        $1.87$ &        $1.91$ &        $2.04$ &        $3.11$ &        $8.27$ &       $50.14$ &       $46.81$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
     \t{RecurJac} &        $0.14$ &        $0.31$ &        $0.36$ &        $1.28$ &       $10.81$ &       $29.23$ &       $12.47$ &       $38.94$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ & $\tle{60.00}$ \\
\hline
\rowcolor{tabgray}
PGD Attack &        $0.26$ &        $0.32$ &        $0.30$ &        $0.34$ &        $0.43$ &        $0.49$ &        $0.33$ &        $0.38$ &        $0.45$ &        $0.48$ &        $0.47$ &        $0.51$ &        $0.52$ &        $0.54$ \\
\hline
   Normal Inference &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ \\
\bottomrule

    \end{tabular}
    }
    \vspace{-1.25em}
    \label{tab:exp-A-mnist-verify-time}
\end{table*}



==> tables/exp-A-models-originalacc.tex <==
% This file is automatically generated by experiments/model_summary.py

\begin{table*}[!t]
    \centering
    \captionof{table}{Clean accuracy and empirical robust accuracy for each set of weights.
    The clean accuracy is measured on the whole original test set.
    The empirical robust accuracy is measured on the inputs generated by PGD attacks from the whole original test set.
    For \texttt{reg} weights, due to low robustness, we do not report empirical robust accuracy~(which is typically close to zero).\\
    On MNIST:
    for \texttt{adv1} and \texttt{cadv1}, the adversarial examples are bounded by radius $\epsilon=0.1$ under $\cL_\infty$ metric;
    for \texttt{adv3} and \texttt{cadv3}, bounded by radius $\epsilon=0.3$.
    On CIFAR-10:
    for \texttt{adv2} and \texttt{cadv2}, bounded by radius $\epsilon=2/255$;
    for \texttt{adv8} and \texttt{cadv8}, bounded by radius $\epsilon=8/255$.
    }
    \resizebox{0.80\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c||c|c|c|c|c}
    \toprule
        Dataset &           Model &         Weights &      Clean Acc. &   Empirical Rob. Acc. &
        Dataset &           Model &         Weights &      Clean Acc. &   Empirical Rob. Acc. \\
    \midrule
          \multirow{35}{*}{MNIST} &      \multirow{5}{*}{\sc{FCNNa}} &    \texttt{reg} &       $93.63\%$ &               / &
       \multirow{35}{*}{CIFAR-10} &      \multirow{5}{*}{\sc{FCNNa}} &    \texttt{reg} &       $38.46\%$ &               / \\
                &                 &   \texttt{adv1} &       $93.36\%$ &       $78.39\%$ &
                &                 &   \texttt{adv2} &       $41.17\%$ &       $39.49\%$ \\
                &                 &  \texttt{cadv1} &       $88.35\%$ &       $80.99\%$ &
                &                 &  \texttt{cadv2} &       $38.97\%$ &       $38.71\%$ \\
                &                 &   \texttt{adv3} &       $76.77\%$ &       $31.67\%$ &
                &                 &   \texttt{adv8} &       $34.13\%$ &       $31.36\%$ \\
                &                 &  \texttt{cadv3} &       $45.79\%$ &       $41.35\%$ &
                &                 &  \texttt{cadv8} &       $30.59\%$ &       $30.36\%$ \\
    \cline{2-5}
    \cline{7-10}
                &      \multirow{5}{*}{\sc{FCNNb}} &    \texttt{reg} &       $96.12\%$ &               / &
                &      \multirow{5}{*}{\sc{FCNNb}} &    \texttt{reg} &       $41.76\%$ &               / \\
                &                 &   \texttt{adv1} &       $97.12\%$ &       $85.18\%$ &
                &                 &   \texttt{adv2} &       $44.31\%$ &       $42.99\%$ \\
                &                 &  \texttt{cadv1} &       $95.23\%$ &       $90.67\%$ &
                &                 &  \texttt{cadv2} &       $44.18\%$ &       $43.83\%$ \\
                &                 &   \texttt{adv3} &       $89.96\%$ &       $33.30\%$ &
                &                 &   \texttt{adv8} &       $37.68\%$ &       $34.01\%$ \\
                &                 &  \texttt{cadv3} &       $76.21\%$ &       $69.90\%$ &
                &                 &  \texttt{cadv8} &       $32.05\%$ &       $31.40\%$ \\
    \cline{2-5}
    \cline{7-10}
                &      \multirow{5}{*}{\sc{FCNNc}} &    \texttt{reg} &       $95.05\%$ &               / &
                &      \multirow{5}{*}{\sc{FCNNc}} &    \texttt{reg} &       $46.37\%$ &               / \\
                &                 &   \texttt{adv1} &       $98.00\%$ &       $87.40\%$ &
                &                 &   \texttt{adv2} &       $36.19\%$ &       $35.87\%$ \\
                &                 &  \texttt{cadv1} &       $96.89\%$ &       $93.43\%$ &
                &                 &  \texttt{cadv2} &       $46.34\%$ &       $45.42\%$ \\
                &                 &   \texttt{adv3} &       $83.27\%$ &       $33.31\%$ &
                &                 &   \texttt{adv8} &       $25.21\%$ &       $25.87\%$ \\
                &                 &  \texttt{cadv3} &       $35.87\%$ &       $34.08\%$ &
                &                 &  \texttt{cadv8} &       $30.30\%$ &       $29.59\%$ \\
    \cline{2-5}
    \cline{7-10}
                &       \multirow{5}{*}{\sc{CNNa}} &    \texttt{reg} &       $98.48\%$ &               / &
                &       \multirow{5}{*}{\sc{CNNa}} &    \texttt{reg} &       $59.45\%$ &               / \\
                &                 &   \texttt{adv1} &       $99.01\%$ &       $95.48\%$ &
                &                 &   \texttt{adv2} &       $60.40\%$ &       $57.39\%$ \\
                &                 &  \texttt{cadv1} &       $98.52\%$ &       $97.18\%$ &
                &                 &  \texttt{cadv2} &       $54.78\%$ &       $54.17\%$ \\
                &                 &   \texttt{adv3} &       $98.20\%$ &       $86.06\%$ &
                &                 &   \texttt{adv8} &       $49.42\%$ &       $41.87\%$ \\
                &                 &  \texttt{cadv3} &       $96.26\%$ &       $93.06\%$ &
                &                 &  \texttt{cadv8} &       $40.51\%$ &       $39.93\%$ \\
    \cline{2-5}
    \cline{7-10}
                
                &       \multirow{5}{*}{\sc{CNNb}} &    \texttt{reg} &       $98.85\%$ &               / &
                &       \multirow{5}{*}{\sc{CNNb}} &    \texttt{reg} &       $65.65\%$ &               / \\
                &                 &   \texttt{adv1} &       $99.33\%$ &       $96.09\%$ &
                &                 &   \texttt{adv2} &       $68.66\%$ &       $64.01\%$ \\
                &                 &  \texttt{cadv1} &       $98.87\%$ &       $98.12\%$ &
                &                 &  \texttt{cadv2} &       $58.81\%$ &       $58.76\%$ \\
                &                 &   \texttt{adv3} &       $99.01\%$ &       $92.84\%$ &
                &                 &   \texttt{adv8} &       $55.15\%$ &       $45.35\%$ \\
                &                 &  \texttt{cadv3} &       $98.14\%$ &       $95.88\%$ &
                &                 &  \texttt{cadv8} &       $40.05\%$ &       $39.36\%$ \\
    \cline{2-5}
    \cline{7-10}
                
                &       \multirow{5}{*}{\sc{CNNc}} &    \texttt{reg} &       $98.85\%$ &               / &
                &       \multirow{5}{*}{\sc{CNNc}} &    \texttt{reg} &       $58.60\%$ &               / \\
                &                 &   \texttt{adv1} &       $99.24\%$ &       $96.35\%$ &
                &                 &   \texttt{adv2} &       $65.59\%$ &       $62.05\%$ \\
                &                 &  \texttt{cadv1} &       $98.83\%$ &       $98.41\%$ &
                &                 &  \texttt{cadv2} &       $59.46\%$ &       $59.25\%$ \\
                &                 &   \texttt{adv3} &       $99.16\%$ &       $93.47\%$ &
                &                 &   \texttt{adv8} &       $54.01\%$ &       $45.91\%$ \\
                &                 &  \texttt{cadv3} &       $98.11\%$ &       $96.10\%$ &
                &                 &  \texttt{cadv8} &       $40.11\%$ &       $39.50\%$ \\
    \cline{2-5}
    \cline{7-10}
                
                &       \multirow{5}{*}{\sc{CNNd}} &    \texttt{reg} &       $99.20\%$ &               / &
                &       \multirow{5}{*}{\sc{CNNd}} &    \texttt{reg} &       $83.53\%$ &               / \\
                &                 &   \texttt{adv1} &       $99.37\%$ &       $97.64\%$ &
                &                 &   \texttt{adv2} &       $83.65\%$ &       $76.41\%$ \\
                &                 &  \texttt{cadv1} &       $99.13\%$ &       $98.50\%$ &
                &                 &  \texttt{cadv2} &       $60.74\%$ &       $59.88\%$ \\
                &                 &   \texttt{adv3} &       $99.38\%$ &       $95.09\%$ &
                &                 &   \texttt{adv8} &       $72.25\%$ &       $53.86\%$ \\
                &                 &  \texttt{cadv3} &       $98.58\%$ &       $96.72\%$ &
                &                 &  \texttt{cadv8} &       $40.61\%$ &       $39.94\%$ \\
    \bottomrule
    \end{tabular}
    }
    \label{table:expA-models-originalacc}
\end{table*}
        

==> tables/exp-A-models-stats.tex <==
% This file is automatically generated by experiments/model_summary.py


\begin{table*}[!t]
    \centering
    \caption{Statistics of the models used in the evaluation of deterministic verification approaches.
    In the ``Structure'' column, the rightarrow $\to$ stands for the connection from previous to the next layer, ``Flatten'' stands for the flatten layer, ``FC'' stands for the fully connected layer, and ``Conv'' stands for the convolutional layer.}
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|l}
    \toprule
        Dataset &           Model &      \# Neurons &   \# Parameters &       Structure &          Source \\
    \midrule
          MNIST &      \sc{FCNNa} &            $50$ &        $16,330$ & Flatten $\to$ 3 FCs & $2 \times [20]$ from \cite{weng2018towards,zhang2019recurjac} \\
                &      \sc{FCNNb} &           $310$ &        $99,710$ & Flatten $\to$ 4 FCs & $3 \times [100]$ enlarged from \cite{weng2018towards,zhang2019recurjac} \\
                &      \sc{FCNNc} &         $7,178$ &     $7,111,690$ & Flatten $\to$ 8 FCs & $7 \times [1024]$ from \cite{weng2018towards,zhang2018efficient} \\
    \cline{2-6}
                &       \sc{CNNa} &         $4,814$ &       $166,406$ & 2 Convs $\to$ Flatten $\to$ 2 FCs & Conv-Small in \cite{wong2018provable,wong2018scaling} \\
                &       \sc{CNNb} &        $24,042$ &       $833,786$ & 4 Convs $\to$ Flatten $\to$ 2 FCs & Half sized Conv-Large in \cite{wong2018scaling} \\
                &       \sc{CNNc} &        $48,074$ &     $1,974,762$ & 4 Convs $\to$ Flatten $\to$ 3 FCs & Conv-Large in \cite{wong2018scaling} \\
                &       \sc{CNNd} &       $176,138$ &    $13,314,634$ & 5 Convs $\to$ Flatten $\to$ 2 FCs & Double sized Conv-Large in \cite{wong2018scaling} \\
    \hline
       CIFAR-10 &      \sc{FCNNa} &            $50$ &        $62,090$ & Flatten $\to$ 3 FCs & $2 \times [20]$ from \cite{weng2018towards,zhang2019recurjac} \\
                &      \sc{FCNNb} &           $310$ &       $328,510$ & Flatten $\to$ 4 FCs & $3 \times [100]$ enlarged from \cite{weng2018towards,zhang2019recurjac} \\
                &      \sc{FCNNc} &         $7,178$ &     $9,454,602$ & Flatten $\to$ 8 FCs & $7 \times [1024]$ from \cite{weng2018towards,zhang2018efficient} \\
    \cline{2-6}
                &       \sc{CNNa} &         $6,254$ &       $214,918$ & 2 Convs $\to$ Flatten $\to$ 2 FCs & Conv-Small in \cite{wong2018provable,wong2018scaling} \\
                &       \sc{CNNb} &        $31,242$ &     $1,079,834$ & 4 Convs $\to$ Flatten $\to$ 2 FCs & Half sized Conv-Large in \cite{wong2018scaling} \\
                &       \sc{CNNc} &        $62,474$ &     $2,466,858$ & 4 Convs $\to$ Flatten $\to$ 3 FCs & Conv-Large in \cite{wong2018scaling} \\
                &       \sc{CNNd} &       $229,898$ &    $17,247,946$ & 5 Convs $\to$ Flatten $\to$ 2 FCs & Double sized Conv-Large in \cite{wong2018scaling} \\
    \bottomrule
    \end{tabular}
    }
    \label{table:expA-models-stats}
\end{table*}
        


==> tables/exp-A-robust-acc-tables.tex <==
% This file is automatically generated by experiments/model_summary.py



\begin{table}
    \caption{\emph{Robust accuracy} on MNIST \texttt{reg} models of different verification approaches. The verification is on $\cL_\infty$ ball with $\epsilon=0.02$ radius. We include results from PGD attack as the reference, which provides an upper bound.}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
              & \mc{1}{\sc{FCNNa}} & \mc{1}{\sc{FCNNb}} & \mc{1}{\sc{FCNNc}} & \mc{1}{\sc{CNNa}} & \mc{1}{\sc{CNNb}} & \mc{1}{\sc{CNNc}} & \emc{1}{\sc{CNNd}}\\
\cline{2-8}
              & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean}\\
\midrule
 Bounded MILP &        $80\%$ &        $24\%$ &         $0\%$ &               &               &               &               \\
          AI2 &        $80\%$ &               &               &               &               &               &               \\
      LP-Full &        $70\%$ &               &               &               &               &               &               \\
     DeepPoly &        $79\%$ &        $85\%$ &         $0\%$ &        $89\%$ &        $90\%$ &         $0\%$ &         $0\%$ \\
     Fast-Lin &        $68\%$ &        $56\%$ &         $0\%$ &        $72\%$ &        $28\%$ &         $5\%$ &               \\
        CROWN &        $79\%$ &        $85\%$ &         $0\%$ &        $89\%$ &        $90\%$ &         $0\%$ &         $0\%$ \\
     CNN-Cert &        $70\%$ &        $67\%$ &         $0\%$ &        $73\%$ &        $44\%$ &         $0\%$ &         $0\%$ \\
    CROWN-IBP &        $77\%$ &         $0\%$ &         $0\%$ &        $13\%$ &         $0\%$ &         $0\%$ &         $0\%$ \\
          IBP &         $3\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ \\
           WK &        $68\%$ &        $56\%$ &         $0\%$ &        $72\%$ &        $28\%$ &         $5\%$ &         $0\%$ \\
       k-ReLU &        $79\%$ &        $85\%$ &         $0\%$ &        $89\%$ &         $0\%$ &         $0\%$ &         $0\%$ \\
   RefineZono &        $79\%$ &               &               &               &               &               &               \\
    SDPVerify &         $0\%$ &               &               &               &               &               &               \\
    LMIVerify &         $0\%$ &               &               &               &               &               &               \\
      Op-norm &         $0\%$ &         $0\%$ &               &         $0\%$ &         $0\%$ &         $0\%$ &               \\
      FastLip &        $60\%$ &         $4\%$ &               &         $6\%$ &         $0\%$ &         $0\%$ &               \\
     RecurJac &        $70\%$ &        $52\%$ &         $0\%$ &        $33\%$ &         $0\%$ &         $0\%$ &               \\
\hline
          PGD &        $80\%$ &        $86\%$ &        $85\%$ &        $92\%$ &        $95\%$ &        $93\%$ &        $97\%$ \\
\hline
        Clean &        $89\%$ &        $92\%$ &        $95\%$ &        $99\%$ &       $100\%$ &       $100\%$ &       $100\%$ \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-robust-accuracy-mnist-0}
\end{table}
    

\begin{table}
    \caption{\emph{Average running time for single-instance robustness verification} in seconds per correctly-predicted instance on MNIST \texttt{reg} models of different verification approaches. In addition, the number in the parenthesis is the timeout instances out of $100$ evaluations. The verification is on $\cL_\infty$ ball with $\epsilon=0.02$ radius. We stop the execution when time exceeds $\SI{60}{s}$ per instance.We include running time of PGD attack as the reference.}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
              & \mc{1}{\sc{FCNNa}} & \mc{1}{\sc{FCNNb}} & \mc{1}{\sc{FCNNc}} & \mc{1}{\sc{CNNa}} & \mc{1}{\sc{CNNb}} & \mc{1}{\sc{CNNc}} & \emc{1}{\sc{CNNd}}\\
\cline{2-8}
              & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean}\\
\midrule
 Bounded MILP &  $6.77$~($0$) & $55.92$~($60$) & $60.00$~($95$) &               &               &               &               \\
          AI2 &  $0.09$~($0$) &               &               &               &               &               &               \\
      LP-Full &  $0.41$~($0$) &               &               &               &               &               &               \\
     DeepPoly &  $0.03$~($0$) &  $0.25$~($0$) & $60.00$~($95$) &  $2.45$~($0$) & $49.04$~($0$) & $60.00$~($100$) & $60.00$~($100$) \\
     Fast-Lin &  $0.03$~($0$) &  $0.03$~($0$) &  $1.71$~($0$) &  $0.35$~($0$) &  $4.70$~($0$) & $15.95$~($0$) &               \\
        CROWN &  $0.01$~($0$) &  $0.01$~($0$) &  $0.03$~($0$) &  $0.02$~($0$) &  $0.13$~($0$) & $60.00$~($100$) & $60.00$~($100$) \\
     CNN-Cert &  $0.12$~($0$) &  $0.43$~($0$) & $60.00$~($95$) &  $1.13$~($0$) & $28.40$~($0$) & $59.67$~($98$) & $60.00$~($100$) \\
    CROWN-IBP &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) \\
          IBP &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) \\
           WK &  $0.01$~($0$) &  $0.01$~($0$) &  $0.04$~($0$) &  $0.01$~($0$) &  $0.03$~($0$) &  $0.08$~($0$) & $60.00$~($100$) \\
       k-ReLU & $12.49$~($0$) & $26.05$~($0$) & $60.00$~($95$) & $30.49$~($0$) & $60.00$~($100$) & $60.00$~($100$) & $60.00$~($100$) \\
   RefineZono &  $3.40$~($0$) &               &               &               &               &               &               \\
    SDPVerify & $60.00$~($89$) &               &               &               &               &               &               \\
    LMIVerify & $60.00$~($89$) &               &               &               &               &               &               \\
      Op-norm &  $0.00$~($0$) &  $0.00$~($0$) &               &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &               \\
      FastLip &  $0.20$~($0$) &  $0.20$~($0$) &               &  $5.81$~($0$) & $25.47$~($0$) & $54.26$~($56$) &               \\
     RecurJac &  $0.81$~($0$) &  $2.25$~($0$) & $43.29$~($10$) & $50.35$~($17$) & $60.00$~($100$) & $60.00$~($100$) &               \\
\hline
          PGD &  $0.26$~($0$) &  $0.30$~($0$) &  $0.42$~($0$) &  $0.33$~($0$) &  $0.43$~($0$) &  $0.46$~($0$) &  $0.51$~($0$) \\
\hline
        Clean &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-robust-accuracy-time-mnist-0}
\end{table}
        

\begin{table*}
    \caption{\emph{Robust accuracy} on MNIST \texttt{adv1}/\texttt{cadv1} models of different verification approaches. The verification is on $\cL_\infty$ ball with $\epsilon=0.1$ radius. We include results from PGD attack as the reference, which provides an upper bound.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1}\\
\midrule
 Bounded MILP &        $70\%$ &        $68\%$ &         $0\%$ &        $84\%$ &         $0\%$ &         $0\%$ &               &               &               &               &               &               &               &               \\
          AI2 &        $70\%$ &        $68\%$ &               &               &               &               &               &               &               &               &               &               &               &               \\
      LP-Full &         $8\%$ &        $46\%$ &               &               &               &               &               &               &               &               &               &               &               &               \\
     DeepPoly &        $47\%$ &        $64\%$ &         $4\%$ &        $72\%$ &         $0\%$ &        $52\%$ &        $32\%$ &        $93\%$ &         $2\%$ &        $93\%$ &         $0\%$ &         $0\%$ &         $0\%$ &               \\
     Fast-Lin &         $5\%$ &        $35\%$ &         $0\%$ &        $36\%$ &         $0\%$ &         $0\%$ &         $0\%$ &        $90\%$ &         $0\%$ &        $89\%$ &         $0\%$ &        $86\%$ &               &               \\
        CROWN &        $47\%$ &        $64\%$ &         $4\%$ &        $72\%$ &         $0\%$ &        $52\%$ &        $32\%$ &        $93\%$ &         $2\%$ &        $93\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ \\
     CNN-Cert &         $5\%$ &        $36\%$ &         $0\%$ &        $44\%$ &         $0\%$ &         $0\%$ &         $0\%$ &        $92\%$ &         $0\%$ &        $93\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ \\
    CROWN-IBP &         $2\%$ &        $67\%$ &         $0\%$ &        $76\%$ &         $0\%$ &        $73\%$ &         $0\%$ &        $93\%$ &         $0\%$ &        $94\%$ &         $0\%$ &        $88\%$ &         $0\%$ &        $94\%$ \\
          IBP &         $0\%$ &        $68\%$ &         $0\%$ &        $85\%$ &         $0\%$ &        $80\%$ &         $0\%$ &        $95\%$ &         $0\%$ &        $91\%$ &         $0\%$ &        $89\%$ &         $0\%$ &        $90\%$ \\
           WK &         $5\%$ &        $35\%$ &         $0\%$ &        $36\%$ &         $0\%$ &         $0\%$ &         $0\%$ &        $90\%$ &         $0\%$ &        $89\%$ &         $0\%$ &        $86\%$ &         $0\%$ &         $1\%$ \\
       k-ReLU &        $51\%$ &        $68\%$ &         $4\%$ &        $85\%$ &         $0\%$ &         $0\%$ &         $3\%$ &        $95\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ \\
   RefineZono &        $49\%$ &        $63\%$ &               &               &               &               &               &               &               &               &               &               &               &               \\
    SDPVerify &         $0\%$ &         $0\%$ &               &               &               &               &               &               &               &               &               &               &               &               \\
    LMIVerify &         $0\%$ &         $0\%$ &               &               &               &               &               &               &               &               &               &               &               &               \\
      Op-norm &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &               &               &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &               &               \\
      FastLip &         $0\%$ &        $30\%$ &         $0\%$ &        $31\%$ &               &               &         $0\%$ &        $86\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &               &               \\
     RecurJac &         $2\%$ &        $30\%$ &         $0\%$ &        $31\%$ &         $0\%$ &         $0\%$ &         $0\%$ &        $85\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &               &               \\
\hline
          PGD &        $71\%$ &        $69\%$ &        $80\%$ &        $85\%$ &        $82\%$ &        $89\%$ &        $94\%$ &        $95\%$ &        $95\%$ &        $97\%$ &        $95\%$ &        $96\%$ &        $97\%$ &        $99\%$ \\
\hline
        Clean &        $92\%$ &        $88\%$ &        $97\%$ &        $97\%$ &        $98\%$ &        $96\%$ &       $100\%$ &        $99\%$ &       $100\%$ &        $99\%$ &       $100\%$ &       $100\%$ &       $100\%$ &       $100\%$ \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-robust-accuracy-mnist-1}
\end{table*}
    

\begin{table*}
    \caption{\emph{Average running time for single-instance robustness verification} in seconds per correctly-predicted instance on MNIST \texttt{adv1}/\texttt{cadv1} models of different verification approaches. In addition, the number in the parenthesis is the timeout instances out of $100$ evaluations. The verification is on $\cL_\infty$ ball with $\epsilon=0.1$ radius. We stop the execution when time exceeds $\SI{60}{s}$ per instance.We include running time of PGD attack as the reference.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1}\\
\midrule
 Bounded MILP &  $7.55$~($0$) &  $4.40$~($0$) & $28.91$~($1$) & $24.83$~($0$) & $60.00$~($98$) & $60.00$~($96$) &               &               &               &               &               &               &               &               \\
          AI2 &  $0.52$~($0$) &  $0.23$~($0$) &               &               &               &               &               &               &               &               &               &               &               &               \\
      LP-Full &  $0.43$~($0$) &  $0.35$~($0$) &               &               &               &               &               &               &               &               &               &               &               &               \\
     DeepPoly &  $0.03$~($0$) &  $0.02$~($0$) &  $0.24$~($0$) &  $0.15$~($0$) & $60.00$~($98$) &  $7.97$~($0$) &  $1.61$~($0$) &  $1.34$~($0$) & $41.59$~($0$) & $23.53$~($0$) & $60.00$~($100$) & $60.00$~($100$) & $60.00$~($100$) &               \\
     Fast-Lin &  $0.01$~($0$) &  $0.01$~($0$) &  $0.03$~($0$) &  $0.02$~($0$) &  $2.06$~($0$) &  $1.71$~($0$) &  $0.39$~($0$) &  $0.41$~($0$) &  $5.63$~($0$) &  $4.80$~($0$) & $17.31$~($0$) & $19.13$~($0$) &               &               \\
        CROWN &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.03$~($0$) &  $0.03$~($0$) &  $0.02$~($0$) &  $0.02$~($0$) &  $0.13$~($0$) &  $0.13$~($0$) & $60.00$~($100$) & $60.00$~($100$) & $60.00$~($100$) & $60.00$~($100$) \\
     CNN-Cert &  $0.02$~($0$) &  $0.03$~($0$) &  $0.05$~($0$) &  $0.31$~($0$) & $60.00$~($98$) & $60.00$~($96$) &  $0.21$~($0$) &  $1.35$~($0$) &  $4.18$~($0$) & $36.00$~($0$) & $60.00$~($100$) & $60.00$~($100$) & $60.00$~($100$) & $60.00$~($100$) \\
    CROWN-IBP &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) \\
          IBP &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) \\
           WK &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.04$~($0$) &  $0.04$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.07$~($0$) &  $0.03$~($0$) &  $0.21$~($0$) &  $0.09$~($0$) & $60.00$~($100$) & $59.41$~($99$) \\
       k-ReLU & $12.87$~($0$) & $11.92$~($0$) & $34.56$~($0$) & $38.43$~($0$) & $60.00$~($98$) & $60.00$~($96$) & $59.35$~($97$) & $34.48$~($0$) & $60.00$~($100$) & $60.00$~($99$) & $60.00$~($100$) & $60.00$~($100$) & $60.00$~($100$) & $60.00$~($100$) \\
   RefineZono &  $7.27$~($0$) & $14.51$~($0$) &               &               &               &               &               &               &               &               &               &               &               &               \\
    SDPVerify & $60.00$~($92$) & $60.00$~($88$) &               &               &               &               &               &               &               &               &               &               &               &               \\
    LMIVerify & $60.00$~($92$) & $60.00$~($88$) &               &               &               &               &               &               &               &               &               &               &               &               \\
      Op-norm &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &               &               &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &               &               \\
      FastLip &  $0.02$~($0$) &  $0.03$~($0$) &  $0.05$~($0$) &  $0.12$~($0$) &               &               &  $2.52$~($0$) &  $5.51$~($0$) & $20.05$~($0$) & $60.00$~($99$) & $46.69$~($11$) & $60.00$~($100$) &               &               \\
     RecurJac &  $0.36$~($0$) &  $0.35$~($0$) &  $0.88$~($0$) &  $1.77$~($0$) & $24.96$~($0$) & $57.75$~($84$) & $28.61$~($0$) & $49.91$~($1$) & $60.00$~($100$) & $60.00$~($99$) & $60.00$~($100$) & $60.00$~($100$) &               &               \\
\hline
          PGD &  $0.26$~($0$) &  $0.30$~($0$) &  $0.30$~($0$) &  $0.33$~($0$) &  $0.42$~($0$) &  $0.48$~($0$) &  $0.33$~($0$) &  $0.37$~($0$) &  $0.44$~($0$) &  $0.48$~($0$) &  $0.47$~($0$) &  $0.50$~($0$) &  $0.52$~($0$) &  $0.54$~($0$) \\
\hline
        Clean &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-robust-accuracy-time-mnist-1}
\end{table*}
        

\begin{table*}
    \caption{\emph{Robust accuracy} on MNIST \texttt{adv3}/\texttt{cadv3} models of different verification approaches. The verification is on $\cL_\infty$ ball with $\epsilon=0.3$ radius. We include results from PGD attack as the reference, which provides an upper bound.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3}\\
\midrule
 Bounded MILP &         $6\%$ &        $25\%$ &         $0\%$ &        $52\%$ &         $0\%$ &         $0\%$ &               &               &               &               &               &               &               &               \\
          AI2 &         $6\%$ &        $25\%$ &               &               &               &               &               &               &               &               &               &               &               &               \\
      LP-Full &         $0\%$ &        $15\%$ &               &               &               &               &               &               &               &               &               &               &               &               \\
     DeepPoly &         $0\%$ &        $23\%$ &         $0\%$ &        $27\%$ &         $0\%$ &        $16\%$ &         $0\%$ &        $40\%$ &         $0\%$ &         $7\%$ &         $0\%$ &         $0\%$ &         $0\%$ &               \\
     Fast-Lin &         $0\%$ &         $4\%$ &         $0\%$ &         $1\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $6\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &               &               \\
        CROWN &         $0\%$ &        $23\%$ &         $0\%$ &        $27\%$ &         $0\%$ &        $16\%$ &         $0\%$ &        $40\%$ &         $0\%$ &         $7\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ \\
     CNN-Cert &         $0\%$ &        $13\%$ &         $0\%$ &         $5\%$ &         $0\%$ &         $0\%$ &         $0\%$ &        $39\%$ &         $0\%$ &         $1\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ \\
    CROWN-IBP &         $0\%$ &        $23\%$ &         $0\%$ &        $45\%$ &         $0\%$ &        $20\%$ &         $0\%$ &        $76\%$ &         $0\%$ &        $71\%$ &         $0\%$ &        $75\%$ &         $0\%$ &        $65\%$ \\
          IBP &         $0\%$ &        $25\%$ &         $0\%$ &        $54\%$ &         $0\%$ &        $22\%$ &         $0\%$ &        $88\%$ &         $0\%$ &        $85\%$ &         $0\%$ &        $87\%$ &         $0\%$ &        $89\%$ \\
           WK &         $0\%$ &         $4\%$ &         $0\%$ &         $1\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $6\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ \\
       k-ReLU &         $0\%$ &        $25\%$ &         $0\%$ &        $54\%$ &         $0\%$ &         $0\%$ &         $0\%$ &        $57\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ \\
   RefineZono &         $0\%$ &        $21\%$ &               &               &               &               &               &               &               &               &               &               &               &               \\
    SDPVerify &         $0\%$ &         $0\%$ &               &               &               &               &               &               &               &               &               &               &               &               \\
    LMIVerify &         $0\%$ &         $0\%$ &               &               &               &               &               &               &               &               &               &               &               &               \\
      Op-norm &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &               &               &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &               &               \\
      FastLip &         $0\%$ &         $1\%$ &         $0\%$ &         $2\%$ &               &               &         $0\%$ &         $2\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &               &               \\
     RecurJac &         $0\%$ &         $1\%$ &         $0\%$ &         $2\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $2\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &               &               \\
\hline
          PGD &        $19\%$ &        $26\%$ &        $26\%$ &        $64\%$ &        $26\%$ &        $26\%$ &        $81\%$ &        $90\%$ &        $91\%$ &        $94\%$ &        $90\%$ &        $93\%$ &        $92\%$ &        $94\%$ \\
\hline
        Clean &        $75\%$ &        $37\%$ &        $88\%$ &        $76\%$ &        $78\%$ &        $28\%$ &        $97\%$ &        $95\%$ &       $100\%$ &        $98\%$ &        $99\%$ &        $98\%$ &       $100\%$ &        $98\%$ \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-robust-accuracy-mnist-3}
\end{table*}
    

\begin{table*}
    \caption{\emph{Average running time for single-instance robustness verification} in seconds per correctly-predicted instance on MNIST \texttt{adv3}/\texttt{cadv3} models of different verification approaches. In addition, the number in the parenthesis is the timeout instances out of $100$ evaluations. The verification is on $\cL_\infty$ ball with $\epsilon=0.3$ radius. We stop the execution when time exceeds $\SI{60}{s}$ per instance.We include running time of PGD attack as the reference.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3}\\
\midrule
 Bounded MILP &  $3.34$~($0$) &  $4.85$~($0$) & $38.86$~($26$) & $14.79$~($0$) & $60.00$~($78$) & $60.00$~($28$) &               &               &               &               &               &               &               &               \\
          AI2 &  $0.72$~($0$) &  $0.29$~($0$) &               &               &               &               &               &               &               &               &               &               &               &               \\
      LP-Full &  $0.49$~($0$) &  $0.39$~($0$) &               &               &               &               &               &               &               &               &               &               &               &               \\
     DeepPoly &  $0.02$~($0$) &  $0.02$~($0$) &  $0.29$~($0$) &  $0.15$~($0$) & $60.00$~($78$) &  $5.14$~($0$) &  $1.75$~($0$) &  $1.28$~($0$) & $40.27$~($0$) & $27.57$~($0$) & $60.00$~($99$) & $60.00$~($98$) & $60.00$~($100$) &               \\
     Fast-Lin &  $0.01$~($0$) &  $0.01$~($0$) &  $0.03$~($0$) &  $0.03$~($0$) &  $2.14$~($0$) &  $1.96$~($0$) &  $0.34$~($0$) &  $0.44$~($0$) &  $5.66$~($0$) &  $5.28$~($0$) & $18.63$~($0$) & $20.04$~($0$) &               &               \\
        CROWN &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.03$~($0$) &  $0.03$~($0$) &  $0.02$~($0$) &  $0.02$~($0$) &  $0.13$~($0$) &  $0.13$~($0$) & $60.00$~($99$) & $60.00$~($98$) & $60.00$~($100$) & $60.00$~($98$) \\
     CNN-Cert &  $0.01$~($0$) &  $0.02$~($0$) &  $0.06$~($0$) &  $0.12$~($0$) & $60.00$~($78$) & $60.00$~($28$) &  $0.17$~($0$) &  $0.89$~($0$) &  $4.20$~($0$) &  $5.91$~($0$) & $60.00$~($99$) & $60.00$~($98$) & $60.00$~($100$) & $60.00$~($98$) \\
    CROWN-IBP &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.02$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.02$~($0$) &  $0.01$~($0$) \\
          IBP &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) \\
           WK &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.04$~($0$) &  $0.04$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.07$~($0$) &  $0.06$~($0$) &  $0.38$~($0$) &  $0.19$~($0$) & $60.00$~($100$) & $60.00$~($98$) \\
       k-ReLU & $12.37$~($0$) & $12.78$~($0$) & $45.15$~($0$) & $44.37$~($0$) & $60.00$~($78$) & $60.00$~($28$) & $60.00$~($97$) & $48.59$~($22$) & $60.00$~($100$) & $60.00$~($98$) & $60.00$~($99$) & $60.00$~($98$) & $60.00$~($100$) & $60.00$~($98$) \\
   RefineZono & $12.08$~($0$) & $18.52$~($0$) &               &               &               &               &               &               &               &               &               &               &               &               \\
    SDPVerify & $60.00$~($75$) & $60.00$~($37$) &               &               &               &               &               &               &               &               &               &               &               &               \\
    LMIVerify & $60.00$~($75$) & $60.00$~($37$) &               &               &               &               &               &               &               &               &               &               &               &               \\
      Op-norm &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &               &               &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &               &               \\
      FastLip &  $0.01$~($0$) &  $0.03$~($0$) &  $0.02$~($0$) &  $0.07$~($0$) &               &               &  $2.04$~($0$) &  $3.11$~($0$) &  $8.27$~($0$) & $50.14$~($36$) & $46.81$~($2$) & $60.00$~($98$) &               &               \\
     RecurJac &  $0.14$~($0$) &  $0.31$~($0$) &  $0.36$~($0$) &  $1.28$~($0$) & $10.81$~($0$) & $29.23$~($2$) & $12.47$~($0$) & $38.94$~($0$) & $60.00$~($100$) & $60.00$~($98$) & $60.00$~($99$) & $60.00$~($98$) &               &               \\
\hline
          PGD &  $0.26$~($0$) &  $0.32$~($0$) &  $0.30$~($0$) &  $0.34$~($0$) &  $0.43$~($0$) &  $0.49$~($0$) &  $0.33$~($0$) &  $0.38$~($0$) &  $0.45$~($0$) &  $0.48$~($0$) &  $0.47$~($0$) &  $0.51$~($0$) &  $0.52$~($0$) &  $0.54$~($0$) \\
\hline
        Clean &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-robust-accuracy-time-mnist-3}
\end{table*}
        

\begin{table}
    \caption{\emph{Robust accuracy} on CIFAR-10 \texttt{reg} models of different verification approaches. The verification is on $\cL_\infty$ ball with $\epsilon=0.5/255$ radius. We include results from PGD attack as the reference, which provides an upper bound.}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
              & \mc{1}{\sc{FCNNa}} & \mc{1}{\sc{FCNNb}} & \mc{1}{\sc{FCNNc}} & \mc{1}{\sc{CNNa}} & \mc{1}{\sc{CNNb}} & \mc{1}{\sc{CNNc}} & \emc{1}{\sc{CNNd}}\\
\cline{2-8}
              & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean}\\
\midrule
 Bounded MILP &        $40\%$ &         $1\%$ &               &               &               &               &               \\
          AI2 &               &               &               &               &               &               &               \\
      LP-Full &        $40\%$ &        $43\%$ &               &               &               &               &               \\
     DeepPoly &               &               &               &               &               &               &               \\
     Fast-Lin &        $40\%$ &        $42\%$ &        $49\%$ &        $51\%$ &        $49\%$ &        $45\%$ &               \\
        CROWN &        $40\%$ &        $43\%$ &        $51\%$ &        $51\%$ &        $52\%$ &         $0\%$ &         $0\%$ \\
     CNN-Cert &        $40\%$ &        $43\%$ &         $0\%$ &        $51\%$ &        $52\%$ &         $0\%$ &         $0\%$ \\
    CROWN-IBP &        $40\%$ &        $24\%$ &         $0\%$ &        $13\%$ &         $0\%$ &         $0\%$ &         $0\%$ \\
          IBP &        $29\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ \\
           WK &        $40\%$ &        $42\%$ &        $49\%$ &        $51\%$ &        $49\%$ &        $45\%$ &         $3\%$ \\
       k-ReLU &               &               &               &               &               &               &               \\
   RefineZono &               &               &               &               &               &               &               \\
    SDPVerify &               &               &               &               &               &               &               \\
    LMIVerify &               &               &               &               &               &               &               \\
      Op-norm &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &               \\
      FastLip &        $40\%$ &        $40\%$ &         $0\%$ &        $36\%$ &         $0\%$ &         $0\%$ &               \\
     RecurJac &        $40\%$ &        $42\%$ &         $0\%$ &         $0\%$ &         $0\%$ &               &               \\
\hline
          PGD &        $40\%$ &        $43\%$ &        $53\%$ &        $51\%$ &        $61\%$ &        $49\%$ &        $76\%$ \\
\hline
        Clean &        $41\%$ &        $47\%$ &        $54\%$ &        $57\%$ &        $68\%$ &        $54\%$ &        $85\%$ \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-robust-accuracy-cifar10-0}
\end{table}
    

\begin{table}
    \caption{\emph{Average running time for single-instance robustness verification} in seconds per correctly-predicted instance on CIFAR-10 \texttt{reg} models of different verification approaches. In addition, the number in the parenthesis is the timeout instances out of $100$ evaluations. The verification is on $\cL_\infty$ ball with $\epsilon=0.5/255$ radius. We stop the execution when time exceeds $\SI{60}{s}$ per instance.We include running time of PGD attack as the reference.}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
              & \mc{1}{\sc{FCNNa}} & \mc{1}{\sc{FCNNb}} & \mc{1}{\sc{FCNNc}} & \mc{1}{\sc{CNNa}} & \mc{1}{\sc{CNNb}} & \mc{1}{\sc{CNNc}} & \emc{1}{\sc{CNNd}}\\
\cline{2-8}
              & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean}\\
\midrule
 Bounded MILP &  $8.09$~($0$) & $53.97$~($39$) &               &               &               &               &               \\
          AI2 &               &               &               &               &               &               &               \\
      LP-Full &  $0.71$~($0$) & $33.68$~($0$) &               &               &               &               &               \\
     DeepPoly &               &               &               &               &               &               &               \\
     Fast-Lin &  $0.03$~($0$) &  $0.02$~($0$) &  $1.03$~($0$) &  $1.49$~($0$) & $11.07$~($0$) & $32.62$~($0$) &               \\
        CROWN &  $0.00$~($0$) &  $0.01$~($0$) &  $0.08$~($0$) &  $0.03$~($0$) &  $0.32$~($0$) & $60.00$~($54$) & $60.00$~($85$) \\
     CNN-Cert &  $0.19$~($0$) &  $0.71$~($0$) & $60.00$~($54$) &  $1.43$~($0$) & $35.36$~($0$) & $59.69$~($53$) & $60.00$~($85$) \\
    CROWN-IBP &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) \\
          IBP &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) \\
           WK &  $0.00$~($0$) &  $0.01$~($0$) &  $0.05$~($0$) &  $0.01$~($0$) &  $0.06$~($0$) &  $0.10$~($0$) & $54.42$~($77$) \\
       k-ReLU &               &               &               &               &               &               &               \\
   RefineZono &               &               &               &               &               &               &               \\
    SDPVerify &               &               &               &               &               &               &               \\
    LMIVerify &               &               &               &               &               &               &               \\
      Op-norm &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.03$~($0$) &               \\
      FastLip &  $0.09$~($0$) &  $0.43$~($0$) &  $1.35$~($0$) & $21.28$~($0$) & $49.81$~($35$) & $60.00$~($54$) &               \\
     RecurJac &  $1.56$~($0$) &  $5.67$~($0$) & $60.00$~($54$) & $57.99$~($53$) & $60.00$~($68$) &               &               \\
\hline
          PGD &  $0.23$~($0$) &  $0.27$~($0$) &  $0.35$~($0$) &  $0.30$~($0$) &  $0.35$~($0$) &  $0.39$~($0$) &  $0.54$~($0$) \\
\hline
        Clean &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-robust-accuracy-time-cifar10-0}
\end{table}
        

\begin{table*}
    \caption{\emph{Robust accuracy} on CIFAR-10 \texttt{adv2}/\texttt{cadv2} models of different verification approaches. The verification is on $\cL_\infty$ ball with $\epsilon=2/255$ radius. We include results from PGD attack as the reference, which provides an upper bound.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2}\\
\midrule
 Bounded MILP &        $35\%$ &        $27\%$ &         $0\%$ &         $8\%$ &               &               &               &               &               &               &               &               &               &               \\
          AI2 &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
      LP-Full &        $35\%$ &        $33\%$ &        $36\%$ &        $37\%$ &               &               &               &               &               &               &               &               &               &               \\
     DeepPoly &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
     Fast-Lin &        $35\%$ &        $33\%$ &        $35\%$ &        $34\%$ &         $0\%$ &               &        $33\%$ &        $45\%$ &        $14\%$ &               &        $13\%$ &               &               &               \\
        CROWN &        $35\%$ &        $33\%$ &        $36\%$ &        $35\%$ &         $1\%$ &               &        $34\%$ &        $46\%$ &        $19\%$ &        $45\%$ &         $0\%$ &               &         $0\%$ &               \\
     CNN-Cert &        $35\%$ &        $33\%$ &        $35\%$ &        $35\%$ &         $0\%$ &               &        $34\%$ &        $46\%$ &        $19\%$ &        $45\%$ &         $0\%$ &               &         $0\%$ &               \\
    CROWN-IBP &        $30\%$ &        $33\%$ &         $0\%$ &        $34\%$ &         $0\%$ &               &         $0\%$ &        $46\%$ &         $0\%$ &        $46\%$ &         $0\%$ &               &         $0\%$ &               \\
          IBP &         $6\%$ &        $33\%$ &         $0\%$ &        $35\%$ &         $0\%$ &        $32\%$ &         $0\%$ &        $45\%$ &         $0\%$ &        $49\%$ &         $0\%$ &        $51\%$ &         $0\%$ &        $51\%$ \\
           WK &        $35\%$ &        $33\%$ &        $35\%$ &        $34\%$ &         $0\%$ &               &        $33\%$ &        $45\%$ &        $14\%$ &        $43\%$ &        $13\%$ &               &         $0\%$ &               \\
       k-ReLU &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
   RefineZono &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
    SDPVerify &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
    LMIVerify &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
      Op-norm &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &               &         $0\%$ &         $0\%$ &         $0\%$ &               &         $0\%$ &               &               &               \\
      FastLip &        $33\%$ &        $32\%$ &        $15\%$ &        $32\%$ &         $0\%$ &               &         $3\%$ &        $40\%$ &         $0\%$ &               &         $0\%$ &               &               &               \\
     RecurJac &        $34\%$ &        $32\%$ &        $33\%$ &        $32\%$ &         $0\%$ &               &         $0\%$ &         $0\%$ &         $0\%$ &               &               &               &               &               \\
\hline
          PGD &        $36\%$ &        $35\%$ &        $41\%$ &        $39\%$ &        $26\%$ &        $38\%$ &        $43\%$ &        $49\%$ &        $52\%$ &        $50\%$ &        $49\%$ &        $53\%$ &        $62\%$ &        $54\%$ \\
\hline
        Clean &        $44\%$ &        $40\%$ &        $48\%$ &        $43\%$ &        $35\%$ &        $46\%$ &        $54\%$ &        $55\%$ &        $66\%$ &        $60\%$ &        $59\%$ &        $63\%$ &        $81\%$ &        $62\%$ \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-robust-accuracy-cifar10-2}
\end{table*}
    

\begin{table*}
    \caption{\emph{Average running time for single-instance robustness verification} in seconds per correctly-predicted instance on CIFAR-10 \texttt{adv2}/\texttt{cadv2} models of different verification approaches. In addition, the number in the parenthesis is the timeout instances out of $100$ evaluations. The verification is on $\cL_\infty$ ball with $\epsilon=2/255$ radius. We stop the execution when time exceeds $\SI{60}{s}$ per instance.We include running time of PGD attack as the reference.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2}\\
\midrule
 Bounded MILP & $11.75$~($0$) &  $9.64$~($0$) & $52.70$~($37$) & $49.96$~($24$) &               &               &               &               &               &               &               &               &               &               \\
          AI2 &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
      LP-Full &  $0.74$~($0$) &  $0.77$~($0$) & $34.64$~($0$) & $26.08$~($0$) &               &               &               &               &               &               &               &               &               &               \\
     DeepPoly &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
     Fast-Lin &  $0.01$~($0$) &  $0.03$~($0$) &  $0.02$~($0$) &  $0.05$~($0$) &  $1.36$~($0$) &               &  $1.48$~($0$) &  $1.45$~($0$) & $11.77$~($0$) &               & $33.87$~($0$) &               &               &               \\
        CROWN &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.07$~($0$) &               &  $0.03$~($0$) &  $0.03$~($0$) &  $0.33$~($0$) &  $0.47$~($0$) & $60.00$~($59$) &               & $60.00$~($81$) &               \\
     CNN-Cert &  $0.05$~($0$) &  $0.17$~($0$) &  $0.67$~($0$) &  $0.70$~($0$) & $10.71$~($0$) &               &  $1.18$~($0$) &  $1.26$~($0$) & $18.84$~($0$) & $33.65$~($0$) & $42.77$~($28$) &               & $60.00$~($81$) &               \\
    CROWN-IBP &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &               &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &               &  $0.01$~($0$) &               \\
          IBP &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) \\
           WK &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.06$~($0$) &               &  $0.02$~($0$) &  $0.01$~($0$) &  $0.08$~($0$) &  $0.10$~($0$) &  $0.15$~($0$) &               & $60.00$~($81$) &               \\
       k-ReLU &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
   RefineZono &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
    SDPVerify &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
    LMIVerify &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
      Op-norm &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &               &  $0.01$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &               &  $0.01$~($0$) &               &               &               \\
      FastLip &  $0.06$~($0$) &  $0.09$~($0$) &  $0.30$~($0$) &  $0.30$~($0$) &  $1.30$~($0$) &               & $11.90$~($0$) & $11.24$~($0$) & $37.44$~($7$) &               & $60.00$~($59$) &               &               &               \\
     RecurJac &  $0.90$~($0$) &  $1.43$~($0$) &  $4.83$~($0$) &  $5.14$~($0$) & $60.00$~($35$) &               & $59.51$~($53$) & $59.17$~($53$) & $60.00$~($66$) &               &               &               &               &               \\
\hline
          PGD &  $0.24$~($0$) &  $0.27$~($0$) &  $0.28$~($0$) &  $0.30$~($0$) &  $0.37$~($0$) &  $0.40$~($0$) &  $0.30$~($0$) &  $0.37$~($0$) &  $0.36$~($0$) &  $0.45$~($0$) &  $0.37$~($0$) &  $0.46$~($0$) &  $0.55$~($0$) &  $0.64$~($0$) \\
\hline
        Clean &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-robust-accuracy-time-cifar10-2}
\end{table*}
        

\begin{table*}
    \caption{\emph{Robust accuracy} on CIFAR-10 \texttt{adv8}/\texttt{cadv8} models of different verification approaches. The verification is on $\cL_\infty$ ball with $\epsilon=8/255$ radius. We include results from PGD attack as the reference, which provides an upper bound.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8}\\
\midrule
 Bounded MILP &        $19\%$ &        $21\%$ &         $0\%$ &        $11\%$ &               &               &               &               &               &               &               &               &               &               \\
          AI2 &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
      LP-Full &        $15\%$ &        $27\%$ &         $6\%$ &        $25\%$ &               &               &               &               &               &               &               &               &               &               \\
     DeepPoly &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
     Fast-Lin &        $15\%$ &        $25\%$ &         $4\%$ &        $18\%$ &         $0\%$ &               &         $3\%$ &        $26\%$ &         $0\%$ &               &         $0\%$ &               &               &               \\
        CROWN &        $15\%$ &        $27\%$ &         $6\%$ &        $20\%$ &         $0\%$ &               &         $8\%$ &        $33\%$ &         $1\%$ &        $20\%$ &         $0\%$ &               &         $0\%$ &               \\
     CNN-Cert &        $15\%$ &        $27\%$ &         $5\%$ &        $20\%$ &         $0\%$ &               &         $7\%$ &        $33\%$ &         $0\%$ &               &         $0\%$ &               &         $0\%$ &               \\
    CROWN-IBP &         $9\%$ &        $27\%$ &         $0\%$ &        $22\%$ &         $0\%$ &               &         $0\%$ &        $34\%$ &         $0\%$ &        $31\%$ &         $0\%$ &               &         $0\%$ &               \\
          IBP &         $0\%$ &        $27\%$ &         $0\%$ &        $25\%$ &         $0\%$ &        $30\%$ &         $0\%$ &        $34\%$ &         $0\%$ &        $35\%$ &         $0\%$ &        $38\%$ &         $0\%$ &        $28\%$ \\
           WK &        $15\%$ &        $25\%$ &         $4\%$ &        $18\%$ &         $0\%$ &               &         $3\%$ &        $26\%$ &         $0\%$ &        $15\%$ &         $0\%$ &               &         $0\%$ &               \\
       k-ReLU &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
   RefineZono &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
    SDPVerify &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
    LMIVerify &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
      Op-norm &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &         $0\%$ &               &         $0\%$ &         $0\%$ &         $0\%$ &               &         $0\%$ &               &               &               \\
      FastLip &        $12\%$ &        $27\%$ &         $0\%$ &        $17\%$ &         $0\%$ &               &         $0\%$ &        $24\%$ &         $0\%$ &               &         $0\%$ &               &               &               \\
     RecurJac &        $14\%$ &        $27\%$ &         $2\%$ &        $17\%$ &         $0\%$ &               &         $0\%$ &         $0\%$ &         $0\%$ &               &               &               &               &               \\
\hline
          PGD &        $22\%$ &        $28\%$ &        $23\%$ &        $26\%$ &        $19\%$ &        $34\%$ &        $34\%$ &        $34\%$ &        $33\%$ &        $39\%$ &        $36\%$ &        $40\%$ &        $41\%$ &        $31\%$ \\
\hline
        Clean &        $33\%$ &        $31\%$ &        $37\%$ &        $30\%$ &        $26\%$ &        $39\%$ &        $44\%$ &        $46\%$ &        $53\%$ &        $48\%$ &        $52\%$ &        $46\%$ &        $66\%$ &        $46\%$ \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-robust-accuracy-cifar10-8}
\end{table*}
    

\begin{table*}
    \caption{\emph{Average running time for single-instance robustness verification} in seconds per correctly-predicted instance on CIFAR-10 \texttt{adv8}/\texttt{cadv8} models of different verification approaches. In addition, the number in the parenthesis is the timeout instances out of $100$ evaluations. The verification is on $\cL_\infty$ ball with $\epsilon=8/255$ radius. We stop the execution when time exceeds $\SI{60}{s}$ per instance.We include running time of PGD attack as the reference.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8}\\
\midrule
 Bounded MILP & $26.79$~($0$) &  $8.25$~($0$) & $28.21$~($1$) & $40.54$~($11$) &               &               &               &               &               &               &               &               &               &               \\
          AI2 &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
      LP-Full &  $1.02$~($0$) &  $0.82$~($0$) & $51.35$~($1$) & $20.84$~($0$) &               &               &               &               &               &               &               &               &               &               \\
     DeepPoly &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
     Fast-Lin &  $0.01$~($0$) &  $0.01$~($0$) &  $0.03$~($0$) &  $0.02$~($0$) &  $1.44$~($0$) &               &  $1.49$~($0$) &  $1.24$~($0$) & $11.77$~($0$) &               & $38.27$~($0$) &               &               &               \\
        CROWN &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.07$~($0$) &               &  $0.03$~($0$) &  $0.03$~($0$) &  $0.33$~($0$) &  $0.46$~($0$) & $60.00$~($52$) &               & $60.00$~($66$) &               \\
     CNN-Cert &  $0.04$~($0$) &  $0.05$~($0$) &  $0.25$~($0$) &  $0.50$~($0$) & $10.94$~($0$) &               &  $0.48$~($0$) &  $1.03$~($0$) &  $4.11$~($0$) &               & $14.79$~($0$) &               & $60.00$~($66$) &               \\
    CROWN-IBP &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &               &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &               &  $0.01$~($0$) &               \\
          IBP &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) \\
           WK &  $0.01$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &  $0.01$~($0$) &  $0.06$~($0$) &               &  $0.02$~($0$) &  $0.01$~($0$) &  $0.09$~($0$) &  $0.11$~($0$) &  $0.40$~($0$) &               & $60.00$~($66$) &               \\
       k-ReLU &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
   RefineZono &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
    SDPVerify &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
    LMIVerify &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
      Op-norm &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &               &  $0.01$~($0$) &  $0.00$~($0$) &  $0.01$~($0$) &               &  $0.01$~($0$) &               &               &               \\
      FastLip &  $0.05$~($0$) &  $0.06$~($0$) &  $0.12$~($0$) &  $0.19$~($0$) &  $1.44$~($0$) &               &  $8.40$~($0$) &  $8.36$~($0$) & $28.66$~($1$) &               & $60.00$~($52$) &               &               &               \\
     RecurJac &  $0.74$~($0$) &  $0.90$~($0$) &  $2.81$~($0$) &  $4.04$~($0$) & $48.90$~($14$) &               & $57.64$~($41$) & $58.93$~($45$) & $60.00$~($53$) &               &               &               &               &               \\
\hline
          PGD &  $0.23$~($0$) &  $0.27$~($0$) &  $0.27$~($0$) &  $0.32$~($0$) &  $0.38$~($0$) &  $0.39$~($0$) &  $0.29$~($0$) &  $0.37$~($0$) &  $0.38$~($0$) &  $0.43$~($0$) &  $0.39$~($0$) &  $0.47$~($0$) &  $0.55$~($0$) &  $0.65$~($0$) \\
\hline
        Clean &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) &  $0.00$~($0$) \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-robust-accuracy-time-cifar10-8}
\end{table*}
        


==> tables/exp-A-robust-radius-tables.tex <==
% This file is automatically generated by experiments/model_summary.py



\begin{table}
    \caption{\emph{Average robust radius} on MNIST \texttt{reg} models of different verification approaches. The verification is on $\cL_\infty$ ball. We include results from PGD attack as the reference, which provides an upper bound.}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
              & \mc{1}{\sc{FCNNa}} & \mc{1}{\sc{FCNNb}} & \mc{1}{\sc{FCNNc}} & \mc{1}{\sc{CNNa}} & \mc{1}{\sc{CNNb}} & \mc{1}{\sc{CNNc}} & \emc{1}{\sc{CNNd}}\\
\cline{2-8}
              & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean}\\
\midrule
 Bounded MILP &       $0.054$ &       $0.000$ &               &               &               &               &               \\
          AI2 &       $0.054$ &               &               &               &               &               &               \\
      LP-Full &       $0.027$ &               &               &               &               &               &               \\
     DeepPoly &       $0.045$ &       $0.035$ &       $0.000$ &       $0.039$ &       $0.000$ &       $0.000$ &       $0.000$ \\
     Fast-Lin &       $0.026$ &       $0.018$ &       $0.000$ &       $0.021$ &       $0.014$ &       $0.009$ &               \\
        CROWN &       $0.045$ &       $0.035$ &       $0.005$ &       $0.039$ &       $0.030$ &       $0.000$ &       $0.000$ \\
     CNN-Cert &       $0.027$ &       $0.020$ &       $0.000$ &       $0.022$ &       $0.015$ &       $0.000$ &       $0.000$ \\
    CROWN-IBP &       $0.033$ &       $0.006$ &       $0.000$ &       $0.011$ &       $0.000$ &       $0.000$ &       $0.000$ \\
          IBP &       $0.006$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ \\
           WK &       $0.026$ &       $0.018$ &       $0.000$ &       $0.021$ &       $0.014$ &       $0.009$ &       $0.000$ \\
       k-ReLU &       $0.046$ &       $0.001$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ \\
   RefineZono &       $0.045$ &               &               &               &               &               &               \\
    SDPVerify &       $0.000$ &               &               &               &               &               &               \\
    LMIVerify &       $0.000$ &               &               &               &               &               &               \\
      Op-norm &       $0.003$ &       $0.001$ &               &       $0.000$ &       $0.000$ &       $0.000$ &               \\
      FastLip &       $0.020$ &       $0.008$ &               &       $0.009$ &       $0.000$ &       $0.000$ &               \\
     RecurJac &       $0.030$ &       $0.021$ &       $0.000$ &       $0.009$ &       $0.000$ &       $0.000$ &               \\
\hline
          PGD &       $0.057$ &       $0.060$ &       $0.046$ &       $0.073$ &       $0.087$ &       $0.090$ &       $0.103$ \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-average-radius-mnist-0}
\end{table}
    

\begin{table}
    \caption{\emph{Average running time for robust radius computation} in seconds per correctly-predicted instance on MNIST \texttt{reg} models of different verification approaches. The verification is on $\cL_\infty$ ball. We stop the execution when time exceeds $\SI{120}{s}$ per instance. We include running time of PGD attack as the reference.}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
              & \mc{1}{\sc{FCNNa}} & \mc{1}{\sc{FCNNb}} & \mc{1}{\sc{FCNNc}} & \mc{1}{\sc{CNNa}} & \mc{1}{\sc{CNNb}} & \mc{1}{\sc{CNNc}} & \emc{1}{\sc{CNNd}}\\
\cline{2-8}
              & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean}\\
\midrule
 Bounded MILP &       $29.17$ &      $120.00$ &               &               &               &               &               \\
          AI2 &        $3.95$ &               &               &               &               &               &               \\
      LP-Full &        $2.63$ &               &               &               &               &               &               \\
     DeepPoly &        $0.17$ &        $1.50$ &      $120.00$ &       $13.42$ &      $120.00$ &      $120.00$ &      $120.00$ \\
     Fast-Lin &        $0.04$ &        $0.17$ &       $12.30$ &        $2.04$ &       $32.25$ &      $103.94$ &               \\
        CROWN &        $0.03$ &        $0.05$ &        $0.17$ &        $0.09$ &        $0.80$ &      $120.00$ &      $120.00$ \\
     CNN-Cert &        $0.11$ &        $1.19$ &      $120.00$ &        $3.23$ &       $75.62$ &      $120.00$ &      $120.00$ \\
    CROWN-IBP &        $0.03$ &        $0.03$ &        $0.07$ &        $0.04$ &        $0.06$ &        $0.08$ &        $0.08$ \\
          IBP &        $0.02$ &        $0.02$ &        $0.03$ &        $0.02$ &        $0.03$ &        $0.04$ &        $0.05$ \\
           WK &        $0.04$ &        $0.06$ &        $0.22$ &        $0.08$ &        $0.32$ &        $1.06$ &      $120.00$ \\
       k-ReLU &       $70.72$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ \\
   RefineZono &       $32.98$ &               &               &               &               &               &               \\
    SDPVerify &      $120.00$ &               &               &               &               &               &               \\
    LMIVerify &      $120.00$ &               &               &               &               &               &               \\
      Op-norm &        $0.00$ &        $0.00$ &               &        $0.00$ &        $0.00$ &        $0.01$ &               \\
      FastLip &        $0.15$ &        $0.57$ &               &       $19.23$ &      $111.50$ &      $120.00$ &               \\
     RecurJac &        $6.81$ &       $29.75$ &      $120.00$ &      $114.36$ &      $120.00$ &      $120.00$ &               \\
\hline
          PGD &        $1.61$ &        $1.81$ &        $2.59$ &        $2.03$ &        $2.68$ &        $2.85$ &        $3.13$ \\

    \bottomrule
    \end{tabular}
    \label{table:exp-A-average-radius-time-mnist-0}
    }
\end{table}
        

\begin{table*}
    \caption{\emph{Average robust radius} on MNIST \texttt{adv1}/\texttt{cadv1} models of different verification approaches. The verification is on $\cL_\infty$ ball. We include results from PGD attack as the reference, which provides an upper bound.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1}\\
\midrule
 Bounded MILP &       $0.135$ &       $0.131$ &       $0.000$ &       $0.133$ &               &               &               &               &               &               &               &               &               &               \\
          AI2 &       $0.135$ &       $0.131$ &               &               &               &               &               &               &               &               &               &               &               &               \\
      LP-Full &       $0.063$ &       $0.097$ &               &               &               &               &               &               &               &               &               &               &               &               \\
     DeepPoly &       $0.095$ &       $0.120$ &       $0.064$ &       $0.118$ &       $0.000$ &       $0.096$ &       $0.086$ &       $0.152$ &       $0.008$ &       $0.160$ &       $0.000$ &       $0.000$ &       $0.000$ &               \\
     Fast-Lin &       $0.060$ &       $0.083$ &       $0.036$ &       $0.080$ &       $0.007$ &       $0.056$ &       $0.061$ &       $0.142$ &       $0.051$ &       $0.149$ &       $0.041$ &       $0.138$ &               &               \\
        CROWN &       $0.095$ &       $0.120$ &       $0.064$ &       $0.118$ &       $0.019$ &       $0.096$ &       $0.086$ &       $0.152$ &       $0.075$ &       $0.168$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ \\
     CNN-Cert &       $0.062$ &       $0.084$ &       $0.039$ &       $0.085$ &       $0.000$ &       $0.000$ &       $0.066$ &       $0.150$ &       $0.056$ &       $0.161$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ \\
    CROWN-IBP &       $0.055$ &       $0.123$ &       $0.009$ &       $0.135$ &       $0.000$ &       $0.133$ &       $0.030$ &       $0.154$ &       $0.001$ &       $0.176$ &       $0.000$ &       $0.179$ &       $0.000$ &       $0.174$ \\
          IBP &       $0.011$ &       $0.128$ &       $0.000$ &       $0.142$ &       $0.000$ &       $0.143$ &       $0.005$ &       $0.154$ &       $0.000$ &       $0.174$ &       $0.000$ &       $0.175$ &       $0.000$ &       $0.168$ \\
           WK &       $0.060$ &       $0.083$ &       $0.036$ &       $0.080$ &       $0.007$ &       $0.056$ &       $0.061$ &       $0.142$ &       $0.051$ &       $0.149$ &       $0.041$ &       $0.139$ &       $0.000$ &       $0.000$ \\
       k-ReLU &       $0.100$ &       $0.129$ &       $0.014$ &       $0.097$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ \\
   RefineZono &       $0.097$ &       $0.120$ &               &               &               &               &               &               &               &               &               &               &               &               \\
    SDPVerify &       $0.000$ &       $0.000$ &               &               &               &               &               &               &               &               &               &               &               &               \\
    LMIVerify &       $0.000$ &       $0.000$ &               &               &               &               &               &               &               &               &               &               &               &               \\
      Op-norm &       $0.002$ &       $0.002$ &       $0.001$ &       $0.002$ &               &               &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &               &               \\
      FastLip &       $0.041$ &       $0.078$ &       $0.016$ &       $0.074$ &               &               &       $0.032$ &       $0.131$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &               &               \\
     RecurJac &       $0.060$ &       $0.081$ &       $0.035$ &       $0.078$ &       $0.000$ &       $0.000$ &       $0.032$ &       $0.107$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &               &               \\
\hline
          PGD &       $0.145$ &       $0.157$ &       $0.155$ &       $0.190$ &       $0.151$ &       $0.213$ &       $0.163$ &       $0.194$ &       $0.168$ &       $0.233$ &       $0.169$ &       $0.278$ &       $0.181$ &       $0.320$ \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-average-radius-mnist-1}
\end{table*}
    

\begin{table*}
    \caption{\emph{Average running time for robust radius computation} in seconds per correctly-predicted instance on MNIST \texttt{adv1}/\texttt{cadv1} models of different verification approaches. The verification is on $\cL_\infty$ ball. We stop the execution when time exceeds $\SI{120}{s}$ per instance. We include running time of PGD attack as the reference.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1} & \texttt{adv1} & \texttt{cadv1}\\
\midrule
 Bounded MILP &       $37.89$ &       $28.84$ &      $120.00$ &      $114.57$ &               &               &               &               &               &               &               &               &               &               \\
          AI2 &        $5.28$ &        $6.44$ &               &               &               &               &               &               &               &               &               &               &               &               \\
      LP-Full &        $2.77$ &        $2.33$ &               &               &               &               &               &               &               &               &               &               &               &               \\
     DeepPoly &        $0.16$ &        $0.12$ &        $1.50$ &        $0.99$ &      $120.00$ &       $65.62$ &        $9.55$ &        $8.65$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &               \\
     Fast-Lin &        $0.03$ &        $0.04$ &        $0.16$ &        $0.17$ &       $11.18$ &        $9.15$ &        $2.11$ &        $2.62$ &       $32.73$ &       $28.51$ &       $96.23$ &      $119.36$ &               &               \\
        CROWN &        $0.03$ &        $0.03$ &        $0.05$ &        $0.05$ &        $0.17$ &        $0.18$ &        $0.09$ &        $0.09$ &        $0.80$ &        $0.80$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ \\
     CNN-Cert &        $0.16$ &        $0.16$ &        $1.48$ &        $1.70$ &      $120.00$ &      $120.00$ &        $4.09$ &        $4.69$ &       $94.97$ &      $115.68$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ \\
    CROWN-IBP &        $0.03$ &        $0.03$ &        $0.03$ &        $0.03$ &        $0.10$ &        $0.07$ &        $0.04$ &        $0.04$ &        $0.06$ &        $0.07$ &        $0.08$ &        $0.08$ &        $0.08$ &        $0.08$ \\
          IBP &        $0.02$ &        $0.02$ &        $0.02$ &        $0.03$ &        $0.03$ &        $0.04$ &        $0.02$ &        $0.03$ &        $0.03$ &        $0.04$ &        $0.04$ &        $0.05$ &        $0.05$ &        $0.06$ \\
           WK &        $0.04$ &        $0.04$ &        $0.06$ &        $0.06$ &        $0.21$ &        $0.20$ &        $0.08$ &        $0.08$ &        $0.33$ &        $0.23$ &        $1.03$ &        $0.77$ &      $120.00$ &      $120.00$ \\
       k-ReLU &       $65.10$ &       $69.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ \\
   RefineZono &       $56.38$ &      $100.87$ &               &               &               &               &               &               &               &               &               &               &               &               \\
    SDPVerify &      $120.00$ &      $120.00$ &               &               &               &               &               &               &               &               &               &               &               &               \\
    LMIVerify &      $120.00$ &      $120.00$ &               &               &               &               &               &               &               &               &               &               &               &               \\
      Op-norm &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &               &               &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ &               &               \\
      FastLip &        $0.16$ &        $0.16$ &        $0.67$ &        $0.69$ &               &               &       $20.61$ &       $25.84$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &               &               \\
     RecurJac &        $5.87$ &        $5.62$ &       $29.77$ &       $28.10$ &      $120.00$ &      $120.00$ &      $119.21$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &               &               \\
\hline
          PGD &        $1.70$ &        $2.04$ &        $1.91$ &        $2.25$ &        $2.67$ &        $2.96$ &        $2.11$ &        $2.33$ &        $2.74$ &        $2.97$ &        $2.85$ &        $3.21$ &        $3.16$ &        $3.40$ \\

    \bottomrule
    \end{tabular}
    \label{table:exp-A-average-radius-time-mnist-1}
    }
\end{table*}
        

\begin{table*}
    \caption{\emph{Average robust radius} on MNIST \texttt{adv3}/\texttt{cadv3} models of different verification approaches. The verification is on $\cL_\infty$ ball. We include results from PGD attack as the reference, which provides an upper bound.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3}\\
\midrule
 Bounded MILP &       $0.157$ &       $0.256$ &       $0.001$ &       $0.267$ &               &       $0.000$ &               &               &               &               &               &               &               &               \\
          AI2 &       $0.157$ &       $0.256$ &               &               &               &               &               &               &               &               &               &               &               &               \\
      LP-Full &       $0.079$ &       $0.229$ &               &               &               &               &               &               &               &               &               &               &               &               \\
     DeepPoly &       $0.119$ &       $0.239$ &       $0.076$ &       $0.224$ &       $0.000$ &       $0.228$ &       $0.174$ &       $0.254$ &       $0.105$ &       $0.188$ &       $0.000$ &       $0.000$ &       $0.000$ &               \\
     Fast-Lin &       $0.074$ &       $0.202$ &       $0.043$ &       $0.151$ &       $0.008$ &       $0.033$ &       $0.117$ &       $0.221$ &       $0.106$ &       $0.174$ &       $0.083$ &       $0.143$ &               &               \\
        CROWN &       $0.119$ &       $0.239$ &       $0.076$ &       $0.224$ &       $0.021$ &       $0.228$ &       $0.174$ &       $0.254$ &       $0.141$ &       $0.204$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ \\
     CNN-Cert &       $0.078$ &       $0.210$ &       $0.048$ &       $0.189$ &       $0.000$ &       $0.000$ &       $0.130$ &       $0.253$ &       $0.120$ &       $0.179$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ \\
    CROWN-IBP &       $0.069$ &       $0.239$ &       $0.005$ &       $0.256$ &       $0.000$ &       $0.288$ &       $0.074$ &       $0.283$ &       $0.000$ &       $0.272$ &       $0.000$ &       $0.277$ &       $0.000$ &       $0.272$ \\
          IBP &       $0.008$ &       $0.256$ &       $0.000$ &       $0.275$ &       $0.000$ &       $0.295$ &       $0.018$ &       $0.294$ &       $0.000$ &       $0.296$ &       $0.000$ &       $0.292$ &       $0.000$ &       $0.299$ \\
           WK &       $0.074$ &       $0.202$ &       $0.043$ &       $0.151$ &       $0.008$ &       $0.033$ &       $0.117$ &       $0.221$ &       $0.106$ &       $0.174$ &       $0.085$ &       $0.143$ &       $0.000$ &       $0.000$ \\
       k-ReLU &       $0.125$ &       $0.256$ &       $0.002$ &       $0.209$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.227$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ \\
   RefineZono &       $0.120$ &       $0.237$ &               &               &               &               &               &               &               &               &               &               &               &               \\
    SDPVerify &       $0.000$ &       $0.000$ &               &               &               &               &               &               &               &               &               &               &               &               \\
    LMIVerify &       $0.000$ &       $0.000$ &               &               &               &               &               &               &               &               &               &               &               &               \\
      Op-norm &       $0.001$ &       $0.000$ &       $0.000$ &       $0.001$ &               &               &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &               &               \\
      FastLip &       $0.053$ &       $0.189$ &       $0.015$ &       $0.153$ &               &               &       $0.067$ &       $0.199$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &               &               \\
     RecurJac &       $0.072$ &       $0.193$ &       $0.039$ &       $0.157$ &       $0.000$ &       $0.000$ &       $0.058$ &       $0.146$ &       $0.000$ &       $0.000$ &       $0.000$ &       $0.000$ &               &               \\
\hline
          PGD &       $0.199$ &       $0.309$ &       $0.216$ &       $0.331$ &       $0.231$ &       $0.427$ &       $0.308$ &       $0.302$ &       $0.313$ &       $0.318$ &       $0.328$ &       $0.316$ &       $0.366$ &       $0.325$ \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-average-radius-mnist-3}
\end{table*}
    

\begin{table*}
    \caption{\emph{Average running time for robust radius computation} in seconds per correctly-predicted instance on MNIST \texttt{adv3}/\texttt{cadv3} models of different verification approaches. The verification is on $\cL_\infty$ ball. We stop the execution when time exceeds $\SI{120}{s}$ per instance. We include running time of PGD attack as the reference.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3} & \texttt{adv3} & \texttt{cadv3}\\
\midrule
 Bounded MILP &       $37.26$ &       $29.85$ &      $120.00$ &       $83.86$ &               &      $120.00$ &               &               &               &               &               &               &               &               \\
          AI2 &        $4.96$ &        $3.74$ &               &               &               &               &               &               &               &               &               &               &               &               \\
      LP-Full &        $2.51$ &        $2.39$ &               &               &               &               &               &               &               &               &               &               &               &               \\
     DeepPoly &        $0.16$ &        $0.13$ &        $1.76$ &        $0.94$ &      $120.00$ &       $32.34$ &       $10.85$ &        $8.12$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &               \\
     Fast-Lin &        $0.03$ &        $0.04$ &        $0.17$ &        $0.15$ &       $11.21$ &        $8.92$ &        $1.78$ &        $2.40$ &       $29.16$ &       $28.74$ &      $115.24$ &      $106.29$ &               &               \\
        CROWN &        $0.03$ &        $0.03$ &        $0.05$ &        $0.05$ &        $0.17$ &        $0.18$ &        $0.09$ &        $0.09$ &        $0.80$ &        $0.80$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ \\
     CNN-Cert &        $0.16$ &        $0.16$ &        $1.41$ &        $1.95$ &      $120.00$ &      $120.00$ &        $4.71$ &        $5.14$ &      $112.83$ &      $117.19$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ \\
    CROWN-IBP &        $0.03$ &        $0.03$ &        $0.03$ &        $0.03$ &        $0.07$ &        $0.08$ &        $0.04$ &        $0.04$ &        $0.10$ &        $0.07$ &        $0.08$ &        $0.08$ &        $0.08$ &        $0.08$ \\
          IBP &        $0.02$ &        $0.02$ &        $0.02$ &        $0.03$ &        $0.03$ &        $0.04$ &        $0.02$ &        $0.03$ &        $0.03$ &        $0.04$ &        $0.04$ &        $0.05$ &        $0.05$ &        $0.06$ \\
           WK &        $0.04$ &        $0.04$ &        $0.06$ &        $0.06$ &        $0.21$ &        $0.18$ &        $0.07$ &        $0.08$ &        $0.18$ &        $0.21$ &        $0.57$ &        $0.78$ &      $120.00$ &      $120.00$ \\
       k-ReLU &       $64.68$ &       $63.76$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ \\
   RefineZono &       $79.13$ &       $21.92$ &               &               &               &               &               &               &               &               &               &               &               &               \\
    SDPVerify &      $120.00$ &      $120.00$ &               &               &               &               &               &               &               &               &               &               &               &               \\
    LMIVerify &      $120.00$ &      $120.00$ &               &               &               &               &               &               &               &               &               &               &               &               \\
      Op-norm &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &               &               &        $0.00$ &        $0.00$ &        $0.01$ &        $0.00$ &        $0.01$ &        $0.01$ &               &               \\
      FastLip &        $0.16$ &        $0.19$ &        $0.62$ &        $0.74$ &               &               &       $31.29$ &       $25.23$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &               &               \\
     RecurJac &        $5.37$ &        $5.92$ &       $29.40$ &       $30.22$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &      $120.00$ &               &               \\
\hline
          PGD &        $1.81$ &        $2.38$ &        $2.00$ &        $2.23$ &        $2.79$ &        $3.08$ &        $2.10$ &        $2.24$ &        $2.71$ &        $2.82$ &        $2.92$ &        $3.10$ &        $3.25$ &        $3.32$ \\

    \bottomrule
    \end{tabular}
    \label{table:exp-A-average-radius-time-mnist-3}
    }
\end{table*}
        

\begin{table}
    \caption{\emph{Average robust radius} on CIFAR-10 \texttt{reg} models of different verification approaches. The verification is on $\cL_\infty$ ball. We include results from PGD attack as the reference, which provides an upper bound.}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
              & \mc{1}{\sc{FCNNa}} & \mc{1}{\sc{FCNNb}} & \mc{1}{\sc{FCNNc}} & \mc{1}{\sc{CNNa}} & \mc{1}{\sc{CNNb}} & \mc{1}{\sc{CNNc}} & \emc{1}{\sc{CNNd}}\\
\cline{2-8}
              & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean}\\
\midrule
 Bounded MILP &   $4.847/255$ &   $0.000/255$ &               &               &               &               &               \\
          AI2 &               &               &               &               &               &               &               \\
      LP-Full &   $3.966/255$ &   $0.000/255$ &               &               &               &               &               \\
     DeepPoly &               &               &               &               &               &               &               \\
     Fast-Lin &   $3.723/255$ &   $2.596/255$ &   $0.812/255$ &   $1.503/255$ &   $0.637/255$ &   $0.000/255$ &               \\
        CROWN &   $3.984/255$ &   $2.888/255$ &   $1.065/255$ &   $1.669/255$ &   $0.765/255$ &   $0.000/255$ &   $0.000/255$ \\
     CNN-Cert &   $3.893/255$ &   $2.819/255$ &   $0.000/255$ &   $1.625/255$ &   $0.699/255$ &   $0.000/255$ &   $0.000/255$ \\
    CROWN-IBP &   $2.187/255$ &   $0.000/255$ &   $0.000/255$ &   $0.000/255$ &   $0.000/255$ &   $0.000/255$ &   $0.000/255$ \\
          IBP &   $1.026/255$ &   $0.011/255$ &   $0.000/255$ &   $0.000/255$ &   $0.000/255$ &   $0.000/255$ &   $0.000/255$ \\
           WK &   $2.818/255$ &   $1.738/255$ &   $0.000/255$ &   $0.734/255$ &   $0.000/255$ &   $0.000/255$ &   $0.000/255$ \\
       k-ReLU &               &               &               &               &               &               &               \\
   RefineZono &               &               &               &               &               &               &               \\
    SDPVerify &               &               &               &               &               &               &               \\
    LMIVerify &               &               &               &               &               &               &               \\
      Op-norm &   $0.183/255$ &   $0.071/255$ &   $0.000/255$ &   $0.002/255$ &   $0.001/255$ &   $0.000/255$ &               \\
      FastLip &   $2.988/255$ &   $1.256/255$ &   $0.000/255$ &   $0.599/255$ &   $0.000/255$ &   $0.000/255$ &               \\
     RecurJac &   $3.596/255$ &   $2.400/255$ &   $0.000/255$ &   $0.000/255$ &   $0.000/255$ &               &               \\
\hline
          PGD &   $5.679/255$ &   $5.521/255$ &   $6.037/255$ &   $3.482/255$ &   $2.560/255$ &   $4.187/255$ &   $1.819/255$ \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-average-radius-cifar10-0}
\end{table}
    

\begin{table}
    \caption{\emph{Average running time for robust radius computation} in seconds per correctly-predicted instance on CIFAR-10 \texttt{reg} models of different verification approaches. The verification is on $\cL_\infty$ ball. We stop the execution when time exceeds $\SI{120}{s}$ per instance. We include running time of PGD attack as the reference.}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
              & \mc{1}{\sc{FCNNa}} & \mc{1}{\sc{FCNNb}} & \mc{1}{\sc{FCNNc}} & \mc{1}{\sc{CNNa}} & \mc{1}{\sc{CNNb}} & \mc{1}{\sc{CNNc}} & \emc{1}{\sc{CNNd}}\\
\cline{2-8}
              & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean} & \texttt{clean}\\
\midrule
 Bounded MILP &       $93.28$ &      $120.00$ &               &               &               &               &               \\
          AI2 &               &               &               &               &               &               &               \\
      LP-Full &        $8.96$ &      $120.00$ &               &               &               &               &               \\
     DeepPoly &               &               &               &               &               &               &               \\
     Fast-Lin &        $0.05$ &        $0.22$ &       $12.19$ &       $13.14$ &      $112.11$ &      $120.00$ &               \\
        CROWN &        $0.03$ &        $0.05$ &        $0.43$ &        $0.20$ &        $2.96$ &      $120.00$ &      $120.00$ \\
     CNN-Cert &        $0.24$ &        $3.05$ &      $120.00$ &        $5.03$ &      $102.79$ &      $120.00$ &      $120.00$ \\
    CROWN-IBP &        $0.02$ &        $0.02$ &        $0.04$ &        $0.03$ &        $0.04$ &        $0.05$ &        $0.06$ \\
          IBP &        $0.02$ &        $0.02$ &        $0.04$ &        $0.02$ &        $0.04$ &        $0.05$ &        $0.08$ \\
           WK &        $0.03$ &        $0.05$ &        $0.25$ &        $0.11$ &        $0.70$ &      $120.00$ &      $120.00$ \\
       k-ReLU &               &               &               &               &               &               &               \\
   RefineZono &               &               &               &               &               &               &               \\
    SDPVerify &               &               &               &               &               &               &               \\
    LMIVerify &               &               &               &               &               &               &               \\
      Op-norm &        $0.00$ &        $0.00$ &        $0.00$ &        $0.01$ &        $0.01$ &        $0.03$ &               \\
      FastLip &        $0.41$ &        $1.98$ &       $13.48$ &       $77.41$ &      $120.00$ &      $120.00$ &               \\
     RecurJac &        $5.72$ &       $26.99$ &      $120.00$ &      $120.00$ &      $120.00$ &               &               \\
\hline
          PGD &        $2.54$ &        $2.87$ &        $3.68$ &        $2.89$ &        $3.48$ &        $3.69$ &        $4.81$ \\

    \bottomrule
    \end{tabular}
    \label{table:exp-A-average-radius-time-cifar10-0}
    }
\end{table}
        

\begin{table*}
    \caption{\emph{Average robust radius} on CIFAR-10 \texttt{adv2}/\texttt{cadv2} models of different verification approaches. The verification is on $\cL_\infty$ ball. We include results from PGD attack as the reference, which provides an upper bound.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2}\\
\midrule
 Bounded MILP &   $6.141/255$ &   $7.427/255$ &   $0.000/255$ &   $0.000/255$ &               &               &               &               &               &               &               &               &               &               \\
          AI2 &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
      LP-Full &   $4.930/255$ &   $8.747/255$ &   $0.000/255$ &   $0.000/255$ &               &               &               &               &               &               &               &               &               &               \\
     DeepPoly &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
     Fast-Lin &   $4.714/255$ &   $7.103/255$ &   $3.211/255$ &   $4.036/255$ &   $0.655/255$ &               &   $2.269/255$ &   $4.079/255$ &   $1.294/255$ &               &   $0.000/255$ &               &               &               \\
        CROWN &   $5.009/255$ &   $7.408/255$ &   $3.683/255$ &   $4.720/255$ &   $0.847/255$ &               &   $2.601/255$ &   $4.682/255$ &   $1.551/255$ &   $3.030/255$ &   $0.000/255$ &               &   $0.000/255$ &               \\
     CNN-Cert &   $4.856/255$ &   $7.321/255$ &   $3.575/255$ &   $4.911/255$ &   $0.000/255$ &               &   $2.532/255$ &   $4.578/255$ &   $1.339/255$ &               &   $0.000/255$ &               &   $0.000/255$ &               \\
    CROWN-IBP &   $2.717/255$ &   $7.863/255$ &   $0.000/255$ &   $5.004/255$ &   $0.000/255$ &               &   $0.000/255$ &   $5.415/255$ &   $0.000/255$ &   $3.889/255$ &   $0.000/255$ &               &   $0.000/255$ &               \\
          IBP &   $0.826/255$ &   $8.324/255$ &   $0.016/255$ &   $5.027/255$ &   $0.000/255$ &   $3.508/255$ &   $0.028/255$ &   $5.958/255$ &   $0.000/255$ &   $4.611/255$ &   $0.000/255$ &   $4.411/255$ &   $0.000/255$ &   $4.233/255$ \\
           WK &   $3.939/255$ &   $7.103/255$ &   $2.407/255$ &   $4.036/255$ &   $0.000/255$ &               &   $1.476/255$ &   $4.079/255$ &   $0.423/255$ &   $2.486/255$ &   $0.000/255$ &               &   $0.000/255$ &               \\
       k-ReLU &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
   RefineZono &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
    SDPVerify &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
    LMIVerify &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
      Op-norm &   $0.174/255$ &   $0.011/255$ &   $0.068/255$ &   $0.000/255$ &   $0.000/255$ &               &   $0.002/255$ &   $0.000/255$ &   $0.001/255$ &               &   $0.000/255$ &               &               &               \\
      FastLip &   $3.696/255$ &   $6.319/255$ &   $1.359/255$ &   $3.399/255$ &   $0.000/255$ &               &   $0.742/255$ &   $3.523/255$ &   $0.000/255$ &               &   $0.000/255$ &               &               &               \\
     RecurJac &   $4.550/255$ &   $6.375/255$ &   $2.765/255$ &   $3.509/255$ &   $0.000/255$ &               &   $0.000/255$ &   $0.000/255$ &   $0.000/255$ &               &               &               &               &               \\
\hline
          PGD &   $7.856/255$ &  $13.485/255$ &   $8.581/255$ &  $10.864/255$ &   $9.292/255$ &   $9.181/255$ &   $7.185/255$ &  $11.432/255$ &   $6.629/255$ &  $10.301/255$ &   $7.901/255$ &   $9.578/255$ &   $5.472/255$ &   $9.981/255$ \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-average-radius-cifar10-2}
\end{table*}
    

\begin{table*}
    \caption{\emph{Average running time for robust radius computation} in seconds per correctly-predicted instance on CIFAR-10 \texttt{adv2}/\texttt{cadv2} models of different verification approaches. The verification is on $\cL_\infty$ ball. We stop the execution when time exceeds $\SI{120}{s}$ per instance. We include running time of PGD attack as the reference.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2} & \texttt{adv2} & \texttt{cadv2}\\
\midrule
 Bounded MILP &       $93.79$ &       $84.55$ &      $120.00$ &      $115.20$ &               &               &               &               &               &               &               &               &               &               \\
          AI2 &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
      LP-Full &        $8.89$ &        $8.65$ &      $120.00$ &      $120.00$ &               &               &               &               &               &               &               &               &               &               \\
     DeepPoly &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
     Fast-Lin &        $0.05$ &        $0.08$ &        $0.22$ &        $0.27$ &       $12.10$ &               &       $13.27$ &       $13.08$ &      $108.53$ &               &      $120.00$ &               &               &               \\
        CROWN &        $0.03$ &        $0.03$ &        $0.05$ &        $0.05$ &        $0.43$ &               &        $0.20$ &        $0.20$ &        $3.00$ &        $4.26$ &      $120.00$ &               &      $120.00$ &               \\
     CNN-Cert &        $0.25$ &        $0.34$ &        $3.17$ &        $2.66$ &      $120.00$ &               &        $5.60$ &        $5.75$ &      $113.73$ &               &      $120.00$ &               &      $120.00$ &               \\
    CROWN-IBP &        $0.02$ &        $0.03$ &        $0.02$ &        $0.03$ &        $0.05$ &               &        $0.03$ &        $0.04$ &        $0.04$ &        $0.10$ &        $0.05$ &               &        $0.06$ &               \\
          IBP &        $0.02$ &        $0.02$ &        $0.02$ &        $0.03$ &        $0.04$ &        $0.05$ &        $0.03$ &        $0.04$ &        $0.04$ &        $0.05$ &        $0.04$ &        $0.05$ &        $0.08$ &        $0.10$ \\
           WK &        $0.03$ &        $0.04$ &        $0.05$ &        $0.07$ &        $0.25$ &               &        $0.11$ &        $0.13$ &        $0.79$ &        $1.35$ &      $120.00$ &               &      $120.00$ &               \\
       k-ReLU &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
   RefineZono &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
    SDPVerify &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
    LMIVerify &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
      Op-norm &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &               &        $0.00$ &        $0.00$ &        $0.01$ &               &        $0.03$ &               &               &               \\
      FastLip &        $0.42$ &        $0.40$ &        $1.88$ &        $1.74$ &       $16.78$ &               &       $99.47$ &       $65.69$ &      $120.00$ &               &      $120.00$ &               &               &               \\
     RecurJac &        $5.83$ &        $6.41$ &       $27.72$ &       $28.83$ &      $120.00$ &               &      $120.00$ &      $120.00$ &      $120.00$ &               &               &               &               &               \\
\hline
          PGD &        $2.79$ &        $3.64$ &        $3.04$ &        $3.60$ &        $4.15$ &        $4.26$ &        $3.19$ &        $4.13$ &        $3.79$ &        $4.57$ &        $4.01$ &        $4.73$ &        $5.05$ &        $6.63$ \\

    \bottomrule
    \end{tabular}
    \label{table:exp-A-average-radius-time-cifar10-2}
    }
\end{table*}
        

\begin{table*}
    \caption{\emph{Average robust radius} on CIFAR-10 \texttt{adv8}/\texttt{cadv8} models of different verification approaches. The verification is on $\cL_\infty$ ball. We include results from PGD attack as the reference, which provides an upper bound.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8}\\
\midrule
 Bounded MILP &  $10.519/255$ &  $16.419/255$ &   $0.000/255$ &   $2.266/255$ &               &               &               &               &               &               &               &               &               &               \\
          AI2 &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
      LP-Full &   $8.542/255$ &  $21.593/255$ &   $0.000/255$ &  $10.625/255$ &               &               &               &               &               &               &               &               &               &               \\
     DeepPoly &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
     Fast-Lin &   $7.825/255$ &  $17.946/255$ &   $4.637/255$ &  $11.422/255$ &   $0.881/255$ &               &   $4.471/255$ &   $9.171/255$ &   $2.396/255$ &               &   $0.000/255$ &               &               &               \\
        CROWN &   $8.882/255$ &  $20.870/255$ &   $5.398/255$ &  $15.780/255$ &   $1.226/255$ &               &   $5.156/255$ &  $11.617/255$ &   $2.890/255$ &   $8.093/255$ &   $0.000/255$ &               &   $0.000/255$ &               \\
     CNN-Cert &   $8.444/255$ &  $20.163/255$ &   $5.169/255$ &  $14.900/255$ &   $0.000/255$ &               &   $4.952/255$ &  $11.601/255$ &   $2.523/255$ &               &   $0.000/255$ &               &   $0.000/255$ &               \\
    CROWN-IBP &   $5.614/255$ &  $21.014/255$ &   $0.108/255$ &  $20.603/255$ &   $0.000/255$ &               &   $0.589/255$ &  $15.012/255$ &   $0.000/255$ &  $14.604/255$ &   $0.000/255$ &               &   $0.000/255$ &               \\
          IBP &   $1.517/255$ &  $22.276/255$ &   $0.074/255$ &  $22.271/255$ &   $0.000/255$ &  $15.880/255$ &   $0.277/255$ &  $19.115/255$ &   $0.000/255$ &  $18.770/255$ &   $0.000/255$ &  $18.920/255$ &   $0.000/255$ &  $15.553/255$ \\
           WK &   $7.003/255$ &  $17.946/255$ &   $3.877/255$ &  $11.422/255$ &   $0.000/255$ &               &   $3.577/255$ &   $9.171/255$ &   $1.541/255$ &   $6.469/255$ &   $0.000/255$ &               &   $0.000/255$ &               \\
       k-ReLU &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
   RefineZono &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
    SDPVerify &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
    LMIVerify &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
      Op-norm &   $0.117/255$ &   $0.020/255$ &   $0.052/255$ &   $0.000/255$ &   $0.000/255$ &               &   $0.002/255$ &   $0.000/255$ &   $0.001/255$ &               &   $0.000/255$ &               &               &               \\
      FastLip &   $6.309/255$ &  $18.002/255$ &   $1.992/255$ &  $10.019/255$ &   $0.000/255$ &               &   $2.173/255$ &   $8.147/255$ &   $0.000/255$ &               &   $0.000/255$ &               &               &               \\
     RecurJac &   $7.539/255$ &  $18.002/255$ &   $3.971/255$ &  $10.027/255$ &   $0.000/255$ &               &   $0.000/255$ &   $0.000/255$ &   $0.000/255$ &               &               &               &               &               \\
\hline
          PGD &  $15.500/255$ &  $35.723/255$ &  $15.783/255$ &  $35.278/255$ &  $19.558/255$ &  $25.796/255$ &  $15.219/255$ &  $31.399/255$ &  $13.128/255$ &  $34.687/255$ &  $14.913/255$ &  $37.088/255$ &  $12.040/255$ &  $28.578/255$ \\

    \bottomrule
    \end{tabular}
    }
    \label{table:exp-A-average-radius-cifar10-8}
\end{table*}
    

\begin{table*}
    \caption{\emph{Average running time for robust radius computation} in seconds per correctly-predicted instance on CIFAR-10 \texttt{adv8}/\texttt{cadv8} models of different verification approaches. The verification is on $\cL_\infty$ ball. We stop the execution when time exceeds $\SI{120}{s}$ per instance. We include running time of PGD attack as the reference.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
              &         \mc{2}{\sc{FCNNa}} &         \mc{2}{\sc{FCNNb}} &         \mc{2}{\sc{FCNNc}} &          \mc{2}{\sc{CNNa}} &          \mc{2}{\sc{CNNb}} &          \mc{2}{\sc{CNNc}} &         \emc{2}{\sc{CNNd}}\\
\cline{2-15}
              & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8} & \texttt{adv8} & \texttt{cadv8}\\
\midrule
 Bounded MILP &      $108.25$ &       $82.45$ &      $117.77$ &      $111.77$ &               &               &               &               &               &               &               &               &               &               \\
          AI2 &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
      LP-Full &        $9.56$ &        $8.43$ &      $120.00$ &      $120.00$ &               &               &               &               &               &               &               &               &               &               \\
     DeepPoly &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
     Fast-Lin &        $0.05$ &        $0.06$ &        $0.23$ &        $0.23$ &       $12.23$ &               &       $12.97$ &       $13.05$ &      $106.36$ &               &      $120.00$ &               &               &               \\
        CROWN &        $0.03$ &        $0.03$ &        $0.05$ &        $0.05$ &        $0.43$ &               &        $0.20$ &        $0.20$ &        $3.00$ &        $4.15$ &      $120.00$ &               &      $120.00$ &               \\
     CNN-Cert &        $0.28$ &        $0.27$ &        $3.56$ &        $3.52$ &      $120.00$ &               &        $6.38$ &        $6.27$ &      $112.92$ &               &      $120.00$ &               &      $120.00$ &               \\
    CROWN-IBP &        $0.02$ &        $0.03$ &        $0.02$ &        $0.03$ &        $0.05$ &               &        $0.03$ &        $0.04$ &        $0.04$ &        $0.09$ &        $0.05$ &               &        $0.06$ &               \\
          IBP &        $0.02$ &        $0.03$ &        $0.03$ &        $0.03$ &        $0.04$ &        $0.05$ &        $0.03$ &        $0.03$ &        $0.04$ &        $0.05$ &        $0.05$ &        $0.06$ &        $0.08$ &        $0.09$ \\
           WK &        $0.03$ &        $0.04$ &        $0.05$ &        $0.07$ &        $0.24$ &               &        $0.10$ &        $0.13$ &        $0.74$ &        $1.19$ &      $120.00$ &               &      $120.00$ &               \\
       k-ReLU &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
   RefineZono &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
    SDPVerify &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
    LMIVerify &               &               &               &               &               &               &               &               &               &               &               &               &               &               \\
      Op-norm &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &        $0.00$ &               &        $0.01$ &        $0.00$ &        $0.01$ &               &        $0.03$ &               &               &               \\
      FastLip &        $0.45$ &        $0.45$ &        $2.05$ &        $1.79$ &       $17.55$ &               &      $102.45$ &       $70.16$ &      $120.00$ &               &      $120.00$ &               &               &               \\
     RecurJac &        $6.91$ &        $7.11$ &       $30.71$ &       $34.06$ &      $120.00$ &               &      $120.00$ &      $120.00$ &      $120.00$ &               &               &               &               &               \\
\hline
          PGD &        $3.41$ &        $4.58$ &        $3.80$ &        $5.17$ &        $4.95$ &        $5.52$ &        $4.04$ &        $5.66$ &        $4.48$ &        $6.73$ &        $4.58$ &        $6.66$ &        $5.67$ &        $8.05$ \\

    \bottomrule
    \end{tabular}
    \label{table:exp-A-average-radius-time-cifar10-8}
    }
\end{table*}
        


==> tables/exp-B-main-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[!ht]
\caption{\emph{Robust accuracy} on CIFAR-10 and ImageNet models of \emph{probabilistic approaches}. The models are trained with various robust training approaches and built using smoothing distributions labelled as ``Smooth Dist.''. 
Each group is variable-controlled. 
The \textbf{bolded} numbers mark the highest ones within the group.}
    \label{tab:exp-B-main-table}
    \centering
    \vspace{-0.75em}
    \resizebox{0.98\textwidth}{!}{
\begin{tabular}{c||c|c|l||l|l|l||cccccc}
\toprule
\multicolumn{1}{c||}{Group \#} & \multicolumn{1}{c|}{Adversary} & \multicolumn{1}{c|}{Dataset} & \multicolumn{1}{l||}{Model Structure} & \multicolumn{1}{l|}{Verification} & \multicolumn{1}{l|}{Robust Training}           & \multicolumn{1}{l||}{Smooth Dist.} & \multicolumn{6}{l}{Certified Robust Accuracy under Radius $r$}                               \\ 
\hline\hline
\multicolumn{7}{r}{$r=$} & $0.25$        & $0.50$         & $0.75$        & $1.00$         & $1.25$        & $1.50$         \\
\hline
\multirow{3}{*}{I}               & \multirow{8}{*}{$\cL_2$}       & \multirow{8}{*}{CIFAR-10}    & \multirow{3}{*}{Wide ResNet 40-2}    & Differential Privacy                       & \multirow{3}{*}{Data Augmentation}                      & \multirow{8}{*}{Gaussian}            & $34.2\%$      & $14.8\%$      & $6.8\%$       & $2.2\%$       & $0.0\%$       & $0.0\%$       \\
\cline{5-5}
                                 &                                &                              &                                      & Neyman-Pearson                             &                                                         &                                      & $\mb{68.8\%}$ & $\mb{46.8\%}$ & $\mb{36.0\%}$ & $\mb{25.4\%}$ & $\mb{19.8\%}$ & $\mb{15.6\%}$ \\
\cline{5-5}
                                 &                                &                              &                                      & $f$-Divergence                             &                                                         &                                      & $62.2\%$      & $41.8\%$      & $27.2\%$      & $19.2\%$      & $14.2\%$      & $11.4\%$      \\
\cline{1-1}\cline{4-6}\cline{8-13}
\multirow{5}{*}{II}              &                                &                              & \multirow{5}{*}{ResNet-110}          & \multirow{5}{*}{Neyman-Pearson}            & Data Augmentation                                       &                                      & $61.2\%$      & $43.2\%$      & $32.0\%$      & $22.4\%$      & $17.2\%$      & $14.0\%$      \\
\cline{6-6}
                                 &                                &                              &                                      &                                            & Adversarial Training                                    &                                      & $73.0\%$      & $57.8\%$      & $48.2\%$      & $\mb{37.2\%}$ & $33.6\%$      & $\mb{28.2\%}$ \\
\cline{6-6}
                                 &                                &                              &                                      &                                            & Adversarial + Pretraining                               &                                      & $\mb{81.8\%}$ & $\mb{62.6\%}$ & $\mb{52.4\%}$ & $37.2\%$      & $\mb{34.0\%}$ & $30.2\%$      \\
\cline{6-6}
                                 &                                &                              &                                      &                                            & \t{MACER}                                                   &                                      & $68.8\%$      & $52.6\%$      & $40.4\%$      & $33.0\%$      & $27.8\%$      & $25.0\%$      \\
\cline{6-6}
                                 &                                &                              &                                      &                                            & \t{ADRE}                                                    &                                      & $68.0\%$      & $50.2\%$      & $37.8\%$      & $30.2\%$      & $23.0\%$      & $17.0\%$      \\
\hline \hline
\multicolumn{7}{r}{$r=$}   & $0.5$         & $1.0$         & $1.5$         & $2.0$         & $2.5$         & $3.0$         \\
\hline
\multirow{3}{*}{III}             & \multirow{7}{*}{$\cL_2$}       & \multirow{7}{*}{ImageNet}    & \multirow{7}{*}{ResNet-50}           & Differential Privacy                       & \multirow{3}{*}{Data Augmentation}                      & \multirow{7}{*}{Gaussian}            & $26.0\%$      & $12.2\%$      & $4.4\%$       & $0.0\%$       & $0.0\%$       & $0.0\%$       \\
\cline{5-5}
                                 &                                &                              &                                      & Neyman-Pearson                             &                                                         &                                      & $\mb{49.2\%}$ & $\mb{37.4\%}$ & $\mb{29.0\%}$ & $\mb{19.2\%}$ & $\mb{14.8\%}$ & $\mb{12.0\%}$ \\
\cline{5-5}
                                 &                                &                              &                                      & $f$-Divergence                             &                                                         &                                      & $43.4\%$      & $30.4\%$      & $13.6\%$      & $3.2\%$       & $0.0\%$       & $0.0\%$       \\
\cline{1-1}\cline{5-6}\cline{8-13}
\multirow{4}{*}{IV}              &                                &                              &                                      & \multirow{4}{*}{Neyman-Pearson}            & Data Augmentation                                       &                                      & $49.2\%$      & $37.4\%$      & $29.0\%$      & $19.2\%$      & $14.8\%$      & $12.0\%$      \\
\cline{6-6}
                                 &                                &                              &                                      &                                            & Adversarial Training                                    &                                      & $56.4\%$      & $\mb{44.8\%}$ & $\mb{38.2\%}$ & $\mb{28.0\%}$ & $\mb{25.6\%}$ & $\mb{20.0\%}$ \\
\cline{6-6}
                                 &                                &                              &                                      &                                            & \t{MACER}                                                   &                                      & $\mb{57.0\%}$ & $43.2\%$      & $31.4\%$      & $24.8\%$      & $17.6\%$      & $14.0\%$      \\
\cline{6-6}
                                 &                                &                              &                                      &                                            & \t{ADRE}                                                    &                                      & $\mb{57.0\%}$ & $41.8\%$      & $30.0\%$      & $23.6\%$      & $17.8\%$      & $14.2\%$      \\
\hline \hline
\multicolumn{7}{r}{$r=$}  & $0.5$         & $1.0$         & $1.5$         & $2.0$         & $3.0$         & $4.0$         \\
\hline
\multirow{4}{*}{V}               & \multirow{8}{*}{$\cL_1$}       & \multirow{4}{*}{CIFAR-10}    & \multirow{4}{*}{Wide ResNet 40-2}    & Differential Privacy                       & \multirow{8}{*}{Data Augmentation}                      & \multirow{3}{*}{Laplace}             & $43.0\%$      & $20.8\%$      & $12.2\%$      & $7.2\%$       & $1.4\%$       & $0.0\%$       \\
\cline{5-5}
                                 &                                &                              &                                      & R\'enyi Divergence          &                                                         &                                      & $58.2\%$      & $39.4\%$      & $27.0\%$      & $16.8\%$      & $9.2\%$       & $4.0\%$       \\
\cline{5-5}
                                 &                                &                              &                                      & \multirow{2}{*}{Neyman-Pearson}            &                                                         &                                      & $58.4\%$      & $39.6\%$      & $27.0\%$      & $17.2\%$      & $9.2\%$       & $4.2\%$       \\
\cline{7-7}
                                 &                                &                              &                                      &                                            &                                                         & Uniform                              & $\mb{69.2\%}$ & $\mb{56.6\%}$ & $\mb{48.0\%}$ & $\mb{39.4\%}$ & $\mb{26.0\%}$ & $\mb{20.4\%}$ \\
\cline{1-1}\cline{3-5}\cline{7-13}
\multirow{4}{*}{VI}              &                                & \multirow{4}{*}{ImageNet}    & \multirow{4}{*}{ResNet-50}           & Differential Privacy                       &                                                         & \multirow{3}{*}{Laplace}             & $39.0\%$      & $26.2\%$      & $17.8\%$      & $13.0\%$      & $6.8\%$       & $0.0\%$       \\
\cline{5-5}
                                 &                                &                              &                                      & R\'enyi Divergence          &                                                         &                                      & $48.2\%$      & $40.4\%$      & $31.0\%$      & $25.8\%$      & $19.0\%$      & $13.6\%$      \\
\cline{5-5}
                                 &                                &                              &                                      & \multirow{2}{*}{Neyman-Pearson}            &                                                         &                                      & $49.0\%$      & $40.8\%$      & $31.2\%$      & $26.0\%$      & $19.0\%$      & $13.6\%$      \\
\cline{7-7}
                                 &                                &                              &                                      &                                            &                                                         & Uniform                              & $\mb{55.2\%}$ & $\mb{49.0\%}$ & $\mb{45.6\%}$ & $\mb{42.0\%}$ & $\mb{32.8\%}$ & $\mb{24.8\%}$ \\
\hline \hline
\multicolumn{7}{r}{$r=$}   & $1/255$       & $2/255$       & $4/255$       & $8/255$       &               &               \\
\hline
\multirow{2}{*}{VII}                              & \multirow{4}{*}{$\cL_\infty$}  & \multirow{2}{*}{CIFAR-10}    & \multirow{2}{*}{Wide ResNet 40-2}    & \multirow{4}{*}{Neyman-Pearson}            & Data Augmentation                                       & \multirow{4}{*}{Gaussian}            & $71.4\%$      & $52.0\%$      & $29.0\%$      & $12.8\%$      &               &               \\
\cline{6-6}
                                 &                                &                              &            &              & Adversarial Training          &      & $\mb{83.2\%}$      & $\mb{65.0\%}$      & $\mb{49.6\%}$      & $\mb{25.4\%}$      &               &   \\
\cline{1-1}\cline{3-4}\cline{6-6}\cline{8-13}
\multirow{2}{*}{VIII}                             &                                &  \multirow{2}{*}{ImageNet}                    &  \multirow{2}{*}{ResNet-50}                            &                                            & Data Augmentation        &                  & $28.2\%$      & $11.4\%$      & $0.0\%$       & $0.0\%$       &               &              \\
\cline{6-6}
                                 &                                &                              &            &              & Adversarial Training          &      & $\mb{38.2\%}$      & $\mb{20.4\%}$      & $\mb{4.6\%}$      & $0.0\%$      &               &   \\
\bottomrule
\end{tabular}
}
\vspace{-1.25em}
\end{table*}
